Global Optimality Guarantees For Policy Gradient Methods

Policy gradients methods apply to complex, poorly understood, control problems by performing stochastic gradient descent over a parameterized class of polices. Unfortunately, even for simple control problems solvable by standard dynamic programming techniques, policy gradient algorithms face non-convex optimization problems and are widely understood to converge only to a stationary point. This work identifies structural properties -- shared by several classic control problems -- that ensure the policy gradient objective function has no suboptimal stationary points despite being non-convex. When these conditions are strengthened, this objective satisfies a Polyak-lojasiewicz (gradient dominance) condition that yields convergence rates. We also provide bounds on the optimality gap of any stationary point when some of these conditions are relaxed.

==> analysis.tex <==
%!TEX root = policy_grad_optimality.tex
\section{Analysis}
The key to proving our main results is a sharp relationship between policy gradient methods and the weighted policy iteration scheme 
\begin{equation}\label{eq:weighted_constrained_PI}
\pi_{k+1}= \argmin_{\theta \in \Theta} \Bc(\theta| \eta, J_{\pi_{\theta_k}})  \quad k=1,2,\cdots,
\end{equation} 
In particular, Lemma \ref{lem: PG theorem} provides the policy gradient formula $\nabla \ell(\theta)=\nabla_{\thetabar} \, \Bc(\thetabar \mid \eta_{\pi_{\theta}}, J_{\pi_{\theta}}) \bigg\vert_{ \thetabar=\theta_t}$. 
When $\Theta=\mathbb{R}^d$ is unconstrained, allows us to write gradient descent on $\ell(\theta)$ as %with a constant stepsize $\alpha$ is equivalent to making gradient updates with respect to the weighted policy iteration objective:
\[ 
\theta_{t+1}  \theta_t - \alpha \nabla_{\thetabar} \, \Bc(\thetabar \mid \eta_{\pi_{\theta_t}}, J_{\pi_{\theta_t}}) \bigg\vert_{ \thetabar=\theta_t} .
\] 
Policy gradient is closely related differs from the weighted PI scheme \eqref{eq: weighted PI objective}
in two important ways.  First, policy gradient methods are incremental, making a parameter update based on a gradient of \eqref{eq: weighted PI objective} rather than solving it exactly. Second, the state-relevance weights  $\eta$ are updated over time to reflect the frequency of states visited by the current policy. The sharpness of the relation between the two, however, allows us to derive properties of the multi-period policy gradient cost directly from those of the single-period weighted PI cost function. 

\subsection{General results}
\paragraph{Performance difference and telescoping sums.} A basic formula for Markov reward processes will be useful for much of the analysis. The difference in cost-to-go functions is related to the the gap in Bellman's equation at future states as
\begin{align}\nonumber
\E_{\nu}^{\pi} \left[ J_{\pi}(s_0) \right] = \E_{\nu}^{\pi}\left[  \sum_{t=0}^{\infty} \gamma^t g_{\pi}(s_t) \right] &=    \E_{\nu}^{\pi}\left[J(s_0)+  \sum_{t=0}^{\infty} \gamma^t \left[g_{\pi}(s_t) +  (P_{\pi}J)(s_t) - J(s_t) \right]\right]\\ &=\E_{\nu}^{\pi}[J(s_0)]+ \E_{\nu}^{\pi}\left[  \sum_{t=0}^{\infty} \gamma^t \left( T_{\pi}J(s_t) - J(s_t) \right)  \right]. \label{eq: perf diff 1}
\end{align}
In the calculation we use the notation $(P_{\pi}J)(s) = \intop J(s') P(ds'| s, \pi(s))$. The second equality follows by noting that $(P_{\pi}J)(s_t) = \E^{\pi}\left[ J(s_{t+1}) | s_t \right]$ and using the tower property of conditional expectation to simplify the telescoping sum. The same technique is central to the study of average cost MDPs. See \cite{makowski2002poisson} or \cite[Prop.~5.5.6]{hernandez2012discrete}.
\cite{kakade2002approximately} write this in a particular convenient form, which they call the \emph{performance difference lemma}. Choosing $J=J_{\pibar}$, $\nu=\rho$, and recalling that  $\ell(\pi)=(1-\gamma)\E_{\rho}[J_{\pi}(s_0)]$, one obtains from \eqref{eq: perf diff 1}, 
\begin{equation}\label{eq: perf diff 2}
\ell(\pi) - \ell(\pibar) = (1-\gamma) \E_{\rho}^{\pi}\left[  \sum_{t=0}^{\infty} \gamma^t \left( T_{\pi}J_{\pibar}(s_t) - J_{\pibar}(s_t) \right)  \right] = \intop \left( T_{\pi}J_{\pibar}-J_{\pi}\right) d\eta_{\pi}.
\end{equation}
The second equality follows from the definition $\eta_{\pi}(S) := (1-\gamma)\E_{\rho}^{\pi} \left[\sum_{t=0}^{\infty} \gamma^t \mathbf{1}(s_t\in S )\right]$. The phenomenon where $\eta_{\pi}$, not $\rho$, appears on the right hand side is sometimes called ``distribution shift''. 



\paragraph{A policy gradient formula.}
%\label{subsec:PG_PI_connection}
Although Condition  \ref{cond: diff}  may initially appear unnatural, the proof shows that it arises naturally in calculating the derivative of $\ell(\theta)$.  



%The policy gradient theorem below which enables this connection can essentially be derived from the result of \cite{silver2014deterministic}. While they call this result a deterministic policy gradient theorem, it actually generalizes the stochastic policy gradient theorem of \cite{sutton2000policy} when $\pi_\theta(s)\in \Delta^{k-1}$ specifies a probability distribution over $k$ base actions. We provide a short proof sketch here, since the presentation of the result and the proof differ from \cite{silver2014deterministic} and \cite{sutton2000policy}. 
\begin{restatable}[Policy gradient theorem]{lem}{pgTheorem}\label{lem: PG theorem}
	Under Condition \ref{cond: diff}, $\ell(\theta)$ is continuously differentiable and
	\[
	\nabla \ell(\theta) =  \nabla_{\thetabar} \, \Bc(\thetabar \mid \eta_{\pi_\theta}, J_{\pi_\theta}) \bigg\vert_{\thetabar=\theta}  %=  \sum_{s \in \Sc} \eta_{\pi_\theta}(s) \left[ \nabla_{\thetabar} \, Q_{\pi_\theta}(s, \pi_{\thetabar}(s)) \bigg\vert_{\thetabar = \theta} \right]. 
	\]
\end{restatable}
\begin{proof}
	From \eqref{eq: perf diff 2}, and the observation that $\Bc(\theta | \eta_{ \thetabar} \, ,\,   J_{\theta} ) = \intop J_{\pi_{\theta}} d\eta_{ \pi_{\thetabar}}$, we have 
	\[
	\ell(\thetabar) - \ell(\theta) =  \intop  \left[ (T_\thetabar J_\theta - J_\theta) \right]d\eta_{\thetabar} = \Bc(\thetabar | \eta_{\thetabar} \, ,\,   J_{\theta} ) -  \Bc(\theta | \eta_{ \thetabar} \, ,\,   J_{\theta} ).
	\]
	Expanding the total derivative in terms of partial derivatives gives,
	\begin{align*}
	\nabla \ell(\thetabar) &=  \nabla_{\thetabar} \, \Bc(\thetabar | \eta_{\thetabar}\, ,\,   J_{\theta} ) \bigg\vert_{\thetabar=\theta} - \nabla_{\thetabar} \, \Bc(\theta | \eta_{\thetabar}\, ,\,   J_{\theta} ) \bigg\vert_{\thetabar=\theta} =\nabla_{\thetabar} \, \Bc(\thetabar | \eta_{\theta}\, ,\,   J_{\theta} ) \bigg\vert_{\thetabar=\theta}. 
	%&=\nabla_{\thetabar} \, \Bc(\thetabar | \eta_{\theta}\, ,\,   J_{\theta} ) \bigg\vert_{\thetabar=\theta} + \underbrace{\nabla_{\thetabar} \, \Bc(\theta | \eta_{\thetabar}\, ,\,   J_{\theta} ) \bigg\vert_{\thetabar=\theta} - \nabla_{\thetabar} \, \Bc(\theta | \eta_{\thetabar}\, ,\,   J_{\theta} ) \bigg\vert_{\thetabar=\theta}}_{=0}.
	\end{align*}
\end{proof}
\begin{rem} 
	Our presentation differs from the familiar form the the policy gradient theorem, which is $\nabla \ell(\theta) = \E\left[ Q_{\pi_{\theta}} (S,A)  \nabla \log \pi_{\theta}(A|S) \right]$ where $\pi_{\theta}(A|S)$ is the probability of selecting a deterministic action $A$ in state $S$ and the expectation is over the distribution of states and actions under $\pi_{\theta}$. See \cite{sutton2018reinforcement}. This form is useful for gradient estimation, but it applies only to stochastic policies and seems to obscure the connections with weighted PI. When the exchange of differentiation and integration is permitted, gradients of $\Bc$ can be rewritten in the more familiar form,
	\begin{equation}\label{eq: pg theorem alternate} 
	\nabla_{\theta} \Bc(\theta | \eta\, J_{\pi} ) = \nabla_{\theta}\, \intop  Q_{\pi}(s, \pi_{\theta}(s)) s\eta(s)  = \intop  \left[ \nabla_{\theta} \, Q_{\pi}(s, \pi_{\theta}(s)) \right] d\eta(s).
	\end{equation}
	In examples \ref{ex:tabularMDPs} and \ref{ex:vanishin_grads_softmax}, stochastic policies are treated as a special case by taking $\pi_{\theta}(s)$ to be a probability vector. The expression \eqref{eq: pg theorem alternate} has been derived before under somewhat stringent regularity conditions by \cite{silver2014deterministic}. Condition \ref{cond: diff} and this short proof appear to be new. 
\end{rem} 







%\begin{rem}
%Suppose 
%
%First consider differentiating the function 
%\[ 
%\theta \mapsto \Bc(\theta | \eta_\pi, J_{\pi} ) = \intop  \left(g(s, \pi_{\theta}(s)) + \gamma\intop J_{\pi}(s') P(s' |  s, \pi_{\theta}(s) ) \right) \eta_{\pi}(s)ds
%\]
%The Leibniz rule shows $\frac{\partial}{\partial \theta_i} \intop g(s, \pi_{\theta}(s) \eta_{\pi}(s)ds$ exists $\frac{\partial}{\partial \theta_i} g(s, \pi_{\theta}(s)$   exists and is integrable---meaning that $\intop \left| \frac{\partial}{\partial \theta_i} g(s, \pi_{\theta}(s)\right| ds <\infty$. The second partial derivative $\frac{\partial^2}{\partial \theta_i \partial \theta_j} \intop g(s, \pi_{\theta}(s) \eta_{\pi}(s)ds$ exists --- implying the first partial derivative is continuous --- if $\frac{\partial^2}{\partial \theta_i \partial \theta_j}  g(s, \pi_{\theta}(s)$ exists and is integrable. 
%Similarly, applying the Leibinz rule twice shows  the derivative of the second term exists if $P(s| s', \pi_{\theta})$ exists and is integrable, here meaning $\intop \intop \left|\frac{\partial }{\partial \theta_i} P(s'|s, \pi_{\theta}(s)) J_{\pi}(s') \right|  \eta_{\pi}(s) ds'ds <\infty$. 
%
%Now consider the differentiability of 
%\[
%\theta \mapsto \Bc(\pi | \eta_{\pi_{\theta}}, J_{\pi} ) = \intop J_{\pi}(s) \eta_{\pi_{\theta}}(ds).
%\]
%
%
%\end{rem} 

%\subsection{Proof of Theorem \ref{thm: no bad stationary points general}}
%\label{subsec: proof of main thm}

\paragraph{A Modified Bellman equation.}


The next lemma establishes Bellman-type equation that holds when the single period objective $\thetabar \mapsto \Bc(\thetabar \mid \eta_{\pi_\theta}, J_{\pi_\theta})$ has no bad stationary points. 
\begin{lem}\label{lem: bellman for stationary points}
	Suppose Condition \ref{cond: stationary} is satisfied. If $\theta$ is a stationary point of $\ell:\Theta \to \mathbb{R}$, then 
	\[ 
	\intop  J_{\pi_\theta} d\eta_{\pi_\theta}  = \min_{\pi\in \Pi_{\Theta}}\intop \left[ T_{\pi}J_{\pi_{\theta}}\right]  d\eta_{\pi_\theta}.
	\] 
\end{lem}
\begin{proof} 
	If $\theta$ is a stationary point of $\ell: \Theta \to \mathbb{R}$, then by Lemma \ref{lem: PG theorem}, it is a stationary point of the function $\thetabar \mapsto \Bc(\thetabar \mid \eta_{\pi_\theta}, J_{\pi_\theta})$. Since Condition \ref{cond: stationary} holds, this means 
	\begin{equation*}
	\Bc(\theta   \mid \eta_{\pi_\theta}, J_{\pi_\theta}) =  \min_{\thetabar \in \Theta} \Bc(\thetabar \mid \eta_{\pi_\theta}, J_{\pi_\theta}).
	\end{equation*}
	Recalling the definition of $\Bc(\theta   \mid \eta, J_\pi)$ in \eqref{eq: weighted PI objective} lets us rewrite both sides of this equation.% To simplify the expressions, take $S$ to be a random state drawn from $\eta_{\pi_\theta}$. Then,
	\begin{equation*}%\label{eq: no bad stationary points in term of bellman}
	\intop J_{\pi_\theta} d\eta_{ \pi_{\theta}} = \intop \left[ T_{\pi_\theta} J_{\pi_\theta}\right] d\eta_{ \pi_{\theta}}  =  \Bc(\theta   \mid \eta_{\pi_\theta}, J_{\pi_\theta})= \min_{\bar{\theta}\in \Theta} \Bc(\bar{\theta} \mid \eta_{\pi_\theta}, J_{\pi_\theta}) = \min_{\bar{\theta}\in \Theta} \intop \left[ (T_{\pi_{\thetabar}}J_{\pi_{\theta}}) \right] d\eta_{\pi_\theta}.
	\end{equation*}
\end{proof} 

\subsection{Proof of Theorem \ref{thm: no bad stationary points general}}
Lemma \ref{lem: on average bellman equation} below provides an ``average'' form of Bellman's equation, which states that a policy is optimal from every possible start state if and only its cost-to-go function has zero average error in Bellman's equation at initial states. The proof is given in Appendix \ref{app: on average Bellman}. The result relies critically on the assumption that the initial distribution is exploratory, formalized in Assumption \ref{ass: exploratory rho}, which essentially implies that all relevant states have a chance of being the initial state. % The proof leverages this 
\begin{restatable}[On average Bellman equation]{lem}{onAvgBellman}\label{lem: on average bellman equation}
	For any $\pi \in \Pi$ , 
	\begin{equation*}%\label{eq: on average Bellman equation}
	J_{\pi}  = J^*  \,\, \rho \,\, a.s.  \iff   \intop (J_{\pi}-TJ_{\pi}) d\rho = 0
	\end{equation*}
\end{restatable}
We now complete the proof. 
\begin{proof}[Proof of Theorem \ref{thm: no bad stationary points general}]
	Since $\ell(\theta) = \intop J_{\pi_{\theta}}d\rho \geq  \intop J^* d\rho$,  if $J_{\pi_{\theta}} = J^*$ $\rho$ almost surely, then $\theta$ is certainly a minimizer of $\ell(\cdot)$. By the first order necessary conditions of optimality, $\theta$ must be a stationary point of $\ell(\cdot)$.
	
	Now suppose $\theta$ is a stationary point of $\ell(\cdot)$. Using Conditions \ref{cond: closure} (and its implication Lemma \ref{lem: bellman for stationary points}) and \ref{cond: stationary} shows
	\[
	\intop  J_{\pi_\theta} d\eta_{\pi_\theta}  = \min_{\pi\in \Pi_{\Theta}}\intop \left[ T_{\pi}J_{\pi_{\theta}}\right]  d\eta_{\pi_\theta} = \intop  [TJ_{\pi_\theta}] d\eta_{\pi_\theta}. 
	\]  
	Next, using that $\eta_{ \pi}\succeq (1-\gamma) \rho$ by definition and using twice that $J_{\pi} \succeq T J_{\pi}$, implies
	\[ 
	0 = \intop \left[ J_{\pi_\theta}- TJ_{\pi_\theta}\right] d\eta_{\pi_\theta} \geq  (1-\gamma) \intop \left[ J_{\pi_\theta}- TJ_{\pi_\theta}\right] d\rho  \geq  0.
	\]
	The result now follows immediately from the ``On average Bellman equation'' in Lemma \ref{lem: on average bellman equation}. 	
\end{proof}

\subsection{Proof of Theorem \ref{thm: convergence_rates}}
The proof can be divided into two key steps. First, we use closure of the policy class (condition \ref{cond: closure}) to upper bound the optimality gap of the policy gradient objective with that of the weighted policy iteration objective. Essentially, this result shows that the current policy is \textit{nearly optimal} if the weighted policy iteration step offers little improvement over the current policy. It is important to note that this crucially depends on the use of an exploratory initial distribution under which $\kappa_{\rho}<\infty$. The second step of the proof translates gradient dominance of the  policy iteration objective to that of $\ell(\cdot)$ by using the policy gradient formula in Lemma \ref{lem: PG theorem}. 
\begin{proof}[Proof of Theorem \ref{thm: convergence_rates}]
	We first derive a consequence of the closure condition. We have, 	
	\begin{align*}
	\ell(\pi_{\theta}) - \min_{\pi}\ell(\pi) &= (1-\gamma) \intop \left[ J_{\pi_{\theta}} - J^* \right] d\rho   \\
	&\overset{(a)}{=} (1-\gamma)\| J_{\pi_{\theta}} - J^{*}\|_{1,\rho} \\
	&\overset{(b)}{\leq} \kappa_\rho \|  J_{\pi_{\theta}} - TJ_{\pi_{\theta}} \|_{1, \rho} \\
	&\overset{(c)}{\leq} \frac{\kappa_\rho}{(1-\gamma)} \|  J_{\pi_{\theta}} - TJ_{\pi_{\theta}} \|_{1, \eta_{\pi_{\theta}}} \\
	&= \frac{\kappa_\rho}{(1-\gamma)} \intop \left[ J_{\pi_\theta}- T J_{\pi_{\theta}} \right]d\eta_{\pi_{\theta}} \\
	&\overset{(d)}{=} \frac{\kappa_\rho}{(1-\gamma)} \left(  \intop J_{\pi_\theta}d\eta_{\pi_{\theta}}  -   \min_{\pi \in \Pi_{\Theta}}  \intop (T_{\pi} J_{\pi_\theta})d\eta_{\pi_{\theta}}    \right) \\
	&= \frac{\kappa_\rho}{(1-\gamma)} \left( \Bc(\theta \mid \eta_{\pi_{\theta}}, J_{\pi_{\theta}}) - \min_{\theta' \in \Theta} \, \Bc(\theta' \mid \eta_{\pi_{\theta}}, J_{\pi_{\theta}})  \right)
	\end{align*}
	Here (a) uses that $J_{\pi_{\theta}} \succeq TJ_{\pi_\theta}$, (b) directly applies the definition of  $\kappa_\rho$ in Definition \ref{def:concentrability_measure}, (c) uses that $\eta_{\pi_{\theta}} \succeq (1-\gamma) \rho$ (by definition, see \eqref{eq: discounted_state_occupancy_measure}) and  (d) directly applies the policy closure condition in Condition \ref{cond: closure}. 
	
	By assumption, $\thetabar \mapsto \Bc(\thetabar \mid \eta_{\theta}, J_{\pi_{\theta}})$ is ($c$, $\mu$)--gradient dominated. Applying this gives
	\begin{align*}
	\Bc(\theta \mid \eta_{\pi_{\theta}}, J_{\pi_{\theta}}) - \min_{\theta' \in \Theta} \Bc(\theta' \mid \eta_{\pi_{\theta}}, J_{\pi_{\theta}}) &\leq - \min_{v \in \Theta} \, \left[ c \, \langle \nabla_{\thetabar} \, \Bc(\thetabar \mid \eta_{\pi_{\theta}}, J_{\pi_{\theta}}) \bigg\vert_{\thetabar = \theta}, v-\theta \rangle + \frac{\mu}{2} \norm{v-\theta}^2_2 \right] \\
	&\leq - \min_{v \in \Theta} \, \left[ c \, \langle \nabla_{\theta} \ell(\theta), v-\theta \rangle + \frac{\mu}{2} \norm{v-\theta}^2_2 \right],
	\end{align*}
	which gives our desired result. The second inequality above uses the policy gradient formula in Lemma \ref{lem: PG theorem}. 
\end{proof}

The next result relaxes the closure condition in Theorem \ref{thm: no bad stationary points general}. When the policy class is closed under $\epsilon-$policy-improvement steps, in the sense formalized in Condition \ref{cond:approx_closure}, we bound the suboptimality of any stationary point of $\ell(\cdot)$. 
\begin{thm}\label{thm: approximate closure}
	Suppose Conditions \ref{cond: diff}, \ref{cond:approx_closure}, and  \ref{cond: stationary} hold. Then, $\ell$ is continuously differentiable and any stationary point  $\theta$  of $\ell(\cdot)$ satisfies, 
	\[ 
	\ell(\pi_\theta) - \ell(\pi^*) \leq  \frac{\kappa_\rho}{(1-\gamma)} \cdot \epsilon 
	\]
\end{thm}

\subsection{Proof of Theorem \ref{thm: approximate closure}}
\begin{proof}
	Suppose $\theta$ is a stationary point of $\ell:\Theta \to \mathbb{R}$. Let $S$ denote a random draw from $\eta_{\pi_\theta}$. Since condition \ref{cond: stationary} holds, Lemma \ref{lem: bellman for stationary points} implies 
	\[ 
	\E\left[ \left(J_{\pi_\theta}-TJ_{\pi_{\theta}}\right)(S) \right]  \leq   \left( \min_{\pi\in \Pi_{\Theta}}\E\left[ T_{\pi}J_{\pi_{\theta}}(S)  \right] - \E[TJ_{\pi_{\theta}}(S)]\right)=  \min_{\pi \in \Pi_{\Theta}}  \|   T_{\pi} J_{\pi_\theta} - TJ_{\pi_\theta} \|_{1, \eta_{\pi_\theta}}  := \epsilon.
	\]
	where the final equality uses $T_{\pi}J_{\pi_{\theta}} \succeq TJ_{\pi_\theta}$ for any $\pi \in \Pi_{\Theta}$. Then, we have
	\begin{align*}
	\ell(\pi_{\theta}) - \min_{\pi}\ell(\pi) = (1-\gamma)\sum_{s \in \Sc}\rho(s)\left( J_{\pi_{\theta}}(s) - J^*(s)\right) &= (1-\gamma)\| J_{\pi_{\theta}} - J^{*}\|_{1,\rho} \\
	&\leq \kappa_\rho \|  J_{\pi_{\theta}} - TJ_{\pi_{\theta}} \|_{1, \rho} \\
	&\leq \frac{\kappa_\rho}{(1-\gamma)} \|  J_{\pi_{\theta}} - TJ_{\pi_{\theta}} \|_{1, \eta_{\pi_{\theta}}} \\
	&= \frac{\kappa_\rho \cdot \epsilon}{(1-\gamma)},
	\end{align*}
	where the first inequality follows from the definition of $\kappa_\rho$ as given in \eqref{def:concentrability_measure} and the second inequality uses that $\eta_{\pi_{\theta}} \geq (1-\gamma) \rho$ (by definition, see \eqref{eq: discounted_state_occupancy_measure}).
	
	
	%	We want to show this means $\|J_{\pi_\theta}-TJ_{\pi_{\theta}}\|_\infty$ is small. We have 
	%	\begin{align*}
	%	\|  J_{\pi_{\theta}} - TJ_{\pi_{\theta}} \|_\infty  \leq \kappa_\rho \|  J_{\pi_{\theta}} - TJ_{\pi_{\theta}} \|_{1, \rho} 
	%	\leq \frac{\kappa_\rho}{1-\gamma} \|  J_{\pi_{\theta}} - TJ_{\pi_{\theta}} \|_{1, \eta_{\pi_{\theta}}} = \frac{\kappa_\rho \cdot \epsilon}{1-\alpha},
	%	\end{align*}
	%	where the first inequality directly applies the definition of $\kappa_\rho$ and the second inequality uses that $\eta_{\pi_{\theta}} \geq (1-\gamma) \rho$. From the contractivity of $T$, this implies (See \eqref{eq: near solutions to bellmans equation}), 
	%	\[ 
	%	\|  J_{\pi_{\theta}} - J^* \|_\infty \leq \frac{\kappa_\rho \cdot \epsilon}{(1-\gamma)^2}.
	%	\]	
	%	Of course, $\ell(\pi_{\theta}) - \min_{\pi}\ell(\pi) = (1-\gamma)\sum_{s}\rho(s)\left( J_{\pi_{\theta}}(s) - J^*(s)\right) \leq (1-\gamma) \| J_{\pi} - J^{*}\|_\infty$, so we reach our conclusion.   
\end{proof}

\section{Conclusion}
\textcolor{red}{WRITE THIS}.

==> app_agrawal_discussion.tex <==
%!TEX root = policy_grad_optimality.tex
\section{Discussion of \cite{agarwal2020optimality}}\label{sec: app_agrawal_discussion}

\jb{Here we provide some comparisons to the approach of \cite{agarwal2020optimality}, offering perspective on the strengths and shortcomings of our approach and highlighting some connections between our technical results and theirs.}

\jb{Our work is not primarily focused on particular algorithms, but rather on the landscape of the loss function $\ell(\cdot)$. Consider Theorems \ref{thm: no bad stationary points general}, \ref{thm: finite_horizon}, or \ref{thm: approximate closure}. These results about the quality of stationary points can be understood as addressing the following question:
\begin{itemize}
	\item Given a parameterized policy class $\Pi_{\Theta}=\{\pi_{ \theta}: \theta \in \Theta\}\subset \Pi$ and a suboptimal policy $\pi \in \Pi_{\Theta}$, does there exists a smooth curve $\{\pi_{\alpha}: \alpha \in (-1,1) \}$ with $\pi_0=\pi$ and $\frac{d}{d\alpha} \ell(\pi_\alpha) \vert_{\alpha=0}<0$?  
\end{itemize}
Such a study is mostly focused on understanding when local policy search is a sensible approach for reaching a (near) optimal policy. We take a broad algorithm-independent view, being mostly focused on whether good feasible descent directions exist, and mostly agnostic to how a descent direction is picked. The work of \cite{agarwal2020optimality} is mostly around specific algorithms, with a special focus on natural-gradient actor-critic algorithms. Explicit bounds on the convergence rates of algorithms are given. Our choice of focus yields several results and insights that are not covered by their work: 
\begin{itemize}
	\item In Example \ref{ex: counterexample}, we provide a simple illustration of how the multi-period nature of the decision problem can lead to bad local minima. \item When the policy class is closed under policy improvement, we show that the challenges raised in that example largely disappear, and the problem reduced to studying the single period objective function in \eqref{eq:weighted_pi_objective}. This approach --- reducing reasoning about long-horizon problems into reasoning about single period problems --- is core to almost all dynamic programming. For us, the approach helps clarify our thinking. 
	\item In addition to treating some examples covered by \cite{agarwal2020optimality}, like linear MDPs, our analysis seamlessly covers problems with infinite action spaces, structured cost functions, and deterministic policies. We show that this includes problems like linear quadratic control and optimal stopping. 
	\item Theorem \ref{thm: finite_horizon}, which is about the nonstationary policy classes an finite horizon problems, is not contained in the simultaneous work by \cite{agarwal2020optimality}. We instantiate this theory on one important problem: a finite horizon inventory control problem. 
\end{itemize}
Our focus on an algorithm-agnostic study of the landscape of $\ell(\cdot)$ comes at a cost. This is felt most clearly when studying the softmax parameterization. Our theory reduces the problem of policy search in long-horizon decision-making to policy search in single-period decision problems,  but the use of softmax parameterization leads to very unusual optimization challenges even in the case of a finite action space, single state, and single time-period (i.e. in the seemingly simple problem of picking the best action among $k$ options). There is no optimal solution to this optimization problem; instead optimal performance is attained only as certain components of the parameter vector tend to infinity. The policy functions themselves are poorly conditioned. Our theory applies easily to problems with some entropy regularization (see e.g. Example \ref{ex:linear_mdp}), in which case optimal solutions exist and are attained by some finite parameter vector. In cases without regularization, it seems this somewhat unique optimization problem requires a detailed study of specific algorithms. \cite{agarwal2020optimality} provide such a study, with a particularly masterful analysis of the rate of convergence of natural policy gradient methods.}

\jb{The next subsection tries to clarify some connections between our theory and that appearing in \cite{agarwal2020optimality}. 
\paragraph{Connecting closure conditions to conditions on  value function approximation}
Our notion of approximate closure of the policy appears, at first glance, to be quite different from conditions in \cite{agarwal2020optimality}, which revolve around the accuracy of certain parametric approximations to the value function. Here we aim to draw tight connections.}

\jb{There is natural duality between a parametric class of policies and a parametric class of value functions. In Example \ref{ex:linear_mdp}, for instance, we began with a class of value function $\{Q^{\theta}: \theta \in \Theta\}$ and derived from this a class of polices $\{ \pi_{\theta} : \theta \in \Theta \}$ where $\pi_{ \theta}$ is greedy with respect to $Q^{\theta}$. Classic work by \cite{konda2000actor,sutton2000policy} works in the reverse direction --- deriving features for approximating $Q_{\pi_{ \theta}}$ from the score function of a stochastic policy.}

\jb{The next result shows that if a parametric class of value functions $\{Q^{\theta}: \theta \in \Theta\}$ can approximate each $Q_{\pi}$, then the class of greedy policies induced by this class of value functions is closed under policy improvement. A similar observation was used in our analysis of Example \ref{ex:linear_mdp}. One can view our treatment of LQ control through this lens. In that case, the state-action value function of any linear policy can be fit within the class of quadratic functions. Greedy optimization of a quadratic value functions induces a linear policy. 
\begin{lem}
	For each $\theta \in \Theta$, let $Q^{\theta}:\Sc \times \Ac \to \mathbb{R}$ and define $\pi_{ \theta}:\Sc \to \Ac$ by $\pi_{ \theta}(s) \in \argmin_{a\in \Ac_s} Q^{\theta}(s,a)$. Take $\mathcal{Q}_{\Theta} = \{Q_{\theta} : \theta \in \Theta \}$. If $Q_{\pi_{ \theta}} \in \mathcal{Q}_{\Theta}$ for each $\theta \in \Theta$, then $\Pi_{\Theta}$ satisfies Condition \ref{cond: closure} (closure). 
\end{lem} 
\begin{proof}
	Pick $\pi_{\theta} \in \Pi_\Theta$. Choose $w \in \Theta$ such that $Q^{w} = Q_{\pi_{ \theta}}$. Then $\pi_w\in \Pi_{\Theta}$ is a PI update to $\pi_{ \theta}$. 
\end{proof}}

\jb{A similar observation holds for approximate closure, as in Condition \ref{cond:approx_closure}. For concreteness, we show this for a class of linearly parameterized value functions together with the softmax policies they induce. Accuracy of value function approximation is shown to imply 
approximate closure of the class of softmax policies.} 

\jb{The measure of least-squares error in \eqref{eq:accurate_Q} is essentially the same as the measure of approximation error in Corollary 21 of \cite{agarwal2020optimality}. Highlighting the connection between this measure and approximate closure is our main motivation behind presenting this example.  
\begin{example}\label{ex:linear_softmax} As in Example \ref{ex:tabularMDPs}, we assume the set of feasible actions $\Ac_s$ is the same for every state $s$ and denote this by $\Ac$. We also assume there is a finite set of $k$ deterministic actions to choose from and take $\Ac=\Delta^{k-1}$ to be the set of all probability distributions over these actions. Suppose $g(s,a)$ and $P(s' | s,a)$ are linear in $a$, as in \eqref{eq: tabular costs and transitions}. Fix a feature mapping $\phi:\Sc\times \{1,\cdots, k\}$. Consider the class of policies, $\Pi_{\Theta} = \{\pi_{\theta} : \theta \in \mathbb{R}^d\}$ where $\pi_{\theta}(s) = (\pi_{\theta}(1|s), \cdots \pi_{ \theta}(k|s)) \in \Delta^{k-1}$ has components $\pi_{\theta}(s,i) \propto  \exp\{ \theta^\top \phi(s,i) \}$.
\end{example}
\begin{restatable}[Accurate function approximation implies approximate closure]{lem}{score-function-approx}\label{lemma:score_function_approx}
	In the setting of Example \ref{ex:linear_softmax}, suppose that for each $\pi \in \Pi_{\Theta}$,
	\begin{equation}\label{eq:accurate_Q}
		\min_{w \in \mathbb{R}^d}  \E_{(s,i)\sim \eta_{ \pi}\otimes {\rm Unif}}\left[ \left(Q_{\pi}(s,e_i) - w^\top \phi(s,i)  \right)^2\right] < \epsilon^2/k. %\left\| Q_{\pi} - \sum_{j=1}^{d} w_j \phi_j \right\|_{2,\eta_{\pi} \otimes {\rm unif} }^2  < k\epsilon^2.
	\end{equation}
	Then $\Pi_{\Theta}$ satisfies Condition \ref{cond:approx_closure}. 
\end{restatable}}
\begin{proof}
	\jb{Given $\pi$, let $\hat{w}$ satisfy  $\E_{(s,i)\sim \eta_{ \pi}\otimes {\rm Unif}}\left[ \left(Q_{\pi}(s,e_i) - w^\top \phi(s,i)  \right)^2\right] =  \epsilon_0^2/k$ where $\epsilon_0<\epsilon_0$. Set 
	\[
	\hat{Q}_{\pi}(s,a) = \sum_{i=1}^{k} a_i (\hat{w}^\top \phi(s,i)). 
	\]
	to be the resulting approximate $Q$--function. For a scalar $c>0$, consider the policy $\pi_{c \hat{w}}$. This policy assigns probability $\pi_{ c \hat{w}}(i|s) \propto \exp\{c \cdot \hat{Q}_{\pi}(s,e_i) \}$ to base action $i$ in state $s$.} 
	
	\jb{We show that $\pi_{c\hat{w}}$ approximately optimizes the policy iteration objective when $c$ is large. First, 
	\begin{align*}
		\Bc(\pi_{c \hat{w}} \mid \eta_{ \pi}, J_{\pi}) &=  \intop \left(Q_{\pi}(s, \pi_{c \hat{w}(s)}) \right)  \eta_{ \pi}(ds)\\
		&\leq \intop \left(\hat{Q}_{\pi}(s, \pi_{c \hat{w}}(s)) \right)  \eta_{ \pi}(ds) + \intop \max_{a\in \Ac}\left| \hat{Q}_{\pi}(s, a) - Q_{\pi}(s,a) \right|\eta_{ \pi}(ds) \\
		&= \intop \left(\hat{Q}_{\pi}(s, \pi_{c \hat{w}}(s)) \right)  \eta_{ \pi}(ds) + \intop \max_{a\in \Ac} \sum_{i=1}^{k}\left| \hat{Q}_{\pi}(s, e_i) - Q_{\pi}(s,e_i) \right|a_i\eta_{ \pi}(ds) \\	
		&\leq \intop \left(\hat{Q}_{\pi}(s, \pi_{c \hat{w}}(s)) \right)  \eta_{ \pi}(ds) + \intop \sum_{i=1}^{k}\left| \hat{Q}_{\pi}(s, e_i) - Q_{\pi}(s,e_i) \right|\eta_{ \pi}(ds)\\
		&= \intop \left(\hat{Q}_{\pi}(s, \pi_{c \hat{w}}(s)) \right)  \eta_{ \pi}(ds) +k \intop k^{-1}\sum_{i=1}^{k}\left| \hat{Q}_{\pi}(s, e_i) - Q_{\pi}(s,e_i) \right|\eta_{ \pi}(ds)\\
		&\leq\left(\hat{Q}_{\pi}(s, \pi_{c \hat{w}}(s)) \right)  \eta_{ \pi}(ds) +k \sqrt{\intop k^{-1}\sum_{i=1}^{k}\left( \hat{Q}_{\pi}(s, e_i) - Q_{\pi}(s,e_i) \right)^2\eta_{ \pi}(ds)} \\
		&\leq \intop \left(\hat{Q}_{\pi}(s, \pi_{c \hat{w}}(s)) \right)  \eta_{ \pi}(ds) + \epsilon_0.
	\end{align*}
	This implies,
	\begin{align*}
		\lim_{c\to \infty} \Bc(\pi_{c \hat{w}} \mid \eta_{ \pi}, J_{\pi}) \leq \lim_{c\to \infty} \intop \left(\hat{Q}_{\pi}(s, \pi_{c \hat{w}}(s)) \right)  \eta_{ \pi}(ds) + \epsilon_0 &= \intop \lim_{c\to \infty} \left(\hat{Q}_{\pi}(s, \pi_{c \hat{w}}(s)) \right)  \eta_{ \pi}(ds) + \epsilon_0 \\
		&= \intop \min_{a\in \Ac} \left(\hat{Q}_{\pi}(s, a) \right)  \eta_{ \pi}(ds) + \epsilon_0  \\
		&=\max_{\pi^+ \in \Pi} \Bc( \pi^+ \mid \eta_{ \pi}, J_{\pi} ) + \epsilon_0. 
	\end{align*}
	The first and second equality use the monotone convergence theorem together with the fact that, for each $s$, $\hat{Q}_{\pi}(s, \pi_{c \hat{w}}(s))\uparrow \max_{a\in \Ac}\hat{Q}_{\pi}(s, a)$. Since $\epsilon_0 <\epsilon$ we can choose a  $\hat{c}\in \mathbb{R}$ such that $\Bc(\pi_{\hat{c} \hat{w}} \mid \eta_{ \pi}, J_{\pi}) \leq \min_{\pi^+ \in \Pi}\Bc( \pi^+ \mid \eta_{ \pi}, J_{\pi} ) + \epsilon$.}
\end{proof}

\jb{The theory in \cite{agarwal2020optimality} is a tour-de-force, containing many ideas which are not reflected in the result above. Let us remark on two of them:
\begin{enumerate}
	\item \cite{agarwal2020optimality} treat generalizations of Example \ref{ex:linear_softmax} where policies are still stochastic but are not log-linear. If $\pi_{ \theta}(s,i) \propto \exp\{f_{\theta}(s,i)\}$ their assumption is that $Q_{\pi}(s,e_i) \approx w^\top \nabla_{\theta} f_{\theta}(s,i)$ for some choice of weights $w\in \mathbb{R}^d$. Roughly, this assumption ensures that through infinitesimally adjusting the parameter vector, 
	one can tilt the policies' action probabilities toward selecting actions with higher $Q$-values. Because it is local in nature, such a property appears to no longer imply closure of the policy class under policy improvement steps, which involves global properties of the policy class. 
	\item \cite{agarwal2020optimality} state their results in terms of a notion called \emph{transfer error.} This measures implicitly depends on both issues of approximation, as in \eqref{eq:accurate_Q}, and issues of distribution shift, as in our term $\kappa_{\rho}$. It is a very nice insight that this term is what is really needed in the analysis. 
	%\item \cite{agarwal2020optimality} provide a deep study of the convergence rates of natural gradient methods. This method overcomes an issue with softmax policies. Namely, the policy's action probabilities become extremely insensitive to changes in the parameter. There is a mismatch between vanialla gradient updates, which make small changes to the policy parameter, and the true constraint in local policy search, which is to make small changes to the policy. Natural gradient methods overcome this by performing steepest descent in an alternative metric.   
	%
	%Our theory handles cases with softmax style policies, but usually only when applied to objectives with minor entropy regularization (see for instance Example \ref{ex:linear_mdp}). This regularization produces a more standard (though nonconvex) optimization problem, where the optimum is attained by some setting of the policy parameter. 
\end{enumerate}}




%\subsection{Proof of Theorem \ref{thm: approximate closure}}
%\begin{proof}
%	Suppose $\theta$ is a stationary point of $\ell:\Theta \to \mathbb{R}$. 
%	
%	Let $S$ denote a random draw from $\eta_{\pi_\theta}$. Since condition \ref{cond: stationary} holds, Lemma \ref{lem: bellman for stationary points} implies 
%	\[ 
%	\E\left[ \left(J_{\pi_\theta}-TJ_{\pi_{\theta}}\right)(S) \right]  \leq   \left( \min_{\pi\in \Pi_{\Theta}}\E\left[ T_{\pi}J_{\pi_{\theta}}(S)  \right] - \E[TJ_{\pi_{\theta}}(S)]\right)=  \min_{\pi \in \Pi_{\Theta}}  \|   T_{\pi} J_{\pi_\theta} - TJ_{\pi_\theta} \|_{1, \eta_{\pi_\theta}}  := \epsilon.
%	\]
%	where the final equality uses $T_{\pi}J_{\pi_{\theta}} \succeq TJ_{\pi_\theta}$ for any $\pi \in \Pi_{\Theta}$. Then, we have
%	\begin{align*}
%		\ell(\pi_{\theta}) - \min_{\pi}\ell(\pi) = (1-\gamma)\sum_{s \in \Sc}\rho(s)\left( J_{\pi_{\theta}}(s) - J^*(s)\right) &= (1-\gamma)\| J_{\pi_{\theta}} - J^{*}\|_{1,\rho} \\
%		&\leq \kappa_\rho \|  J_{\pi_{\theta}} - TJ_{\pi_{\theta}} \|_{1, \rho} \\
%		&\leq \frac{\kappa_\rho}{(1-\gamma)} \|  J_{\pi_{\theta}} - TJ_{\pi_{\theta}} \|_{1, \eta_{\pi_{\theta}}} \\
%		&= \frac{\kappa_\rho \cdot \epsilon}{(1-\gamma)},
%	\end{align*}
%	where the first inequality follows from the definition of $\kappa_\rho$ as given in \eqref{def:concentrability_measure} and the second inequality uses that $\eta_{\pi_{\theta}} \geq (1-\gamma) \rho$ (by definition, see \eqref{eq: discounted_state_occupancy_measure}).
%\end{proof}


%So far, we have studied some classical dynamic programming problems that are ideally suited to policy iteration. The  key property we used is that certain structured policy classes were closed under policy improvement, so that exact policy iteration can be performed when only considering that policy class. Although simple structured policy classes are common in some applications of stochastic approximation based policy search \cite[e.g.][]{l1994stochastic,karaesmen2004overbooking,van2008simulation}, they are not widely used in the reinforcement learning literature. Instead, flexible policy classes like those parameterized by a deep neural network, a Kernel method \cite{rajeswaran2017towards}, or using state aggregation \cite{singh1995reinforcement,ferns2004metrics,bertsekas2019feature} are preferred. Here we conclude by presenting some preliminary but interesting progress toward understanding why, for highly expressive policy classes, any local minimum of the policy gradient cost function might be near-optimal. We conjecture this theory can at least be clearly instantiated in special case of state aggregation given in Appendix \ref{section:app_state_aggregation}. 
%
%Given an expressive policy class $\Pi_{\Theta}$,
%\begin{equation}\label{eq: approximate closure}
%\inf_{\pi \in \Pi_\Theta} \left\|T_{\pi}J_{\pi_{\theta}} - TJ_{\pi_{\theta}}\right\|_{1, \eta_{\pi_{\theta}}}  
%\end{equation} 
%measures the approximation error of the best approximate policy iteration update in the policy class to the current policy $\pi_{\theta}$. If $\Pi_\Theta$ were closed under policy improvement steps, the approximation error would be zero since there would exist a $\pi\in \Pi_{\Theta}$ such that  $T_{\pi}J_{\pi{\theta}}(s) = TJ_{\pi_{\theta}}(s)$ for every $s\in \Sc$. Equation \eqref{eq: approximate closure} measures the deviation from this ideal case, in a norm that weights states by the discounted-state-occupancy distribution $\eta_{\pi_\theta}$ under the policy $\pi_{\theta}$. Our formal result stated below in Theorem \ref{thm: approximate closure} bounds the optimiality gap at a stationary point by the approximation error in \eqref{eq: approximate closure}. Our result in Theorem \ref{thm: approximate closure} is reminiscent of results in the study of approximate policy iteration methods, pioneered by \cite{bertsekas1996neuro, munos2003error, antos2008learning, munos2008finite, bertsekas2011approximate}, among others. The primary differences are that (1) we directly consider an approximate policy class whereas that line of work considers the error in parametric approximations to the $Q$-function and (2) we make a specific link with the stationary points of a policy gradient method. The abstract framework of \citet{kakade2002approximately} is also closely related, though they do not study the stationary points of $\ell(\cdot)$. Recall the definition of the effective concentrability coefficient, $\kappa_\rho$, which relates errors in the Bellman equation to errors in the cost-to-go functions wieghted under the initial distribution $\rho$.


%The proof of Theorem \ref{thm:approximation} relates the Bellman  $\|TJ_{\pi_{\theta}}-J_{\pi_{\theta}}\|_{1,\eta_{\pi_{\theta}}}$  measured in this same norm is to the approximation error in \eqref{eq: approximate closure}. 
%
%But when does a small Bellman error $\| TJ_{\pi_{\theta}}-J_{\pi_{\theta}} \|_{1,\eta_{\theta}}$ imply the policy is near optimal?  We relate the Bellman error in the supremum norm to the average Bellman error over states sampled from the initial distribution $\rho$. Define $\Jc=\{ J_{\pi_{\theta}} : \theta \in \mathbb{R}^d \}$ and
%\begin{equation}\label{eq: exploration constant}
%\kappa_{\rho} = \inf_{J \in \Jc_{\Theta} }  \frac{\| TJ-J \|_{1,\rho}}{\| TJ-J \|_{\infty}}.
%\end{equation}
%The constant $\kappa_{\rho}$ measures the extent to which errors $TJ(s) - J(s)$ at some state must be detectable by random sampling, which depends both on the initial state distribution $\rho$ and on properties of the set of cost-to-go functions $\Jc_{\Theta}$. If the state space is finite, $\kappa_{\rho} \leq 1/(\min_{s\in \Sc} \rho(s))$ and naturally captures the ability of the distribution $\rho$ to uniformly explore the state space. This is similar to constants that depend on the worst-case likelihood ratio between state occupancy measures  \cite{kakade2002approximately}. However, those constants can equal zero for continuous state problems. It seems \eqref{eq: exploration constant} could still be meaningful for such problems\footnote{To give some intuition, consider quadratic function $f(s)=s^{\trans} K s$ on the unit sphere $\Sc=\{s\in \mathbb{R}^n: \| s\|_2 \leq 1\}$. For $\rho$ denoting the uniform density of $\Sc$, we have $\intop_{[0,1]} |f(s)| d\rho(s) \geq  (1/n)\| f\|_{\infty}$.} since it also captures regularity properties of $\Jc_\Theta$. The second part of Theorem 2 is reminiscent of results in the study of approximate policy iteration methods, pioneered by \cite{bertsekas1996neuro, munos2003error, antos2008learning, munos2008finite, bertsekas2011approximate}, among others. The primary differences are that (1) we directly consider an approximate policy class whereas that line of work considers the error in parametric approximations to the $Q$-function and (2) we make a specific link with the stationary points of a policy gradient method. The abstract framework of \citet{kakade2002approximately} is also closely related, though they do not study the stationary points of $\ell(\cdot)$. 


%\begin{thm}\label{thm: approximate closure}
%	Suppose Condition \ref{cond: stationary} holds. Then, if $\theta$ is a stationary point of $\ell(\cdot)$, 
%	\[ 
%	\ell(\pi_\theta) - \min_{\pi \in \Pi} \ell(\pi) \leq  \frac{\kappa_\rho}{(1-\gamma)}  \, \min_{\pi \in \Pi_{\Theta}}  \|   T_{\pi} J_{\pi_\theta} - TJ_{\pi_\theta} \|_{1, \eta_{\pi_\theta}}
%	\]
%\end{thm}
%\begin{proof}
%	Suppose $\theta$ is a stationary point of $\ell:\Theta \to \mathbb{R}$. Let $S$ denote a random draw from $\eta_{\pi_\theta}$. Since condition \ref{cond: stationary} holds, Lemma \ref{lem: bellman for stationary points} implies 
%	\[ 
%	\E\left[ \left(J_{\pi_\theta}-TJ_{\pi_{\theta}}\right)(S) \right]  \leq   \left( \min_{\pi\in \Pi_{\Theta}}\E\left[ T_{\pi}J_{\pi_{\theta}}(S)  \right] - \E[TJ_{\pi_{\theta}}(S)]\right)=  \min_{\pi \in \Pi_{\Theta}}  \|   T_{\pi} J_{\pi_\theta} - TJ_{\pi_\theta} \|_{1, \eta_{\pi_\theta}}  := \epsilon.
%	\]
%	where the final equality uses $T_{\pi}J_{\pi_{\theta}} \succeq TJ_{\pi_\theta}$ for any $\pi \in \Pi_{\Theta}$. Then, we have
%	\begin{align*}
%	\ell(\pi_{\theta}) - \min_{\pi}\ell(\pi) = (1-\gamma)\sum_{s \in \Sc}\rho(s)\left( J_{\pi_{\theta}}(s) - J^*(s)\right) &= (1-\gamma)\| J_{\pi_{\theta}} - J^{*}\|_{1,\rho} \\
%	&\leq \kappa_\rho \|  J_{\pi_{\theta}} - TJ_{\pi_{\theta}} \|_{1, \rho} \\
%	&\leq \frac{\kappa_\rho}{(1-\gamma)} \|  J_{\pi_{\theta}} - TJ_{\pi_{\theta}} \|_{1, \eta_{\pi_{\theta}}} \\
%	&= \frac{\kappa_\rho \cdot \epsilon}{(1-\gamma)},
%	\end{align*}
%	where the first inequality follows from the definition of $\kappa_\rho$ as given in \eqref{def:concentrability_measure} and the second inequality uses that $\eta_{\pi_{\theta}} \geq (1-\gamma) \rho$ (by definition, see \eqref{eq: discounted_state_occupancy_measure}).


%	We want to show this means $\|J_{\pi_\theta}-TJ_{\pi_{\theta}}\|_\infty$ is small. We have 
%	\begin{align*}
%	\|  J_{\pi_{\theta}} - TJ_{\pi_{\theta}} \|_\infty  \leq \kappa_\rho \|  J_{\pi_{\theta}} - TJ_{\pi_{\theta}} \|_{1, \rho} 
%	\leq \frac{\kappa_\rho}{1-\gamma} \|  J_{\pi_{\theta}} - TJ_{\pi_{\theta}} \|_{1, \eta_{\pi_{\theta}}} = \frac{\kappa_\rho \cdot \epsilon}{1-\alpha},
%	\end{align*}
%	where the first inequality directly applies the definition of $\kappa_\rho$ and the second inequality uses that $\eta_{\pi_{\theta}} \geq (1-\gamma) \rho$. From the contractivity of $T$, this implies (See \eqref{eq: near solutions to bellmans equation}), 
%	\[ 
%	\|  J_{\pi_{\theta}} - J^* \|_\infty \leq \frac{\kappa_\rho \cdot \epsilon}{(1-\gamma)^2}.
%	\]	
%	Of course, $\ell(\pi_{\theta}) - \min_{\pi}\ell(\pi) = (1-\gamma)\sum_{s}\rho(s)\left( J_{\pi_{\theta}}(s) - J^*(s)\right) \leq (1-\gamma) \| J_{\pi} - J^{*}\|_\infty$, so we reach our conclusion.   
%\end{proof}











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%
%\subsection{General results}
%
%Let us generalize \eqref{eq: convexity lqr} by introducing the weighted policy iteration objective 
%\begin{equation}\label{eq: weighted PI objective}
%C(\pi' \mid \eta, \pi)  = \E_{s\sim \eta}\left[  Q_{\pi}(s, \pi'(s))  \right] =\E_{s\sim \eta}\left[ (T_{\pi'} J_{\pi})(s)\right]  %= \E_{s\sim \eta}\left[  g(s, \pi'(s)) + \gamma\sum_{s'} P(s' \mid s, \pi'(s)) J_{\pi}(s') \right]  
%\end{equation}
%and overload notation to write $C(\theta \mid \eta, \pi)  = C(\pi_\theta \mid \eta, \pi)$. When $\eta$ is supported on all states, minimizing \eqref{eq: weighted PI objective} over all policies $\pi'$ is equivalent to classical policy iteration. Policy gradient methods are more closely related to the weighted policy iteration scheme
%\begin{equation}\label{eq: weighted constrained PI}
%\theta_{t+1} = \argmin_{\theta \in \Theta} C(\theta \mid \eta, \pi_{\theta_t}),
%\end{equation}  
%which preforms policy iteration style updates over the parameterized policy class. In general, this scheme may chatter endlessly. But, it is assured to converge to an optimal policy when the policy class is closed under policy improvement. As explained in the introduction, this condition is stronger than the requirement that $\Pi_{\Theta}$ contains an optimal policy. This is necessary, since Example \ref{ex: counterexample} shows policy gradient methods can get stuck in bad local minima even in extremely simple examples in which $\Pi_{\Theta}$ contains an optimal policy. However, Condition \ref{cond: closure} is much weaker than requiring the policy class is rich enough to contain nearly all policies, accommodating examples like linear policies in linear quadratic control or threshold policies in optimal stopping in which a certain class of policies is naturally aligned with the decision task. 
%\begin{cond}[Closure under policy improvement]\label{cond: closure}
%	For each $\pi \in \Pi_\Theta$ there is a $\pi^+ \in \Pi_\Theta$  such that
%	$T_{\pi^+} J_{\pi} = T J_{\pi}$. Equivalently, $Q_{\pi}(s, \pi^+(s)) = \min_{a \in \Ac(s)} Q_{\pi}(s,a)$ for all $s\in \Sc$.
%\end{cond}
%As a first order method, policy gradient methods require additional local optimization structure to succeed.  The following condition ensures that the weighted policy iteration problem is amenable to first-order optimization methods. It is worth emphasizing that the total cost function $\ell(\theta)$ is complicated and non-convex even in the simple examples we have considered so far. This is due to the multi-period nature of the decision problem, in which changes to the policy can have a compounding effect over time. Since it considers only a single period decision problem, the weighted PI objective $\theta' \mapsto C(\theta' | \eta_{\pi_{\theta}} , \pi_{\theta} )$ is typically much simpler: in the finite action example in Section \ref{sec: tabuluar} it is a linear function and in the LQ control problem in Example \ref{ex: lq control} it is a quadratic function. 
%
%\begin{cond}[Stationary points of the policy improvement objective]\label{cond: stationary}
%	For each $\pi \in \Pi_\Theta$ and distribution $\eta$ over $\Sc$, the function $\theta \mapsto C(\theta \mid \eta, \pi)$ has no sub-optimal stationary points. 
%\end{cond}
%
%\begin{thm}\label{thm: no bad stationary points general}
%	Suppose Conditions \ref{cond: closure} and \ref{cond: stationary} hold. Then, $\theta$ is a stationary point of $\ell(\cdot)$ if and only if $J_{\pi_\theta}=J^*$.  
%\end{thm}
%
%\subsection{A sharp connection between policy gradient and weighted policy iteration}
%
%The key to our approach is a sharp relation between between policy gradient methods and the weighted policy iteration scheme
%\begin{equation}\label{eq: weighted constrained PI}
%\theta_{t+1} = \argmin_{\theta \in \Theta} C(\theta \mid \eta, \pi_{\theta_t}),
%\end{equation}  
%which performs policy iteration style updates over the parameterized policy class. In light of the policy gradient theorem below, when $\Theta=\mathbb{R}^d$ is unconstrained, gradient descent on $\ell(\theta)$ with constant stepsize $\alpha$ is the iteration 
%\[ 
%\theta_{t+1} = \theta_t - \alpha \nabla_{\thetabar} \, C(\thetabar \mid \eta_{\pi_{\theta_t}}, \pi_{\theta_t}) \bigg\vert_{ \thetabar=\theta_t}. 
%\]  
%These methods differ in two ways.  First, policy gradient methods are incremental, making a parameter update based on a gradient of \eqref{eq: weighted PI objective} rather than solving it exactly. Second, the state-weighting $\eta$ is updated over time to reflect the states visited by the current policy. 
%
%The policy gradient theorem below could essentially be derived from the result of \cite{silver2014deterministic}. While they call this result a deterministic policy gradient theorem, it actually generalizes the stochastic policy gradient theorem of \cite{sutton2000policy} when $\pi_\theta(s)\in \Delta^{k-1}$ specifies a probability distribution over $k$ base actions. We provide a short proof sketch here, since the presentation of the result and the proof differ from \cite{silver2014deterministic} and \cite{sutton2000policy}. 
%\begin{lem}[Policy gradient theorem]\label{lem: PG theorem} $\ell(\theta)$ is differentiable and
%	\[
%	\nabla \ell(\theta) =  \frac{1}{1-\gamma} \nabla_{\thetabar} \, C(\thetabar \mid \eta_{\pi_\theta}, \pi_\theta) \bigg\vert_{\thetabar=\theta}  =  \sum_{s \in \Sc} \eta_{\pi_\theta}(s) \left[ \nabla_{\thetabar} \, Q_{\pi_\theta}(s, \pi_{\thetabar}(s)) \bigg\vert_{\thetabar = \theta} \right]. 
%	\]
%\end{lem}
%\begin{proof}[Proof sketch.]
%	Put $J_{\pi_\theta} \equiv J_\theta$, $Q_\theta\equiv Q_{\pi_\theta}$, $P_\theta\equiv P_{\pi_\theta}$ and $T_\theta\equiv T_{\pi_\theta}$ and $\eta_\theta \equiv \eta_{\pi_\theta}$. Then,
%	\begin{align*}
%	\ell(\thetabar) - \ell(\theta) = \rho \left(J_{\thetabar} -J_{\theta}\right) &= \rho \left( (I - \gamma P_{\thetabar})^{-1} (T_\thetabar J_\theta - J_\theta) \right)  \\
%	&= (1-\gamma)^{-1}  \eta_\thetabar \left( T_\thetabar J_\theta - J_\theta \right) \\
%	%&= \sum_{s} \eta_{\thetabar}(s)  \left( Q_{\theta}(s, \pi_{\thetabar}(s))- J_\theta(s) \right)
%	&= (1-\gamma)^{-1}\eta_\theta  \left( T_\thetabar J_\theta - J_\theta \right) +\underbrace{ (1-\gamma)^{-1}  \left[  (\eta_\thetabar - \eta_\theta)\left( T_\thetabar J_\theta - T_{\theta} J_\theta \right)\right]}_{ O(\|\thetabar - \theta \|^2_2)}.  
%	\end{align*}
%	Note that $\eta_{\theta} \left( T_{\thetabar} J_{\theta} \right)= \E_{s \sim \eta_\theta }\left[ Q_{\theta}(s, \pi_{\thetabar}(s))\right] = C(\thetabar \mid \eta_\theta, \pi_\theta)$.  Evaluating the derivative with respect to $\thetabar$ at $\thetabar=\theta$ yields the result. 
%	To make this rigorous, we need to justify the interchange of the expectation and derivative and to show formally that $\|\eta_\thetabar - \eta_\theta\|_\infty =O(\|\thetabar - \theta \|_2)$ and $\| T_\thetabar J_\theta - T_{\theta} J_\theta \|_\infty = O(\| \thetabar - \theta\|_2)$. See Appendix (\textcolor{red}{Add this}) for a detailed proof. 
%\end{proof}
%
%\subsection{Proof of Theorem \ref{thm: no bad stationary points general}}
%We first give a key lemma, which can be viewed as a Bellman-type equation that holds when the single period objective $\thetabar \mapsto C(\thetabar \mid \eta_{\pi_\theta}, \pi_\theta)$ has no bad stationary points. 
%\begin{lem}\label{lem: bellman for stationary points}
%	Suppose Condition \ref{cond: stationary} is satisfied. If $\theta$ is a stationary point of $\ell:\Theta \to \mathbb{R}$, then 
%	\[ 
%	\E\left[ J_{\pi_\theta}(S) \right] = \min_{\pi\in \Pi_{\Theta}}\E\left[ T_{\pi}J_{\pi_{\theta}}(S) \right],
%	\] 
%	where the expectation is over $S$ drawn from $\eta_{\pi_\theta}$. 
%\end{lem}
%\begin{proof} 
%	If $\theta$ is a stationary point of $\ell: \Theta \to \mathbb{R}$, then by \eqref{eq: policy gradient expression 2}, it is a stationary point of the function $\thetabar \mapsto C(\thetabar \mid \eta_{\pi_\theta}, \pi_\theta)$. Since Condition \ref{cond: stationary} holds, this means 
%	\begin{equation*}
%	C(\theta   \mid \eta_{\pi_\theta}, \pi_\theta) =  \min_{\thetabar \in \Theta} C(\thetabar \mid \eta_{\pi_\theta}, \pi_\theta).
%	\end{equation*}
%	Recalling the definition of $C(\theta   \mid \eta, \pi)$ in \eqref{eq: weighted PI objective} lets us rewrite both sides of this equation. To simplify the expressions, take $S$ to be a random state drawn from $\eta_{\pi_\theta}$. Then,
%	\begin{equation*}%\label{eq: no bad stationary points in term of bellman}
%	\E\left[ J_{\pi_\theta}(S) \right] = \E\left[ T_{\pi_\theta}J_{\pi_{\theta}}(S) \right] =  C(\theta   \mid \eta_{\pi_\theta}, \pi_\theta)= \min_{\theta'\in \Theta} C(\theta' \mid \eta_{\pi_\theta}, \pi_\theta) = \min_{\theta'\in \Theta}\E\left[ T_{\pi_{\theta'}}J_{\pi_{\theta}}(S) \right].
%	\end{equation*}
%\end{proof} 
%
%The proof of Theorem \ref{thm: no bad stationary points general} now follows as an immediate consequence of the closure assumption. 
%\begin{proof}[Proof of Theorem \ref{thm: no bad stationary points general}]
%	Suppose $\theta$ is a stationary point of $\ell(\cdot)$. Condition \ref{cond: closure} gives that for $S$ drawn from $\eta_{\pi_\theta}$,
%	\[
%	\min_{ \pi \in \Pi_\Theta} \E\left[ T_{\pi }J_{\pi_{\theta}}(S) \right] = \E\left[ T J_{\pi_\theta}(S) \right].
%	\]
%	Now, since Condition \ref{cond: stationary} holds, applying this together with Lemma \ref{lem: bellman for stationary points} shows  $\E\left[TJ_{\pi_\theta}(S) - J_{\pi_\theta}(S) \right] =0$. The difference in the expectation is non-negative by the basic fact \eqref{eq: bellman update reduces cost}. Therefore, we must have $TJ_{\pi_\theta}(S) = J_{\pi_\theta}(S)$ almost surely over $S$ drawn from $\eta_{\pi_\theta}$. Since $\eta_{\pi} \succeq (1-\gamma)\rho \succ 0$, this means $TJ_{\pi_\theta}(s)= J_{\pi_\theta}(s)$ for all $s\in \Sc$, which implies $J_{\pi_\theta} = J^*$. 
%\end{proof}
%
%
%
%\subsection{Beyond closed policy classes: nonstaionary policy classes}
%For finite horizon problems, we can guarantee that there are no spurious local minima for policy gradient under a much weaker condition. Rather than require the policy class is closed under improvement -- which would imply the policy class contains the optimal policy -- it is sufficient that the policy class contain the optimal policy. For this reason, our theory will cover as special cases a broad variety of finite horizon dynamic programming problems for which structured policy classes are known to be optimal. 
%
%Unfortunately, we do not have space in this short paper to develop specialized notation for finite horizon problems. We do so and give a more detailed treatment in Appendix \ref{section:app_finite_horizon}. We can state our formal result without rewriting our problem formulation, by a well known trick that treats finite-horizon time-inhomogenous MDPs as a special case of infinite horizon MDPs (see e.g. \cite{osband2017deep}). Under the following assumption, the state space factorizes into $H+1$ components, thought of as stages or time periods of the decision problem. Under any policy, any state will transition to some state in the next stage until stage $H+1$ is reached and the interaction effectively ends. This assumption on the policy class allows us to change the policy in stage $h$ without influencing the policy at other stages, essentially encoding time-inhomogenous policies. 
%\begin{assumption}\label{assumption: finite horizon}
%	Suppose the state space factors as $\Sc=\Sc_1 \cup \cdots \cup \Sc_{H} \cup \Sc_{H+1}$, where for a state $s\in \Sc_h$ with $h\leq H$, $\sum_{s'\in \Sc_{h+1}} p(s'| s, a)=1$ for all $a\in \Ac(s)$. The final subset $\Sc_{H+1}=\{T\}$ contains a single costless absorbing state, with $P(T| T,a)=1$ and $g(T,a)=0$ for any action $a$. The policy parameter $\theta=(\theta^{1}, \ldots, \theta^{H})$ is the concatenation of $H$ sub-vectors, where for any fixed $s\in \Sc_h$, $\pi_{\theta}(s)$ depends only on $\theta^{h}$. 
%\end{assumption}
%\begin{thm}\label{thm: finite horizon}
%	Suppose Assumption \ref{assumption: finite horizon} holds and, for any distribution $\eta$ over $\Sc$, $\theta \mapsto C(\theta \mid \pi^*, \eta)$ has no suboptimal stationary points. Suppose the parameterized policy class $\Pi_\Theta$ contains some optimal policy $\pi^*$. Then, any stationary point $\theta$ of $\ell:\Theta \to \mathbb{R}$ satisfies $\ell(\theta)=\ell(\pi^*)$. 
%\end{thm}
%\begin{proof}
%	Simple consequence of $\E\left[ J_{\pi_\theta}(S) \right] = \min_{\pi\in \Pi_{\Theta}}\E\left[ T_{\pi}J_{\pi_{\theta}}(S) \right]$\ldots     
%\end{proof}
%
%
%\subsubsection{Policy classes closed under approximate policy improvement}
%
%\begin{thm}
%	Suppose Condition \ref{cond: stationary} holds. Then, if $\theta$ is a stationary point of $\ell(\cdot)$, 
%	\[ 
%	\ell(\pi_\theta) - \min_{\pi \in \Pi} \ell(\pi) \leq  \frac{\kappa_\rho}{(1-\alpha)^2}  \, \min_{\pi \in \Pi_{\Theta}}  \|   T_{\pi} J_{\pi_\theta} - TJ_{\pi_\theta} \|_{1, \eta_{\pi_\theta}}
%	\]
%\end{thm}
%\begin{proof}
%	Suppose $\theta$ is a stationary point of $\ell:\Theta \to \mathbb{R}$. Let $S$ denote a random draw from $\eta_{\pi_\theta}$. Since condition \ref{cond: stationary} holds, Lemma \ref{lem: bellman for stationary points} implies 
%	\[ 
%	\E\left[ \left(J_{\pi_\theta}-TJ_{\pi_{\theta}}\right)(S) \right]  \leq   \left( \min_{\pi\in \Pi_{\Theta}}\E\left[ T_{\pi}J_{\pi_{\theta}}(S)  \right] - \E[TJ_{\pi_{\theta}}(S)]\right)=  \min_{\pi \in \Pi_{\Theta}}  \|   T_{\pi} J_{\pi_\theta} - TJ_{\pi_\theta} \|_{1, \eta_{\pi_\theta}}  := \epsilon.
%	\]
%	Here the first equality uses the nonegativity of $T_{\pi}J_{\pi_{\theta}} - TJ_{\pi_\theta}$. We want to show this means $\|J_{\pi_\theta}-TJ_{\pi_{\theta}}\|_\infty$ is small. We have 
%	\begin{align*}
%	\|  J_{\pi_{\theta}} - TJ_{\pi_{\theta}} \|_\infty  \leq \kappa_\rho \|  J_{\pi_{\theta}} - TJ_{\pi_{\theta}} \|_{1, \rho} 
%	\leq \frac{\kappa_\rho}{1-\alpha} \|  J_{\pi_{\theta}} - TJ_{\pi_{\theta}} \|_{1, \eta_{\pi_{\theta}}} = \frac{\kappa_\rho \cdot \epsilon}{1-\alpha},
%	\end{align*}
%	where the first inequality directly applies the definition of $\kappa_\rho$ and the second inequality uses that $\eta_{\pi_{\theta}} \geq (1-\gamma) \rho$. From the contractivity of $T$, this implies (See \eqref{eq: near solutions to bellmans equation}), 
%	\[ 
%	\|  J_{\pi_{\theta}} - J^* \|_\infty \leq \frac{\kappa_\rho \cdot \epsilon}{(1-\alpha)^2}.
%	\]	
%	Of course, $\ell(\pi_{\theta}) - \min_{\pi}\ell(\pi) = \sum_{s}\rho(s)\left( J_{\pi_{\theta}}(s) - J^*(s)\right) \leq \| J_{\pi} - J^{*}\|_\infty$, so we reach our conclusion.   
%\end{proof}
%
%
%
%




%\paragraph{Overview of \cite{agarwal2020optimality}}
%
%We provide a more detailed discussion of the relationship of our work to concurrent work by \cite{agarwal2020optimality}. Their paper provides many results. 
%
%They consider problems where $\Ac = \Delta^{k-1}$ consists of probability distributions over $k$ deterministic actions. For $a\in \Ac$, $Q_{\pi}(s,a)=\sum_{i=1}^{k} Q_{\pi}(s,e_i) a_i$, where the $i$th standard basis vector $e_i$ can be thought of as a deterministic action. Similarly, the advantage function $A_{\pi}(s,a)=-(Q_{\pi}(s,a) - J_{\pi}(s))$ is linear in $a$. Because we have taken the negative sign, the advantage $A(s,e_i)$ is positive if a action $i$ offers lower cost than sampling an action from $\pi(\cdot \mid s)$. 
%
%Consider the set of policies
%\[
%\pi_{\theta}(i|s) =  Z\exp\{ \phi(s,i)^\top \theta \}  \quad \text{where } \quad Z= \left(\sum_{j=1}^{k } \exp\{\phi(s,i)^\top  \theta\} \right)^{-1}.    
%\]
%\cite{agarwal2020optimality} focus primarily on a particularly clean algorithm for optimizing over policies in this case. A natural policy gradient method with an estimated critic forms an estimate of the actor
%\[ 
%\hat{w}_k=\argmin_{w}\| A_{\pi_{\theta_k}} - \Phi w \|_{k}^2 \quad \text{and} \quad \hat{A}_k = \Phi w_k = \argmin_{ A \in {\rm Col}(\Phi)} \| A_{\pi_{\theta_k}} - A\|_k^2
%\] 
%where $\| A\|_k^2 = \sum_{s,i} \eta_{\pi(s)} \pi(i|s) A(s,e_i)^2$ in the 2-norm weighted by the occupancy measure of the current policy and we assume, that nonzero weight is placed on each state-action pair so this is a norm. The natural policy gradient update is
%\[
%\theta_{k_1}=\theta_k + \alpha_k \hat{w}_k \quad \text{and} \quad \pi_{\theta_{k+1}}(i|s) \propto \pi_{\theta_k}(i|s) \exp\left\{ \alpha_{k} \hat{A}_k(s,e_i) \right\}. 
%\]
%These two formulas are equivalent, but one expresses it in terms of the policy parameter and one in terms of action probabilities. The action-probabilities are updated by an exponential--weights iteration which reinforces actions with positive advantage. 
%
%Under a realizability condition, each policy .
%\begin{cond}[Realizability]For each $\theta \in \mathbb{R}^d$, $A_{\pi_{\theta}} \in {\rm Col}(\Phi)$, the span of the columns of the $\Phi$. 
%\end{cond}
%It is not hard to see that this condition also implies the policy class is closed\footnote{Technically, policy iteration updates are contained only in the the closure of the policy class. The policy iteration update is typically a deterministic policy. Such a policy can be approximated arbitrarily well by a softmax policy but is not a softmax policy itself.} (Condition \ref{cond: closure}). To see this, notice that if one takes $\alpha_k \to \infty$, then $\pi_{\theta_{k+1}}$ converges to the policy iteration update to $\pi_{\theta}$. 
%
%\begin{enumerate}
%	\item They provide a detailed analysis of convergence rates, by deftly modifying ideas from the analysis of exponential weights type updates in online optimization.   
%	\item They generalize beyond linear parameterizations. In the generalization, one essentially requires that for each $\theta$, there exists a weight vector $w$ such that $A_{\pi_{\theta}}(s,e_i) = w \cdot \nabla \log \pi_{\theta}(i \mid s)$. The advantage function should be in the span of the policy's score function. When this is true, $\log \left(\frac{\pi_{\theta+\alpha w}(i|s)}{\pi_{\theta}(i|s)}\right) \approx w \cdot \nabla \log \pi_{\theta}(i \mid s) = A_{\pi_{\theta}}(s, e_i)$. Locally, the action probabilities are tilted toward those of a policy iteration update. 	
%	\item They provide detailed bounds on how much performance loss degrades if realizability is relaxed. This is stated in terms of a notion of transfer error, which requires that the least squares solution produces under the current policy's occupancy measure has low mean squared error under another a different evaluation distribution. 
%\end{enumerate}
%
%
%



==> app_bellman_background.tex <==
%!TEX root = policy_grad_optimality.tex

\section{Background on Bellman operators and policy iteration}
\label{sec: app_bellman_background}
We make repeated use of the basic element-wise inequalities
\begin{align}\label{eq: bellman update reduces cost}  
TJ \preceq T_{\pi}J    \quad \text{and} \quad TJ_{\pi} \preceq J_{\pi}
\end{align}
which hold for any policy $\pi$. The first inequality follows since $T$ minimizes over actions, $TJ(s) = \min_{a \in \Ac} Q(s,a)$ (see Equation \eqref{eq: q to bellman}). The second inequality follows by the first since $J_{\pi} = T_{\pi} J_{\pi}$. An important property that we repeatedly make use of is that for bounded cost-to-go functions, $J,J': \Sc \to \mathbb{R}$, both bellman optimality operator $T$ and the Bellman operator $T_{\pi}$ for a stationary policy $\pi$ are contraction operators with respect to the maximum norm with modulus $\gamma$. Precisely, 
\begin{align}
\|  J - J' \|_{\infty} \leq \gamma \|J - J' \|_{\infty}  && \| T_{\pi} J - T_{\pi}J' \|_{\infty} \leq \gamma \|J - J' \|_{\infty}.
\end{align}  
These operators are also monotone, meaning the element-wise inequality $J \preceq J'$ implies $TJ\preceq TJ'$ and $T_{\pi}J \preceq T_{\pi}J'$. A simple argument using contractivity of $T$ and $T_{\pi}$ together with the triangle inequality shows that for any bounded cost function $J_{\pi}$,
\begin{align}\label{eq: simple near solutions to Bellmans equation}
\| J_{\pi} - J^* \|_{\infty}\leq \frac{1}{1-\alpha} \| J_{\pi} - TJ_{\pi}  \|_{\infty} 
\end{align}
Using the definitions: $J_{\pi}=T_{\pi}J_{\pi}$ and $J^*=TJ^*$,
\begin{align*}
\norm{J_{\pi}-J^*}_{\infty} = \norm{T_{\pi}J_{\pi} - TJ_{\pi} + TJ_{\pi} - J^*}_{\infty} &\leq \norm{T_{\pi}J_{\pi} - TJ_{\pi}}_{\infty} + \norm{ TJ_{\pi} - TJ^*}_{\infty} \\
&\leq \norm{T_{\pi}J_{\pi} - TJ_{\pi}}_{\infty} + \gamma \norm{J_{\pi} - J^*}_{\infty}
\end{align*}
%\begin{align}\label{eq: simple near solutions to Bellmans equation}
%\|  J^* - J \|_{\infty}\leq \frac{1}{1-\alpha} \|  TJ - J \|_{\infty}  && \|  J_{\pi} - J \|_{\infty}\leq \frac{1}{1-\alpha} \|  T_{\pi}J - J \|_{\infty} 
%\end{align}
Equation \eqref{eq: simple near solutions to Bellmans equation} is very useful for our analysis as it indicates that near-solutions to the the Bellman equation $J^*=TJ^*$ must themselves be close to the optimal cost-to-go function $J^*$. The reinforcement learning literature widely uses versions of this inequality that are sensitive to the state distribution. For each bounded function $J$,
\begin{equation}\label{eq: near solutions to bellmans equation}
J - J_{\pi} = J-T_{\pi}J + T_{\pi}J - T_{\pi}J_{\pi} = J-T_{\pi}J + \gamma P_{\pi} \left( J - J_{\pi} \right) = \cdots = \sum_{t=0}^{\infty} \gamma^{t} P^t_{\pi} \cdot \left(J-T_{\pi}J\right).
\end{equation}
This expresses the difference of $J$ from $J_{\pi}$ in terms of the gap in Bellman's equations at the states visited by the policy $\pi$. An especially usesful case of this result arises when $\pi=\pi^*$ is an optimal policy in which case, 
\begin{equation}\label{eq: performance difference like relation}
J - J^* \preceq \sum_{t=0}^{\infty} \alpha^{t} P^t_{\pi^*} \cdot \left(J-T J\right),
\end{equation}
where the inequality uses \eqref{eq: bellman update reduces cost} to conclude $TJ\preceq T_{\pi*} J$. Related inequalities are sometimes called the \emph{Performance difference lemma} in the reinforcement learning literature, after crucial lemma of \cite{kakade2002approximately}.

The classic policy iteration algorithm due to \cite{howard1960dynamic} can be expressed compactly in terms of Bellman operators. Starting with an initial policy $\pi$, the algorithm first evalues evaluates the corresponding cost to go function $J_{\pi}$, and then finds the policy $\pi^+$ that attains the minimum in the Bellman update, $\pi^+ = \argmin_{\tilde{\pi}} T_{\tilde{\pi}} J_{\pi}$. Equivalently, this can be written as $T_{\pi^+} J_{\pi} = TJ_{\pi}$. One finds
\[ 
J_{\pi} \succeq T_{\pi^+} J_{\pi} \succeq T^{2}_{\pi^+} J_{\pi} \succeq \cdots \succeq J_{\pi^+}  
\]
where the first inequality applies \eqref{eq: bellman update reduces cost} and the rest follow by inductively applying $T_{\pi^+}$ to each side and using the monotonicity property of the Bellman operator. The first inequality is strict unless $J_{\pi} = T_{\pi^+} J_{\pi}= TJ_{\pi}$, in which case $J_\pi=J^*$ and $\pi$ is an optimal policy. From Equation \eqref{eq: near solutions to bellmans equation} or its more refined variant \eqref{eq: performance difference like relation}, we can see that each step of policy iteration leads to a substantial cost reduction unless the policy is near optimal. We conclude with a proof of a basic extension of Bellman's equation used in our analysis, which we restate here. Recall, $\eta_{\pi}$ to be the discunted state-occupancy measure under policy $\pi$ (see \eqref{eq: discounted_state_occupancy_measure}).
\onAvgBellman*
\begin{proof}
	First note that standard results in dynamic programming imply $J_{\pi} \succeq TJ_{\pi}$ and $J_{\pi} \succeq J^*$ (these in fact hold for any arbitrary policy $\pi$ and not just for $\pi \in \Pi_{\Theta}$). 
	
	Let $J : \Sc \to \mathbb{R}$ be an arbitray cost-to-go function such that $J\succeq 0$. Then, we have $\E[J(S)]= 0 \iff J=0$. To see this, note that the non-negativity of $J$ implies we must have $J(S)=0$ almost surely. Since $S\sim \eta_{\pi} \succeq (1-\gamma)\rho$ and by assumption, $\rho(s)>0$ for all $s\in \Sc$, $J(S)=0$ almost surely if and only if $J(s)=0$ for all $s\in \Sc$. Applying this with choice of $J=J_{\pi}-J^*$ or $J=J_{\pi}-TJ_{\pi}$ shows the average Bellman equation above is equivalent to the standard result, 
	\begin{equation*}
	J_{\pi} = J* \iff J_{\pi} = TJ_{\pi}.
	\end{equation*}
\end{proof} 



==> app_example_details_full.tex <==
%!TEX root = policy_grad_optimality.tex

%\section{Further details on LQ control}
%\label{app:LQ_details}
%\subsection{Proof of Lemma \ref{lem: bellman operators for LQ}:  Properties of the Bellman operator  }
%Recall the statement of Lemma \ref{lem: bellman operators for LQ}. 
%\LQBellman*
%\begin{proof}
%	These results can be found (or straightforwardly derived from) in any standard textbook on dynamic programming, for example \cite{bertsekas1995dynamic}. Details are only provided to aid the readers who might be unfamilier with some of the relevant material. 
%	
%	We prove each of the three claims in order. Consider any two cost-to-go functions $J, \bar{J} \in \Jc_{q}$ as:
%	\[
%	J(s) = s^\top K s \quad \bar{J}(s) = s^\top \bar{K} s
%	\]
%	defined for some $K, \bar{K} \succ 0$. Consider a stable linear policy $\pi_{\theta}(s) = \theta s$ for all $s \in \mathbb{R}^n$ and $\theta \in \mathbb{R}^{k \times n}$. Recall the set-up for LQ control from Section \ref{subsec:Motivation_LQ} where for action $a \in \mathbb{R}^k$, the state evolution follows $s' = As + Ba$ and the per-period cost $g(s,a)=a^\top R a + s^\top Cs$ for some cost matrices $R, C \succ 0$.
%	
%	\paragraph{Part (1)} By definition of the Bellman operator for policy $\pi_{\theta}$, we have:
%	\begin{align}
%	(T_{\pi_\theta} J)(s) &= (\theta s)^\top R (\theta s) + s^\top C s + \gamma J(As+B\theta s) \nonumber \\
%	&=s^\top \left( \theta^\top R \theta  +C + [A+B\theta]^\top K [A+B\theta] \right) s \label{eq:Bellman_LQ_equation}
%	\end{align} 
%	which simply follows by taking $a = \pi_{\theta}(s) = \theta s$. Note that $\theta^\top R \theta  +C + [A+B\theta]^\top K [A+B\theta] \succ 0$ as $R, C, K \succ 0$ and so $T_{\pi_\theta} J \in \Jc_{q}$.
%	Next, by definition, 
%	\begin{align}
%	\label{eq:Bellman_optimality_appendix}
%	 TJ(s) = \min_{a\in \mathbb{R}^k} \, \left[a^\top R a +s^\top C s +  \gamma(As+Ba)^\top K(As+Ba)\right]
%	 \end{align}
%	 Clearly, the minimizing action here is $a^*=-\gamma(R+\gamma B^\top K_{\theta} B)^{-1} B^\top K_{\theta} A s$ and therefore $TJ = T_{\pi_{\thetabar}} J$ for $\pi_{\thetabar}(s)=\thetabar s$ with $\thetabar =-\gamma(R+\gamma B^\top K B)^{-1} B^\top K_{\theta} A$. Using Equation \eqref{eq:Bellman_LQ_equation}, it is easy to see that $TJ \in \Jc_{q}$ as well. 
%	 
%	\paragraph{Part (2)} These inequalities can be checked immediately from the definitions of the Bellman operators. For $J\preceq \bar{J}$ and any $s$,
%	\begin{align*}
%	T_{\pi_{\theta}}J(s) &=  (\theta s)^\top R (\theta s) + s^\top C s + \gamma J(As + B \theta s) \\
%	&\leq (\theta s)^\top R (\theta s) + s^\top C s + \gamma \bar{J}(As + B \theta s) = T_{\pi_{\theta}}\bar{J}(s)
%	\end{align*}
%	We can similarly show that $TJ(s) \leq T \bar{J}(s)$ for all s, by minimizing over $a \in \mathbb{R}^k$ on both sides of the following inequality which holds as $J \preceq \bar{J}$.
%	\[
%	\left[a^\top R a +s^\top C s +  \gamma J(As+Ba)\right] \leq \left[a^\top R a +s^\top C s +  \gamma \bar{J}(As+Ba)\right]
%	\]
%	
%	\paragraph{Part (3)} As the per-period costs are unbounded for LQ control, there is some subtelty involed in showing the Bellman equaltions. We refer the readers to Chapter 4 in \citep{bertsekas1995dynamic} for a detailed proof which essentially uses the fact that per-period costs are non-negative. 
%	
%\end{proof}


\section{Example details.}
\label{appendix: example details}
%\subsection{Tabuluar MDPs with natural parameterization}\label{subsec:finite_mdp}
%We verify Condition \ref{cond: diff} for the tabular MDP case as formulated in Example \ref{ex:tabularMDPs}. Recall the policy class in that case is the set of all stationary randomized policies, $\Pi  = \{ \pi \in \mathbb{R}^{n\times k}_{+}  :  \sum_{i=1}^{k} \pi_{s,i}  =1  \,\, \forall s\in \{1,\cdots, n\}  \}$. As argued in Section \ref{sec:examples}, for any $\pi, \pibar \in \Pi$ and $s \in \Sc$, the Q-function is linear in $\pibar$, as $Q_{\pi}(s,\pibar(s)) = \langle Q_{\pi}(s, e_i), \pibar(s)$. Therefore, $\Bc(\pibar|\eta, J_{\pi}) = \sum_{s \in \Sc} \eta(s) \,  Q_{\pi}\left(s,\pibar(s)\right)$ is linear and hence differentiable in $\pibar$.
%
%Similarly, for any $s,s' \in \Sc$, the probability transition matrix $P_{\pi}(s'|s)  \in \R^{n \times n}$ is linear, $P_{\pi}(s'|s)=\langle P(s'|s, e_i), \pi'(s) \rangle$ and hence differentiable in $\pi'$. Also note that $P_{\pi}$ is a stochastic matrix, $\|P_{\pi}\|_{\infty} \leq 1$ and hence $(I-\gamma P_{\pi})$ is invertible. Therefore, $\eta_{\pi'}(\cdot) = (1-\gamma) \sum_{t=0}^\infty \gamma^t \rho P^t_{\pi'} = (1-\gamma) \rho (I-\gamma P_{\pi})^{-1}$ is differentiable\footnote{For finite states, it is easy to see that discounted state occupancy measure in \eqref{eq: discounted_state_occupancy_measure} can be simplified to this form.} in $\pibar$ (using the inverse function theorem). 

\subsection{Regularized finite state and action MDPs with nonlinear parameterization.}\label{app:softmax}
We continue the discussion of Example \ref{ex:vanishin_grads_softmax}. Given a feasible descent direction $D$, which by definition means  $\pi_{ \theta}+\alpha D \in \Pi$ is a feasible policy for sufficiently small $\alpha$, our goal is to verify that there exists $N$ solving the linear system $\left[ \frac{\partial \pi_{ \theta}}{\partial \theta} \right] N = D.$  For simplicity, imagine there is only a single state, so that a policy is described by the vector $(\pi_{\theta}(1),\cdots, \pi_{\theta}(k))$.
If there were multiple states, the same argument  could be repeated for each block of parameters corresponding to a distinct state. 	

 Since we have effectively fixed a choice of $\theta_1=0$ in Example \ref{ex:vanishin_grads_softmax},  $\left[ \frac{\partial \pi_{ \theta}}{\partial \theta} \right] N = D$ is a system of $k$ equations with $k-1$ variables, denoted $N=(N_2, \cdots, N_k)$. We first temporarily ignore the first linear equality and show we can solve the remaining $k-1$ equations: 
 $\frac{\partial \pi_{ \theta}(i) }{\partial \theta_2}N_2 + \cdots + \frac{\partial \pi_{ \theta}(i) }{\partial \theta_k}N_k = D_i$ for each $i\geq 2$. To see this, consider the  $(k-1)\times (k-1)$ submatrix of the Jacobian that comes from dropping the first row:
 \[
 \left[ \frac{\partial \pi_{ \theta}(i)}{\partial\theta_j } \right]_{i,j>2} = \begin{bmatrix}
 	\pi_{ \theta}(2)(1-\pi_{ \theta}(2)) & -\pi_{ \theta}(2)\pi_{ \theta}(3) & \cdots & -\pi_{ \theta}(2)\pi_{ \theta}(k)\\
 	-\pi_{ \theta}(2)\pi_{ \theta}(3)  & \pi_{ \theta}(3)(1-\pi_{ \theta}(3)) & \cdots & -\pi_{ \theta}(3)\pi_{ \theta}(k) \\   
 	\vdots & \vdots & \vdots & \vdots \\
 	-\pi_{ \theta}(2)\pi_{ \theta}(k) & -\pi_{ \theta}(3)\pi_{ \theta}(k) & \cdots & \pi_{ \theta}(k)(1-\pi_{ \theta}(k))
 \end{bmatrix}.
 \]
 This matrix is diagonally dominant and therefore non-singular, implying a solution to these $k-1$ linear equations exist.

We now show that the first linear equation is redundant and follows from the other $k-1$. In particular, we have 
\[
\sum_{j=2}^{k} \frac{\partial \pi_{ \theta}(1) }{\partial \theta_j}N_j = \sum_{j=2}^{k} \left( - \sum_{i=2}^{k} \frac{\partial \pi_{ \theta}(i) }{\partial \theta_j}N_j \right) =   \sum_{i=2}^{k}\left( - \sum_{j=2}^{k} \frac{\partial \pi_{ \theta}(i) }{\partial \theta_j}N_j \right) = -\sum_{i=2}^{k} D_i = D_1,
\]
where the first equality uses that $\pi_{\theta}(1)+\cdots+\pi_{ \theta}(k)=1$ and the final equality uses that $D_1 + \cdots + D_k = 0$ for any feasible descent direction. 

	
\subsection{LQ control}
\label{app:LQ}
\paragraph{Preliminaries.} We consider the LQ control problem as described in Example \ref{ex: lq control} with all the notations and assumptions introduced there. Even though this example doesn't fit our general formulation as the per period costs are not uniformly bounded, the important properties of Bellman operators that are used in our proofs hold when restricting attention to stable linear policies and quadratic value functions. Define the set of strictly convex quadratic cost to go functions as 
\[
\Jc_q = \{J : s\in \mathbb{R}^n \mapsto s^\top K s   \mid K \in \mathbb{R}^{n\times n},  K\succ 0  \}. 
\]


%Lemma \ref{lem: bellman operators for LQ} lists important properties of the Bellman operators that hold when restricting attention to stable policies. In this context, we define $\Jc_{\Theta_{\rm S}} = \{ J: s \in \R^n \mapsto s^\top K_{\theta} \, s \,\,|\,\, \theta \in \Theta_{\rm S}, K_{\theta} \in \R^{n \times n}, K_{\theta} \succ 0 \}$ to be the set of strictly convex quadratic cost-to-go functions corresponding to stable linear policies.

%Unfortunately, the per step costs for LQ control are not uniformly bounded. However, for stable policies, the Bellman operators still obey crucial properties like monotonicity and satisfy the Bellman equation. Let $\Jc_{\Theta_{\rm S}} = \{ J: s \in \R^n \mapsto s^\top K_{\theta} \, s \,\,|\,\, \theta \in \Theta_{\rm S}, K_{\theta} \in \R^{n \times n}, K_{\theta} \succeq 0 \}$ be the set of convex quadratic cost-to-go functions corresponding to stable policies. Then, 
\begin{restatable}[Bellman operators for LQ control]{lem}{LQBellman}
	\label{lem: bellman operators for LQ}
	Consider the LQ control problem formulated in Example \ref{ex: lq control}. For $J, \bar{J}\in \Jc_{q}$ and a stable linear policy $\pi\in \{ \pi_{ \theta} : \theta \in \Theta_S \} $, the following hold: 
	\begin{enumerate}
		\item (Closure on the set of quadratic cost-to-go functions)   $T_{\pi} J \in \Jc_{q}$ and $TJ \in \Jc_{q}$.
		\item (Monotonicity) If $J\preceq \bar{J}$, then $T_{\pi} J \preceq T_{\pi} \bar{J}$ and $TJ \preceq T \bar{J}$. 
		\item (Bellman equation) $J_{\pi} = T_{\pi}J_{\pi}$ and $J_{\pi}= \lim_{k\to \infty} T_{\pi}^k J$. Moreover, $J=TJ$ if and only if $J=J^*$. 
	\end{enumerate}
\end{restatable}
We use these properties extensively for our analysis but omit the proofs as these results can be found\footnote{It is worth mentioning that many references state such results in terms of the cost matrices instead of the functions $J\in \Jc_{q}$. For example, the uniqueness of solutions to the Bellman optimality equation within $\Jc_q$ is identical to the more common statement that the algebraic Riccatti equation has a unique positive definite solution.} in standard textbooks \cite[e.g.][]{bertsekas1995dynamic}. In addition, we use the following standard property of the trace operator repeatedly in our analysis. This can be found in \citep{fang1994inequalities}, for example. Let $\lambda_{\min}(A)$ and $\lambda_{\max}(A)$ denote the minimum and maximum eigenvalues of a symmetric matrix respectively. 
\begin{lem}\label{lem:trace}
For any two symmetric and positive semi-definite symmetric matrices $A, B \in \mathbb{R}^{n\times n}$,
\[
\lambda_{\min}(A) {\rm Trace}(B) \leq {\rm Trace} (AB) \leq \lambda_{\max}(A) {\rm Trace}(B)
\]
\end{lem} 

Finally, we use several times the following observation. Recall that the second moment matrix of the initial state, denoted $\Sigma_{\rho} = \E_\rho\left[ s_0 s_0^\top\right]$ is assumed to be finite and positive definite.
\begin{lem}\label{lem:lq_trace_argument}
	For a square matrix $M$ with Frobenius norm $\| M\|_{F} = \sqrt{{\rm Trace}(M^\top M)}$,  
	\[ 
	\lambda_{\min}\left( \Sigma_\rho  \right)  \| M\|_F^2  \leq \E_{\rho}\left[\| Ms_0\|_2^2 \right]\leq \lambda_{\max}\left( \Sigma_\rho  \right)  \| M\|_F^2. 
	\]
\end{lem}
\begin{proof}
	Using Lemma \ref{lem:trace} gives
\begin{align*}
	\E_{\rho}\left[\| Ms_0\|_2^2 \right] = \E_{\rho}\left[s_0^\top M^\top M s_0 \right] = \E\left[ {\rm Trace}\left(s_0^\top M^\top M s_0   \right)\right]   &= {\rm Trace}\left( M^\top M  \Sigma_\rho \right) \\
	&\geq  \lambda_{\min}\left( \Sigma_\rho  \right) {\rm Trace}(M^\top M)\\
	&= \lambda_{\min}\left( \Sigma_\rho  \right)  \| M\|_F^2.
\end{align*}
 An identical argument yields a corresponding upper bound.
\end{proof}

 

%Before giving a simple analysis of the stationary points of the policy gradient loss functions, we need some basic preliminaries that are specialized to linear quadratic control. First, notice that the LQ control example does not fit within our general problem formulation, which assumed single period costs to be uniformly bounded. For linear quadratic control, costs tend to infinity as the norm of the state grows and unstable policies will have infinite cost-to-go from some initial states. However, by restricting to quadratic cost-to-go functions and stable linear policies, important properties of Bellman operators still hold. The following lemma states the three properties we use. These are standard results\footnote{Many references state such results in terms of the cost matrices instead of the functions $J\in \Jc_{q}$. For example, the uniqueness of solutions to the Bellman optimality equation within $\Jc_{q}$ is identical to the more common statement that the algebraic Riccatti equation has a unique positive definite solution.}  and the proofs is omitted.  Define the set of strictly convex quadratic cost-to-go functions, as
%\[ 
%\Jc_q   = \{ J:s\in \mathbb{R}^n \mapsto s^\top K s  \,\big\vert \,\, K\in \mathbb{R}^{n\times n}\, ,\, K\succ 0   \,\,   \}. 
%\]

%With this choice, for any cost-to-go function of the form $J(s)=s^\top K s$, we have $\|J(s)\|_{\infty, w} = \| K \|_2$, where $ \| K \|_2$ is the spectral norm of the matrix $K$. 
%a natural measure of the magnitude of a cost-to-go function. 
%The next result confirms the Bellman operator $T_{\pi_\theta}$ corresponding to a stable linear policies and the Bellman optimality operator $T$ are monotone contraction operators with respect to this weighted maximum norm. For completeness, we provide details in Appendix (\textcolor{red}{Add this}).  %Let $S^n_{++}$ denote the set of $n$ by $n$ symmetric positive definite matrices and 
%Take $\Jc_{q}$ to be the set of quadratic cost-to-go functions. That is, $J \in \Jc_q$ if and only if there exists some symmetric positive definite $K\in \mathbb{R}^{n\times n}$ such that $J(s)=s^\top K s$ for all $s$. 
%We equip this vector space with the induced norm $\| J \| = \sup_{x : \| x\|\leq 1} |J(x)|$. If  $J(s)=s^\top K s$, then $\| J\|$  is the spectral norm or maximum singular value of $K$. For the Bellman operator $T_{\pi_\theta} : \Jc_q \to \Jc_q$ corresponding to a stable linear policy and the Bellman optimality operator $T: \Jc_q \to \Jc_q$ map quadratic cost-to-go functions to quadratic cost to go functions. They are defined by 


%\begin{restatable}[Bellman operators for LQ control]{lem}{LQBellman}
%	\label{lem: bellman operators for LQ}
%	Consider the linear quadratic control problem formulated in Example \ref{ex: lq control}. For $J, \bar{J}\in \Jc_q$ and a stable linear policy $\pi_{\theta}$, the following properties hold: 
%	\begin{enumerate}
%		\item (Closure on the set of quadratic cost functions) $T_{\pi_\theta} J \in \Jc_q$  and  $TJ \in \Jc_q$. 
%		\item (Monotonicity) If $J\preceq \bar{J}$ then $T_{\pi_\theta} J \preceq T_{\pi_\theta} \bar{J}$ and $TJ \preceq T \bar{J}$.
%		\item (Bellman equation) $J_{\pi_{\theta}} = T_{\pi_{\theta}}J_{\pi_{\theta}}$ and $J_{\pi_{\theta}}= \lim_{k\to \infty} T_{\pi_{\theta}}^k J$. Moreover, $J=TJ$ if and only if $J=J^*$. 
%	\end{enumerate}
	
	%Fix $R\in S^n_{++}$, $C\in S_{++}^n$ and $A, B \in \mathbb{R}^{n \times n}$. For any function $f: \mathbb{R}^n \to \mathbb{R}$ let $\|f\|_2 = \sup_{x: \| x\|_2 \leq 1}   |f(x)| $ denote the operator norm. Let $\theta$ satisfy $ \| A+B\theta \|_2 \leq 1$. For each $J\in \Jc_q$, define 
	%	\begin{align*}
	%	(T_{\pi_\theta} J)(s) &= (\theta s)^\top R \theta s + s^\top C s + \gamma J(As+B\theta s) \\
	%	(TJ)(s) &= \min_{a\in \mathbb{R}^k} \, a^\top R a + s^\top C s + \gamma J(As+Ba ).
	%	\end{align*}
%\end{restatable}



%\subsection{Cost function for LQ control is smooth on sublevel sets}

\paragraph{Stability in LQ control.}
The following lemma adapts classical understanding of stability in linear dynamical systems to our setting, which considers the cumulative discounted cost incurred from a random initial state. 
\begin{lem}\label{lem:lq_stability}  In the LQ control problem formulated in Example \ref{ex: lq control}, 
	$\ell(\theta)<\infty$ if and only if $\theta \in \Theta_S$. 
\end{lem}
\begin{proof}
	The average cost can be written as
	\[
	\ell(\theta) = (1-\gamma)\E^{\pi_{\theta} }_{\rho}\left[ \sum_{t=0}^{\infty} \gamma^t \left( s_t^\top \left[ \theta R \theta + C  \right] s_t \right)  \right]  
	\]
	where the expectation is over $s_0\sim \rho$ and it is implicit that the state evolves according to the linear dynamical system $s_{t+1}=(A+B\theta)s_t$ for $t=0,1\cdots$. 	
     We can bound $\ell(\theta)$ above and below as, 
	\[ 
	\lambda_{\min}(\theta R \theta + C )  \E^{\pi_{\theta} }_{\rho}\left[\sum_{t=0}^{\infty}  \| \sqrt{\gamma} s_t  \|_2^2\right]\leq (1-\gamma)^{-1}\ell(\theta) \leq \lambda_{\max}(\theta R \theta + C )  \E^{\pi_{\theta} }_{\rho}\left[\sum_{t=0}^{\infty}  \| \sqrt{\gamma} s_t  \|_2^2\right]. 
	\]
	 Since $s_t= \left[A+B\theta\right]^t s_0$, applying Lemma \ref{lem:lq_trace_argument} at each timestep with a choice of $M=(\sqrt{\lambda}\left[A+B\theta\right] )^t$ yields 
	 \[ 
	 \lambda_{\min}\left( \Sigma_\rho  \right) \sum_{t=0}^{\infty }  \| (\sqrt{\gamma}\left[A+B\theta\right] )^t \|_F^2 \leq \E^{\pi_{\theta} }_{\rho}\left[\sum_{t=0}^{\infty}  \| \sqrt{\gamma} s_t  \|_2^2\right] \leq \lambda_{\max}\left( \Sigma_\rho  \right)   \sum_{t=0}^{\infty }\| (\sqrt{\gamma}\left[A+B\theta\right] )^t \|_F^2.
	 \] 
	 We recall Gelfand's formula, which says that for any square matrix $M$ with spectral radius $\rho(M)$ and any matrix norm $\|\cdot\|$, we have $\| M^t\|^{1/t} \to \rho(M)$ as $t\to \infty$. This implies  $\sum_{t=0}^{\infty }\| (\sqrt{\gamma}\left[A+B\theta\right] )^t \|_F^2$ is finite if and only if $\sqrt{\gamma}\left[A+B\theta\right]$ has spectral radius strictly less than one.  
\end{proof}



\paragraph{Smoothness properties for LQ control.} We do not verify Condition \ref{cond: diff} for LQ control as it is well known that for any stable policy, $\ell(\theta)$ is twice continuously differentiable \citep{rautert1997computational}. Studying only stable linear policies is appropriate, as we argued in Section \ref{sec:Motivation_LQ} that beginning with a stable linear policy, iterates produced by first order methods with appropriate step-sizes are assured to stay in the sublevel set, which by Lemma \ref{lem: lqr loss function} only contain stable policies. %The following result strengthens the conclusion that  $\ell(\theta)$ is twice continuously differentiable to show its Hessian is uniformly bounded on sublevel sets. 



\LQloss*
\begin{proof}
That any sublevel set only contains stable policies, i.e. $C_{\alpha} \subseteq \Theta_{\text{S}}$, is an immediate consequence of Lemma \ref{lem:lq_stability}. With a little bit of algebraic simplification (see \cite{rautert1997computational}), it is easy to see that $\ell(\theta)$ is twice continuously differentiable for any $\theta \in \Theta_{\text{S}}$ and hence over sublevel sets (as $C_{\alpha} \subseteq \Theta_{\text{S}})$. 



 We show that sublevel sets are compact by showing that they are closed and bounded. As $\ell(\cdot)$ is continuous over $\Theta_{\rm S}$, by definition its sublevel sets are closed. We show $\ell(\theta)$ is a coercive function, meaning  $\lim_{\|\theta\| \to \infty} \ell(\theta) = \infty$. (By the equivalence of norms in finite dimensional spaces, the definition does not depend on the choice of matrix norm.)  By definition, sublevel sets of a coercive function are bounded, (see for example \citep{peressini1988mathematics}) so this completes our argument.
 To show $\ell(\cdot)$ is coercive, we lower bound it using Lemma \ref{lem:lq_trace_argument} as 
 \begin{align*}
 (1-\gamma)^{-1}\ell(\theta) = \E_{\rho} \left[ \sum_{t=0}^\infty \gamma^t s_t^\top (\theta^\top R \theta + C)s_t \right] \geq \E_{\rho}\left[ (\theta s_0)^\top R (\theta s_0) \right] &\geq \lambda_{\min}(R) \E_{\rho}\left[ \| \theta s_0\|_2^2\right] \\
 &\geq \lambda_{\min}(R) \lambda_{\min}(\Sigma_\rho) \| \theta \|_F^2,  
 \end{align*}
 which clearly tends to infinity as $ \| \theta \|_F^2 \to \infty$. 
 
 To prove the final claim, observe that as $\ell(\cdot)$ is twice continuously differentiable, $\|\nabla^2 \ell(\theta) \|_2$ is a continuous function. Because any sublevel set $C_{\alpha}$ of $\ell(\cdot)$ is compact, the Extreme Value Theorem implies $\|\nabla^2 \ell(\theta) \|_2$ is bounded on any sublevel set, i.e. $\max_{\theta \in C_{\alpha}} \|\nabla^2 \ell(\theta) \|_2 < \infty$.
 

\end{proof}


\paragraph{Optimality of stationary points for LQ control: Proof of Lemma \ref{lem: lqr stationary}.}

\LQstationary*
\begin{proof}
	If $\theta$ defines an optimal policy, then the first order necessary conditions imply $\nabla \ell(\theta)=0$. Now consider a sub-optimal stable linear policy $\pi_{\theta}$ and let $\pi_{\thetabar}$ be the policy iteration update to $\pi_{\theta}$. That is, $\thetabar$ satisfies 
	$T_{\pi_{\thetabar}} J_{\pi_{\theta}} = T J_{\pi_{\theta}}$. Set $\theta^{\alpha} = (1-\alpha)\theta + \alpha \thetabar$ for some $\alpha \in [0,1]$. As both $\pi_{\theta}$ and $\pi_{\thetabar}$ are linear policies, this implies, $\pi_{\theta^\alpha}(s)=(1-\alpha)\theta s + \alpha \thetabar s$ . For every $s\in \mathbb{R}^n$,
	\begin{align}
	T_{\pi_{\theta^{\alpha}}} J_{\pi_{\theta}}(s) = Q_{\pi_{\theta}}(s,\pi_{\theta^{\alpha}}(s) ) &=Q_{\pi_{\theta}}(s, (1-\alpha)\theta s+ \alpha \thetabar s ) \nonumber \\
	&\leq (1-\alpha)Q_{\pi_{\theta}}(s, \theta s) + \alpha  Q_{\pi_{\theta}}(s, \thetabar s) \nonumber \\
	& = (1-\alpha) 	T_{\pi_{\theta}} J_{\pi_{\theta}}(s) + \alpha	T_{\pi_{\thetabar}} J_{\pi_{\theta}}(s) \nonumber \\
	&= (1-\alpha) J_{\pi_{\theta}}(s) + \alpha	T J_{\pi_{\theta}}(s) \nonumber \\
	&=J_{\pi_{\theta}}(s) - \alpha \left(J_{\pi_{\theta}}(s)- T J_{\pi_{\theta}}(s)\right) \label{eq: LQ cost reduction descent direction}
	\end{align}
	where the first inequality uses that $a\mapsto Q_{\pi_{\theta}}(s,a)$ is convex, as noted in Section \ref{sec:Motivation_LQ}. As $J_{\pi_{\theta}} \succeq TJ_{\pi_{\theta}}$, we conclude from \eqref{eq: LQ cost reduction descent direction} that $J_{\pi_{\theta}} \succeq T_{\pi_{\theta^{\alpha}}} J_{\pi_{\theta}}$. Repeatedly applying the Bellman operator and using the monotonicity property gives,
	\begin{equation}
		\label{eq: LQ Appendix monotonicity}
	J_{\pi_{\theta}} \succeq T_{\pi_{\theta^{\alpha}}} J_{\pi_{\theta}} \succeq T_{\pi_{\theta^{\alpha}}}^2 J_{\pi_{\theta}} \succeq \cdots \succeq \lim_{k \to \infty} T^k_{\pi_{\theta^{\alpha}}}J_{\pi_{\theta^\alpha}} = J_{\pi_{\theta^\alpha}}.
	\end{equation}
	As, $J_{\pi_{\theta^\alpha}} \preceq J_{\pi_{\theta}}$, the interpolated policy $\pi_{\theta^{\alpha}}$ is stable. Then from \eqref{eq: LQ cost reduction descent direction} and \eqref{eq: LQ Appendix monotonicity}, we have 
	\[ 
	\frac{J_{\pi_{\theta^\alpha}}- J_{\pi_{\theta}} }{\alpha} \preceq \frac{ T_{\pi_{\theta^{\alpha}}}J_{\pi_{\theta}}- J_{\pi_{\theta}} }{\alpha} \preceq \left[ TJ_{\pi_{\theta}}-J_{\pi_{\theta}} \right].
	\]
	Multiplying each side by $(1-\gamma)$, taking the expectation over $s_0$ drawn from the initial distribution $\rho$, and then taking $\alpha \to 0$ gives 
	\begin{equation}
		\label{eq:LQ descent}
	\frac{d}{d\alpha} \ell(\theta^\alpha) \bigg\vert_{ \alpha=0}  \leq  (1-\gamma) \, \E_{\rho} \left[ TJ_{\pi_{\theta}}(s_0)- J_{\pi_{\theta}}(s_0) \right] = -(1-\gamma) \E_{\rho}\left[ E(s_0) \right]    
	\end{equation}
where we have denoted the error in Bellman's equation by $E(s) \triangleq J_{\pi_{\theta}}(s) - TJ_{\pi_{\theta}}(s)$. 

We know $E(s)\geq 0$ for all $s$ because $J_{\pi_{\theta}} \succeq T J_{\pi_{\theta}}$ and the inequality is strict at some $s$ because the policy $\pi_{ \theta}$ is sub-optimal by assumption and therefore  $J_{\pi_{\theta}} \neq T J_{\pi_{\theta}}$. We argue that $\E_{\rho}[E(s_0) ]>0$, showing that the right hand side of \eqref{eq:LQ descent} is negative and hence $\theta$ cannot be a stationary point. To show this, we first observe that, since $J_{\pi_{\theta}}  \in \Jc_{q}$ and $T J_{\pi_{\theta}} \in \Jc_{q}$ are both quadratic functions (See Lemma \ref{lem: bellman operators for LQ}), $E(s)$ is a quadratic function. We can then write $E(s) = s^\top K s$ for some symmetric matrix $K$ satisfying $K\succeq 0$ and $K\neq 0$. Applying Lemma \ref{lem:lq_trace_argument} gives,
\[
\E_{\rho}\left[ E(s_0) \right] =   \E_{\rho}\left[ s_0^\top K s_0 \right] = \E_{\rho}\left[ \|  K^{1/2} s_0\|_2^2 \right] \geq \lambda_{\min}(\Sigma_\rho) \| K^{1/2}\|_F^2 =\lambda_{\min}(\Sigma_\rho) \cdot {\rm Trace}(K) >0.   
\] 

%We know $E(s)\leq 0$ for all $s$ as $J_{\pi_{\theta}} \succeq T J_{\pi_{\theta}}$, and $E(s)<0$ for some $s$ since $\pi_{ \theta}$ is suboptimal 

%	We show that for a stable suboptimal policy $\pi_{\theta}$, moving along the policy iteration update as in \eqref{eq:LQ descent}, is a feasible descent direction and therefore $\theta$ cannot be a stationary point. Consider the error in Bellman's equation $E(s) \triangleq TJ_{\pi_{\theta}}(s) - J_{\pi_{\theta}}(s)$. We know $E(s)\leq 0$ for all $s$ as $J_{\pi_{\theta}} \succeq T J_{\pi_{\theta}}$. We argue that $\E_{\rho}\left[ E(s_0)\right] < 0$ by using the fact that $\Sigma :=\E_{\rho}\left[ s_0 s_0^\top \right]$ is assumed to be positive definite. 
%	 To show this, note that as $J_{\pi_{\theta}}  \in \Jc_{q}$ and $T J_{\pi_{\theta}} \in \Jc_{q}$, $E(s)$ is clearly a quadratic function. Since $E(s) \leq 0$, it can be written as $E(s)=  s^\top K s$ for some symmetric $K\preceq 0 $ with $K\neq 0$. Therefore, the matrix $K$ has spectral decomposition $K= \sum_{i=1}^{n} \lambda_i q_i q_i^\top$, where $(q_1, \cdots, q_n)$ is an orthonormal basis of eigenvectors, each eigenvalue is non-positive, and at least one eigenvalue is strictly negative as $E(s)<0$ for some state $s$. We get our result by noting, 
%	\[
%	\E_{\rho} \left[ E(s_0) \right] = \sum_{i=1}^{n} \lambda_i  \E_{\rho} \left[ (q_i^\top s_0)^2 \right] = \sum_{i=1}^{n} \lambda_i  q_i^\top  \Sigma q_i<0.
%	\]

%	 Clearly, if $\theta$ is suboptimal, $E(s) < 0$ for some state $s$. We argue that this also implies $\intop \left[ TJ_{\pi_{\theta}}(s)- J_{\pi_{\theta}}(s) \right] d\rho(s) <0$ as $\Sigma :=\E_{s\sim \rho}\left[ ss^\top \right]$ is assumed to be positive definite.
%	 
%	  That $\E_{s\sim \rho}[E(s)]<0$ follows because $\Sigma :=\E_{s\sim \rho}\left[ ss^\top \right]$ is assumed to be positive definite. To show this note that $E(s)$ is the difference in quadratic functions, so it is a quadratic function and we can write $E(s)=  s^\top K s$ for some symmetric $K\preceq 0 $ with $K\neq 0$. The matrix $K$ has spectral decomposition $K= \sum_{i=1}^{n} \lambda_i q_i q_i^\top$, where $(q_1, \cdots, q_n)$ is an orthonormal basis of eigenvectors, each eigenvalue is non-positive, and at least one eigenvalue is strictly negative. We have $\E_{s\sim \rho}[ E(s)] = \sum_{i=1}^{n} \lambda_i  \E_{s\sim \rho} [(q_i^\top s)^2] = \sum_{i=1}^{n} \lambda_i  q_i^\top  \Sigma q_i<0$.
\end{proof} 



\paragraph{Concentrability coefficient for LQ control.}
We first recall the lemma statement from Section \ref{sec:concentrability}. 
\concentrabilityLQ*

The proof leverages the performance difference lemma, described in Subsection \ref{subsec:app_general_results} and equation \eqref{eq: perf diff 2} in particular. Here, to make precise the result used in the proof, we state an analogue of that formula in linear quadratic control, which restricts to  stable policies to rule out divergent sums. The proof is essentially identical to that leading to \eqref{eq: perf diff 2} and is therefore omitted.  Observe that, since the dynamics are deterministic with states evolving according to $s_{t+1} = (A+B\thetabar) s_t$, all randomness is due to the initial state $s_0$ drawn from $\rho$.  
\begin{lem}[Performance difference lemma for LQ control] Consider the LQ control problem formulated in Example \ref{ex: lq control}. For any $\theta, \thetabar\in  \Theta_S$,
	\begin{equation*}
	\ell(\thetabar) - \ell(\theta) = (1-\gamma) \E_{\rho}^{\pi_{\thetabar}}\left[  \sum_{t=0}^{\infty} \gamma^t \left( T_{\pi_\thetabar}J_{\pi_\theta}(s_t) - J_{\pi_\theta}(s_t) \right)  \right] = \intop \left[ T_{\pi_{\thetabar}}J_{\pi_\theta} -J_{\pi_{\theta}} \right] d\eta_{\pi_{\thetabar}}.
\end{equation*}
\end{lem}

%	\begin{equation}
%	%	\label{eq: perf diff 1}
%	\E^{\pi}_{\nu} \left[ J_{\pi_{\thetabar}}(s_0) - J(s_0) \right] = \E^{\pi_{\thetabar}}_{\nu} \left[ \sum_{t=0}^{\infty} \gamma^t \left[ T_{\pi_{\thetabar}}J(s_t) - J(s_t)  \right] \right].
%\end{equation}
%
%
%\begin{proof}
%	The argument is essentially identical to that leading to \eqref{eq: perf diff 2} and is therefore omitted. 
%\end{proof}


\begin{proof}[Proof of Lemma \ref{lemma: concentrability LQ}]
	For any $\pi_{\theta} \in \Theta_{\rm S}$, by Lemma \ref{lem: bellman operators for LQ}, $J_{\pi_{\theta}} \in \Jc_{q}$ and $TJ_{\pi_{\theta}} \in \Jc_{q}$. Therefore $J_{\pi_{\theta}} - TJ_{\pi_{\theta}}\in \Jc_{q}$, which means there exists symmetric $K\in \mathbb{R}^{n\times n}$ such that $J_{\pi_{\theta}}(s) - TJ_{\pi_{\theta}}(s)=s^\top K s$ for all $s$.  Since $J_{\pi_{\theta}} \succeq TJ_{\pi_{\theta}}$, we have that $K\succeq 0$. We get 
	\begin{equation}\label{eq: lq control rhs concentrability}
	\| J_{\pi_{\theta}}- T J_{\pi_{\theta}} \|_{1,\rho} = \E_{\rho} \left[ J_{\pi_{\theta}}(s_0) - T J_{\pi_{\theta}}(s_0) \right] = \E_{\rho} \left[ s_0^\top K s_0 \right] = {\rm Trace}(K \Sigma_\rho).
	\end{equation}
	This simplifies the right hand side in the definition of $\kappa_{\rho}$. To simplify the left hand side, we use the performance difference lemma above (with a choice $\thetabar=\theta^*$), 
	\begin{align*}
		(1-\gamma )\|  J_{\pi_{ \theta}} - J^*\|_{1,\rho}  = -  \left( \ell(\theta^*) - \ell(\theta) \right) =   \intop \left[ J_{\pi_{\theta}} - T_{\pi_{\thetabar}}J_{\pi_\theta} \right] d\eta_{\pi_{\theta^*}} &\leq  \intop \left[ J_{\pi_{\theta}} - TJ_{\pi_\theta} \right] d\eta_{\pi_{\theta^*}}\\
		& = \E_{\eta_{\theta^*}}\left[s_0^\top K s_0 \right] \\
		&= {\rm Trace}\left( K \Sigma_{\eta_{ \pi_{\theta^*}}} \right), 
	\end{align*}
	 where the inequality used that $TJ \preceq T_{\pi_{ \theta^*}} J$ holds for all cost-to-go functions $J$.  Combining this with \eqref{eq: lq control rhs concentrability} and applying Lemma \ref{lem:trace} gives, 
	 \[
	 \frac{	\|  J_{\pi_\theta}  - J^* \|_{1,\rho} }{\|  J_{\pi_\theta}  - TJ\|_{1, \rho}} \leq \frac{1}{1-\gamma} \cdot \frac{ {\rm Trace}(K \Sigma_{\eta_{ \pi_{\theta^*}}}) }{{\rm Trace}(K \Sigma_\rho)  } \leq \frac{1}{1-\gamma} \cdot \frac{ \lambda_{\max} \left( \Sigma_{\eta_{ \pi_{\theta^*}}} \right)  }{ \lambda_{\min}(\Sigma_\rho) }. 
	 \]
\end{proof} 


%\concentrabilityLQ*


\subsection{Optimal Stopping}
\label{subsec:app_optimalstopping}
We now consider the optimal stopping problem as described in Example \ref{ex:stopping}, continuing with the notation and assumptions introduced there. Recall that in our formulation, for each context $x \in \Xc$, the offer distribution is assumed to have a density, $q_x(\cdot)$, with continuous derivative and support $\{ y \in \mathbb{R}  : q_x(y)>0 \}=(y_{\min}, y_{\max})$ where $y_{\min} >0$. We set $\Yc = [y_{\min}, y_{\max}]$. We also assume the initial distribution places zero probability on trivial instances that begin in the terminal state (i.e $\rho(\tau)=0$) and factorizes over continuation states as $\rho(x,dy)=\nu(x) q_x(y)dy$ where $\nu(x) > 0$ for all $x \in \Xc$. 

\paragraph{Preliminaries and notation.} % and $P_{\theta}:= P_{\pi_{\theta}}$ for any $\theta \in \Theta$. 
Technically, the state at time $t$ consists of both the context $x_t$ and the offer $y_t$. But since $y_t$ depends only on $x_t$ and not on the previous state, it is helpful to work directly with the state variable $x_t$ and then separately take expectations over offers drawn from $q_{x_t}(\cdot)$. To this end, we develop some specialized notation. Let $\eta'_{\pi}$ denote the marginal distribution over $\Xc \cup \{\tau\}$ under the discounted state occupancy measure $\eta_{ \pi}$, and note that
\begin{equation}
	\label{eq:eta_factorization optimal stopping}
\eta_{\pi}\Big( \{ x\} \times (y_1, y_2) \Big) = \eta'_{\pi}(x)  \intop_{y_1}^{y_2} q_{x}(y) dy. 
\end{equation}

We find it convenient to directly work with $\eta'_{\pi}$ and $q_{x}(y)$. We now state several formulas in terms of $\eta'_{\pi}$ and $q_{x}(y)$ that will be used throughout the analysis. For an action $a\in [0,1]$, indicating a probability of stopping, 
\[
Q_{\pi}((x,y),a) = \left[ ay + (1-a) \gamma\sum_{x' \in \Xc} p(x'|x) \int_{\Yc} J_{\pi}((x', y')) q_{x'}(y') dy' \right] = ay + (1-a) c_{\pi}(x)
\]
where
\begin{equation}
	c_{\pi}(x) := \gamma \sum_{x'\in \Xc} p(x'|x) \int_{\Yc} J_{\pi}(x', y') q_{x'}(y') dy' \in [0, \gamma y_{\max}] 
\end{equation}
is called the ``continuation value'' from context $x$ under policy $\pi$. That $c_{\pi}(x) \leq \gamma y_{\max}$ is due the basic fact that $ J_{\pi}(x', y')\leq y_{\max}$, i.e. no policy can accrue expected reward exceeding the maximum possible offer.  Similarly, the weighted policy iteration objective becomes,
\begin{align}\nonumber
\Bc\left( \theta \mid \eta_{ \pi}, J_{\pi}  \right) &= \sum_{x \in \Xc} \eta'_{ \pi}(x) \intop_{y_{\min}}^{y_{\max}} Q_{\pi}( (x,y)\, ,\,    \mathbbm{1}(y > \theta_x)  ) q_{x}(y)dy   \\
&= \sum_{x\in \Xc} \eta'_{ \pi}(x) \intop_{y_{\min}}^{y_{\max} } \left[y\mathbbm{1}(y > \theta_x) + c_{\pi}(x)\mathbbm{1}(y < \theta_x)    \right] q_{x}(y)dy. \label{eq:stopping_formula_for_B}
\end{align}
Here we use that there is zero value-to-go from the terminal state $\tau$ to restrict the sum to continuation states. We now proceed to verify all the conditions needed to apply our general results. 
 
 

\paragraph{Condition \ref{cond: closure}: Closure under policy improvement.}
It is easy to verify that the class of threshold policies is closed under policy improvement. For any $\pi \in \Pi_{\Theta}$, the policy iteration update for any state $s=(x,y) \in \Sc_{\rm C}$ is given by
\[
\pi^+(x,y) = \argmax_{a \in \{0,1\}} \, Q_{\pi}((x,y),a) = \mathbbm{1}(y > c_{\pi}(x)). 
\]
This result can be seen immediately from the formula for $Q_{\pi}(\cdot)$ given above. Clearly the policy iteration update is another threshold policy. In particular, the policy iteration update to $\pi$ is a new threshold policy $\pi_{ \theta^+}$ with parameters
\begin{equation}\label{eq:stopping_pi_update}
\theta_x^+  = \max\{y_{\min} \, , \, c_{\pi}(x) \}.
\end{equation}
for each $x\in \Xc$. This works because a policy with stopping threshold $y_{\min}$ accepts the next offer with probability one when $c_{\pi}(x)<y_{\min}$ and otherwise and we are assured that $c_{\pi}(x)\in [y_{\min}, \gamma y_{\max}]$ is a feasible choice for $\theta_x^+$.  


\paragraph{Condition \ref{cond: stationary}: No suboptimal stationary points for the weighted PI objective.} \emph{This result here is implied by the gradient dominance result that follows, but it provides a warmup for that analysis.}

We now show that $\theta \mapsto \Bc(\theta|\eta_{\pi}, J_{\pi})$ has no suboptimal stationary points for each $\pi \in \Pi_{\Theta}$. As we formulate the optimal stopping example as a maximization problem, any stationary point $\theta$ satisfies,
\begin{equation*}
	\frac{\partial }{\partial \theta_x} \Bc(\theta|\eta, J_\pi) \cdot (\theta'_x - \theta_x) \leq 0 \qquad \forall\theta'_x \in \Yc , 
\end{equation*}
for every $x\in \Xc$. It is possible to separate the stationarity condition into a componentwise inequality in this manner because the parameters space is the Cartesian product $\Theta= \Yc^{\Xc}$.

From \eqref{eq:stopping_formula_for_B}, we have the following formula for the derivative:
\begin{equation}\label{eq:policy_grad_opt_stopping}
	\frac{\partial}{\partial \theta_x} \Bc(\theta \mid \eta_{ \pi}, J_\pi) =  \left(c_{\pi}(x) - \theta_x  \right)  \eta'_{\pi}(x)q_x(\theta_x) 
\end{equation}
Therefore, $\theta$ is stationary point when $\left(c_{\pi}(x) - \theta_x  \right)  \cdot (\theta'_x  - \theta_x) \leq 0$ for all $\theta'_x \in  [y_{\min}, y_{\max}]$. If $c_{\pi}(x) \in (y_{\min}, y_{\max})$ is in the interior of the feasible region, this implies $\theta_x = c_{\pi}(x)$.  Otherwise (since it is impossible to have $c_{\pi}(x) \geq y_{\max}$), we have  $c_{\pi}(x)\leq y_{\min}$  and a stationary point must satisfy $\theta_x = y_{\min}$. We have found any stationary point $\theta$ satisfies, $\theta_x = \max\{ y_{\min}, c_{\pi}(x) \}$, which matches the formula \eqref{eq:stopping_pi_update} for the policy iteration update  that minimizes $\theta \mapsto \Bc(\theta \mid \eta_{ \pi}, J_{\pi})$. 


\paragraph{Condition \ref{cond: convexity_strong}: Gradient dominance.} We now establish a gradient dominance result that strengthens the previous analysis. We first recall the claim. 
\graddomoptstopp*
\begin{proof}
	Fix any $\pi \in \Pi_{\Theta}$. As we formulate the optimal stopping as a reward maximization problem, following our notion of gradient dominance in Definition \ref{def:gradient_dominance}, we want to show that
	\begin{equation}\label{eq:opt_stopping_grad_dominance}
		\max_{\theta' \in \Theta} \, \langle \nabla_{\theta} \Bc(\theta | \eta_{\pi}, J_{\pi}), \theta' - \theta \rangle \geq \frac{1}{\beta} \left( \Bc(\theta^+ | \eta_{\pi}, J_{\pi}) - \Bc(\theta | \eta_{\pi}, J_{\pi})  \right)
	\end{equation}
	where $\theta^+$ is the parameter of a policy iteration update to $\pi$, i.e. $\theta^+ = \argmax_{\theta \in \Theta} \, \Bc(\theta|\eta_{\pi}, J_{\pi})$. As shown in \eqref{eq:stopping_pi_update}, $\theta^+_x=\max\{y_{\min}, c_{\pi}(x)  \}$. 	
	 We first lower bound the left hand side of \eqref{eq:opt_stopping_grad_dominance} as,
	\begin{align}
		\max_{\theta' \in \Theta} \, \langle \nabla_{\theta} \Bc(\theta | \eta_{\pi}, J_{\pi}), \theta' - \theta \rangle &= \sum_{x \in \X}  \max_{\theta'_x \in \Yc }  \frac{\partial  \Bc(\theta | \eta_{\pi}, J_{\pi})}{\partial \theta_x} \cdot (\theta'_x - \theta_x) \nonumber \\
		&= \sum_{x \in \X}  \max_{\theta'_x \in \Yc }  \left(c_\pi(x)-\theta_x\right) \cdot   \eta'_{\pi}(x)q_{x}(\theta_x) \cdot (\theta'_x - \theta_x) \nonumber \\
		&\geq \left(\min_{x' \in \Xc, y'\in \Yc}q_{x'}(y')\right)   \sum_{x \in \X}  \eta'_{\pi}(x) \left\{ \max_{\theta'_x \in \Yc }  \, \left[ \left(c_\pi(x)-\theta_x\right) \cdot (\theta'_x - \theta_x) \right] \right\}, \label{eq:gradient dominance stopping LHS}
	\end{align}
	where second equality uses the derivative calculation in \eqref{eq:policy_grad_opt_stopping}. We now upper bound the right hand side of \eqref{eq:opt_stopping_grad_dominance}: 
	\begin{align*}
			& \Bc(\theta^+ | \eta_{\pi}, J_{\pi}) - \Bc(\theta | \eta_{\pi}, J_{\pi})  \\ =& \sum_{x \in \Xc} \eta'_{ \pi}(x) \intop_{y_{\min}}^{y_{\max}} \left[ Q_{\pi}( (x,y)\, ,\,    \mathbbm{1}(y > \theta^+_x)  ) - Q_{\pi}( (x,y)\, ,\,    \mathbbm{1}(y > \theta_x)  ) \right] q_{x}(y)dy   \\
			\leq & \left(\max_{x' \in \Xc, y'\in \Yc}q_{x'}(y')\right)  \sum_{x \in \Xc} \eta'_{ \pi}(x) \underbrace{\intop_{y_{\min}}^{y_{\max}} \left[ Q_{\pi}( (x,y)\, ,\,    \mathbbm{1}(y > \theta^+_x)  ) - Q_{\pi}( (x,y)\, ,\,    \mathbbm{1}(y > \theta_x)  ) \right] dy}_{:=G_{x}(\theta^+_x, \theta_x )}.   
	\end{align*}
The result follows if we can conclude,
\begin{equation}\label{eq:opt_stopp_grad_dominance_ineq}
\max_{\theta'_x \in \Yc }  \, \left[ \left(c_\pi(x)-\theta_x\right) \cdot (\theta'_x - \theta_x) \right] \geq G_{x}(\theta^+_x, \theta_x), 
\end{equation}
which we do below by separately considering two cases. For this purpose, it is helpful to use a more explicit formula for $G_{x}(\theta^+_x, \theta_x )$, which follows directly from the formula for the $Q$ function given in this section's preliminaries:
\[
G_{x}(\theta^+_x, \theta_x ) = 
\begin{cases}
	\intop_{\theta_x}^{\theta^+_x} ( c_{\pi}(x)-y  )dy, & \text{for  } \theta_x \leq \theta^+\\
	\intop_{\theta^+_x}^{\theta_x} ( y- c_{\pi}(x)  )dy, & \text{for  } \theta_x > \theta^+
\end{cases}
\]


\paragraph{Case (1):} Assume that $c_{\pi}(x)  \in (y_{\min}, y_{\max})$ in which case $\theta^+_x  = c_{\pi}(x)$. Then,
\begin{align*}
G_{x}(\theta^+_x, \theta_x) = \frac{1}{2}\left( c_{\pi}(x) - \theta_x    \right)^2  &\leq \left( c_{\pi}(x) - \theta_x    \right)^2 \leq \max_{\theta'_x \in \Yc }  \left(c_\pi(x)-\theta_x\right) \cdot (\theta'_x - \theta_x)  
\end{align*}
where the formula for $G_{x}(\theta_x^+, \theta_x)$ follows by calculating the integral and the final inequality uses that a choice of $\theta'_x=c_{\pi}(x)$ is feasible. The establishes \eqref{eq:opt_stopp_grad_dominance_ineq}. 


\paragraph{Case (2): } Now assume that $c_{\pi}(x)  \not \in (y_{\min}, y_{\max})$ in which case we know $c_{\pi}(x) \leq y_{\min}$ (since $c_{\pi}(x)\leq \gamma y_{\max}$) and therefore $\theta^+_x  = y_{\min}$. One can check that 
\begin{align*}
		G_{x}(\theta^+_x, \theta_x) = 	\intop_{y_{\min} }^{\theta_x} ( y- c_{\pi}(x)  )dy \leq \left( \theta_x - c_{\pi}(x) \right) \left( \theta_x - y_{\min} \right) \leq \max_{\theta'_x \in \Yc }  \left(c_\pi(x)-\theta_x\right) \cdot (\theta'_x - \theta_x) 
\end{align*}
where again the final inequality is immediate since $\theta'_x=y_{\min}$ is a feasible choice. This establishes \eqref{eq:opt_stopp_grad_dominance_ineq}. 
\end{proof}

	

	
%	Using that $T_{\pi_{\theta^+}} J_{\pi} = T J_{\pi}$, we have
%	\begin{align}
%		\label{eq:grad dominance objective stopping}
%		\Bc(\theta^+ | \eta_{\pi}, J_{\pi}) - \Bc(\theta | \eta_{\pi}, J_{\pi}) &= \sum_{x \in \X} \eta'_{\pi}(x) \int_{\Yc} \left(T J_{\pi}(x,y) - T_{\pi_{\theta}} J_{\pi}(x,y) \right) q_x(y) dy \nonumber \\
%		&\leq  \left(\max_{x' \in \Xc, y'\in \Yc}q_{x'}(y')\right)  \sum_{x \in \X} \eta'_{\pi}(x) \int_{\Yc} \left(T J_{\pi}(x,y) - T_{\pi_{\theta}} J_{\pi}(x,y) \right) dy.
%	\end{align}
%	We can simplify to write,
%	\begin{align}
%		T_{\pi_{\theta}} J_{\pi}(x,y) &= y \cdot \mathbbm{1} (y \geq \theta_x) + c_{\pi_{\theta}}(x) \cdot \mathbbm{1} (y < \theta_x) 	\label{eq:cost-to-go stopping appendix 1} \\
%		T J_{\pi}(x,y) &=  y \cdot \mathbbm{1} (y \geq \theta^+_x) + c_{\pi_{\theta}}(x) \cdot \mathbbm{1} (y < \theta^+_x) \label{eq:cost-to-go stopping appendix 2}
%	\end{align}
%	We argued above that $c_{\pi}(x) < y_{\max}$ and $\theta^+_x = \max \{c_{\pi}(x), y_{\min} \}$. We consider two cases.
%	\paragraph{Case (1):} Assume that $c_{\pi}(x)  \in (y_{\min}, y_{\max})$ in which case $\theta^+_x  = c_{\pi}(x)$. Using equations \eqref{eq:cost-to-go stopping appendix 1} and \eqref{eq:cost-to-go stopping appendix 2}, it is easy to check that
%	\begin{align}
%		\label{eq:case1 stopping RHS}
%		\int_{\Yc} \left(T J_{\pi}(x,y) - T_{\pi_{\theta}} J_{\pi}(x,y) \right) dy &\leq (c_{\pi}(x) - \theta_x)^2.
%	\end{align}
%	As $c_{\pi}(x)  \in (y_{\min}, y_{\max})$, observing the lower bound in \eqref{eq:gradient dominance stopping LHS}, we find that
%	\begin{align}
%		\max_{\theta'_x \in \Yc }  \left(c_\pi(x)-\theta_x\right) \cdot (\theta'_x - \theta_x)  
%		%&\geq   \left(c_\pi(x)-\theta_x\right)    \cdot (\theta^+_x - \theta_x) 
%		\geq (c_{\pi}(x) - \theta_x)^2 \label{eq:case1 stopping LHS} 
%	\end{align}
%	We get our desired result by using \eqref{eq:case1 stopping RHS} and \eqref{eq:case1 stopping LHS} to compare Equations \eqref{eq:grad dominance objective stopping} and \eqref{eq:gradient dominance stopping LHS} respectively.
%	
%	\paragraph{Case (2):} Now assume that $c_{\pi}(x)  \not \in (y_{\min}, y_{\max})$ in which case $\theta^+_x  = y_{\min}$. Again, using \eqref{eq:cost-to-go stopping appendix 1} and \eqref{eq:cost-to-go stopping appendix 2}, it is easy to check that 
%	\begin{align}
%		\label{eq:case2 stopping RHS} 
%		\int_{\Yc} \left(T J_{\pi}(x,y) - T_{\pi_{\theta}} J_{\pi}(x,y) \right) dy = \intop^{\theta_x}_{\theta^+_x} \left( y - c_{\pi}(x) \right) dy &\leq \intop^{\theta_x}_{\theta^+_x} \left( \theta_x - c_{\pi}(x) \right) dy \nonumber \\
%		&= \left( \theta_x - c_{\pi}(x) \right) \left( \theta_x - \theta^+_{x} \right).
%	\end{align}
%	Similarly, we can lower bound the right hand side of \eqref{eq:gradient dominance stopping LHS} as
%	\begin{align}
%		\max_{\theta'_x \in \Yc }  \left(c_\pi(x)-\theta_x\right) \cdot (\theta'_x - \theta_x) \geq   \left( \theta_x -c_{\pi}(x) \right) \cdot (\theta_x - \theta^+_x). \label{eq:case2 stopping LHS} 
%	\end{align}
%	We get out desired result by using \eqref{eq:case2 stopping RHS} and \eqref{eq:case2 stopping LHS} to compare Equations \eqref{eq:grad dominance objective stopping} and \eqref{eq:gradient dominance stopping LHS} respectively.
%\end{proof}
%
%
%
%
%
%
%
%\newpage
%










%\concentrabilityStopping*
%\subsubsection{Conditions 0 - 3 in Example \ref{ex:stopping}}



%Optimality of threshold policies for this problem is well known (see \cite{bertsekas1995dynamic} for example) and essentially follows from the convergence of policy iteration along with the closure property. 
%We verify the additional smoothness properties in  \ref{subsec:app_optimalstopping}. 

\paragraph{Smoothness results: Condition \ref{cond: diff} and Lemma \ref{lem:smoothness_opt_stopp}}

%\paragraph{Condition \ref{cond: diff} and twice continuous differentiability.}
\emph{Additional notation. } 
 We simplify notation to write $\eta_{\theta}:= \eta_{\pi_{\theta}}$, $\eta'_{\theta}:=\eta'_{\pi_{ \theta}}$, $T_{\theta}:=T_{\pi_{\theta}}$, and $J_{\theta} := J_{\pi_{\theta}}$. We define $J'_{\theta}(x) := \intop_{\Yc} J_{\theta}(x, y) q_x(y) dy$ to be the expected cost-to-go function from context $x$. Similarly, denote $g'_{\theta}(x) := \intop_{\Yc} \mathbbm{1}\left(  y \geq \theta_x \right) y q_x(y) dy$ to be the expected reward earned from context $x$. Take $J'_{\theta}(\tau)=0$ and $g'_{\theta}(\tau)=0$. Recall that $\nu(x)$ is the probability the initial state $(x_0,y_0)$ has $x_0=x$. We extend $\nu$ to be a probability distribution over $\Xc \cup \{\tau\}$ by defining $\nu(\tau)=0$. 
 
   We let $P'_{\theta} \in \mathbb{R}^{ (|\Xc| + 1) \times (|\Xc| + 1)}$ denote the transition matrix over $\Xc \cup \{\tau\}$ under $\pi_{\theta}$, defined as
\begin{equation}
	\label{eq:transition_probability optimal stopping}
	P'_{\theta}(x'|x) = p(x'|x) \int_{\Yc} \mathbbm{1}(y < \theta_x) q_x(y) dy, \quad P'_{\theta}(\tau|x) = \int_{\Yc} \mathbbm{1}(y \geq \theta_x) q_x(y) dy, \quad P'_{\theta}(\tau|\tau) = 1,
\end{equation} %\sum_{x' \in \Xc} P'_{\theta}(x'|x)
for all $x',x \in \Xc$. One can write key quantities in ``vector form'' as
\begin{equation}\label{eq:opt_stopping_smoothness_matrices}
J'_{\theta} = \left(I-\gamma P'_{\theta}\right)^{-1} g'_{\theta}  \qquad \& \qquad  \eta'_{\theta} =  (1-\gamma) \nu (I - \gamma P'_{\theta})^{-1}  
\end{equation}
where $\nu\in \mathbb{R}^{|\Xc|+1}$ is a row vector $g'_{\theta}\in \mathbb{R}^{|\Xc|+1}$ is a column vector.  The matrix $(I-\gamma P'_{\thetabar})$ is invertible as $P'_{\thetabar}$ is a stochastic matrix.




%We now verify all the conditions needed for our main results.

\emph{Verifying Condition \ref{cond: diff}}. We establish the main condition needed to invoke the policy gradient formula in Lemma \ref{lem: PG theorem}. 
  That $\frac{\partial }{\partial \thetabar_x} \Bc(\thetabar|\eta_{\theta}, J_{\theta})$ exists and is continuous in $\thetabar$ is an immediate consequence of \eqref{eq:policy_grad_opt_stopping}
together with the continuity of $q_{x}(\cdot)$.  We also need to verify that $\Bc(\theta | \eta_{\thetabar}, J_{\theta})$ is continuously differentiable as a function of $\thetabar$. Since $J'_{\theta}(\tau)=0$, 
\[ 
\Bc(\theta | \eta_{\thetabar}, J_{\theta}) = \sum_{x \in \X} \eta'_{\thetabar}(x)\intop_{\Yc} Q_{\pi_{\theta} }( (x,y),  \pi_{ \theta}(x,y) )  q_{x}(y)dy = \sum_{x \in \X} \eta'_{\thetabar}(x) J'_{\theta}(x).
\] 
Observe that $P'_{\thetabar}$ is continuously differentiable in $\thetabar$, as $q_{x}(\cdot)$ is assumed to be continuous.  Therefore, $(I-\gamma P_{\thetabar})^{-1}$ is also continuously differentiable and $\eta'_{\thetabar}(\cdot)$ is as well. 

\emph{Verifying Lemma \ref{lem:smoothness_opt_stopp}.} We now establish the following smoothness result for the policy gradient loss $\ell(\cdot)$, which is useful for invoking convergence rate results for first order methods. 
\optstoppcostsmooth*
\begin{proof}
	Using the policy gradient theorem as shown in Lemma \ref{lem: PG theorem} and the derivative calculations in \eqref{eq:policy_grad_opt_stopping}, we have
	\begin{align*}
		\frac{\partial }{\partial \theta_x} \ell(\theta) = 	\frac{\partial }{\partial \thetabar_x} \Bc(\thetabar | \eta_{\theta}\, , J_{\theta}  )  \bigg\vert_{\thetabar = \theta}  %\eta'_{\theta}(x) \frac{\partial }{\partial \thetabar_x} \left[ \int_{\Yc} Q_{\pi_{\theta}}\left( (x,y), \pi_{\thetabar}(x,y) \right) q_x(y) dy \right] \bigg\vert_{\thetabar=\theta} \\
		= \left( c_{\pi_{\theta}}(x) - \theta_x \right) \eta'_{\theta}(x) q_x(\theta_x).
		%	&= \left( \sum_{x' \in \Xc} p(x'|x) J_{\pi_{\theta}}(x') - \theta_x \right) \eta'_{\theta}(x) q_x(\theta_x) 
	\end{align*}
	We argued above when verifying Condition \ref{cond: diff} that $\eta'_{\theta}(x)$ is continuously differentiable. By assumption, $q_{x}(\theta_x)$ is continuously differentiable in $\theta_x$. Therefore, $\nabla \ell(\theta)$ has a continuous derivative if $c_{\pi_{\theta}}(x)$ is continuously differentiable in $\theta$. 
	To show this, recall that by definition, 
	\begin{align}
		\label{eq:continutaion_value_appendix}
		c_{\pi_{\theta}}(x) = \gamma \sum_{x'\in \Xc}p(x'|x) \int_{\Yc} J_{\theta}(x', y') q_{x'}(y') dy = \gamma \sum_{x'\in \Xc}p(x'|x) J'_{\theta}(x') \qquad \forall x \in \Xc.
	\end{align}
  While verifying Condition \ref{cond: diff} above, we argued that  $(I-\gamma P'_{\theta})^{-1}$ is is continuously differentiable. It is also easily shown that $g'_{\theta}$ is continuously differentiable. Due to \eqref{eq:opt_stopping_smoothness_matrices}, this implies $J'_{\theta}$ is continuously differentiable.  Hence using \eqref{eq:continutaion_value_appendix}, we find that $c_{\pi_{\theta}}$ is continuously differentiable in $\theta$. 
	
	We have shown $\nabla^2 \ell(\theta)$ exists and is continuous. Since $\Theta$ is compact, the Extreme Value theorem implies $\max_{\theta \in \Theta} \| \nabla^2 \ell(\theta) \|_2$ exists and is finite.
\end{proof} 




\paragraph{Concentrability coefficient for optimal stopping.} 
We first recall the claim.
\concentrabilityStopping*
\begin{proof}
	We show that the Bellman operator $T$ is a contraction with modulus $\gamma$ in $\| \cdot\|_{1,\mu}$. The proof then follows immediately using part (c) of Theorem \ref{thm: concentrability general}.
	
	For a policy that never stops, the stationary distribution over continuation states, $(x,y) \in \Sc_{\rm C}$ factorizes as $\mu(x,y) = \mu'(x) q_x(y)$ where $\mu'$ is the marginal stationary distribution over context states $\Xc$ such that $\mu'(x') = \sum_{x \in \Xc} \mu'(x) p(x'|x)$. Then, for any bounded cost-to-go functions $J,J'\in \Jc$,
	\begin{align*}
		\|TJ-TJ'\|_{1,\mu} &= \sum_{x \in \Xc} \mu'(x) \int_{\Yc} \left| TJ(x,y) - TJ'(x,y) \right| q_x(y) dy. 
	\end{align*}
	By definition, 
	\[
	T J(x,y) = \max \{y, \gamma \sum_{x' \in \Xc} p(x'|x) \int_{\Yc} J(x',y') q_{x'}(y') dy' \}.
	\]
	Note that for any scalars $(x_1, x_2, y)$, we have $|\max\{y,x_1\} - \max\{y,x_2\}| \leq |x_1 - x_2 |$. Therefore, 
	\begin{align}
		\left| TJ(x,y) - TJ'(x,y) \right| \leq \gamma \sum_{x' \in \Xc} p(x'|x) \int_{\Yc} \left| J(x',y') - J'(x',y') \right| q_{x'}(y') dy'. \label{eq:contraction_opt_stopp_appx}
	\end{align}
	As the right hand side in \eqref{eq:contraction_opt_stopp_appx} is independent of $y$, integrating \eqref{eq:contraction_opt_stopp_appx} with respect to $q_x(\cdot)$ gives
	\[
	\int_{\Yc} \left| TJ(x,y) - TJ'(x,y) \right| q_x(y) dy \leq \gamma \sum_{x' \in \Xc} p(x'|x) \int_{\Yc} \left| J(x',y') - J'(x',y') \right| q_{x'}(y') dy'. 
	\]
	Therefore, 
	\begin{align*}
		\|TJ-TJ'\|_{1,\mu} &= \sum_{x \in \Xc} \mu'(x) \int_{\Yc} \left| TJ(x,y) - TJ'(x,y) \right| q_x(y) dy \\
		&\leq \gamma \sum_{x \in \X} \mu'(x) \sum_{x' \in \Xc} p(x'|x) \int_{\Yc} \left| J(x',y') - J'(x',y') \right| q_{x'}(y') dy' \\
		&\overset{(a)}{=} \gamma \sum_{x' \in \X} \mu'(x') \intop_{\Yc} \left| J(x',y') - J'(x',y') \right| q_{x'}(y') dy' \\
		&= \gamma \| J-J' \|_{1,\mu}
	\end{align*}
	where (a) follows as $\mu'$ is the stationary distribution over $\Xc$. For $\rho = \mu$, we have $C,c=1$ in part (c) of Theorem \ref{thm: concentrability general}, implying that $\kappa_\rho \leq 1$.
\end{proof}


\subsection{Finite horizon inventory control}
We consider the inventory control problem as described in Example \ref{ex:inventorycontrol}. To review notation, recall that in this setting, the inventory level evolves as: $x_{t+1} = x_t + a_t - w_t$ for non-negative orders $a_t$ and i.i.d demands $w_t \in [0, w_{\max}]$. We let $s_t=(x_t,h_t)$ denote the state at time $t$ and consider the class of base-stock policies which orders inventory, $\pi_{\theta}(s_t) =  \max\{0, \theta_{h_t} - x_t\}$ in state $s_t$. We consider the policy class, $\Pi_{\Theta}=\{ \pi_{\theta} : \theta \in \Theta \}$ with bounded parameter space $\Theta =  [0, 2 w_{\max}]^{H}$ which implies the inventory levels, $x_t$, at every period are bounded in $\mathcal{I} = [-w_{\max}, 2 w_{\max}]$. We assume the initial distribution factorizes as, $\rho(dx,h) = \nu(h) q_{h}(x)dx_0$, where $\nu(h) > 0$ for every $h \in \{1, \ldots, H\}$ and $q_{h}(\cdot)$ is a twice differentiable PDF supported over $\mathcal{I}$ for each $h$. Clearly, this choice of $\rho$ satisfies the regularity condition in Assumption \ref{ass: exploratory rho finite horizon}. The problem setup also clearly follows the factorization structure assumed in Condition \ref{cond: finite_horizon}. Here, we verify the differentiability condition along with Condition \ref{cond:finite_horizon_stationarity}, both of which are needed for Theorem \ref{thm: finite_horizon}.




\paragraph{Reminder on the  Leibniz rule.}
We appeal to the Leibniz rule, which states sufficient conditions for differentiating the integral of a function. For a bounded set $\Psi \subset \R$, consider the function $F: \Psi \to \R$ given by 
\[
F(\psi) = \E [ f(\psi, s) ] = \int_{\Sc} f(\psi,s) P(ds)
\]
where $f: \Psi \times \Sc \to \R$ is a real valued function, $P$ is a probability measure supported over $\Sc$ and for each $\psi \in \Psi$, the function $f(\psi,\cdot)$ is $P$-integrable, i.e. $\E [|f(\psi,s)|] < \infty$. Let $\Dc_s(\psi)$ be the set of points $s \in \Sc$ such that $f(\cdot, s)$ is non-differentiable at $\psi$. By the Leibniz rule, $F$ is differentiable at $\psi$ if (i) $\Dc_s(\psi)$ has zero measure under $P$, i.e. $P[\Dc_s(\psi)]=0$ and (ii) $f'(\psi,\cdot)$ is $P$-integrable, in which case $F'(\psi) =  \int_{\Sc} f'(\psi,s) P(ds).$  By applying the same steps again, we can calculate the second derivative of $F(\cdot)$ as well.

The Leibniz rule is useful as a threshold policy, $\pi_{\theta}(z)=\max\{0, \theta - z\}$, is differentiable everywhere except at one point, $z=\theta$.



\paragraph{Condition \ref{cond: diff}: continuous differentiability.}
We make the abbreviation $\eta_{\theta}=\pi_{\theta}$, $J_{\theta}\equiv J_{\pi_\theta}$ and $Q_{\theta}\equiv Q_{\pi_{ \theta}}$. To establish Condition 0, we need to show that the function $\Bc(\theta^+ | \eta_{\thetabar}, \, J_{\theta}) = \intop Q_{\theta}(s, \pi_{\theta^+}(s))\eta_{ \thetabar}(ds),$ is (i) continuously differentiable as a function of $\theta^+$ when $\thetabar=\theta$ and (ii) continuously differentiable in $\thetabar$ when $\theta^+=\theta$. The approach is to (somewhat tediously) rewrite $\Bc(\cdot)$ in terms of a single multi-dimensional integral that appears in \eqref{eq:inventory_smoothness_integral_form} below. From there, the result follows by applying the Leibniz rule to differentiate under the integral. 

We write:
\begin{align*}
	\Bc(\theta^+ | \eta_{\thetabar},\, J_{\theta}) &= (1-\gamma)\E_{\rho}^{\pi_{\thetabar}}\left[\sum_{t=0}^{\infty} \gamma^t Q_{\theta}(s_t, \pi_{ \theta^+}(s_t)  ) \right] \\
	 &= (1-\gamma)\E_{\rho}^{\pi_{\thetabar} }\left[\sum_{t=0}^{H-h_0} \gamma^t Q_{\theta}(s_t, \pi_{ \theta^+}(s_t)  ) \right] \\ 
	&= (1-\gamma)\E_{\rho}^{\pi_{\thetabar} }\left[\sum_{t=0}^{H-h_0} \underbrace{\E_{\rho}^{\pi_{\thetabar} }\left[ \gamma^t  Q_{\theta}(s_t, \pi_{ \theta^+}(s_t)  ) \mid h_0 \right]}_{:= \Bc_{h_0, t}(\theta^+ | \eta_{\thetabar},\, J_{\theta})  }\right].
\end{align*}
The first equality is the definition of the state occupancy measure. The second equality uses that the process transitions to a terminal state after stage $h_t=H+1$ is reached. The final equality is uses the tower property of conditional expectation -- there the outer expectation is over $h_0 \in \{1, \cdots, H\}$ drawn from the initial distribution and the inner expecation is over the state $s_t=(x_t, h_0+t)$, and in particular the inventory level $x_t$, that is reached $t$ periods later under the policy $\pi_{ \thetabar}$. 

We show that each individual term, $\Bc_{h_0, t}(\theta^+ | \eta_{\thetabar},\, J_{\theta}),$ is continuously differentiable in $\thetabar$ or in $\theta^+$. This completes the result, since $\Bc(\theta^+| \eta_{ \thetabar}, J_{\theta})$ a finite mixture of such terms.  Notice that this expression involves three different policies that are applied at different timesteps:
\begin{enumerate}
	\item $\pi_{ \thetabar}$ is applied prior to timestep $t$ and it is these dynamics that determine $s_t$. 
	\item $\pi_{\theta^+}$ is applied during timestep $t$ only. (That is the meaning of the action in the $Q$ function.)
	\item $\pi_{ \theta}$ is applied from timestep $t+1$ until the final stage is reached. (That is the meaning of the subscript of the $Q$ function.) 
\end{enumerate}
 Based on this, we write
 $\tilde{\theta} = (\thetabar_1, \cdots, \thetabar_{h_{t}-1}, \theta^+_{h_t}, \theta_{h_t+1},\, \cdots, \theta_H ).$ Since we condition on $h_0$ and treat a fixed $t$ throughout the remainder of the proof, we omit dependence on these quantities in notation. Then, one can write 
\[
\Bc_{h_0, t}(\theta^+ | \eta_{\thetabar},\, J_{\theta}) = \E_{\rho}^{\pi_{\tilde{\theta} } }\left[ \sum_{\ell=t}^{H-h_0} \gamma^{\ell}  g(s_t, a_t)  \, \bigg\vert \, h_0 \right], 
\] 
where we used the observations 1-3 above together with the definition of a $Q$-function as an expected disctounted sum of single-period costs $g(\cdot)$. In this inventory control problem,  
\begin{equation*}
	g(s_t,a_t) = c \cdot a_t + \E[r(x_t + a_t - w_t) \mid x_t, a_t] = c \cdot a_t + \E[r(x_{t+1}) \mid x_t, a_t],
\end{equation*}
where $r: \mathbb{R} \to \mathbb{R}$ is defined as $r(z) = b\max(0,z) + p\max(0,-z)$ and denotes the holding/backlogging costs. The conditional expectation in the middle equation integrates over the i.i.d draw of the demand $w_t$ and the second equation uses form of inventory dynamics $x_{t+1} = x_t +a_t - w_t$.  By the tower property of conditional expectation, we can rewrite  
\begin{equation}\label{eq:inventory_smoothness_expectation_form}
\Bc_{h_0, t}(\theta^+ | \eta_{\thetabar},\, J_{\theta}) = \E_{\rho}^{\pi_{\tilde{\theta} } }\left[ \sum_{\ell=t}^{H-h_0} \gamma^{\ell}  \left(  c \cdot a_t  + r(x_{t+1}) \right)   \, \bigg\vert \, h_0  \right]. 
\end{equation}
%All randomness in this expression is taken over the initial state $x_0$, drawn from a the continuous density $q_{h_0}(\cdot)$, and the demands $w_0, \cdots, w_H$ that are drawn i.i.d from a continuous density. Write $\xi = (x_0, w_0, \cdots, w_H )$. Then one can write $\Bc_{h_0, t}(\theta^+ | \eta_{\thetabar},\, J_{\theta}) = \E_{\xi}\left[  F( \vec{a}  , \xi ) ]$. Here $F( \vec{a}, \xi )=\sum_{\ell=t}^{H-h_0} \gamma^{\ell}  \left(  c \cdot a_t  + r(x_{t+1}) \right)$ evaluates the costs 

%Conditioned on $\vec{w}$ and $x_0$, 



Finally, we are ready to put this in the form of a single multi-dimensional integral. For any sequence of of inventory levels write $\vec{x}=(x_0, \cdots, x_{H-h_0+1})$. Set $G(\vec{x}, \tilde{\theta}) = \sum_{\ell=t}^{H-h_0} \gamma^{\ell}  \left(  c \cdot [ \tilde{\theta}_{h_t} - x_t ]^+  + r(x_{t+1}) \right)$, representing the cost incurred for an arbitrary sequence of inventory levels $\vec{x}$ assuming the ordering costs are based on the values  $[\tilde{\theta}_{h_t} - x_t ]^+= \max\{0, \tilde{\theta}_{h_t} - x_t  \}$ prescribed by the base-stock levels $\tilde{\theta}$. Now, to assign probabilities over the sequence $\vec{x}$, 
recall that conditioned on $h_0$, the initial inventory level $x_0$ is drawn from a PDF $q_{x}(\cdot)$. 
 Let $f(\cdot)$ denote the PDF of the demand distribution. Both PDFs are assumed to be twice differentiable. Then, 
\begin{equation}\label{eq:inventory_smoothness_integral_form}
\Bc_{h_0, t}(\theta^+ | \eta_{\thetabar},\, J_{\theta}) = \intop G(\vec{x}, \tilde{\theta}) p(\vec{x} \mid \tilde{\theta}) d\vec{x}
\end{equation}
where 
\[ 
p(\vec{x} \mid \tilde{\theta}) = q_{h_0}(x_0) \prod_{t=0}^{H-h_0} f(x_{t+1} - x_t - [\tilde{\theta}_{h_t}-x_t]^+) %f(x_1 - x_0 - [\tilde{\theta}_{h_0}-x_0]^+) \cdots f(x_{H-h_0+1} - x_{H-h_0} - [\tilde{\theta}_{H}-x_{H-h_0}]^+) 
\]
is the probability density function of $\vec{x}$. Here we have used that $x_{t+1}= x_t + a_t - w_t$ to relate the transitions of the inventory level to demand realizations.  

Now,  we can justify that $G(\vec{x}, \tilde{\theta}) p(\vec{x} , \tilde{\theta} )$ is almost surely twice differentiable with bounded first and second derivatives, so the Leibniz rule implies \eqref{eq:inventory_smoothness_integral_form} is twice differentiable (and hence continuously differentiable). Notice that $G(\vec{x}, \tilde{\theta})$ and $p(\vec{x} , \tilde{\theta} )$ may fail to be differentiable at values of $\vec{x}$ where $x_t = \tilde{\theta}_{h_t}$ for some $t$, but the set of such sequences of inventory levels has zero Lebesgue measure. Boundedness of first and second derivatives of $G(\vec{x}, \tilde{\theta})$ is immediate since it involves piece-wise linear functions of $\tilde{theta}$.  Boundedness of first and second derivatives of $p(\vec{x} \mid \tilde{\theta})$ can be shown from the assumption that $f(\cdot)$ and $q_{h_0}(\cdot)$ are twice continuously differentiable and both $\vec{x}$ and $\tilde{\theta}$ take values in bounded sets. (See Example \ref{ex:inventorycontrol} where it is noted that $x_t \in [-w_{\max}, 2w_{\max}]$ almost surely.).

\begin{rem}
	It is also possible to complete the argument by claiming that the discounted sum inside \eqref{eq:inventory_smoothness_expectation_form} is differentiable \emph{pathwise}, i.e for each realization of the random initial inventory level $x_0$ and the demand realizations (except on a set of measure zero). A benefit of this approach is that it does not require differentiability of $f(\cdot)$, whereas directly differentiating $p(\vec{x} | \tilde{\theta})$ in  $\eqref{eq:inventory_smoothness_integral_form}$ does. See \cite[Section 2.6]{bertsekas1997nonlinear} for an introduction on how to calculate pathwise derivatives using the chain rule. \cite{glasserman1995sensitivity} applies this technique rigorously to an inventory control problem. 
\end{rem}

\paragraph{Verifying Condition \ref{cond:finite_horizon_stationarity}.}
The following lemma shows how Condition \ref{cond:finite_horizon_stationarity} holds for the finite horizon inventory control problem.
\begin{lem}
	\label{lemma:no_stationary_points_inventory}
	Consider the finite horizon inventory control problem in Example \ref{ex:inventorycontrol}. Let $J^*$ be the cost-to-go function corresponding to the optimal policy. Then, for any $\pi, \pi_{\theta} \in \Pi_{\Theta}$, the weighted policy iteration objective $\Bc(\theta|\eta_{\pi}, J^*)$ has no suboptimal stationary points.
\end{lem}

\begin{proof}
	Let $Q^*(s,a)$ be the Q-function corresponding to an optimal policy. Following \citep{bertsekas1995dynamic}, it can be shown that $Q^*(s,a)$ is convex in $a$, as both $J^*$ and the per step costs are convex. We show that at any stationary point $\theta$ of $\Bc(\theta | \eta_{\pi}, J^*)$, the corresponding base-stock policy $\pi_{\theta}$ is optimal. Recall, for any state $s=(x,h)$, we have 
	\begin{align*}
		\label{eq:stat_pts_stopping}
		\pi_{\theta}(s) = 
		\begin{cases}
			\theta_h - x \qquad &\text{if } \,\, x < \theta_h,  \\
			0 \qquad &\text{if } \,\, x > \theta_h
		\end{cases}
	\end{align*}
	We can write,
	\begin{align*}
		\frac{\partial}{\partial \theta_h} \Bc(\theta|\eta_{\pi}, J^*) &= \frac{\partial}{\partial \theta_h} \int_{x \in \mathcal{I}} Q^*\left( (x,h),\pi_{\theta}(x,h) \right) \, \eta_{\pi}(dx,h) \\
		&= \frac{\partial}{\partial \theta_h} \left[  \int_{x < \theta_h} Q^*((x,h),\theta_h - x) \, \eta_{\pi}(dx,h) + \int_{x > \theta_h} Q^*((x,h),0) \, \eta_{\pi}(dx,h) \right]\\
		&\overset{(a)}{=} \int_{x < \theta_h} \frac{\partial}{\partial \theta_h} Q^*((x,h),\theta_h - x) \, \eta_{\pi}(dx,h) \\
		&= \int_{x < \theta_h} \frac{\partial}{\partial a} Q^*((x,h),a) \at[\Big]{a=\pi_{\theta}(x,h)} \eta_{\pi}(dx,h)
	\end{align*}
	where we used Leibniz rule for (a). For simplicity, assume that there is a unique optimal policy and let $\theta^*$ be the corresponding optimal threshold. Consider any $\theta$ such that $\theta_h \neq \theta^*_h$ and let $\theta^{\alpha}_h = \theta_h + \alpha (\theta^*_h - \theta_h)$. We argue that $\frac{d}{d\alpha} \Bc(\theta^{\alpha}_h | \eta_{\pi}, J^*) \vert_{\alpha=0} < 0$, which implies that $\theta$ cannot be a stationary point. This follows as $Q^*(s,a)$ is convex in $a$ with a minimum at $a=\pi_{\theta^*}(s)$. Thus, we can reduce $\Bc(\theta|\eta_{\pi},J^*)$\footnote{If we cannot reduce $\Bc(\theta|\eta_{\pi},J^*)$, then $J_{\pi_{\theta}}((x,h))=J^*((x,h))$ holds $\rho$-almost surely. Assumption \ref{ass: exploratory rho finite horizon} then implies that $\theta_h$ must be optimal for period $h$.} by moving $\theta_h$ in the direction of $\theta^*_h$, which is feasible as $\Theta_h=[0,2w_{\max}]$ is a bounded interval of $\mathbb{R}$.
\end{proof}

%We observe that $G(\vec{x}, \tilde{\theta})$ is almost everywhere twice differentiable in $\tilde{\theta}$. It fails to be differentiable at at values of $\vec{x}$ where $x_t = \tilde{\theta}_{h_t}$ for some $t$, but the set of such sequences of inventory levels has zero Lebesgue measure. Moreover, $|\frac{\partial^2 }{ \partial\tilde{\theta_h} \partial\tilde{\theta_{h'}}  } G(\vec{x}, \tilde{\theta} )|$ are uniformly bounded as a function of $\vec{x}$ when derivatives exist. Due to the assumption that $f(\cdot)$ and $q_{h_0}()$ are continuously twice differentiable, $p(\vec{x} \mid \tilde{\theta})$ is continuously twice differentiable as a function of $\tilde{\theta}$ at almost every $\vec{x}$. Since continuous functions are uniformly bounded on bounded sets, and $\vec{x} \in [-w_{\max}, 2 w_{\max}]^{H-h_0+2}$ lies in a bounded hyper-rectangle for every feasible choice of $\tilde{\theta}$, we know that the second derivative of  $p(\vec{x} \mid \tilde{\theta})$ is uniformly bounded almost surely.  



\newpage
\dr{Jalaj's proof}

\paragraph{Condition \ref{cond: diff}: differentiability.}
%We first comment on some differentiability conditions needed for the policy gradient lemma to hold. Recall the setting in Example \ref{ex:inventorycontrol} where the inventory level evolves as: $s_{t+1} = s_t + a_t - w_t \,\, \forall \, t = \{0,\ldots,H-1\}$ for non-negative inventory orders $a_t$ and i.i.d demands $w_t \in [0, w_{\max}]$. We consider the class of base-stock-policies parameterized as $\Pi_{\theta} = \left\{\theta=(\theta_0, \ldots, \theta_{H-1}) \in \mathbb{R}^H : \theta_t > 0\right\}$ which orders inventory $\pi_{\theta}(s_t) =  \max\{0, \theta_t - s_t\}$ at time $t$. Also recall that we treat finite-horizon time-inhomogenous MDPs as a special case of infinite horizon MDP using the following factorization. 
%Proof of Theorem \ref{thm: finite_horizon}}
%\label{subsec: finite horizon proof}
%For the reader's convenience, we restate Condition \ref{cond: finite_horizon} and Theorem \ref{thm: finite_horizon}.
%\condFiniteHorizon*

We appeal to the Leibniz rule which states sufficient conditions for differentiating the integral of a function. For a bounded set $\Psi \subset \R$, consider the function $F: \Psi \to \R$ given by 
\[
F(\psi) = \E [ f(\psi, s) ] = \int_{\Sc} f(\psi,s) P(ds)
\]
where $f: \Psi \times \Sc \to \R$ is a real valued function, $P$ is a probability measure supported over $\Sc$ and for each $\psi \in \Psi$, the function $f(\psi,\cdot)$ is $P$-integrable, i.e. $\E [|f(\psi,s)|] < \infty$. Let $\Dc_s(\psi)$ be the set of points $s \in \Sc$ such that $f(\cdot, s)$ is non-differentiable at $\psi$. By Leibniz rule, $F$ is differentiable at $\psi$ if (i) $\Dc_s(\psi)$ has zero measure under $P$, i.e. $P[\Dc_s(\psi)]=0$ and (ii) $f'(\psi,\cdot)$ is $P$-integrable. Leibniz rule is useful as a threshold policy, $\pi_{\theta}(z)=\max\{0, \theta - z\}$, is differentiable everywhere except at one point, $z=\theta$.

Fix some $\theta = (\theta_0, \ldots, \theta_{H-1}) \in \Theta$. For the inventory control problem, we first argue differentiability of $\eta_{\pi_{\theta}}$. Note that give our problem setup, for any state $s=(x,h)$, the inventory level in the next period lies in the interval $\mathcal{I}$ and the stage advances by one. As $\pi_{\theta}(s)$ is differentiable except at $x\theta_h$, for any measurable set $\Mc \in \mathcal{I}$, the transition kernel
\[
P^{\pi_{\theta}}( (\Mc, h+1) \mid (x,h)) = \E_{w_h} \left[ \mathbbm{1}\left( x + \pi_{\theta}(s) - w_h \in \Mc \right)  \right]
\]
is differentiable in $\theta$ following Leibniz rule. A similar argument shows differentiability of the integral,
\[
\intop P^{\pi_{\theta}}( (\Mc, h+1) \mid (x,h)) \, \rho(dx, h)
\]
by using that $|\frac{\partial}{ \partial \theta_h} P^{\pi_{\theta}}( (\Mc, h+1) \mid s)|$ is bounded as $|\frac{\partial}{\partial \theta_h} \pi_{\theta}(s)| \leq 1$ for all $x \neq \theta_h$ (Leibniz rule requires bounded derivatives). We can write out $\eta_{\pi_{\theta}}$ as,
\begin{align*}
	\eta_{\pi_{\theta}}(M,h) &= \rho(M,h) + \gamma \intop P^{\pi_{\theta}}( (M,h) \mid (x,h-1) ) \rho(dx,h-1) + \\
	&\qquad \quad \gamma^2 \intop \intop P^{\pi_{\theta}} ( (M,h) \mid y, h-1 ) P^{\pi_{\theta}} ( (dy,h-1) \mid (x,h-2)) \rho(dx,h-2) + \ldots 
\end{align*}
where each of the integrals are differentiable in $\theta$ using the same argument as above. This implies differentiability of $\eta_{\pi_{\theta}}$.

%For any period $h \in \{0,\ldots, H-1\}$, state $s_h=(x,h)$ and a measurable set $\Mc \subset \mathcal{I}_{h+1}$, the transition kernel under $\pi_{\theta}$, $P_{\theta_h}(s_h,\Mc) = \E_{w_h} [ \mathbf{1}(x + \pi_{\theta_h}(s_h) - w_h \in \Mc) ]$ is differentiable for any $x \neq \theta_h$. Clearly, $|\partial / \partial \theta_h P_{\theta_h}(s_h, \Mc)|$ is also bounded as $|\partial / \partial \theta_h \pi_{\theta_h}(s_h)| \leq 1 \,\, \forall s_h \neq \theta$. 
%$|\partial / \partial \theta_h \pi_{\theta_h}(s)| \leq 1 \,\, \forall \, s \neq \theta_h$.
%$P_{\theta_h}(s,A) = \int_{\Sc_{h+1}} \mathbbm{1}(x \in A) \Prob_{\theta_h}(s,x)dx$ where $\Prob_{\theta_h}(s,x) = \E_{w_h} [ \mathbbm{1}(s + \pi_{\theta_h}(s) - w_h = x) ]$ \jb{check again}. Clearly, $\Prob_{\theta_h}(s,x)$ and hence $P_{\theta_h}(s,A)$ is differentiable for any $s \neq \theta_h$. 
%Therefore, when $\rho$ is supported over $\Sc_h$, the one step transition kernel
%\begin{align}
%	\label{eq:transition kernel inventory}
%\Prob^{\pi_{\theta}}_\rho(\Mc) = \int_{S_h} P_{\theta_h}(s_h,\Mc) \, d\rho(s_h)
%\end{align}
%is differentiable for any $\theta_h \in \Theta_h$. A similar argument holds for the t-step counterpart of \eqref{eq:transition kernel inventory}, which is a product of the one step transition kernels. Therefore, $\eta_{\theta}$ is differentiable in $\theta$.
%For instance, consider any $A \in \Sc_{h+2}$
%\[
%\lambda P^2_{\theta}(A) = \int_{\Sc_h} P_{\theta_h}(s,dy) P_{\theta_{h+1}}(y,A) \lambda(s) ds
%\]
%which is clearly differentiable in $\theta$. 
%Hence, for any $A \in \Sc_h$ and $h \in \{1,\ldots,H+1\}$, the state-occupancy measure $\eta_{\theta}(A) = \sum_{i=1}^h \rho P^{i}_{\theta}(A)$ is differentiable in $\theta$. It is noteworthy to see that $\eta_{\theta}$ is supported over all $\Sc$ as the start distribution $\rho$ is supported over each $\Sc_h$ for $h \leq H$.

To show differentiability of $\Bc(\thetabar|\eta_{\theta}, J_{\pi_{\theta}})$, consider the Bellman update $T_{\thetabar} J_{\theta}$ for any $\theta, \thetabar \in \Theta$. For any starting state $s_0=(x_0,h_0)$ and $h_0 < H$, we can write
\begin{align}
	\label{eq:Bellman update differentiability inventory}
	T_{\thetabar} J_{\theta}(s_0) = \left[ g(x_0, \pi_{\thetabar}(s_0)) + \sum_{t=1}^{H-h_0} g(x_t,a_t) \right]
\end{align}
where $\pi_{\thetabar}(s_0) = \max\{0, \thetabar_{h_0}-x_0\}$, $a_t = \pi_{\theta}(s_t) = \max\{0, \theta_{h_t} - x_t\}$ and the expected per-step cost function is given by $g(x_t,a_t) = c a_t + \E_{w_t}[r(x_t + a_t - w_t)]$. Here, $r: \mathbb{R} \to \mathbb{R}$ is defined as $r(z) = b\max(0,z) + p\max(0,-z)$ and denotes the holding/backlogging costs. Consider derivatives of the first term, 
\[
\frac{\partial}{\partial \thetabar_{h_0}} g(x_0,\pi_{\thetabar}(s_0)) = c  \cdot \underbrace{\frac{\partial \pi_{\thetabar}(s_0)}{\partial \thetabar_{h_0}}}_{(a)} + \underbrace {\frac{\partial}{\partial \thetabar_{h_0}} \E_{w_0}[r(x_0 + \pi_{\thetabar}(s_0) - w_0)]}_{(b)}
\]
Here, (a) exists everywhere except at $x_0=\thetabar_{h_0}$. For (b), we use that $r(x_0 + \pi_{\thetabar}(s_0) - w_0)$ is differentiable everywhere except at $x_0=\thetabar_{h_0}$ and $x_0 + \pi_{\thetabar}(s_0) = w_0$ as well as the fact that $|\frac{\partial}{\partial \thetabar_{h_0}} r(x_0 + \pi_{\thetabar}(s_0) - w_0)| \leq \max\{b,p\}$. Therefore, using Leibniz rule, the expectation in (b) is differentiable and hence $g(x_0,\pi_{\thetabar}(s_0))$ is differentiable everywhere except $x_0=\thetabar_{h_0}$. Also note that as $|\frac{\partial \pi_{\thetabar}(s_0)}{\partial \thetabar_{h_0}}| \leq 1$, this implies $|\frac{\partial}{\partial \thetabar_{h_0}} g(x_0,\pi_{\thetabar}(s_0))|$ is bounded.

%For the second term, we used that $r(x_0 + \pi_{\thetabar}(s_0) - w_0)$ is differentiable everywhere except at $x_0=\thetabar_{h_0}$ as well as at $x_0 + \pi_{\thetabar}(s_0) = w_0$ and $|\frac{\partial}{\partial \thetabar_{h_0}} r(x_0 + \pi_{\thetabar}(s_0) - w_0)| \leq \max\{b,p\}$. Therefore, using Leibniz rule, the expectation in (b) is differentiable in $\thetabar_{h_0}$. 
Let's now consider the remaining terms,
\[
\frac{\partial}{\partial \thetabar_{h_0}} g(x_t,a_t) = c \cdot \frac{\partial a_t}{\partial \thetabar_{h_0}} + \frac{\partial}{\partial y_t} \E_{w_t} [r(y_t - w_t)] \bigg \vert_{y_t = x_t + a_t} \left(\frac{\partial x_t}{\partial \thetabar_{h_0}} + \frac{\partial a_t}{\partial \thetabar_{h_0}}\right) 
\]
%\begin{align*}
%\frac{\partial}{\partial \thetabar_{h_0}} g(x_t,a_t) &= c \cdot \frac{\partial a_t}{\partial \thetabar_{h_0}} + \frac{\partial}{\partial y_t} \E_{w_t} [r(y_t - w_t)] \bigg \vert_{y_t = x_t + a_t} \frac{\partial y_t}{\partial \thetabar_{h_0}} \\
%&= c \cdot \frac{\partial a_t}{\partial \thetabar_{h_0}} + \frac{\partial}{\partial y_t} \E_{w_t} [r(y_t - w_t)] \bigg \vert_{y_t = x_t + a_t} \left(\frac{\partial x_t}{\partial \thetabar_{h_0}} + \frac{\partial a_t}{\partial \thetabar_{h_0}}\right) 
%\end{align*}
Again, the function $r(y-w_t)$ is differentiable in $y$ except at $y=w_t$ and $|\frac{\partial}{\partial y} r(y - w_t)| \leq \max\{b,p\}$. As the demand distribution is assumed to have a density over $[0, w_{\max}]$, the expectation term is differentiable using Leibniz rule. We can also write
\[
\frac{\partial a_t}{\partial \thetabar_{h_0}} = \frac{\partial \pi_{\theta}(s_t)}{\partial \thetabar_{h_0}} = \frac{\partial \pi_{\theta}(s_t)}{\partial x_t} \cdot \frac{\partial x_t}{\partial \thetabar_{h_0}}
\]
Repeatedly using the fact that threshold policies are differentiable everywhere except at one point, a little bit of algebra shows that $x_t$, $a_t$ and hence $g(x_t,a_t)$ is differentiable in $\thetabar_{h_0}$ except only at a finite number of points and $|\frac{\partial}{\partial \thetabar_{h_0}} g(x_t,a_t)|$ is bounded. Equation \eqref{eq:Bellman update differentiability inventory} shows that the same holds for $T_{\thetabar} J_{\theta}$, implying differentiability of $\Bc(\thetabar|\eta_{\pi_{\theta}},J_{\pi_{\theta}})$. Our arguments can be similarly extended to argue differentiability of $J_{\theta}$ and $\ell(\theta)$. We omit them for brevity.






%	Let $s_h=(x,h) \in \Sc_h$ denote a state in period h. Note that $\pi_{\theta}(s_h) = \theta_h - x$ for all $x < \theta_h$ and $\pi_{\theta}(s_h) = 0$ for all $x > \theta_h$. By Leibniz rule and the fact that $\eta_{\pi}$ is supported over $\Sc_h$ for each $h \leq H-1$, we have
%	\begin{align*}
%		\frac{\partial}{\partial \theta_h} \Bc(\theta|\eta_{\pi}, J^*) &= \frac{\partial}{\partial \theta_h} \int_{\Sc_h} Q^*(s_h,\pi_{\theta}(s_h)) \, d\eta_{\pi}(s_h) \\
%		&= \frac{\partial}{\partial \theta_h} \left[  \int_{x < \theta_h} Q^*(s_h,\theta_h - x) \, d\eta_{\pi}(s_h) + \int_{x > \theta_h} Q^*(s_h,0) \, d\eta_{\pi}(s_h) \right]\\
%		&= \int_{x < \theta_h} \frac{\partial}{\partial \theta_h} Q^*(s_h,\theta_h - x) \, d\eta_{\pi}(s_h) \\
%		&= \int_{x < \theta_h} \frac{\partial}{\partial a} Q^*(s_h,a) \at[\Big]{a=\pi_{\theta}(s_h)} d\eta_{\pi}( s_h)
%	\end{align*}
%	For simplicity, assume that there is a unique optimal policy and let $\theta^*$ be the corresponding optimal threshold. Consider any $\theta$ such that $\theta_h \neq \theta^*_h$ and let $\theta^{\alpha}_h = \theta_h + \alpha (\theta^*_h - \theta_h)$. We argue that $\frac{d}{d\alpha} \Bc(\theta^{\alpha}_h | \eta_{\pi}, J^*) \vert_{\alpha=0} < 0$, which implies a descent direction and therefore $\theta$ cannot be a stationary point. This follows as $Q^*(s_h,a)$ is convex with a minimum at $a=\pi_{\theta^*}(s_h)$. Clearly, we can reduce cost\footnote{If we cannot reduce cost, then $J_{\pi_{\theta}}(s_h) = J^*(s_h) $ $\rho$-almost surely. Assumption \ref{ass: exploratory rho finite horizon} then implies that $\theta_h$ is optimal for period $h$.} by moving $\theta_h$ in the direction of $\theta^*_h$, which is feasible as $\Theta_h$ is a bounded interval of $\mathbb{R}$.

%	\begin{align*}
%	\frac{\partial}{\partial \theta_h} \Bc(\theta|\eta, J^*) = 	\frac{\partial}{\partial \theta_h} \E_{s \sim \eta} \left[ Q^*(s, \pi_{\theta}(s))  \right] &\overset{(a)}{=} \int_{S \in \Sc_h} \frac{\partial}{\partial \theta_h} Q^*(S,\pi_{\theta}(s)) \, \eta(S) \, dS \\
%	&\overset{(b)}{=} \int_{S < \theta_h} \left[ \frac{\partial}{\partial a} Q^*(S,a) \at[\Big]{a=\pi_{\theta}(s)}  \frac{\partial}{\partial \theta_h} \pi_{\theta}(s) \right] \eta(S) \, dS
%	\end{align*}
%	%\jb{Local integrability (which follows from continuity of $\Bc(\theta|\eta,J^*)$) is enough for the interchange of derivative and integral.}
%	Note that $Q^*(S,a)$ is convex with a minimum at $a=\pi_{\theta^*_h}(S)$. Thus, $ \frac{\partial}{\partial a} Q^*(S,a) \at[\Big]{a=\pi_{\theta}(S)} > 0$ for $\theta_h < \theta^*_h$ (as we are ordering more) and $ \frac{\partial}{\partial a} Q^*(S,a) \at[\Big]{a=\pi_{\theta}(S)} < 0$ otherwise. Using this along with the fact that $\frac{\partial}{\partial \theta_h} \pi_{\theta}(S) = 1$ for $S < \theta_h$, we get that for any $S < \theta_h$,
%	\begin{align}
%	\label{eq:subopt_inventory}
%	\Bigl< \frac{\partial}{\partial \theta_h} \Bc(\theta|\eta, J^*), \theta'_h - \theta \Bigr> \geq 0 \,\, \forall \, \theta'_h \in \Theta_h \iff \Bigl< \frac{\partial}{\partial a} Q^*(S,a) \at[\Big]{a=\pi_{\theta}(S)}, \theta'_h - \theta_h \Bigr> \geq 0 \,\, \forall \, \theta'_h \in \Theta_h
%	\end{align}
%	which is sufficient to show that $\pi_{\theta}(S)$ is optimal for $S < \theta_h$ as $Q^*$ is convex. This in turn implies that the thresholds must match, i.e. $\theta_h = \theta^*_h$ (as $\pi_{\theta}(S) > 0$ for $S < \theta_h$).
%	
%	To justify the interchange of derivative and integral in (a), note that while formulating the problem in Example \ref{ex:inventorycontrol}, we argued that $\Sc_h, \Theta_h = \Mc = [-M,M]$ for some finite $M$ using boundedness of the demand distribution. The interchange is then justified using the dominated convergence theorem. For any $\theta_h \in \Theta_h$, clearly $Q^*(S,\pi_{\theta}(S)) \leq \sup_{s \in \Mc, \, a \in [0,2M]} \, |Q^*(S,a)|$. Let $\partial \pi(\theta_h, S)$ denotes the subdifferential of $\pi_{\theta}(S)$ at $\theta_h$. Then, 
%	\begin{align}
%	\label{eq:partial_bound_inventory_control}
%	\frac{\partial }{\partial \theta_h} Q^*(S,\pi_{\theta}(S)) \leq \sup_{s \in \Mc, \, a \in [0,2M]} \, \sup_{g \in \partial \pi(\theta_h, S)} \, \left|\frac{\partial}{\partial a} Q^*(S,a) \right| \cdot g \leq \sup_{s \in \Mc, \, a \in [0,2M]} \, \left|\frac{\partial}{\partial a} Q^*(S,a) \right|
%	\end{align}
%	as $\partial \pi(\theta_h, S) = [0,1]$ and $Q^*(S,a)$ is convex in $a$ for all $S \in \Sc_h$. Equality (b) can be justified using \eqref{eq:partial_bound_inventory_control} above and the fact that $\eta(\cdot)$ is supported over a bounded set (i.e. its not a delta function).









==> app_state_aggregation.tex <==
%!TEX root = policy_grad_optimality.tex

\section{An example of state aggregation}
\label{section:app_state_aggregation}
State aggregation is the simplest form of value function approximation employed in reinforcement learning and comes with strong stability properties \cite{gordon1995stable, tsitsiklis1996feature, van2006performance}. It is common across several academic communities \cite[e.g][]{whitt1978approximations, rust1997using}. 
Numerous theoretical papers carefully construct classes of MDPs with sufficient smooth dynamics, and upper bound the error from planning on a discretized state space \cite[e.g][]{ortner2012online}. The following example considers a continuous state, finite action problem which reduces to the tabular MDP case (in Example \ref{ex:tabularMDPs}) with state aggregation. It is not unreasonable to expect that an appropriate partitioning of the state space results in the policy class (class of stochastic policies over finite aggregated states) being approximately closed under policy improvement.

\begin{example}[State aggregation]
	We consider a problem with finite number of deterministic actions $k$ and take $\Ac=\Delta^{k-1}$ to be the set of probability distributions over actions. Let the state space, $\Sc \subset \mathbb{R}^{n}$, be a bounded convex subset of eucidean space where the dimension $n$ is thought to be small. We consider a partition of the state space into $m$ disjoint subsets, $\Sc = \cup_{i=1}^{m} \Sc_i$ and the set of stochastic policies over these subsets $\Pi  = \{ \pi \in \mathbb{R}^{m\times k}_{+}  :  \sum_{i=1}^{k} \pi(\Sc_j,i)  =1  \,\, \forall j = \{1,\cdots, m\}  \}$ such  that $\pi(s,i) = \pi(\Sc_j,i) \,\, \forall \, s \in \Sc_j$. Our result applies by assuming the partion is effective such that the approximation error, $\inf_{\pi \in \Pi} \, \|T_{\pi'} - T J\|_{1,\eta_{\pi}}$, is small for any cost-to-go function $J: \Sc \to \mathbb{R}$.
\end{example} 

%The following example describes state-aggregation in policy space. It satisfies all of our assumptions other than closure under policy improvement, but we expect it can be shown to be approximately closed under policy improvement. 
%\begin{example}[State aggregation]
%	There are a finite number of deterministic actions $k$, so we take $\Ac=\Delta^{k-1}$ to be the set of probability distributions over actions. 
%	$\Sc \subset \mathbb{R}^{n}$ is a bounded convex subset of eucidean space and the dimension $n$ is thought to be small. Reward functions and state transitions probabilities are smooth in $s$. We therefore expect an effective action in some state $s$ will be effective in another state $s'$ if  $\|s-s'\|$ is sufficiently small. We partition the state space $\Sc = \cup_{i=1}^{m} \Sc_i$ into $m$ disjoint subsets. We consider a modified softmax policy $\pi_{\theta}$ where $\theta = (\theta_{ij} :  1\leq i \leq m, 1\leq j \leq k)$. If $s \in \Sc_i$ lies in the $i$th subset of the state partition, $\pi_{\theta}(s)$ plays action $j\in \{1, \ldots , k\}$ with probability probability $e^{\theta_{ij}} / \sum_{\ell=1}^{k} e^{\theta_{i\ell}}$. 
%\end{example} 



==> app_tabular_rates.tex <==
%!TEX root = policy_grad_optimality.tex

\section{Proof of Theorem \ref{thm: tabular rates}}
We first restate the geometric convergence rate result in Theorem \ref{thm: tabular rates}.
\geometricthm*

Throughout the proof, we use some standard properties of the Bellman operator. For example, $J^*=TJ^*$ and that $T, T_{\pi}$ are a contraction in $\|\cdot\|$ with modulus $\gamma$ for any $\pi \in \Pi$. Refer to Section \ref{sec: app_bellman_background} for details. We denote $\pi^t_+$ to be the policy iteration update to any policy $\pi^t \in \Pi$.

\paragraph{Part (a): Proof for exact line-search:}
First, let us revisit the exact line search method applied for optimizing stepsizes as descibed in Section \ref{section:tabularMDPS}. At any iterate, $\pi^t$, let $\delta^t$ be a descent direction. Then exact linesearch solves for 
\[
\alpha^* = \argmin_{\alpha \geq 0} \ell(\pi^t_\alpha) := \ell(\pi^t + \alpha \delta^t)
\]
and updates to $\pi^{t+1} = \pi^t_{\alpha^*}$. The first-order algorithms we described in Section \ref{section:tabularMDPS} differ in the choice of descent directions. For example, Frank-Wolfe method chooses $\delta_t = \left( \pi^t_+ - \pi^t \right)$ as the descent directon while the projected gradient and natural policy gradient methods use $\nabla \ell(\pi^t)$ and its preconditioned (with the Fisher information matrix) counterpart respectively. We give a unified proof using a simple observation that updates for all the different first-order algorithms exactly equal the policy iteration update for some value of $\alpha$ (see Section \ref{section:tabularMDPS}). Therefore, $\pi^t_+$ is a feasible update for the exact line search method.
\begin{proof}
%Let $\alpha^* = \argmin_{\alpha \geq 0} \ell(\pi^t_{\alpha})$. 
Noting that $\pi^t_{\alpha^*}=\pi^{t+1}$, we have
\begin{align}
\label{eq:progress_linesearch}
\ell(\pi^{t+1}) = \| J_{\pi^{t+1}} \|_{1,\rho} \leq \| T_{\pi^{t+1}} J_{\pi^t} \|_{1,\rho} \leq \| T J_{\pi^t} \|_{1,\rho} 
\end{align}
where the first equality follows by definition. To see the second inequality, observe that 
\[
T_{\pi^{t+1}} J_{\pi^t} \preceq J_{\pi^t}
\]
Essentially, we cannot increase costs as $\pi^{t+1}=\pi^t$, corresponding to $\alpha=0$, is a feasible update. Then, monotonicity of $T_{\pi^{t+1}}$ implies: $J_{\pi^t}(s) \geq T_{\pi^{t+1}} J_{\pi^t}(s) \geq T^2_{\pi^{t+1}} J_{\pi^t}(s) \geq \ldots \geq J_{\pi^{t+1}}(s)$ using the definition $J_{\pi^{t+1}}(s) =  \lim_{n \to \infty} T^n_{\pi^{t+1}} J_{\pi^t}(s)$. The final inequality follows as $\pi^t_+$ is feasible update for all the four policy gradent methods with linesearch as explained above. Equation \eqref{eq:progress_linesearch} gives us a lower bound on the progress made with line search. Denote $\rho_{\min} := \min_{s \in \Sc} \rho(s)$. Then,
\begin{align}
	\label{eq:progress2_linesearch}
	\ell(\pi^t) - \ell(\pi^{t+1}) \geq \| J_{\pi^t} - T J_{\pi^t} \|_{1,\rho} &\geq \rho_{\min} \| J_{\pi^t} - T J_{\pi^t} \|_\infty \nonumber \\
	&= \rho_{\min} \| J_{\pi^t} - J^* - \left(T J_{\pi^t} - J^*\right) \|_\infty \nonumber \\
	&\geq \rho_{\min} \left\{ \| J_{\pi^t} - J^*\|_\infty - \|T J_{\pi^t} - TJ^*\|_\infty \right\} \nonumber \\
	&\geq \rho_{\min} \left( 1-\gamma \right)  \| J_{\pi^t} - J^*\|_\infty 
\end{align}
where we use that $\|J\|_{1,\rho} \geq \min_{s \in \Sc} \rho(s) \|J\|_\infty$ along with $J^*=TJ^*$ and contraction of $T$. It is easy to see,
\begin{align}
\label{eq:linesearch_intermediate}
\| J_{\pi^t} - J^*\|_\infty + \| J^* - J_{\pi^{t+1}} \|_\infty \geq \| J_{\pi^t} - J_{\pi^{t+1}}\|_\infty \geq \ell(\pi^t) - \ell(\pi^{t+1})
\end{align}
We get our desired result combining \eqref{eq:progress2_linesearch} and \eqref{eq:linesearch_intermediate} as well as using the fact that $J^* \preceq J_{\pi^{t+1}}$.
\begin{align*}
	J_{\pi^{t+1}} - J^*\|_\infty \leq \left( 1 - \rho_{\min}\left( 1-\gamma \right) \right) \| J_{\pi^t} - J^*\|_\infty \ldots \leq \left( 1 - \rho_{\min}\left( 1-\gamma \right)\right)^{t+1}  \| J_{\pi^0} - J^*\|_\infty
\end{align*}
\end{proof}

\paragraph{Part (b): Proof for constant stepsize Frank-Wolfe:}
Recall from Section \ref{section:tabularMDPS}, Frank-Wolfe exactly equals soft-policy iteration:
\[
\pi^{t+1}(s) = (1-\alpha)\pi^t(s) + \alpha \pi^t_+(s)
\]
where we denote $\pi^t_+$ to be the policy iteration update to $\pi^t$. Note that starting from a feasbile policy $\pi^0 \in \Pi$, we always maintain feasibility for $\alpha \in (0,1]$. Hence, for any state $s$
\begin{align*}
	T_{\pi^{t+1}} J_{\pi^t}(s) - T J_{\pi^t}(s) &= \langle \pi^{t+1}(s),Q^t(s,\cdot)  \rangle - \langle \pi^t_+(s),Q^t(s,\cdot)  \rangle \\
	&= (1-\alpha) \langle \pi^t(s),Q^t(s,\cdot)  \rangle - (1-\alpha) \langle \pi^t_+(s),Q^t(s,\cdot)  \rangle \\
	&= (1-\alpha) \left[J_{\pi^t}(s) - T J_{\pi^t}(s) \right]
\end{align*}
Using $T J_{\pi^t} \preceq J_{\pi^t}$, we also get
\[
T_{\pi^{t+1}} J_{\pi^t}(s) = (1-\alpha) J_{\pi^t}(s) + \alpha T J_{\pi^t}(s) \leq J_{\pi^t}(s)
\]
Monotonicty of $T_{\pi^{t+1}}$ implies: $J_{\pi^t}(s) \geq T_{\pi^{t+1}} J_{\pi^t}(s) \geq T^2_{\pi^{t+1}} J_{\pi^t}(s) \geq \ldots \geq J_{\pi^{t+1}}(s)$ using the definition $J_{\pi^{t+1}}(s) =  \lim_{n \to \infty} T^n_{\pi^{t+1}} J_{\pi^t}(s)$. Therefore,
\begin{align*}
		J_{\pi^{t+1}}(s) - T J_{\pi^t}(s) \leq T_{\pi^{t+1}} J_{\pi^t}(s) - T J_{\pi^t}(s) = (1-\alpha) \left[J_{\pi^t}(s) - T J_{\pi^t}(s) \right]
\end{align*}
Subtracting $J^*(s)$ from  both sides and rearranging terms,
\begin{align*}
J_{\pi^{t+1}}(s)- J^*(s) \leq (1-\alpha)\left(J_{\pi^t}(s) - J^*(s)\right) + \alpha \left(T J_{\pi^t}(s) - J^*(s) \right)
\end{align*}
The above inequality holds for any $s$, therefore 
\begin{align*}
\norm{J_{\pi^{t+1}} - J^*}_{\infty} \leq (1-\alpha) \norm{J_{\pi^t} - J^*}_{\infty} +  \alpha \norm{T J_{\pi^t} - J^*}_{\infty} \leq \left[ (1-\alpha) + \gamma \alpha \right] \norm{J_{\pi^t} - J^*}_{\infty}
\end{align*}
where we used that $J^*=TJ^*$ and $\norm{TJ_{\pi^t}-TJ^*}_{\infty}\leq \gamma \norm{J_{\pi^t}-J^*}_{\infty}$ (as $T(\cdot)$ is a contraction). Iterating over the above equation gives us our final result.
\begin{align*}
\norm{J_{\pi^{t+1}} - J^*}_{\infty} \leq \left(1 - \alpha(1-\gamma) \right) \norm{J_{\pi^t} - J^*}_{\infty} \leq \left(1 - \alpha(1-\gamma) \right)^t \norm{J_{\pi^0} - J^*}_{\infty}
\end{align*}


\paragraph{Part (c): Proof for constant stepsize natural policy gradient:}
Recall that for $\theta \in \mathbb{R}^{n \times k}$, the softmax policy parameterization takes action $i$ in state $s$ with probability $\pi_{\theta}(i|s)$:
\[
\pi_{\theta}(i|s) = \frac{e^{\theta_{s,i}}}{\sum_{j=1}^k e^{\theta_{s,j}}} \qquad i = 1,\ldots,k.
\]
As shown in Section \ref{section:tabularMDPS}, the natural policy gradient (NPG) updates with a constant stepsize $\alpha$ take the simple form:
\begin{equation}
\label{eq:NPG_updates}
\pi^{t+1}(i|s) = \frac{\pi^{t}(i|s) \cdot e^{-\alpha Q^{t}(i,s)}}{\sum_{j=1}^k \pi^{t}(j|s) \cdot e^{-\alpha Q^{t}(j,s)}},
\end{equation}
where we use the shorthand notation $\pi^{t}(\cdot)$ to denote $\pi_{\theta^{t}}(\cdot)$ and $Q^{t}(s,i)$ to denote $Q_{\pi_{\theta^t}}(s,i)$. 

Our proof strategy follows essentially shows that for any state $s \in \Sc$, the NPG update decrease the probability of \textit{sub-optimal} actions by a multiplicative factor. Informally, the set of sub-optimal actions (per state) can be understood as the set of actions with action gap\footnote{The action gap of any action $i \in \{1,\ldots,k\}$ is the difference between Q-values of the action and Q-value of the optimal action.} larger than some threshold. Essentially, this shows the NPG update is equivalent to a soft policy iteration update upto some small additive error. We divide the proof into three steps.
	
\paragraph{Step 1: NPG update for \textit{sub-optimal} actions:}
Fix some state $s \in \Sc$. Without loss of generality, we assume the following ordering on the Q-values: $Q^t(s,1) < Q^t(s,2) \ldots < Q^t(s,k)$ which implies that action 1 is optimal in state $s$ under policy $\pi^t$. For any $c \in (0,1)$, define $O_t^-(s)$ and $O_t^+(s)$ as:
\begin{align*}
O_t^-(s) &:= \left\{ i \,\, |\,\, Q^t(s,i) - Q^t(s,1) \geq \frac{\log (1/c)}{\alpha} \right\} \\
O_t^+(s) &:= \left\{ i \,\, |\,\, Q^t(s,i) - Q^t(s,1) \leq \frac{\log (1/c)}{\alpha} \right\}
\end{align*}
For simplicity, we will take $c=\frac{1}{2}$ although all our results hold for any $c \in (0,1)$. Denote $\epsilon := \frac{\log 2}{\alpha}$. The set $O_t^-(s)$ can be interpreted as the set of \textit{sub-optimal} actions with the \textit{action gap}, $Q^t(s,i) - Q^t(s,1)$, larger than the threshold $\epsilon$. Similarly, $O_t^+(s)$ can be interpreted to be the set of \textit{nearly optimal} actions according to the policy $\pi^t$. The following lemma shows that the NPG updates decrease the probability of playing sub-optimal actions by a multiplicative factor.

\begin{restatable}[]{lem}{}
	\label{lemma:suboptimal_actions}
	For any state $s$, $\frac{\pi^{t+1}(i|s)}{\pi^t(i|s)} \leq \frac{1}{2} \,\,\, \forall \, i \in O_t^-(s)$.
\end{restatable}
\begin{proof}
	The proof follows a simple argument. By definition, for any $i \in O_t^-(s)$:
	\begin{align*}
	\alpha \left( Q^t(s,i) - Q^t(s,1) \right) &\geq \log (2) \\
	\Rightarrow \, \alpha \left( Q^t(s,i) - Q^t(s,1) \right) &\geq \log (2) - \log(\pi^t(1|s))
	\end{align*}
	which follows as $\pi^t(1|s) \in (0,1)$. Rearranging, we get
	\[
	\log \left(\pi^{t}(1|s) e^{-\alpha Q^{t}(s,1)} \right) + \log(\frac{1}{2}) \geq -\alpha Q^{t}(s,i)
	\]
	This implies,
	\[
	\log \left( \sum_{j=1}^k \pi^{t}(j|s) e^{-\alpha Q^{t}(s,j)} \right) + \log(\frac{1}{2}) \geq \log \left(\pi^{t}(1|s) e^{-\alpha Q^{t}(s,1)} \right) + \log(\frac{1}{2}) \geq -\alpha Q^{t}(s,i).
	\]
	which holds as all the terms in the summation are positive, $\pi^{t}(j|s) e^{-\alpha Q^{t}(s,j)} > 0 \,\,\, \forall \, j \in \{1,2,\ldots,k\}$ and $\log(\cdot)$ is a monotonic transformation. Our result holds by noting
	\[
	\frac{1}{2} \left( \sum_{j=1}^k \pi^{t}(j|s) e^{-\alpha Q^{t}(s,j)} \right) \geq e^{-\alpha Q^{t}(s,i)} \quad \Rightarrow \quad \frac{\pi^{t+1}(i|s)}{\pi^t(i|s)} = \frac{e^{-\alpha Q^{t}(s,i)}}{\sum_{j=1}^k \pi^{t}(j|s) e^{-\alpha Q^{t}(s,j)}} \leq \frac{1}{2}.
	\]
\end{proof}

\paragraph{Step 2: NPG updates as soft policy iteration:}
Recall that the policy iteration update, $\pi^t_+(s)=\argmin_{i \in \{1,2,\ldots,k\}} \,\, Q^t(s,i)$, which puts the entire mass on the best action (according to Q-values) and zeros out the probability of playing other actions. On the other hand, Lemma \ref{lemma:suboptimal_actions} shows how the NPG update decays the probabilities of \textit{sub-optimal} actions (in the set $O_t^-(s)$) by a multiplicative factor instead of zeroing them out\footnote{This defintion of sub-optimal actions based on action gap threshold, $\epsilon=\log(2)/\alpha$, is essentially an artifact that we are taking gradient steps with finite stepsizes. As $\alpha \to \infty$, the threshold $\epsilon \to 0$ making the NPG update equivalent to a soft-policy iteration update.}. Thus intuitively, the NPG update resemble a \textit{soft} policy iteration update for the set of actions $O_t^-(s)$. We formalize this intuition in the following lemma which characterizes the progress made by an NPG update vis-a-vis the policy iteration update.
\begin{restatable}[Progress quantification]{lem}{}
	\label{lemma:progress_quanitification}
	Let $J_{\pi^t}(s)$ denote the cost-to-go function for policy $\pi^t$ from any starting state $s$. Then, 
	\[
	T_{\pi^{t+1}} J_{\pi^t}(s) - J_{\pi^t}(s) \leq  \frac{1}{2} \cdot \left( T J_{\pi^t}(s) - J_{\pi^t}(s) \right) + \epsilon 
	\]
\end{restatable}
\begin{proof}
	Recall, we assumed that: $Q^t(s,1) < Q^t(2) \ldots < Q^t(s,k)$ which implies that the policy iteration update, $\pi^{+}_t$ puts the entire mass on action 1. That is,
	$\pi^t_+(1|s)=1$ and $\pi^t_+(i|s)=0 \,\,\, \forall \,\, i \neq 1$. Consider,
	\begin{align}
	T_{\pi^{t+1}} J_{\pi^t}(s) - T J_{\pi^t}(s) &= \langle \pi^{t+1}(\cdot|s) - \pi^+_t(\cdot|s), Q^t(s,\cdot) \rangle \nonumber \\
	&= (\pi^{t+1}(1|s)-1) Q^t(s,1) + \sum_{j=2}^k \pi^{t+1}(j|s) Q^t(s,j) \nonumber \\
	&= - \sum_{j=2}^k \pi^{t+1}(j|s) Q^t(s,1) + \sum_{j=2}^k \pi^{t+1}(j|s) Q^t(s,j) \nonumber \\
	&= \sum_{j=2}^k \pi^{t+1}(j|s) \left( Q^t(s,j) - Q^t(s,1) \right) \nonumber \\
	&= \sum_{j \in \mathcal{O}_{t}^{-}} \pi^{t+1}(j|s) \left( Q^t(s,j) - Q^t(s,1) \right) + \sum_{j \in \mathcal{O}_{t}^{+}} \pi^{t+1}(j|s) \left( Q^t(s,j) - Q^t(s,1) \right) \nonumber \\
	&= \sum_{j \in \mathcal{O}_{t}^{-}} \frac{\pi^{t+1}(j|s)}{\pi^t(j|s)} \pi^t(j|s) \left( Q^t(s,j) - Q^t(s,1) \right) + \sum_{j \in \mathcal{O}_{t}^{+}} \pi^{t+1}(j|s) \underbrace{\left( Q^t(s,j) - Q^t(s,1)\right)}_{\leq \epsilon} \nonumber \\
	&\leq \frac{1}{2} \sum_{j \in \mathcal{O}_{t}^{-}} \pi^t(j|s) \left( Q^t(s,j) - Q^t(s,1) \right) + \epsilon \nonumber \\
	&\leq \frac{1}{2} \left( \sum_{j=2}^k \pi^t(j|s) ( Q^t(s,j) - Q^t(s,1) ) \right) + \epsilon \nonumber \\
	&= \frac{1}{2} \left( \sum_{j=2}^k \pi^t(j|s) Q^t(s,j) - \sum_{j=2}^k \pi^t(j|s) Q^t(s,1)\right) + \epsilon \nonumber \\
	&= \frac{1}{2} \left( \left(\pi^t(j|s)-1\right) Q^t(s,1) + \sum_{j=2}^k \pi^t(j|s) Q^t(s,j) \right) + \epsilon \nonumber \\
	&= \frac{1}{2} \, \langle \pi^t(\cdot|s) - \pi^+_t(\cdot|s), Q^t(s,\cdot) \rangle + \epsilon \nonumber \\
	&= \frac{1}{2} \, \left( J_{\pi^t}(s) - T J_{\pi^t}(s) \right) + \epsilon
	\label{eq:NPG_intermediate}
	\end{align}
	where we used that $\frac{\pi^{t+1}(j|s)}{\pi^t(j|s)} \leq \frac{1}{2} \,\,\, \forall \, j \in \mathcal{O}_{t}^{-}(s)$ as shown above in Lemma \ref{lemma:suboptimal_actions} along with the fact that $\left( Q^t(s,j) - Q^t(s,1) \right) \leq \epsilon \,\,\, \forall \, j \in \mathcal{O}_{t}^{+}(s)$ which follows by definition. Subtracting $J_{\pi^t}(s)$ from both sides in Equation \eqref{eq:NPG_intermediate} and rearranging terms gives our desired result
	\[
	T_{\pi^{t+1}} J_{\pi^t}(s) - J_{\pi^t}(s) \leq  \frac{1}{2} \cdot \left( T J_{\pi^t}(s) - J_{\pi^t}(s) \right) + \epsilon 
	\]
%	\[
%	J_{\pi^t}(s) - T_{\pi^{t+1}} J_{\pi^t}(s) \leq  \frac{1}{2} \, \left( J_{\pi^t}(s) - T J_{\pi^t}(s) \right) + \epsilon 
%	\]
\end{proof}
	
\paragraph{Step 3: Completing the proof:}
Lemma \ref{lemma:progress_quanitification} clearly quantifies the relationship between an NPG update with constant stepsize $\alpha$ and a soft policy iteration update with an additive error $\epsilon$. With this connection, we give a simple proof of geometric convergence for the natural policy gradient method. We claim that $J_{\pi^{t+1}}(s) \leq J_{\pi^t}(s)$. To see this, note that for any stepsize $\alpha$, the NPG update for state $s$ can be equivalently written as:
\[
\pi^{t+1}(s) = \argmin_{a \in \Delta^{k-1}} \left[ Q^t(s,a) + \frac{\eta_{\pi^t(s)}}{\alpha} D_{\rm KL}(a||\pi^t(s)) \right]
\]
As $a = \pi^t(s)$ is feasible for the optimization problem above, 
\[
T_{\pi^{t+1}} J_{\pi^t}(s) = Q^t(s,\pi^{t+1}(s)) \leq Q^t(s,\pi^t(s)) = J_{\pi^t}(s)
\]
By monotonicty property of $T_{\pi^{t+1}}$, we have $J_{\pi^t}(s) \geq T_{\pi^{t+1}} J_{\pi^t}(s) \geq T^2_{\pi^{t+1}} J_{\pi^t}(s) \geq \ldots \geq J_{\pi^{t+1}}(s)$ by noting that $J_{\pi^{t+1}}(s) =  \lim_{n \to \infty} T^n_{\pi^{t+1}} J_{\pi^t}(s)$. From Lemma \ref{lemma:progress_quanitification}, we get
\[
J_{\pi^{t+1}}(s) - J_{\pi^t}(s) \leq T_{\pi^{t+1}}J_{\pi^t}(s) - J_{\pi^t}(s) \leq \frac{1}{2} \cdot \left( T J_{\pi^t}(s) - J_{\pi^t}(s) \right) + \epsilon
\]
Subtracting $J^*(s)$ from  both sides and rearranging terms,
\begin{align*}
J_{\pi^{t+1}}(s)- J^*(s) &\leq \frac{1}{2} J_{\pi^t}(s) + \frac{1}{2} T J_{\pi^t}(s) - J^*(s) + \epsilon  \\
&= \frac{1}{2} \left(J_{\pi^t}(s) - J^*(s)\right) +  \frac{1}{2} \left(T J_{\pi^t}(s) - J^*(s) \right) + \epsilon
\end{align*}
which implies,
\begin{align*}
\norm{J_{\pi^{t+1}} - J^*}_{\infty} &\leq \frac{1}{2} \norm{J_{\pi^t} - J^*}_{\infty} +  \frac{1}{2} \norm{T J_{\pi^t} - J^*}_{\infty} + \epsilon \\
&\leq \left[ \frac{1}{2} + \frac{\gamma}{2} \right] \norm{J_{\pi^t} - J^*}_{\infty} + \epsilon
\end{align*}
where we used that $\norm{TJ_{\pi^t}-J^*}_{\infty}=\norm{TJ_{\pi^t}-TJ^*}_{\infty}\leq \gamma \norm{J_{\pi^t}-J^*}_{\infty}$ which follows from the contraction property of, $T(\cdot)$. Rewriting $\left( \frac{1}{2} + \frac{\gamma}{2}\right) = \left( 1 - \frac{1}{2}(1-\gamma) \right)$ and iterating over the above equation gives us our final result.
\begin{align*}
%\label{eq:NPGfinal}
\norm{J_{\pi^{t+1}} - J^*}_{\infty} &\leq \left(1 - \frac{(1-\gamma)}{2} \right) \norm{J_{\pi^t} - J^*}_{\infty} + \epsilon \\
&\leq \left(1 - \frac{(1-\gamma)}{2}\right)^t \norm{J_{\pi^0} - J^*}_{\infty} + \epsilon \sum_{i=0}^{t-1} \left( 1 - \frac{(1-\gamma)}{2}\right)^i \\
&\leq \left(1 - \frac{(1-\gamma)}{2}\right)^t \norm{J_{\pi^0} - J^*}_{\infty} + \frac{2\epsilon}{(1-\gamma)}
%&= \left(1 - \frac{(1-\gamma)}{2}\right)^t \norm{J^* - J_{\pi^0}}_{\infty} + \frac{2\log 2}{\alpha (1-\gamma)} \\
%%&= \left(1 - \frac{(1-\gamma)}{2}\right)^t \norm{J^* - J_{\pi^0}}_{\infty} + \frac{2\log 2}{\eta}
\end{align*}
%where the final equality follows by the definition: $\alpha = \frac{\eta}{(1-\gamma)}$. 
%Essentially, a larger stepsize $\alpha$ decreases the constant error $\epsilon$. 
As $\alpha \to \infty$, constant error term $\epsilon \to 0$ and therefore NPG update is exactly the policy iteration step.



==> app_tabular_rates_old.tex <==
%!TEX root = policy_grad_optimality.tex

\section{Proof of Theorem \ref{thm: tabular rates}}

\subsection{Part 3: Natural policy gradient with constant stepsize}
\textcolor{red}{NEED TO RETURN TO MAKE THIS CONSISTENT}\\
In the previous sections, we exploited a powerful connection between policy gradients and weighted policy iteration to show polynomial convergence rates to the optimal policy for MDPs with special structural properties. Surprisingly, for finite MDPs, it turns out that the natural policy gradient (NPG) update with softmax policies decouples across states and mimics a policy iteration update up to a constant error term. It is easy to show that policy iteration converges geometrically to the optimal policy; hence using this connection, we show a geometric convergence rate result for NPG with softmax policies which is \textit{dimension free}\footnote{The rate is independent of the number of states and actions in the finite MDP.}. This result is an improvement over the recent result of \cite{agarwal2019optimality} which gives an $\mathcal{O}(1/T)$ dimension free convergence rate for NPG updates with softmax policies.

We briefly review the exact form of NPG updates for softmax policy parameterization. For unconstrained $\theta \in \mathbb{R}^{|\Sc||\Ac|}$, the softmax policy parameterization takes action $a$ in state $s$ with probability $\pi_{\theta}(a|s)$:
\[
\pi_{\theta}(a|s) = \frac{e^{\theta_{s,a}}}{\sum_{a' \in \Ac} e^{\theta_{s,a'}}}
\]
Let the Fisher information matrix induced by the policy $\pi(\theta)$ be defined as:
\[
F_{\rho}(\theta) = \E_{s \sim \eta^{\pi_{\theta}}_{\rho}} \E_{a \sim \pi_{\theta(\cdot | s)}} \left[ \nabla_{\theta} \log \pi_{\theta}(a|s) \left( \nabla_{\theta} \log \pi_{\theta}(a|s) \right)^{T} \right]
\]
where $\eta^{\pi_{\theta}}_{\rho}$ is the steady state distribution associated with $\pi_{\theta}(\cdot)$ and the start state distribution $\rho(\cdot)$ as defined in Equation \eqref{}. The natural policy gradient algorithm uses the Fisher information matrix to precondition the policy gradient updates as:
\[
\theta^{t+1} = \theta^t + \eta F_{\rho}(\theta^t)^{\dagger} \nabla_{\theta} \ell(\theta^t) 
\]
where $M^{\dagger}$ denotes the Moore-Penrose pseudoinverse of matrix M. As shown in \citep{kakade2002natural,agarwal2019optimality}, the NPG updates for softmax policies decouple across states and take a very simple form:
\begin{equation}
\label{eq:NPG_updates}
\pi^{t+1}(i|s) = \frac{\pi^{t}(i|s) \cdot e^{\eta Q^{t}(i,s)/(1-\gamma)}}{\sum_{j \in \Ac} \pi^{t}(j|s) \cdot e^{\eta Q^{t}(j,s)/(1-\gamma)}},
\end{equation}
where we use the shorthand notation $\pi^{t}(\cdot)$ to denote $\pi_{\theta^{t}}(\cdot)$ and $Q^{t}(i,s)$ to denote $Q_{\pi_{\theta_t}}(i,s)$, the state-action value function corresponding to policy $\pi_{\theta_t}$. Careful readers will note a striking similarity of NPG updates to the multiplicative weight updates algorithm of \citep{freund1995desicion,cesa2006prediction} for online linear optimization over the probability simplex\footnote{The NPG updates shown in \citep{kakade2002natural,agarwal2019optimality} use the advantage function, $A^{t}(i,s) = Q^t(i,s) - V^t(s)$, where $A^{t}(i,s)$ denotes the advantage of playing action $i$ in state $s$ under policy $\pi^t(\cdot)$. As $V^t(s)$ is constant for a given state, we can replace $A^{t}(i,s)$ by the q-values $Q^t(i,s)$ due to the normalized form of the updates.}. We emphasize the readers to note how the NPG updates decouple across states; we use this fact crucially to make a connection with policy iteration. We state our result formally in Theorem \ref{thrm:NPG_updates} below. Importantly, as the step-size $\eta \to \infty$, the constant error term vanishes and the results looks exactly like what one would expect with \textit{policy iteration updates}. This is no coincidence, as $\eta \to \infty$, the NPG updates can be shown to exactly mimic the policy iteration update. 

\begin{restatable}[Geometric convergence of NPG with softmax policies]{thm}{}
	\label{thrm:NPG_updates}
	Consider the Natural policy gradient updates for softmax policies \eqref{eq:NPG_updates} for any initial guess $\theta^0$ and start state distribution $\rho \in \Delta(\Sc)$. Let $J^*$ denotes the optimal cost-to-go function and $J_{\pi^t}$ denote the cost-to-go function corresponding to policy $\pi_{\theta_t}$. Fix any constant step-size $\eta > 0$. Then,
	\[
	\norm{J_{\pi^{t+1}}-J^*}_{\infty} \leq \left(1 - \frac{(1-\gamma)}{2}\right)^t \norm{J_{\pi^0}-J^*}_{\infty} + \frac{2\log 2}{\eta}
	\]
\end{restatable}
The proof strategy follows essentially from a very simple idea. For any state $s \in \Sc$, we show that the NPG update decrease the probability of \textit{sub-optimal} actions by a multiplicative factor. The set of sub-optimal actions (per state) can be understood to be those with action gap\footnote{The difference between the Q-values of the best action and the selected action.} larger than a threshold (that inversely depends on the step-size $\eta$).

\begin{proof}[Proof of Theorem \ref{thrm:NPG_updates}]
	Throughout, we assume the action space for each state $s \in \Sc$ to have $K$ possible actions, $\Ac(s) = \{1,2,\ldots,K\}$. Define $\alpha := \frac{\eta}{(1-\gamma)}$. The NPG update with stepsize $\eta$ updates the probability of taking action $i$ in state $s$ as,
	\begin{equation*}
	\pi^{t+1}_{\alpha}(i|s) = \frac{\pi^{t}(i|s) e^{\alpha Q^{t}(s,i)}}{\sum_{j=1}^K \pi^{t}(j|s) e^{\alpha Q^{t}(s,j)}}.
	\end{equation*}
	Notice how the updated probabilities decouple across states\footnote{The updated probabilities for a state-action pair do not depend on the Q-values of actions in other states.}, a nice property of the NPG update we critically exploit to make an explicit connection with policy iteration updates. Without loss of generality, we fix state $s$. The proof idea is simple and can broadly be divide into three steps. 
	
	\paragraph{Step 1: NPG update for \textit{sub-optimal} actions:}
	We first show that for any state, an NPG update decreases the probabilities of \textit{sub-optimal} arms by atleast a multiplicative factor. We formalize this below. Recall that $\pi^t(\cdot|s)$ denotes the policy at time $t$ (corresponding to the iterate $\theta_t$) and and $Q^t(s,\cdot)$ denotes its state-action value function. Without loss of generality, we assume the following ordering on the Q-values: $Q^t(s,1) < Q^t(s,2) \ldots < Q^t(s,K)$. As we are minimizing costs, action 1 is thus optimal for state $s$ under policy $\pi^t$. For any $k \in (0,1)$, we define two sets, $O_t^-(s)$ and $O_t^+(s)$, as:
	\begin{align*}
	O_t^-(s) &:= \left\{ i \,\, |\,\, Q^t(s,i) - Q^t(s,1) \geq \frac{\log (1/k)}{\alpha} \right\} \\
	O_t^+(s) &:= \left\{ i \,\, |\,\, Q^t(s,i) - Q^t(s,1) \leq \frac{\log (1/k)}{\alpha} \right\}
	\end{align*}
	For simplicity, we will take $k=\frac{1}{2}$ although all our results hold for any $k \in (0,1)$. The set $O_t^-(s)$ can be interpreted as the set of \textit{sub-optimal} actions with the \textit{action gap}, the difference between Q-values when compared to the optimal action: $Q^t(s,a) - Q^t(s,1)$, being larger than the threshold $\epsilon := \frac{\log 2}{\alpha}$. Similarly, $O_t^+(s)$ can be interpreted to be the set of \textit{nearly optimal} actions according to the policy $\pi^t(\cdot|s)$. The following lemma shows that the NPG updates decrease the probability of playing sub-optimal actions by a multiplicative factor.
	
	\begin{restatable}[]{lem}{}
		\label{lemma:suboptimal_actions}
		For any state $s$, $\frac{\pi^{t+1}_\alpha(i|s)}{\pi^t(i|s)} \leq \frac{1}{2} \,\,\, \forall \, i \in O_t^-(s)$.
	\end{restatable}
	\begin{proof}
		The proof follows a simple argument. By definition, for any $i \in O_t^-(s)$:
		\begin{align*}
		\alpha \left( Q^t(s,1) - Q^t(s,i) \right) &\geq \log \left( 2 \right) \\
		\Rightarrow \, \alpha \left( Q^t(s,1) - Q^t(s,i) \right) &\geq \log \left( 2\right) - \log(\pi^t(1))
		\end{align*}
		which follows as $\pi^t(1|s) \in (0,1)$. Rearranging, we get
		\[
		\log \left(\pi^{t}(1|s) e^{\alpha Q^{t}(s,1)} \right) + \log(\frac{1}{2}) \geq \alpha Q^{t}(s,i)
		\]
		This implies,
		\[
		\log \left( \sum_{j=1}^K \pi^{t}(j|s) e^{\alpha Q^{t}(s,j)} \right) + \log(\frac{1}{2}) \geq \log \left(\pi^{t}(1|s) e^{\alpha Q^{t}(s,1)} \right) + \log(\frac{1}{2}) \geq \alpha Q^{t}(s,i).
		\]
		which holds as all the terms in the summation are positive, $\pi^{t}(j|s) e^{\alpha Q^{t}(s,j)} > 0 \,\,\, \forall \, j \in \{1,2,\ldots,K\}$ and $\log(\cdot)$ is a monotonic transformation. Our result holds by noting
		\[
		\frac{1}{2} \left( \sum_{j=1}^K \pi^{t}(j|s) e^{\alpha Q^{t}(s,j)} \right) \geq e^{\alpha Q^{t}(s,i)} \quad \Rightarrow \quad \frac{\pi^{t+1}_\alpha(i|s)}{\pi^t(i|s)} = \frac{e^{\alpha Q^{t}(s,i)}}{\sum_{j=1}^K \pi^{t}(j|s) e^{\alpha Q^{t}(s,j)}} \leq \frac{1}{2}.
		\]
	\end{proof}
	
	\paragraph{Step 2: NPG updates as soft policy iteration:}
	Lemma \ref{lemma:suboptimal_actions} already gives an intuitive connection to policy iteration. Recall, how the policy iteration update: $\pi^+_t(s)=\argmin_{i \in \{1,2,\ldots,K\}} \,\, Q^t(s,i)$, puts the entire mass on the best action (according to Q-values) and zeros out the probability of playing other actions. On the other hand, the NPG update decays the probabilities of \textit{sub-optimal}\footnote{This defintion of sub-optimal actions based on action gap threshold is essentially an artifact that we are taking gradient steps with finite stepsizes.} actions (in the set $O_t^-(s)$) instead of zeroing them out. Intuitively, the NPG update resemble a \textit{soft} policy iteration update. We formalize this intuition in he following lemma which characterizes the progress made by an NPG update vis-a-vis the policy iteration step.
	\begin{restatable}[Progress quantification]{lem}{}
		\label{lemma:progress_quanitification}
		Let $J_{\pi^t}(s)$ denote the cost-to-go function for policy $\pi^t$ from any starting state $s$. Then, 
		\[
		J_{\pi^t}(s) - T_{\pi^{t+1}_{\alpha}} J_{\pi^t}(s) \leq  \frac{1}{2} \cdot \left( J_{\pi^t}(s) - T J_{\pi^t}(s) \right) + \epsilon 
		\]
	\end{restatable}
	\begin{proof}
		Recall that we assumed without loss of generality that: $Q^t(s,1) < Q^t(2) \ldots < Q^t(s,K)$ which implies the policy iteration update, $\pi^{+}_t$ puts the entire mass on action 1 (the optimal action according to $\pi^t$). That is,
		$\pi^+_t(1)=1$ and $\pi^+_t(i)=0 \,\,\, \forall \,\, i \neq 1$
		Now consider,
		\begin{align}
		T J_{\pi^t}(s) - T_{\pi^{t+1}_{\alpha}} J_{\pi^t}(s) &= \langle \pi^+_t(\cdot|s) - \pi^{t+1}_{\alpha}(\cdot|s), Q^t(s,\cdot) \rangle \nonumber \\
		&= (1-\pi^{t+1}_{\alpha}(1|s)) Q^t(s,1) - \sum_{j=2}^K \pi^{t+1}{\alpha}(j|s) Q^t(s,j) \nonumber \\
		&= \sum_{j=2}^K \pi^{t+1}_{\alpha}(j|s) Q^t(s,1) - \sum_{j=2}^K \pi^{t+1}_{\alpha}(j|s) Q^t(s,j) \nonumber \\
		&= \sum_{j=2}^K \pi^{t+1}_{\alpha}(j|s) \left( Q^t(s,1) - Q^t(s,j) \right) \nonumber \\
		&= \sum_{j \in \mathcal{O}_{t}^{-}} \pi^{t+1}_{\alpha}(j|s) \left( Q^t(s,1) - Q^t(s,j) \right) + \sum_{j \in \mathcal{O}_{t}^{+}} \pi^{t+1}_{\alpha}(j|s) \left( Q^t(s,1) - Q^t(s,j) \right) \nonumber \\
		&= \sum_{j \in \mathcal{O}_{t}^{-}} \frac{\pi^{t+1}_{\alpha}(j|s)}{\pi^t(j|s)} \pi^t(j|s) \left( Q^t(s,1) - Q^t(s,j) \right) + \sum_{j \in \mathcal{O}_{t}^{+}} \pi^{t+1}_{\alpha}(j|s) \underbrace{\left( Q^t(s,1) - Q^t(s,j)\right)}_{\leq \epsilon} \nonumber \\
		&\leq \frac{1}{2} \sum_{j \in \mathcal{O}_{t}^{-}} \pi^t(j|s) \left( Q^t(s,1) - Q^t(s,j) \right) + \epsilon \nonumber \\
		&\leq \frac{1}{2} \left( \sum_{j=2}^K \pi^t(j|s) ( Q^t(s,1) - Q^t(s,j) ) \right) + \epsilon \nonumber \\
		&= \frac{1}{2} \left( \sum_{j=2}^K \pi^t(j|s) Q^t(s,1) - \sum_{j=2}^K \pi^t(j|s) Q^t(s,j)\right) + \epsilon \nonumber \\
		&= \frac{1}{2} \left( \left(1-\pi^t(j|s) \right) Q^t(s,1) - \sum_{j=2}^K \pi^t(j|s) Q^t(s,j) \right) \nonumber \\
		&= \frac{1}{2} \, \langle \pi^+_t(\cdot|s) - \pi^t(\cdot|s), Q^t(s,\cdot) \rangle + \epsilon \nonumber \\
		&= \frac{1}{2} \, \left( T J_{\pi^t}(s) - J_{\pi^t}(s)\right) + \epsilon
		\label{eq:NPG_intermediate}
		\end{align}
		where we used that $\frac{\pi^{t+1}_{\alpha}(j)}{\pi^t(j)} \leq \frac{1}{2} \,\,\, \forall \, j \in \mathcal{O}_{t}^{-}$ as shown above in Lemma \ref{lemma:suboptimal_actions} along with the fact that $\left( Q^t(s,j) - Q^t(s,1) \right) \leq \epsilon \,\,\, \forall \, j \in \mathcal{O}_{t}^{+}$ which follows by definition of the set $\mathcal{O}_{t}^{+}$. Adding $J_{\pi^t}(s)$ to both sides in Equation \eqref{eq:NPG_intermediate} and rearranging terms gives our final result
		\[
		J_{\pi^t}(s) - T_{\pi^{t+1}_{\alpha}} J_{\pi^t}(s) \leq  \frac{1}{2} \, \left( J_{\pi^t}(s) - T J_{\pi^t}(s) \right) + \epsilon 
		\]
	\end{proof}
	
	\paragraph{Step 3: Completing the proof of Theorem \ref{thrm:NPG_updates}:}
	Lemma \ref{lemma:progress_quanitification} clearly quantifies the relationship between an NPG update with a finite step-size and a policy iteration update. With this connection, we give a simple proof of geometric convergence of NPG updates for finite MDPs. First note that using the monotonicity property of the Bellman operator (for example, see Chapter 1 in \citep{bertsekas1995dynamic}), we have
	\[
	J_{\pi^{t+1}_{\alpha}}(s) \geq T_{\pi^{t+1}_{\alpha}} J_{\pi^t}(s).
	\]
	Thus, we conclude
	\[
	J_{\pi^t}(s) - J_{\pi^{t+1}_\alpha}(s) \, \leq \, J_{\pi^t}(s) - T_{\pi^{t+1}_{\alpha}} J_{\pi^t}(s) \, \leq \, \frac{1}{2} \cdot \left( J_{\pi^t}(s) - T J_{\pi^t}(s) \right) + \epsilon 
	\]
	Adding $J^*$ to both sides and rearranging terms, we get
	\begin{align*}
	J^*(s) - J_{\pi^{t+1}_\alpha}(s) &\leq J^*(s) - \frac{1}{2} J_{\pi^t}(s) - \frac{1}{2} T J_{\pi^t}(s) + \epsilon \\
	&= \frac{1}{2} \left( J^*(s) - J_{\pi^t}(s) \right) +  \frac{1}{2} \left( J^*(s) - T J_{\pi^t}(s) \right) + \epsilon
	\end{align*}
	Note, the above holds for any arbitrary state $s$. This implies,
	\begin{align*}
	\norm{J^* - J_{\pi^{t+1}_\alpha}}_{\infty} &\leq \frac{1}{2} \norm{J^* - J_{\pi^t}}_{\infty} +  \frac{1}{2} \norm{J^* - T J_{\pi^t}}_{\infty} + \epsilon \\
	&\leq \left[ \frac{1}{2} + \frac{\gamma}{2} \right] \norm{J^* - J_{\pi^t}}_{\infty} + \epsilon
	\end{align*}
	where we used that $\norm{J^*-TJ_{\pi^t}}_{\infty}=\norm{TJ^*-TJ_{\pi^t}}_{\infty}\leq \gamma \norm{J^*-J_{\pi^t}}_{\infty}$ which follows from our assumption that the Bellman operator, $T(\cdot)$, is a contraction with modulus $\gamma$. Rewriting $\left( \frac{1}{2} + \frac{\gamma}{2}\right) = \left( 1 - \frac{1}{2}(1-\gamma) \right)$ and iterating over the above equation gives us our final result.
	\begin{align*}
	%\label{eq:NPGfinal}
	\norm{J^* - J_{\pi^{t+1}_\alpha}}_{\infty} &\leq \left(1 - \frac{(1-\gamma)}{2} \right) \norm{J^* - J_{\pi^t}}_{\infty} + \epsilon \\
	&\leq \left(1 - \frac{(1-\gamma)}{2}\right)^t \norm{J^* - J_{\pi^0}}_{\infty} + \epsilon \sum_{i=0}^{t-1} \left( 1 - \frac{(1-\gamma)}{2}\right)^i \\
	&\leq \left(1 - \frac{(1-\gamma)}{2}\right)^t \norm{J^* - J_{\pi^0}}_{\infty} + \frac{2\epsilon}{(1-\gamma)} \\
	&= \left(1 - \frac{(1-\gamma)}{2}\right)^t \norm{J^* - J_{\pi^0}}_{\infty} + \frac{2\log 2}{\alpha (1-\gamma)} \\
	&= \left(1 - \frac{(1-\gamma)}{2}\right)^t \norm{J^* - J_{\pi^0}}_{\infty} + \frac{2\log 2}{\eta}
	\end{align*}
	where the final equality follows by the definition: $\alpha = \frac{\eta}{(1-\gamma)}$. 
	Essentially, a larger stepsize $\eta$ decreases the constant error $\epsilon$. This clearly aligns with our intuition: as $\eta \rightarrow \infty$, natural policy gradient steps exactly mimics the policy iteration update which can be easily shown to converge geometrically to the optimal policy.
\end{proof}



==> convergence_rates.tex <==
%!TEX root = policy_grad_optimality.tex

\section{Convergence rates for policy gradient methods}
\label{sec:convergence_rates}
Our result in Theorem \ref{thm: no bad stationary points general} guarantees that any stationary point of the policy gradient objective, $\ell(\cdot)$ is globally optimal assuming (i) the policy class is closed in policy improvement and (ii) the weighted policy iteration objective function, $\theta \mapsto \Bc(\theta \, |\, \eta, J_{\pi})$ has no sub-optimal stationary points for any $\pi \in \Pi_{\Theta}$ and distribution $\eta$ supported over the entire state space $\Sc$. This however only implies an asymptotic result: optimizing the policy gradient objective with first order methods converges asymptotically to a stationary point which is also globally optimal. From a practitioners perspective however, we also care about finite time convergence rates which provide bounds the optimality gap after say a finite number of policy gradient updates. 

Our main insight in this section is to identify conditions which guarantee that the policy gradient objective is gradient dominated. The result follows if the weighted policy iteration objective, $\theta \mapsto \Bc(\theta \, |\, \eta, J_{\pi})$ is gradient dominated as well as closure of the policy class (condition \ref{cond: closure}). We use the policy gradient theorem in Lemma \ref{lem: PG theorem} to show how these conditions translate to gradient dominance of $\ell(\cdot)$. This is useful as under suitable smoothness assumptions, it is well known that first order methods converge rapidly to the globally optimal solutions if the objective is gradient dominated \cite[see e.g][]{nesterov2018lectures}. Such gradient dominance conditions also underly the proof of \cite{fazel2018global} for linear quadratic control.


%Recall the general recipe from Section \ref{section:opt_background} which uses different notions of gradient dominance conditions to show \textit{fast} convergence to globally optimal solutions, see Section \ref{subsec: gradient dominance global optimality} for details. Our main insight here is to identify conditions which guarantee that the policy gradient objective is gradient dominated. In addition to assuming condition \ref{cond: closure}, we impose stricter regularity conditions on the weighted policy iteration objective, $\theta \mapsto \Bc(\theta \, |\, \eta, J_{\pi})$, by assuming it to be convex/strongly convex. We show how this directly translates to  gradient dominance conditions for $\ell(\cdot)$ by using the policy gradient theorem in Lemma \ref{lem: PG theorem}. 


We remark that assuming the policy improvement objective to be convex is not entirely impractical. As noted before in Section \ref{sec:stationary_points}, $\theta \mapsto \Bc(\theta \, |\, \eta, J_{\pi})$, is linear for finite MDPs and quadratic for LQ control problem and therefore our results in this section immediately apply to these examples.
%\jb{Do these apply to inventory control or optimal stopping?}.


\subsection{Background on Gradient Dominance}
Throughout this section, we consider the optimization problem $\min_{x \in \X} f(x)$ where $\X \subseteq \mathbb{R}^d$. When $\Xc \subset \R^d$, we assume it to be a closed convex set and let $f$ be differentiable on an open set containing $\X$. Recall that the defining feature of a convex function is that it lies above its tangents, that is for each $x\in \X$, $f(x') \geq  f(x)+\langle \nabla f(x)\,, \, x'-x  \rangle$  for every $x' \in \Xc$. In analysis of optimization algorithms, this property not only implies that $f(\cdot)$ has no suboptimal stationary points, it can be used to bound the optimality gap by a measure of distance from stationarity, as
\[
\min_{x' \in \X} f(x') \geq f(x) + \min_{x' \in \X} \langle  \nabla f(x) \,  x'-x  \rangle . 
\]
When $\| x -x' \| \leq R$ for all $x,x'\in \X$, one can deduce from this the condition that $\min_{x' \in \X} f(x') \geq f(x) + R \| \nabla f(x)\|$, indicating that the gradient norm bounds sub optimality. When $f(\cdot)$ is strongly convex, this conclusion can be strengthened, leading to faster convergence rates. In particular, if $f$ is $\mu$--strongly convex, then 
\[ 
\min_{x'\in \mathcal{X}} f(x') \geq f(x) + \min_{x'\in \mathcal{X}} \, \left[ \langle \nabla f(x),x'-x\rangle + \frac{\mu}{2} \norm{x-x'}^2_2 \right]. 
\]
When $\Xc=\R^d$, this says $\min_{x'\in \mathcal{X}} f(x') \geq f(x) - \frac{\mu}{2} \| \nabla f(x)\|_{2}^2$,  so the optimality gap is bounded by the \emph{squared} norm of the gradient in this case. 

%Throughout this section, consider the optimization problem $\min_{x \in \X} f(x)$ where $\X \subset \mathbb{R}^d$ is a closed convex set and $f$ is differentiable on an open set containing $\X$. Recall the defining feature of a convex function is that it lies above its tangents, that is for each $x\in \X$, $f(x') \geq  f(x)+\langle \nabla f(x)\,, \, x'-x  \rangle$  for every $x' \in \Xc$. In analysis of optimization algorithms, this property not only implies that $f(\cdot)$ has no suboptimal stationary points, it can be used to bound the optimality gap by a measure of distance from stationarity, as
%\[
%\min_{x' \in \X} f(x') \geq f(x) + \min_{x' \in \X} \langle  \nabla f(x) \,  x'-x  \rangle . 
%\]
%When $\| x -x' \| \leq R$ for all $x,x'\in \X$, one can deduce from this the condition that $\min_{x' \in \X} f(x') \geq f(x) + R \| \nabla f(x)\|$, indicating that the gradient norm bounds sub optimality. When $f(\cdot)$ is strongly convex, this conclusion can be strengthened, leading to faster convergence rates. In particular, if $f$ is $\mu$--strongly convex, then 
%\[ 
%\min_{x'\in \mathcal{X}} f(x') \geq f(x) + \min_{x'\in \mathcal{X}} \, \left[ \langle \nabla f(x),x'-x\rangle + \frac{\mu}{2} \norm{x-x'}^2_2 \right]. 
%\]
%When $\Xc$ is unconstrained, this says $\min_{x'\in \mathcal{X}} f(x') \geq f(x) + \frac{\mu}{2} \| \nabla f(x)\|_{2}^2$, \jb{I think this should be $\min_{x'\in \mathcal{X}} f(x') \geq f(x) - \frac{1}{2 \mu} \| \nabla f(x)\|_{2}^2$} so the optimality gap is bounded by the \emph{squared} norm of the gradient in this case. 

Below, we introduce a notion called gradient dominance. This definition, essentially, assumes a critical implication of convexity or strong convexity rather than assuming the properties themselves. According to the definition below, a convex function is $(1,0)$--gradient dominated. A $\mu$--strongly convex function is $(1,\mu)$--gradient dominated. 
%The definition below is somewhat non-standard because we discuss constrained optimization. Most authors discuss unconstrained optimization, in which case the definition reduces to the usual gradient dominance or so-called Polyak condition, $\min_{x' \in \X} f(x) \geq f(x) - \frac{\mu}{2c}\| \nabla f(x) \|_2^2$ \jb{I think this should be $\min_{x' \in \X} f(x) \geq f(x) - \frac{c^2}{2\mu}\| \nabla f(x) \|_2^2$. I wrote the rate result in lemma \ref{lemma:second_order_convergence_rate} (b) accordingly.}.   
%\begin{definition}
%	\label{def:gradient_dominance}
%	For  a closed convex set  $\X \subset \mathbb{R}^d$ and function $f$ that is differentiable on an open set containing $\X$, we say $f$ is $(c,\mu)$--\textit{gradient dominated} over $\Xc$ if there exists a constant $c>0$ and $\mu\geq 0$ such that
%	\begin{align}\label{eq: second_order_grad_dom}
%	 \min_{x'\in \mathcal{X}} f(x')  \geq f(x) + \min_{x'\in \mathcal{X}} \, \left[ c\, \langle \nabla f(x),x'-x\rangle + \frac{\mu}{2} \norm{x-x'}^2_2 \right]  \,\, \quad \forall \, x\in \Xc. 
%	\end{align}
%	The function is said to be gradient dominated with degree 1 if $\mu=0$ and gradient dominated of degree two if $\mu>0$. 
%\end{definition}
%The definition above is somewhat non-standard because we discuss constrained optimization. Most authors discuss unconstrained optimization, in which case the definition reduces to the usual gradient dominance or so-called Polyak condition, $\min_{x' \in \X} f(x) \geq f(x) - \frac{\mu}{2c}\| \nabla f(x) \|_2^2$ \jb{I think this should be $\min_{x' \in \X} f(x) \geq f(x) - \frac{c^2}{2\mu}\| \nabla f(x) \|_2^2$. I wrote the rate result in lemma \ref{lemma:second_order_convergence_rate} (b) accordingly.}. 
\begin{definition}
	\label{def:gradient_dominance}
	For $\X \subseteq \mathbb{R}^d$, we say $f$ is $(c,\mu)$--\textit{gradient dominated} over $\Xc$ if there exists a constant $c>0$ and $\mu\geq 0$ such that
	\begin{align}\label{eq: second_order_grad_dom}
	\min_{x'\in \mathcal{X}} f(x')  \geq f(x) + \min_{x'\in \mathcal{X}} \, \left[ c\, \langle \nabla f(x),x'-x\rangle + \frac{\mu}{2} \norm{x-x'}^2_2 \right]  \,\, \quad \forall \, x\in \Xc. 
	\end{align}
	The function is said to be gradient dominated with degree 1 if $\mu=0$ and gradient dominated of degree two if $\mu>0$. 
\end{definition}
For $\Xc \subset \R^d$, the definition above may seem somewhat non-standard as authors typically consider unconstrained optimization (see \citep{karimi2016linear,fazel2018global} for example) in which case the definition reduces to the well known Polyak-Lojasiewicz (PL) inequality, $\min_{x' \in \X} f(x) \geq f(x) - \frac{c^2}{2\mu}\| \nabla f(x) \|_2^2$. See \cite{polyak1963gradient}. 

Under gradient dominance conditions, popular first order optimization algorithms are assured to converge to the global minimum and a simple analysis provides finite time rates of convergence as shown in Lemma \ref{lemma:second_order_convergence_rate} below. The first result focuses
on projected gradient descent, strengthening Lemma \ref{lem: pgd reaches global optimum} by providing a convergence rate. This result is obtained by using a well known fact that  projected gradient descent reaches an approximate stationary point rapidly (approximately at $\mathcal{O}(1/\sqrt{T})$ rate), and then using the definition of gradient dominance to relate approximate stationarity to the optimality gap. The second case considers an unconstained problem and analysis here is essentially identical to the typical analysis of gradient descent for strongly convex objectives and shows a geometric convergence rate. Recall that a differentiable function is said to be $L$-smooth if $\nabla f(x)$ is Lipschitz with constant $L$ with respect to the Euclidean norm. 

%Under gradient dominance conditions, popular first order optimization algorithms are assured to converge to the global minimum and a simple analysis provides finite time rates of convergence. For concreteness, we will focus on projected gradient descent, strengthening Lemma \ref{lem: pgd reaches global optimum} by providing a convergence rate. The first result is obtained by using a well known fact that  projected gradient descent reaches an approximate stationary point rapidly (approximately at $\mathcal{O}(1/\sqrt{T})$ rate), and then using the definition of gradient dominance to relate approximate stationarity to the optimality gap. Analysis in the second case is essentially identical to the typical analysis of projected gradient descent for strongly convex objectives and shows a geometric convergence rate. Recall that a differentiable function is said to be $L$-smooth if $\nabla f(x)$ is Lipschitz with constant $L$ with respect to the Euclidean norm. 
\begin{restatable}[Convergence rates for gradient dominated smooth functions]{lem}{ratesgraddominance}
	\label{lemma:second_order_convergence_rate}
	Consider the problem, $\min_{x \in \Xc} f(x)$ where $\Xc \subseteq \R^d$. Assume $f$ be $L$--smooth on $\X$ and a non-empty solution set. Denote $f(x^*)=\min_{x'\in \Xc} f(x')$. Consider the sequence $x_{t+1} = {\rm Proj}_{\Xc}\left( x_t - \alpha \nabla f(x_t) \right)$.
	%Let $\X \subset \mathbb{R}^d$ is a closed convex set and $f$ be $L$--smooth on $\X$. Consider the sequence $x_{t+1} = {\rm Proj}_{\Xc}\left( x_t - \alpha \nabla f(x_t) \right)$ where $\alpha \leq1/L$. Set $f(x^*)=\min_{x'\in \Xc} f(x')$. Then,
	\begin{enumerate}
		\item Let $\Xc \subset \R^d$ such that $\| x-x'\|_{2} \leq R<\infty$ for all $x,x'\in \Xc$. Assume $f$ is $k$-lipschitz and $(c,0)$--gradient-dominated and where $\alpha \leq \min\{\frac{1}{k}, \frac{1}{L} \}$. Then, 
		\[
		\min_{t \leq T}  \left\{ f(x_t) - f(x^*) \right\} \leq \sqrt{\frac{2R^2c \left( f(x_0) - f(x^*) \right)}{\alpha T}}
		\]
		\item \citep{karimi2016linear,polyak1963gradient} Assume $\Xc=\R^d$ and $\alpha=1/L$. If $f$ is $(c,\mu)$--gradient-dominated for $\mu>0$, then, 
		\[ 
		f(x_t) - f(x^*) \leq \left(1-\frac{\mu}{c^2 L}\right)^t  \left( f(x_0) - f(x^*) \right)  
		\]
	\end{enumerate}
\end{restatable}
\begin{proof}
	See Appendix \ref{app:proof_of_convergence_rates} for a detailed proof of Part (1). 
\end{proof}
\begin{rem} Part (2) of Lemma \ref{lemma:second_order_convergence_rate} assumes $\Xc=\mathbb{R}^d$, 
	in which case the sequence $x_{t}$ is produced by gradient descent with a fixed stepsize. 
	It is likely possible to show geometric rates for projected gradient descent on constrained subsets $\Xc \neq \mathbb{R}^d$. We do not consider this case for simplicity and brevity.
\end{rem}

% In practice however, one really cares about how fast the policy gradient method would converge to a globally optimal solution. Can we characterize the optimality gap after optimizing $\ell(\theta)$ using say, a first-order method for a finite number of steps? We precisely answer this question by imposing stricter regularity conditions on the weighted policy iteration objective than assuming the absence of sub-optimal stationary points. In particular, we show that if $\theta \mapsto \Bc(\theta \, |\, \eta, J_{\pi})$ is convex or strongly convex for all $\pi \in \Pi_{\Theta}$, then $\ell(\cdot)$ is gradient dominated. 

% A gradient dominance condition on $\ell(\cdot)$ is very useful as it almost immediately implies convergence rates. Under suitable smoothness assumptions, it is well known that first order methods can converge rapidly to the global optimum of a non-convex function if it is gradient dominated \cite[see e.g][]{nesterov2018lectures}. Such gradient dominance conditions also underly the proof of \cite{fazel2018global} for linear quadratic control. Before formally stating our results in Theorem \ref{}, we first outline the two different notions of gradient dominance conditions along with the convergence rates these for first order methods like the projected gradient descent and the Frank-Wolfe algorithm.

\subsection{Gradient dominance of the policy gradient objective}
We continue to assume that the policy class is closed under policy improvement, as stated in condition \ref{cond: closure}. But now, instead of assuming the policy improvement objective has no sub-optimal stationary points, we impose a stronger property that it is gradient dominated. This condition holds whenever the single period objective solved by policy iteration is convex and therefore immediately applies to the LQ control problem as well as for tabular MDPs.

%\begin{cond}[Gradient dominance of the weighted policy iteration objective]\label{cond: convexity_strong} 
%	For any $\pi \in \Pi_{\Theta}$, the function $\theta \mapsto \Bc(\theta \mid \eta_{\pi}, J_{\pi})$ is $(c,\mu)$--gradient-dominated over $\Theta$. 
%\end{cond}
This gradient dominance condition ensures the single-period objective optimized by policy iteration problem could be solved efficiently by first order methods. Our main result in Theorem \ref{thm: convergence_rates} shows that for closed policy classes, this gradient dominance condition is automatically inherited by the multi-period objective $\ell(\cdot)$, implying convergence rates for first-order methods applied to $\ell(\cdot)$. Notice that the  constants degrade with the horizon and the concentrability coefficient $\kappa_{\rho}$ stated in Definition \ref{def:concentrability_measure}. The Corollary \ref{cor: convexity to gradient dominance of pg} provides a more interpretable statement, which follows because any convex $\Bc(\theta| \eta, J_{\pi})$ is $(1,0)$--gradient-dominated and any $\Bc(\theta| \eta, J_{\pi})$ and any $\mu$--strongly--convex $\Bc(\theta| \eta, J_{\pi})$ is $(1,\mu)$--gradient-dominated. 


\begin{restatable}[]{thm}{mainthm}\label{thm: convergence_rates}
	If Conditions \ref{cond: diff}, \ref{cond: closure}, and \ref{cond: convexity_strong} hold, then $\ell(\cdot)$ is $\left(\frac{1-\gamma}{\kappa_{\rho}}\cdot c\, ,\, \frac{1-\gamma}{\kappa_{\rho}}\cdot \mu \right)$--gradient dominated.
\end{restatable}
\begin{cor}\label{cor: convexity to gradient dominance of pg}
	Suppose Conditions Conditions \ref{cond: diff} and \ref{cond: closure} hold. If, for every $\pi \in \Pi_{\Theta}$, the function $\theta \mapsto \Bc(\theta \mid \eta_\pi, J_{\pi})$ is convex, then $\ell(\theta)$ is gradient dominated of degree one. If $\theta \mapsto \Bc(\theta \mid \eta_\pi, J_{\pi})$ is strongly convex then $\ell(\theta)$ is gradient dominated of degree two. 
\end{cor}
The proof can be divided into two key steps. First, we use closure of the policy class (condition \ref{cond: closure}) to upper bound the optimality gap of the policy gradient objective with that of the weighted policy iteration objective. Essentially, this result shows that the current policy is \textit{nearly optimal} if the weighted policy iteration step offers little improvement over the current policy; assuming the policy iteration step can be performed exactly and sufficient exploration, $\rho(s) > 0 \,\, \forall \, s \in \Sc$. It is important to note how \textit{optimality} here crucially depends on the use of an exploratory initial distribution under which $\kappa_{\rho}<\infty$. The second step of the proof translates gradient dominance of the  policy iteration objective to that of $\ell(\cdot)$ by using the policy gradient theorem in Lemma \ref{lem: PG theorem}. 
\begin{proof}[Proof of Theorem \ref{thm: convergence_rates}]
	We first derive a consequence of the closure condition. We have, 	
	\begin{align*}
	\ell(\pi_{\theta}) - \min_{\pi}\ell(\pi) &= (1-\gamma)\E_{\rho}\left[ J_{\pi_{\theta}}(s_0) - J_{\pi}(s_0) \right]   \\
	&\overset{(a)}{=} (1-\gamma)\| J_{\pi_{\theta}} - J^{*}\|_{1,\rho} \\
	&\overset{(b)}{\leq} \kappa_\rho \|  J_{\pi_{\theta}} - TJ_{\pi_{\theta}} \|_{1, \rho} \\
	&\overset{(c)}{\leq} \frac{\kappa_\rho}{(1-\gamma)} \|  J_{\pi_{\theta}} - TJ_{\pi_{\theta}} \|_{1, \eta_{\pi_{\theta}}} \\
	&= \frac{\kappa_\rho}{(1-\gamma)} \E_{\eta_{\pi_{\theta}}}\left[ J_{\pi_\theta}(s_0)- T J_{\pi_{\theta}}(s_0) \right] \\
	&\overset{(d)}{=} \frac{\kappa_\rho}{(1-\gamma)} \E_{\eta_{\pi_{\theta}}}\left[ J_{\pi_\theta}(s_0)- \min_{\pi' \in \Pi_{\Theta}} T_{\pi'} J_{\pi_{\theta}}(s_0) \right] \\
	& \frac{\kappa_\rho}{(1-\gamma)} \left( \Bc(\theta \mid \eta_{\pi_{\theta}}, J_{\pi_{\theta}}) - \min_{\theta' \in \Theta} \, \Bc(\theta' \mid \eta_{\pi_{\theta}}, J_{\pi_{\theta}})  \right)
	\end{align*}
	Here (a) uses that $J_{\pi_{\theta}} \succeq TJ_{\pi_\theta}$, (b) directly applies the definition of  $\kappa_\rho$ in Definition \ref{def:concentrability_measure}, (c) uses that $\eta_{\pi_{\theta}} \geq (1-\gamma) \rho$ (by definition, see \eqref{eq: discounted_state_occupancy_measure}) and  (d) directly applies the policy closure condition in Condition \ref{cond: closure}. 
	
	By assumption, $\thetabar \mapsto \Bc(\thetabar \mid \eta_{\theta}, J_{\pi_{\theta}})$ is ($c$, $\mu$)--gradient dominated. Applying this gives
	\begin{align*}
	\Bc(\theta \mid \eta_{\pi_{\theta}}, J_{\pi_{\theta}}) - \min_{\theta' \in \Theta} \Bc(\theta' \mid \eta_{\pi_{\theta}}, J_{\pi_{\theta}}) &\leq - \min_{v \in \Theta} \, \left[ c \, \langle \nabla_{\thetabar} \, \Bc(\thetabar \mid \eta_{\pi_{\theta}}, J_{\pi_{\theta}}) \bigg\vert_{\thetabar = \theta}, v-\theta \rangle + \frac{\mu}{2} \norm{v-\theta}^2_2 \right] \\
	&\leq - \min_{v \in \Theta} \, \left[ c \, \langle \nabla_{\theta} \ell(\theta), v-\theta \rangle + \frac{\mu}{2} \norm{v-\theta}^2_2 \right],
	\end{align*}
	which gives our desired result. The second inequality above uses the policy gradient theorem in Lemma \ref{lem: PG theorem}. 
\end{proof}


\subsection{Gradient dominance and smoothness for examples \ref{ex: lq control}-\ref{ex:stopping}}
As noted earlier, the gradient dominance condition for LQ control and finite MDPs follows from (strong) convexity of the weighted policy iteration objective. However, the weighted policy iteration cost function is not convex for the optimal stopping problem as described in Example \ref{ex:stopping}.  Nevertheless, the policy iteration objective is gradient dominated. The gradient dominance constants depend on a measure of the degree of uniformity in the offer distribution $q_{x}(\cdot)$.  For a general start state distribution, Lemma \ref{lem: concentrability with immitation} bounds $\kappa_{\rho} $ but Lemma \ref{lem: concentrability stopping} shows that we get a tighter bound of $\kappa_{\rho} \leq 1$ is possible when $\rho$ is chosen to be the stationary distribution. See Appendix \ref{subsec:app_optimalstopping} for details.

%we show below in Lemma \ref{lem:grad_dom_of_optstopp} that the total cost function, $\ell(\cdot)$ is infact gradient dominated using a more direct argument. See Appendix \ref{subsec:app_optimalstopping} for details. Recall that we assume $\nu(x) > 0 \,\, \forall \, x \in \Xc$ and $q_x(\cdot)$ to be a density supported over $\Yc$ such that the initial distribution $\rho(x,y) = \nu(x) q_x(y)$ is supported over $\Sc$.

\begin{restatable}[Gradient dominance for optimal stopping]{lem}{graddomoptstopp}
	\label{lem:grad_dom_of_optstopp}
	Consider the optimal stopping problem formulated in Example \ref{ex:stopping}. For any $\pi \in \Pi_{\Theta}$,  the function $\theta \mapsto \Bc(\theta | \eta_{\pi}, J_{\pi} )$ is $(2\beta, 0)$--gradient-dominated where $\beta = \max_{x \in \Xc, y\in \Yc} q_{x}(y) / \min_{x \in \Xc, y\in \Yc} q_{x}(y)$. 
	%Denote $\kappa_{\rho}$ to be the concentrability coefficient corresponding to the initial distribution $\rho(x,y) = \nu(x) q_x(y)$ supported on $\Sc$. Define $\psi: \inf_{(x,y) \in \Sc} \, \nu(x) \, q_x(y)$ and $\beta:=\sup_{(x, y) \in \Sc} \, \nu(x) \, q_x(y)$. Then, $\ell(\cdot)$ is $(\frac{\psi}{\kappa_{\rho} \beta},0)$ gradient dominated.
\end{restatable}


In addition to gradient dominance, the convergence rates described in Lemma \ref{lemma:second_order_convergence_rate} apply to smooth objectives. We refer the readers to Lemma E.3 in \cite{agarwal2019optimality} which shows smoothness of $\ell(\cdot)$ for tabular MDPs. 
For the LQ control problem, Lemma \ref{lem: smoothness_LQ} below shows that $\ell(\cdot)$ is smooth on sub-level sets. This is useful as the gradient update, $\theta' = \theta - \nabla \ell(\theta)$, with exact line-search remains in the sublevel set $\{\theta': \ell(\theta') \leq \ell(\theta)\}$. See Appendix \ref{app:LQ_smoothness} for a full proof.
%The following lemma shows that the policy gradient objective for the LQ control problem is smooth on sub-level sets. 
\begin{restatable}[]{lem}{lqcostsmooth}
	\label{lem: smoothness_LQ}
	Consider the LQ control problem in Example \ref{ex: lq control}. For  any $\theta \in \Theta_{\text{S}}$,
	\[
	\max \, \left\{ \| \nabla^2 \ell(\theta') \| : \theta \in \Theta, \ell(\theta') \leq \ell(\theta) \right\} < \infty
	\]
	%Let $\Sigma = \E_{s \sim \rho} \left[ ss^\top \right] \succ 0$. Then, the total cost function for the LQ control problem in Example \ref{ex: lq control}, $\ell(\theta): \Theta_{\text{S}} \to \mathbb{R}$, is smooth in $\theta$ on sublevel sets.	
\end{restatable}
A smoothness results also holds for the optimal stopping objective as shown below in Lemma \ref{lem:smoothness_opt_stopp}. The proof follows by showing that $\ell(\theta)$ is twice continuously differentiable and leveraging that continuous functions are bounded on compact sets. Namely  $\| \nabla^2 \ell(\theta) \|$) is bounded over $\Theta$. See Appendix \ref{subsec:app_optimalstopping} for details.
\begin{restatable}[]{lem}{optstoppcostsmooth}
	\label{lem:smoothness_opt_stopp}
	In the optimal stopping problem in Example \ref{ex:stopping}, $\max_{\theta \in \Theta}  \| \nabla^2 \ell(\theta) \| < \infty$.  % is smooth over $\Theta = \{\theta \in \mathbb{R}^{|\Xc|} : \theta_x \in \Yc \}$.
\end{restatable}


%\subsubsection{Issue of policy parameterization:}
%Problem of conditioning of the policy class for the softmax parameterization case. 

 



==> electronic_companion.tex <==
%!TEX root = policy_grad_optimality.tex
\newpage


\title{Global Optimiality Guarantees For Policy Gradient Methods: Technical Report with Supplementary Materials}


\maketitle

\setcounter{section}{0}
\setcounter{page}{1}


This technical report provide some further details related to our paper \citep{bhandari2019global}. This helps separate our main contribution from either (i) slight adaptations of known results or (ii) technical details of specific examples that are somewhat orthogonal to the paper's main insights. The first part proves results related to the convergence of projected gradient descent in smooth (but possibly nonconvex) optimization. Similar results can be found in nonlinear optimization textbooks like \cite{bertsekas1997nonlinear} or \cite{beck2017first}, but we include careful standalone proofs here. The second part provides some further technical results related to specific examples on which we instantiate our general results. Primarily, the effort here is on certifying that various functions are differentiable.  We also extend our treatment of the optimal stopping example, providing stronger results. 

The document should be read as a direct continuation of \cite{bhandari2019global}. We refer to equations and citations from that paper throughout. 

\section{Convergence proofs for first order methods.}
\label{app:proof_of_convergence_rates}

To start, let us define some standard notions from first order optimization. For a convex set $\Xc \subset \mathbb{R}^d$, we say a function $f:\Xc \to \mathbb{R}$ is $k$-Lipshitz if $\norm{f(x) - f(y)}_2 \leq k \norm{x - y}_2$ for every $x,y \in \Xc$. We say a function is $L$-smooth if $f$ is differentiable throughout $\Xc$ and $\nabla f$ is $L$-Lipschitz. A consequence of smoothness that will be useful throughout our proofs is often called the \textit{descent lemma}. It implies a quadratic upper bound on function values. The proof follows by Taylor expansion and the mean-value theorem \citep{bertsekas1997nonlinear}.
\begin{lem}[Descent Lemma] \label{lemma:smoothness}
	If the function $f:\D\to \mathbb{R}$ is $L$-smooth over a set $\X \subseteq \D$, then for any $(x,y) \in \X$:
	\[
	f(y) \leq f(x) + \langle \nabla f(x), y-x \rangle + \frac{L}{2} \norm{y-x}^2_2.
	\]
\end{lem}

The following interpretation of projected gradient updates will be very useful for our proof. Recall the notation for orthogonal projection: ${\rm Proj}_{\X} (x) = \argmin_{y \in \X} \, \norm{y - x}^2_2$. The projected gradient descent iteration can be equivalently written as 
\begin{align}\label{eq:quad_approx_appendix}
	x_{t+1} = {\rm Proj}_\X \left( x_t - \alpha_t \nabla f(x_t) \right) =  \argmin_{x \in \X} \left[ f(x_t) + \langle \nabla f(x_t), x-x_t \rangle + \frac{1}{2\alpha_t} \norm{x-x_t}^2_2 \right].
\end{align} 
giving a ``proximal'' interpretation of projection as minimizing a local quadratic approximation. See \cite{beck2017first} for a simple proof. 


\subsection{Asymptotic convergence to stationary points: proof of Lemma \ref{lem: pgd reaches global optimum}}
For convenience, we first restate the claim. 
\convergencetostationary*
\begin{proof}
	%Part 1 follows from \cite[Proposition 3.6.3]{bertsekas1997nonlinear} or \cite[Theorem 10.15]{beck2017first}.  
	Part 1 follows from the simple proofs in \citep{beck2002convergence, beck2017first}.
	We show the claim in part 2. Throughout, let $\| x\|$ denotes the Euclidean norm of a vector $x$ and $\|A\|= \max_{\|x\|\leq 2} \| Ax\|$ be induced operator norm of a matrix $A$.  Note that the sub-level set $S := \{x \in \Xc : f(x) \leq f(x_0) \}$ is compact (continuity of $f(\cdot)$ implies its closed and we assume it to be bounded). Also, for a sufficiently small $\epsilon$, $f(\cdot)$ is twice continuously differentiable over the compact set,
	\[
	S_{\epsilon} := \{ x +y:   x\in  S_1, \| y\| \leq \epsilon  \}. 
	\]
	which follows by our assumption that $f(\cdot)$ is twice continuously differentiable on an open set containing $S$. We denote $G = \max_{x\in S} \| \nabla f(x) \| $ and $L = \max_{x \in S_{\epsilon}} \| \nabla^2 f(x) \|$. Note that $G$ and $L$ are finite since $\|\nabla f\|$ and $\|\nabla^2 f\|$ are continuous  over the compact sets $S$ and $S_{\epsilon}$. Fix the step-size $\alpha= \min\{\epsilon / G, 1/L \}$. For any $x\in S_1$, define $x^{+} = {\rm Proj}_\X \left( x - \alpha \nabla f(x) \right)$. For this choice of step-size,  $x^+ \in S_{\epsilon}$ since
	\[
	\| x^{+} - x\|_2  = \|  {\rm Proj}_\X \left( x - \alpha \nabla f(x) \right) - {\rm Proj}_\X(x)  \| \leq \| \alpha \nabla f(x)\| \leq \alpha G \leq \epsilon,
	\]
	which follows as projection operators are non-expansive. The optimality conditions for projection onto a convex set yield the standard property that $\hat{x} = {\rm Proj}_\X \left( x\right)$ if and only if $\langle \hat{x}-x, y-\hat{x} \rangle \geq 0 $ for all $y\in \Xc$. Using this and some algebra, we get 
	\begin{align*}
		\langle x - \alpha \nabla f(x) - x^+, x - x^+ \rangle \leq 0 \,\, \implies \,\, \|x - x^+\|^2 - \alpha \langle \nabla f(x), x - x^+ \rangle  \leq 0.
	\end{align*}
	As $x^+ \in S_{\epsilon}$,
	\begin{flalign*}
		&& f(x^+) &\leq  f(x) + \langle \nabla f(x)\, , \, x^+ - x \rangle  + \frac{L}{2} \| x^+ - x\|^2   && [\text{smoothness of} f(\cdot) \text{ over } S_\epsilon]\\
		&&   &\leq f(x) + \left( \frac{L}{2} - \frac{1}{\alpha} \right) \|x^+ - x\|^2 &&\\
		&&   &\leq f(x). &&  [\alpha  \leq 1/L]  
	\end{flalign*}
	Since the projected gradient update reduces cost, we know $x^+ \in S$. Repeating this argument inductively shows that $f(x_{k+1}) \leq f(x_k)$ and $x_k \in S$ for all $k$. 
	Since $\{x_k\}$ is contained in a compact set $S$, it has a convergent sub-sequence, $\{x_{k_i}\}$ with some limit $x_{\infty}$. We have ,
	\[ 
	\lim_{k\to \infty} f(x_k) = \lim_{i\to \infty} f(x_{k_i}) = f(x_\infty),
	\]
	where the first limit exists since $\{f(x_k) \}$ is monotone-decreasing and bounded below and the final inequality uses continuity of $f(\cdot)$. The proof to show that any limit point is a stationary point follows from \citep{beck2002convergence, beck2017first}. See also \citep[Figure 3.3.2]{bertsekas1997nonlinear}. We omit this for brevity.
\end{proof}


\subsection{Convergence rates under gradient dominance: Proof of Lemma \ref{lemma:second_order_convergence_rate}.}
We first restate the claim. 
\ratesgraddominance*

\begin{proof}[Proof of Lemma \ref{lemma:second_order_convergence_rate}]
	Recall, by Definition \ref{def:gradient_dominance} that a function $f$ is defined to be $(c,\mu)$--\textit{gradient dominated} over $\Xc$ if there exists a constant $c>0$ and $\mu\geq 0$ such that
	\[
	f(x^*)  \geq f(x) + \min_{y\in \mathcal{X}} \, \left[ c\, \langle \nabla f(x),y-x\rangle + \frac{\mu}{2} \norm{y-x}^2_2 \right]  \,\, \quad \forall \, x\in \Xc. 
	\]
	
	\paragraph{Proof of Part (a):}
	We assume $\mu=0$ in which case for any $x\in \Xc$, we have 
	\begin{align}
		\label{eq:first_order_grad_dominance_app}
		\min_{y\in \mathcal{X}} \, \left[ c\, \langle \nabla f(x),y-x\rangle \right] \leq f(x^*) - f(x)
	\end{align}
	Therefore, for any $x \neq x^*$, we have $\min_{y \in \D} \, \langle \nabla f(x_t), y - x \rangle < 0$. Let $\{x_t\}$ be the iterates produced by projected gradient descent. At iterate $x_t$, let $\bar{y} = \argmin_{y \in \X} \, \langle \nabla f(x_t), y-x_t \rangle$ and denote $\delta_t = \min_{y \in \X} \langle \nabla f(x_t), y-x_t \rangle$. Note that $\delta_t \leq 0$ and $|\delta_t| \leq \|\nabla f(x_t)\| \|y-x_t\| \leq k R$ as $f$ is assumed to be $k$-Lipschitz. We take a constant stepsize, $\alpha_t = \alpha \leq \min\{ \frac{1}{k},\frac{1}{L}\}$. Then,
	
	\begin{align}
		f(x_{t+1}) - f(x_t) &\overset{(a)}{\leq} \min_{y \in \D} \, \left[ \langle \nabla f(x_t), y-x_t \rangle + \frac{1}{2\alpha} \norm{y-x_t}^2_2 \right] \nonumber \\
		&\overset{(b)}{=} \min_{\beta \in [0,1]} \left[ \langle \nabla f(x_t), x_t + \beta(\bar{y}-x_t) - x_t \rangle + \frac{1}{2 \alpha} \norm{x_t + \beta(\bar{y}-x_t) - x_t}^2_2 \right] \nonumber \\
		&= \min_{\beta \in [0,1]} \, \left[ \beta \langle \nabla f(x_t), (\bar{y}-x_t) \rangle + \frac{\beta^2}{2\alpha} \norm{\bar{y}-x_t}^2_2 \right] \nonumber \\
		&\leq \min_{\beta \in [0,1]} \, \left[ \beta \delta_t + \frac{\beta^2 R^2}{2\alpha} \right] = \frac{-\alpha \delta_t^2}{2R^2} \label{eq:proj_rates1}
	\end{align}
	where the minimizer $\beta^*=-\delta_t\alpha / R^2 \leq k \alpha / R \leq 1$ as $\alpha \leq \min\{\frac{1}{k}, \frac{1}{L} \}$ (we assume $R>1$ without loss of generality as we can take any upper bound while minimizing in \eqref{eq:proj_rates1}).
	Here (a) follows by using the equivalence shown in \eqref{eq:quad_approx_appendix} and the quadratic upper bound on the function values implied by the descent lemma. Equality (b) uses the fact that right hand side of (a) can be optimized by searching over the steepest descent direction $x_t \to y$. Using \eqref{eq:first_order_grad_dominance_app}, we get
	\[
	f(x_{t+1}) - f(x_t) \leq \frac{-\alpha}{2R^2 c^2} \left( f(x^*) - f(x_t) \right)^2
	\]
	Rearranging, we get our desired result
	\begin{align*}
		\min_{t \leq T}  \left( f(x_t) - f(x^*) \right)^2 \leq \frac{1}{T} \sum_{t=0}^{T-1} \left( f(x_t) - f(x^*) \right)^2 &\leq \frac{2R^2c^2}{\alpha T} \sum_{t=0}^{T-1} f(x_t) - f(x_{t+1}) \\
		&\leq \frac{2R^2c^2}{\alpha T} \left( f(x_0) - f(x_T) \right) \\
		&\leq \frac{2R^2c^2}{\alpha T} \left( f(x_0) - f(x^*) \right)
	\end{align*}
	Since also $f(x_T) \leq f(x_{T-1}) \leq \cdots f(x_1)$, we have
	\[
	f(x_T) - f(x^*) \leq \min_{t \leq T}  \left\{ f(x_t) - f(x^*) \right\} \leq \sqrt{\frac{2R^2c^2 \left( f(x_0) - f(x^*) \right)}{\alpha T}}.
	\]
	
	\paragraph{Proof of Part (b):} We refer readers to the proof in \cite{karimi2016linear}, which can be dated back to \cite{polyak1963gradient}.
\end{proof}	




\section{Example Details}

\subsection{Stability in discounted LQ control: Proof of Lemma \ref{lem:lq_stability}}
We first recall the claim. 
\LQStable* 
\begin{proof}
	The average cost can be written as
	\[
	\ell(\theta) = (1-\gamma)\E^{\pi_{\theta} }_{\rho}\left[ \sum_{t=0}^{\infty} \gamma^t \left( s_t^\top \left[ \theta R \theta + C  \right] s_t \right)  \right]  
	\]
	where the expectation is over $s_0\sim \rho$ and it is implicit that the state evolves according to the linear dynamical system $s_{t+1}=(A+B\theta)s_t$ for $t=0,1\cdots$. 	
	We can bound $\ell(\theta)$ above and below as, 
	\[ 
	\lambda_{\min}(\theta R \theta + C )  \E^{\pi_{\theta} }_{\rho}\left[\sum_{t=0}^{\infty}  \| \sqrt{\gamma} s_t  \|_2^2\right]\leq (1-\gamma)^{-1}\ell(\theta) \leq \lambda_{\max}(\theta R \theta + C )  \E^{\pi_{\theta} }_{\rho}\left[\sum_{t=0}^{\infty}  \| \sqrt{\gamma} s_t  \|_2^2\right]. 
	\]
	Since $s_t= \left[A+B\theta\right]^t s_0$, applying Lemma \ref{lem:lq_trace_argument} at each timestep with a choice of $M=(\sqrt{\lambda}\left[A+B\theta\right] )^t$ yields 
	\[ 
	\lambda_{\min}\left( \Sigma_\rho  \right) \sum_{t=0}^{\infty }  \| (\sqrt{\gamma}\left[A+B\theta\right] )^t \|_F^2 \leq \E^{\pi_{\theta} }_{\rho}\left[\sum_{t=0}^{\infty}  \| \sqrt{\gamma} s_t  \|_2^2\right] \leq \lambda_{\max}\left( \Sigma_\rho  \right)   \sum_{t=0}^{\infty }\| (\sqrt{\gamma}\left[A+B\theta\right] )^t \|_F^2.
	\] 
	We recall Gelfand's formula, which says that for any square matrix $M$ with spectral radius $\rho(M)$ and any matrix norm $\|\cdot\|$, we have $\| M^t\|^{1/t} \to \rho(M)$ as $t\to \infty$. This implies  $\sum_{t=0}^{\infty }\| (\sqrt{\gamma}\left[A+B\theta\right] )^t \|_F^2$ is finite if and only if $\sqrt{\gamma}\left[A+B\theta\right]$ has spectral radius strictly less than one.  
\end{proof}



\subsection{Further results on optimal stopping}
This section continues the analysis from the appendix of the main paper. It is intended t be read side-by-side with the notation and results there.   
\paragraph{Condition \ref{cond: convexity_strong}: Gradient dominance.} We now establish a gradient dominance result that strengthens the previous analysis. We first recall the claim. 
\graddomoptstopp*
\begin{proof}
	Fix any $\pi \in \Pi_{\Theta}$. As we formulate the optimal stopping as a reward maximization problem, following our notion of gradient dominance in Definition \ref{def:gradient_dominance}, we want to show that
	\begin{equation}\label{eq:opt_stopping_grad_dominance}
		\max_{\theta' \in \Theta} \, \langle \nabla_{\theta} \Bc(\theta | \eta_{\pi}, J_{\pi}), \theta' - \theta \rangle \geq \frac{1}{\beta} \left( \Bc(\theta^+ | \eta_{\pi}, J_{\pi}) - \Bc(\theta | \eta_{\pi}, J_{\pi})  \right)
	\end{equation}
	where $\theta^+$ is the parameter of a policy iteration update to $\pi$, i.e. $\theta^+ = \argmax_{\theta \in \Theta} \, \Bc(\theta|\eta_{\pi}, J_{\pi})$. As shown in \eqref{eq:stopping_pi_update}, $\theta^+_x=\max\{y_{\min}, c_{\pi}(x)  \}$. 	
	We first lower bound the left hand side of \eqref{eq:opt_stopping_grad_dominance} as,
	\begin{align}
		\max_{\theta' \in \Theta} \, \langle \nabla_{\theta} \Bc(\theta | \eta_{\pi}, J_{\pi}), \theta' - \theta \rangle &= \sum_{x \in \X}  \max_{\theta'_x \in \Yc }  \frac{\partial  \Bc(\theta | \eta_{\pi}, J_{\pi})}{\partial \theta_x} \cdot (\theta'_x - \theta_x) \nonumber \\
		&= \sum_{x \in \X}  \max_{\theta'_x \in \Yc }  \left(c_\pi(x)-\theta_x\right) \cdot   \eta'_{\pi}(x)q_{x}(\theta_x) \cdot (\theta'_x - \theta_x) \nonumber \\
		&\geq \left(\min_{x' \in \Xc, y'\in \Yc}q_{x'}(y')\right)   \sum_{x \in \X}  \eta'_{\pi}(x) \left\{ \max_{\theta'_x \in \Yc }  \, \left[ \left(c_\pi(x)-\theta_x\right) \cdot (\theta'_x - \theta_x) \right] \right\}, \label{eq:gradient dominance stopping LHS}
	\end{align}
	where second equality uses the derivative calculation in \eqref{eq:policy_grad_opt_stopping}. We now upper bound the right hand side of \eqref{eq:opt_stopping_grad_dominance}: 
	\begin{align*}
		& \Bc(\theta^+ | \eta_{\pi}, J_{\pi}) - \Bc(\theta | \eta_{\pi}, J_{\pi})  \\ =& \sum_{x \in \Xc} \eta'_{ \pi}(x) \intop_{y_{\min}}^{y_{\max}} \left[ Q_{\pi}( (x,y)\, ,\,    \mathbbm{1}(y > \theta^+_x)  ) - Q_{\pi}( (x,y)\, ,\,    \mathbbm{1}(y > \theta_x)  ) \right] q_{x}(y)dy   \\
		\leq & \left(\max_{x' \in \Xc, y'\in \Yc}q_{x'}(y')\right)  \sum_{x \in \Xc} \eta'_{ \pi}(x) \underbrace{\intop_{y_{\min}}^{y_{\max}} \left[ Q_{\pi}( (x,y)\, ,\,    \mathbbm{1}(y > \theta^+_x)  ) - Q_{\pi}( (x,y)\, ,\,    \mathbbm{1}(y > \theta_x)  ) \right] dy}_{:=G_{x}(\theta^+_x, \theta_x )}.   
	\end{align*}
	The result follows if we can conclude,
	\begin{equation}\label{eq:opt_stopp_grad_dominance_ineq}
		\max_{\theta'_x \in \Yc }  \, \left[ \left(c_\pi(x)-\theta_x\right) \cdot (\theta'_x - \theta_x) \right] \geq G_{x}(\theta^+_x, \theta_x), 
	\end{equation}
	which we do below by separately considering two cases. For this purpose, it is helpful to use a more explicit formula for $G_{x}(\theta^+_x, \theta_x )$, which follows directly from the formula for the $Q$ function given in this section's preliminaries:
	\[
	G_{x}(\theta^+_x, \theta_x ) = 
	\begin{cases}
		\intop_{\theta_x}^{\theta^+_x} ( c_{\pi}(x)-y  )dy, & \text{for  } \theta_x \leq \theta^+\\
		\intop_{\theta^+_x}^{\theta_x} ( y- c_{\pi}(x)  )dy, & \text{for  } \theta_x > \theta^+
	\end{cases}
	\]
	
	
	\paragraph{Case (1):} Assume that $c_{\pi}(x)  \in (y_{\min}, y_{\max})$ in which case $\theta^+_x  = c_{\pi}(x)$. Then,
	\begin{align*}
		G_{x}(\theta^+_x, \theta_x) = \frac{1}{2}\left( c_{\pi}(x) - \theta_x    \right)^2  &\leq \left( c_{\pi}(x) - \theta_x    \right)^2 \leq \max_{\theta'_x \in \Yc }  \left(c_\pi(x)-\theta_x\right) \cdot (\theta'_x - \theta_x)  
	\end{align*}
	where the formula for $G_{x}(\theta_x^+, \theta_x)$ follows by calculating the integral and the final inequality uses that a choice of $\theta'_x=c_{\pi}(x)$ is feasible. The establishes \eqref{eq:opt_stopp_grad_dominance_ineq}. 
	
	
	\paragraph{Case (2): } Now assume that $c_{\pi}(x)  \not \in (y_{\min}, y_{\max})$ in which case we know $c_{\pi}(x) \leq y_{\min}$ (since $c_{\pi}(x)\leq \gamma y_{\max}$) and therefore $\theta^+_x  = y_{\min}$. One can check that 
	\begin{align*}
		G_{x}(\theta^+_x, \theta_x) = 	\intop_{y_{\min} }^{\theta_x} ( y- c_{\pi}(x)  )dy \leq \left( \theta_x - c_{\pi}(x) \right) \left( \theta_x - y_{\min} \right) \leq \max_{\theta'_x \in \Yc }  \left(c_\pi(x)-\theta_x\right) \cdot (\theta'_x - \theta_x) 
	\end{align*}
	where again the final inequality is immediate since $\theta'_x=y_{\min}$ is a feasible choice. This establishes \eqref{eq:opt_stopp_grad_dominance_ineq}. 
\end{proof}




%	Using that $T_{\pi_{\theta^+}} J_{\pi} = T J_{\pi}$, we have
%	\begin{align}
%		\label{eq:grad dominance objective stopping}
%		\Bc(\theta^+ | \eta_{\pi}, J_{\pi}) - \Bc(\theta | \eta_{\pi}, J_{\pi}) &= \sum_{x \in \X} \eta'_{\pi}(x) \int_{\Yc} \left(T J_{\pi}(x,y) - T_{\pi_{\theta}} J_{\pi}(x,y) \right) q_x(y) dy \nonumber \\
%		&\leq  \left(\max_{x' \in \Xc, y'\in \Yc}q_{x'}(y')\right)  \sum_{x \in \X} \eta'_{\pi}(x) \int_{\Yc} \left(T J_{\pi}(x,y) - T_{\pi_{\theta}} J_{\pi}(x,y) \right) dy.
%	\end{align}
%	We can simplify to write,
%	\begin{align}
%		T_{\pi_{\theta}} J_{\pi}(x,y) &= y \cdot \mathbbm{1} (y \geq \theta_x) + c_{\pi_{\theta}}(x) \cdot \mathbbm{1} (y < \theta_x) 	\label{eq:cost-to-go stopping appendix 1} \\
%		T J_{\pi}(x,y) &=  y \cdot \mathbbm{1} (y \geq \theta^+_x) + c_{\pi_{\theta}}(x) \cdot \mathbbm{1} (y < \theta^+_x) \label{eq:cost-to-go stopping appendix 2}
%	\end{align}
%	We argued above that $c_{\pi}(x) < y_{\max}$ and $\theta^+_x = \max \{c_{\pi}(x), y_{\min} \}$. We consider two cases.
%	\paragraph{Case (1):} Assume that $c_{\pi}(x)  \in (y_{\min}, y_{\max})$ in which case $\theta^+_x  = c_{\pi}(x)$. Using equations \eqref{eq:cost-to-go stopping appendix 1} and \eqref{eq:cost-to-go stopping appendix 2}, it is easy to check that
%	\begin{align}
%		\label{eq:case1 stopping RHS}
%		\int_{\Yc} \left(T J_{\pi}(x,y) - T_{\pi_{\theta}} J_{\pi}(x,y) \right) dy &\leq (c_{\pi}(x) - \theta_x)^2.
%	\end{align}
%	As $c_{\pi}(x)  \in (y_{\min}, y_{\max})$, observing the lower bound in \eqref{eq:gradient dominance stopping LHS}, we find that
%	\begin{align}
%		\max_{\theta'_x \in \Yc }  \left(c_\pi(x)-\theta_x\right) \cdot (\theta'_x - \theta_x)  
%		%&\geq   \left(c_\pi(x)-\theta_x\right)    \cdot (\theta^+_x - \theta_x) 
%		\geq (c_{\pi}(x) - \theta_x)^2 \label{eq:case1 stopping LHS} 
%	\end{align}
%	We get our desired result by using \eqref{eq:case1 stopping RHS} and \eqref{eq:case1 stopping LHS} to compare Equations \eqref{eq:grad dominance objective stopping} and \eqref{eq:gradient dominance stopping LHS} respectively.
%	
%	\paragraph{Case (2):} Now assume that $c_{\pi}(x)  \not \in (y_{\min}, y_{\max})$ in which case $\theta^+_x  = y_{\min}$. Again, using \eqref{eq:cost-to-go stopping appendix 1} and \eqref{eq:cost-to-go stopping appendix 2}, it is easy to check that 
%	\begin{align}
%		\label{eq:case2 stopping RHS} 
%		\int_{\Yc} \left(T J_{\pi}(x,y) - T_{\pi_{\theta}} J_{\pi}(x,y) \right) dy = \intop^{\theta_x}_{\theta^+_x} \left( y - c_{\pi}(x) \right) dy &\leq \intop^{\theta_x}_{\theta^+_x} \left( \theta_x - c_{\pi}(x) \right) dy \nonumber \\
%		&= \left( \theta_x - c_{\pi}(x) \right) \left( \theta_x - \theta^+_{x} \right).
%	\end{align}
%	Similarly, we can lower bound the right hand side of \eqref{eq:gradient dominance stopping LHS} as
%	\begin{align}
%		\max_{\theta'_x \in \Yc }  \left(c_\pi(x)-\theta_x\right) \cdot (\theta'_x - \theta_x) \geq   \left( \theta_x -c_{\pi}(x) \right) \cdot (\theta_x - \theta^+_x). \label{eq:case2 stopping LHS} 
%	\end{align}
%	We get out desired result by using \eqref{eq:case2 stopping RHS} and \eqref{eq:case2 stopping LHS} to compare Equations \eqref{eq:grad dominance objective stopping} and \eqref{eq:gradient dominance stopping LHS} respectively.
%\end{proof}
%
%
%
%
%
%
%
%\newpage
%










%\concentrabilityStopping*
%\subsubsection{Conditions 0 - 3 in Example \ref{ex:stopping}}



%Optimality of threshold policies for this problem is well known (see \cite{bertsekas1995dynamic} for example) and essentially follows from the convergence of policy iteration along with the closure property. 
%We verify the additional smoothness properties in  \ref{subsec:app_optimalstopping}. 

\paragraph{Smoothness results: Condition \ref{cond: diff} and Lemma \ref{lem:smoothness_opt_stopp}}

%\paragraph{Condition \ref{cond: diff} and twice continuous differentiability.}
\emph{Additional notation. } 
We simplify notation to write $\eta_{\theta}:= \eta_{\pi_{\theta}}$, $\eta'_{\theta}:=\eta'_{\pi_{ \theta}}$, $T_{\theta}:=T_{\pi_{\theta}}$, and $J_{\theta} := J_{\pi_{\theta}}$. We define $J'_{\theta}(x) := \intop_{\Yc} J_{\theta}(x, y) q_x(y) dy$ to be the expected cost-to-go function from context $x$. Similarly, denote $g'_{\theta}(x) := \intop_{\Yc} \mathbbm{1}\left(  y \geq \theta_x \right) y q_x(y) dy$ to be the expected reward earned from context $x$. Take $J'_{\theta}(\tau)=0$ and $g'_{\theta}(\tau)=0$. Recall that $\nu(x)$ is the probability the initial state $(x_0,y_0)$ has $x_0=x$. We extend $\nu$ to be a probability distribution over $\Xc \cup \{\tau\}$ by defining $\nu(\tau)=0$. 

We let $P'_{\theta} \in \mathbb{R}^{ (|\Xc| + 1) \times (|\Xc| + 1)}$ denote the transition matrix over $\Xc \cup \{\tau\}$ under $\pi_{\theta}$, defined as
\begin{equation}
	\label{eq:transition_probability optimal stopping}
	P'_{\theta}(x'|x) = p(x'|x) \int_{\Yc} \mathbbm{1}(y < \theta_x) q_x(y) dy, \quad P'_{\theta}(\tau|x) = \int_{\Yc} \mathbbm{1}(y \geq \theta_x) q_x(y) dy, \quad P'_{\theta}(\tau|\tau) = 1,
\end{equation} %\sum_{x' \in \Xc} P'_{\theta}(x'|x)
for all $x',x \in \Xc$. One can write key quantities in ``vector form'' as
\begin{equation}\label{eq:opt_stopping_smoothness_matrices}
	J'_{\theta} = \left(I-\gamma P'_{\theta}\right)^{-1} g'_{\theta}  \qquad \& \qquad  \eta'_{\theta} =  (1-\gamma) \nu (I - \gamma P'_{\theta})^{-1}  
\end{equation}
where $\nu\in \mathbb{R}^{|\Xc|+1}$ is a row vector $g'_{\theta}\in \mathbb{R}^{|\Xc|+1}$ is a column vector.  The matrix $(I-\gamma P'_{\thetabar})$ is invertible as $P'_{\thetabar}$ is a stochastic matrix.




%We now verify all the conditions needed for our main results.

\emph{Verifying Condition \ref{cond: diff}}. We establish the main condition needed to invoke the policy gradient formula in Lemma \ref{lem: PG theorem}. 
That $\frac{\partial }{\partial \thetabar_x} \Bc(\thetabar|\eta_{\theta}, J_{\theta})$ exists and is continuous in $\thetabar$ is an immediate consequence of \eqref{eq:policy_grad_opt_stopping}
together with the continuity of $q_{x}(\cdot)$.  We also need to verify that $\Bc(\theta | \eta_{\thetabar}, J_{\theta})$ is continuously differentiable as a function of $\thetabar$. Since $J'_{\theta}(\tau)=0$, 
\[ 
\Bc(\theta | \eta_{\thetabar}, J_{\theta}) = \sum_{x \in \X} \eta'_{\thetabar}(x)\intop_{\Yc} Q_{\pi_{\theta} }( (x,y),  \pi_{ \theta}(x,y) )  q_{x}(y)dy = \sum_{x \in \X} \eta'_{\thetabar}(x) J'_{\theta}(x).
\] 
Observe that $P'_{\thetabar}$ is continuously differentiable in $\thetabar$, as $q_{x}(\cdot)$ is assumed to be continuous.  Therefore, $(I-\gamma P_{\thetabar})^{-1}$ is also continuously differentiable and $\eta'_{\thetabar}(\cdot)$ is as well. 

\emph{Verifying Lemma \ref{lem:smoothness_opt_stopp}.} We now establish the following smoothness result for the policy gradient loss $\ell(\cdot)$, which is useful for invoking convergence rate results for first order methods. 
\optstoppcostsmooth*
\begin{proof}
	Using the policy gradient theorem as shown in Lemma \ref{lem: PG theorem} and the derivative calculations in \eqref{eq:policy_grad_opt_stopping}, we have
	\begin{align*}
		\frac{\partial }{\partial \theta_x} \ell(\theta) = 	\frac{\partial }{\partial \thetabar_x} \Bc(\thetabar | \eta_{\theta}\, , J_{\theta}  )  \bigg\vert_{\thetabar = \theta}  %\eta'_{\theta}(x) \frac{\partial }{\partial \thetabar_x} \left[ \int_{\Yc} Q_{\pi_{\theta}}\left( (x,y), \pi_{\thetabar}(x,y) \right) q_x(y) dy \right] \bigg\vert_{\thetabar=\theta} \\
		= \left( c_{\pi_{\theta}}(x) - \theta_x \right) \eta'_{\theta}(x) q_x(\theta_x).
		%	&= \left( \sum_{x' \in \Xc} p(x'|x) J_{\pi_{\theta}}(x') - \theta_x \right) \eta'_{\theta}(x) q_x(\theta_x) 
	\end{align*}
	We argued above when verifying Condition \ref{cond: diff} that $\eta'_{\theta}(x)$ is continuously differentiable. By assumption, $q_{x}(\theta_x)$ is continuously differentiable in $\theta_x$. Therefore, $\nabla \ell(\theta)$ has a continuous derivative if $c_{\pi_{\theta}}(x)$ is continuously differentiable in $\theta$. 
	To show this, recall that by definition, 
	\begin{align}
		\label{eq:continutaion_value_appendix}
		c_{\pi_{\theta}}(x) = \gamma \sum_{x'\in \Xc}p(x'|x) \int_{\Yc} J_{\theta}(x', y') q_{x'}(y') dy = \gamma \sum_{x'\in \Xc}p(x'|x) J'_{\theta}(x') \qquad \forall x \in \Xc.
	\end{align}
	While verifying Condition \ref{cond: diff} above, we argued that  $(I-\gamma P'_{\theta})^{-1}$ is is continuously differentiable. It is also easily shown that $g'_{\theta}$ is continuously differentiable. Due to \eqref{eq:opt_stopping_smoothness_matrices}, this implies $J'_{\theta}$ is continuously differentiable.  Hence using \eqref{eq:continutaion_value_appendix}, we find that $c_{\pi_{\theta}}$ is continuously differentiable in $\theta$. 
	
	We have shown $\nabla^2 \ell(\theta)$ exists and is continuous. Since $\Theta$ is compact, the Extreme Value theorem implies $\max_{\theta \in \Theta} \| \nabla^2 \ell(\theta) \|_2$ exists and is finite.
\end{proof} 




\subsection{Finite horizon inventory control}
We consider the inventory control problem as described in Example \ref{ex:inventorycontrol}. To review notation, recall that in this setting, the inventory level evolves as: $x_{t+1} = x_t + a_t - w_t$ for non-negative orders $a_t$ and i.i.d demands $w_t \in [0, w_{\max}]$. We let $s_t=(x_t,h_t)$ denote the state at time $t$ and consider the class of base-stock policies which orders inventory, $\pi_{\theta}(s_t) =  \max\{0, \theta_{h_t} - x_t\}$ in state $s_t$. We consider the policy class, $\Pi_{\Theta}=\{ \pi_{\theta} : \theta \in \Theta \}$ with bounded parameter space $\Theta =  [0, 2 w_{\max}]^{H}$ which implies the inventory levels, $x_t$, at every period are bounded in $\mathcal{I} = [-w_{\max}, 2 w_{\max}]$. We assume the initial distribution factorizes as, $\rho(dx,h) = \nu(h) q_{h}(x)dx_0$, where $\nu(h) > 0$ for every $h \in \{1, \ldots, H\}$ and $q_{h}(\cdot)$ is a twice differentiable PDF supported over $\mathcal{I}$ for each $h$. Clearly, this choice of $\rho$ satisfies the regularity condition in Assumption \ref{ass: exploratory rho finite horizon}. The problem setup also clearly follows the factorization structure assumed in Condition \ref{cond: finite_horizon}. Here, we verify the differentiability condition along with Condition \ref{cond:finite_horizon_stationarity}, both of which are needed for Theorem \ref{thm: finite_horizon}.




\paragraph{Reminder on the  Leibniz rule.}
We appeal to the Leibniz rule, which states sufficient conditions for differentiating the integral of a function. For a bounded set $\Psi \subset \R$, consider the function $F: \Psi \to \R$ given by 
\[
F(\psi) = \E [ f(\psi, s) ] = \int_{\Sc} f(\psi,s) P(ds)
\]
where $f: \Psi \times \Sc \to \R$ is a real valued function, $P$ is a probability measure supported over $\Sc$ and for each $\psi \in \Psi$, the function $f(\psi,\cdot)$ is $P$-integrable, i.e. $\E [|f(\psi,s)|] < \infty$. Let $\Dc_s(\psi)$ be the set of points $s \in \Sc$ such that $f(\cdot, s)$ is non-differentiable at $\psi$. By the Leibniz rule, $F$ is differentiable at $\psi$ if (i) $\Dc_s(\psi)$ has zero measure under $P$, i.e. $P[\Dc_s(\psi)]=0$ and (ii) $f'(\psi,\cdot)$ is $P$-integrable, in which case $F'(\psi) =  \int_{\Sc} f'(\psi,s) P(ds).$  By applying the same steps again, we can calculate the second derivative of $F(\cdot)$ as well.

The Leibniz rule is useful as a threshold policy, $\pi_{\theta}(z)=\max\{0, \theta - z\}$, is differentiable everywhere except at one point, $z=\theta$.



\paragraph{Condition \ref{cond: diff}: continuous differentiability.}
We make the abbreviation $\eta_{\theta}=\pi_{\theta}$, $J_{\theta}\equiv J_{\pi_\theta}$ and $Q_{\theta}\equiv Q_{\pi_{ \theta}}$. To establish Condition 0, we need to show that the function $\Bc(\theta^+ | \eta_{\thetabar}, \, J_{\theta}) = \intop Q_{\theta}(s, \pi_{\theta^+}(s))\eta_{ \thetabar}(ds),$ is (i) continuously differentiable as a function of $\theta^+$ when $\thetabar=\theta$ and (ii) continuously differentiable in $\thetabar$ when $\theta^+=\theta$. The approach is to (somewhat tediously) rewrite $\Bc(\cdot)$ in terms of a single multi-dimensional integral that appears in \eqref{eq:inventory_smoothness_integral_form} below. From there, the result follows by applying the Leibniz rule to differentiate under the integral. 

We write:
\begin{align*}
	\Bc(\theta^+ | \eta_{\thetabar},\, J_{\theta}) &= (1-\gamma)\E_{\rho}^{\pi_{\thetabar}}\left[\sum_{t=0}^{\infty} \gamma^t Q_{\theta}(s_t, \pi_{ \theta^+}(s_t)  ) \right] \\
	&= (1-\gamma)\E_{\rho}^{\pi_{\thetabar} }\left[\sum_{t=0}^{H-h_0} \gamma^t Q_{\theta}(s_t, \pi_{ \theta^+}(s_t)  ) \right] \\ 
	&= (1-\gamma)\E_{\rho}^{\pi_{\thetabar} }\left[\sum_{t=0}^{H-h_0} \underbrace{\E_{\rho}^{\pi_{\thetabar} }\left[ \gamma^t  Q_{\theta}(s_t, \pi_{ \theta^+}(s_t)  ) \mid h_0 \right]}_{:= \Bc_{h_0, t}(\theta^+ | \eta_{\thetabar},\, J_{\theta})  }\right].
\end{align*}
The first equality is the definition of the state occupancy measure. The second equality uses that the process transitions to a terminal state after stage $h_t=H+1$ is reached. The final equality is uses the tower property of conditional expectation --- there the outer expectation is over $h_0 \in \{1, \cdots, H\}$ drawn from the initial distribution and the inner expecation is over the state $s_t=(x_t, h_0+t)$, and in particular the inventory level $x_t$, that is reached $t$ periods later under the policy $\pi_{ \thetabar}$. 

We show that each individual term, $\Bc_{h_0, t}(\theta^+ | \eta_{\thetabar},\, J_{\theta}),$ is continuously differentiable in $\thetabar$ or in $\theta^+$. This completes the result, since $\Bc(\theta^+| \eta_{ \thetabar}, J_{\theta})$ a finite mixture of such terms.  Notice that this expression involves three different policies that are applied at different timesteps:
\begin{enumerate}
	\item $\pi_{ \thetabar}$ is applied prior to timestep $t$ and it is these dynamics that determine $s_t$. 
	\item $\pi_{\theta^+}$ is applied during timestep $t$ only. (That is the meaning of the action in the $Q$ function.)
	\item $\pi_{ \theta}$ is applied from timestep $t+1$ until the final stage is reached. (That is the meaning of the subscript of the $Q$ function.) 
\end{enumerate}
Based on this, we write
$\tilde{\theta} = (\thetabar_1, \cdots, \thetabar_{h_{t}-1}, \theta^+_{h_t}, \theta_{h_t+1},\, \cdots, \theta_H ).$ Since we condition on $h_0$ and treat a fixed $t$ throughout the remainder of the proof, we omit dependence on these quantities in notation. Then, one can write 
\[
\Bc_{h_0, t}(\theta^+ | \eta_{\thetabar},\, J_{\theta}) = \E_{\rho}^{\pi_{\tilde{\theta} } }\left[ \sum_{\ell=t}^{H-h_0} \gamma^{\ell}  g(s_t, a_t)  \, \bigg\vert \, h_0 \right], 
\] 
where we used the observations 1-3 above together with the definition of a $Q$-function as an expected disctounted sum of single-period costs $g(\cdot)$. In this inventory control problem,  
\begin{equation*}
	g(s_t,a_t) = c \cdot a_t + \E[r(x_t + a_t - w_t) \mid x_t, a_t] = c \cdot a_t + \E[r(x_{t+1}) \mid x_t, a_t],
\end{equation*}
where $r: \mathbb{R} \to \mathbb{R}$ is defined as $r(z) = b\max(0,z) + p\max(0,-z)$ and denotes the holding/backlogging costs. The conditional expectation in the middle equation integrates over the i.i.d draw of the demand $w_t$ and the second equation uses form of inventory dynamics $x_{t+1} = x_t +a_t - w_t$.  By the tower property of conditional expectation, we can rewrite  
\begin{equation}\label{eq:inventory_smoothness_expectation_form}
	\Bc_{h_0, t}(\theta^+ | \eta_{\thetabar},\, J_{\theta}) = \E_{\rho}^{\pi_{\tilde{\theta} } }\left[ \sum_{\ell=t}^{H-h_0} \gamma^{\ell}  \left(  c \cdot a_t  + r(x_{t+1}) \right)   \, \bigg\vert \, h_0  \right]. 
\end{equation}
%All randomness in this expression is taken over the initial state $x_0$, drawn from a the continuous density $q_{h_0}(\cdot)$, and the demands $w_0, \cdots, w_H$ that are drawn i.i.d from a continuous density. Write $\xi = (x_0, w_0, \cdots, w_H )$. Then one can write $\Bc_{h_0, t}(\theta^+ | \eta_{\thetabar},\, J_{\theta}) = \E_{\xi}\left[  F( \vec{a}  , \xi ) ]$. Here $F( \vec{a}, \xi )=\sum_{\ell=t}^{H-h_0} \gamma^{\ell}  \left(  c \cdot a_t  + r(x_{t+1}) \right)$ evaluates the costs 

%Conditioned on $\vec{w}$ and $x_0$, 



Finally, we are ready to put this in the form of a single multi-dimensional integral. For any sequence of of inventory levels write $\vec{x}=(x_0, \cdots, x_{H-h_0+1})$. Set $G(\vec{x}, \tilde{\theta}) = \sum_{\ell=t}^{H-h_0} \gamma^{\ell}  \left(  c \cdot [ \tilde{\theta}_{h_t} - x_t ]^+  + r(x_{t+1}) \right)$, representing the cost incurred for an arbitrary sequence of inventory levels $\vec{x}$ assuming the ordering costs are based on the values  $[\tilde{\theta}_{h_t} - x_t ]^+= \max\{0, \tilde{\theta}_{h_t} - x_t  \}$ prescribed by the base-stock levels $\tilde{\theta}$. Now, to assign probabilities over the sequence $\vec{x}$, 
recall that conditioned on $h_0$, the initial inventory level $x_0$ is drawn from a PDF $q_{x}(\cdot)$. 
Let $f(\cdot)$ denote the PDF of the demand distribution. Both PDFs are assumed to be twice differentiable. Then, 
\begin{equation}\label{eq:inventory_smoothness_integral_form}
	\Bc_{h_0, t}(\theta^+ | \eta_{\thetabar},\, J_{\theta}) = \intop G(\vec{x}, \tilde{\theta}) p(\vec{x} \mid \tilde{\theta}) d\vec{x}
\end{equation}
where 
\[ 
p(\vec{x} \mid \tilde{\theta}) = q_{h_0}(x_0) \prod_{t=0}^{H-h_0} f(x_{t+1} - x_t - [\tilde{\theta}_{h_t}-x_t]^+) %f(x_1 - x_0 - [\tilde{\theta}_{h_0}-x_0]^+) \cdots f(x_{H-h_0+1} - x_{H-h_0} - [\tilde{\theta}_{H}-x_{H-h_0}]^+) 
\]
is the probability density function of $\vec{x}$. Here we have used that $x_{t+1}= x_t + a_t - w_t$ to relate the transitions of the inventory level to demand realizations.  

Now,  we can justify that $G(\vec{x}, \tilde{\theta}) p(\vec{x} , \tilde{\theta} )$ is almost surely twice differentiable with bounded first and second derivatives, so the Leibniz rule implies \eqref{eq:inventory_smoothness_integral_form} is twice differentiable (and hence continuously differentiable). Notice that $G(\vec{x}, \tilde{\theta})$ and $p(\vec{x} , \tilde{\theta} )$ may fail to be differentiable at values of $\vec{x}$ where $x_t = \tilde{\theta}_{h_t}$ for some $t$, but the set of such sequences of inventory levels has zero Lebesgue measure. Boundedness of first and second derivatives of $G(\vec{x}, \tilde{\theta})$ is immediate since it involves piece-wise linear functions of $\tilde{\theta}$.  Boundedness of first and second derivatives of $p(\vec{x} \mid \tilde{\theta})$ can be shown from the assumption that $f(\cdot)$ and $q_{h_0}(\cdot)$ are twice continuously differentiable and both $\vec{x}$ and $\tilde{\theta}$ take values in bounded sets. (See Example \ref{ex:inventorycontrol} where it is noted that $x_t \in [-w_{\max}, 2w_{\max}]$ almost surely.).

\begin{rem}
	It is also possible to complete the argument by claiming that the discounted sum inside \eqref{eq:inventory_smoothness_expectation_form} is differentiable \emph{pathwise}, i.e for each realization of the random initial inventory level $x_0$ and the demand realizations (except on a set of measure zero). A benefit of this approach is that it does not require differentiability of $f(\cdot)$, whereas directly differentiating $p(\vec{x} | \tilde{\theta})$ in  $\eqref{eq:inventory_smoothness_integral_form}$ does. See \cite[Section 2.6]{bertsekas1997nonlinear} for an introduction on how to calculate pathwise derivatives using the chain rule. \cite{glasserman1995sensitivity} applies this technique rigorously to an inventory control problem. 
\end{rem}
 
\end{document}


\newpage
\dr{Jalaj's proof}

\paragraph{Condition \ref{cond: diff}: differentiability.}
%We first comment on some differentiability conditions needed for the policy gradient lemma to hold. Recall the setting in Example \ref{ex:inventorycontrol} where the inventory level evolves as: $s_{t+1} = s_t + a_t - w_t \,\, \forall \, t = \{0,\ldots,H-1\}$ for non-negative inventory orders $a_t$ and i.i.d demands $w_t \in [0, w_{\max}]$. We consider the class of base-stock-policies parameterized as $\Pi_{\theta} = \left\{\theta=(\theta_0, \ldots, \theta_{H-1}) \in \mathbb{R}^H : \theta_t > 0\right\}$ which orders inventory $\pi_{\theta}(s_t) =  \max\{0, \theta_t - s_t\}$ at time $t$. Also recall that we treat finite-horizon time-inhomogenous MDPs as a special case of infinite horizon MDP using the following factorization. 
%Proof of Theorem \ref{thm: finite_horizon}}
%\label{subsec: finite horizon proof}
%For the reader's convenience, we restate Condition \ref{cond: finite_horizon} and Theorem \ref{thm: finite_horizon}.
%\condFiniteHorizon*

We appeal to the Leibniz rule which states sufficient conditions for differentiating the integral of a function. For a bounded set $\Psi \subset \R$, consider the function $F: \Psi \to \R$ given by 
\[
F(\psi) = \E [ f(\psi, s) ] = \int_{\Sc} f(\psi,s) P(ds)
\]
where $f: \Psi \times \Sc \to \R$ is a real valued function, $P$ is a probability measure supported over $\Sc$ and for each $\psi \in \Psi$, the function $f(\psi,\cdot)$ is $P$-integrable, i.e. $\E [|f(\psi,s)|] < \infty$. Let $\Dc_s(\psi)$ be the set of points $s \in \Sc$ such that $f(\cdot, s)$ is non-differentiable at $\psi$. By Leibniz rule, $F$ is differentiable at $\psi$ if (i) $\Dc_s(\psi)$ has zero measure under $P$, i.e. $P[\Dc_s(\psi)]=0$ and (ii) $f'(\psi,\cdot)$ is $P$-integrable. Leibniz rule is useful as a threshold policy, $\pi_{\theta}(z)=\max\{0, \theta - z\}$, is differentiable everywhere except at one point, $z=\theta$.

Fix some $\theta = (\theta_0, \ldots, \theta_{H-1}) \in \Theta$. For the inventory control problem, we first argue differentiability of $\eta_{\pi_{\theta}}$. Note that give our problem setup, for any state $s=(x,h)$, the inventory level in the next period lies in the interval $\mathcal{I}$ and the stage advances by one. As $\pi_{\theta}(s)$ is differentiable except at $x\theta_h$, for any measurable set $\Mc \in \mathcal{I}$, the transition kernel
\[
P^{\pi_{\theta}}( (\Mc, h+1) \mid (x,h)) = \E_{w_h} \left[ \mathbbm{1}\left( x + \pi_{\theta}(s) - w_h \in \Mc \right)  \right]
\]
is differentiable in $\theta$ following Leibniz rule. A similar argument shows differentiability of the integral,
\[
\intop P^{\pi_{\theta}}( (\Mc, h+1) \mid (x,h)) \, \rho(dx, h)
\]
by using that $|\frac{\partial}{ \partial \theta_h} P^{\pi_{\theta}}( (\Mc, h+1) \mid s)|$ is bounded as $|\frac{\partial}{\partial \theta_h} \pi_{\theta}(s)| \leq 1$ for all $x \neq \theta_h$ (Leibniz rule requires bounded derivatives). We can write out $\eta_{\pi_{\theta}}$ as,
\begin{align*}
	\eta_{\pi_{\theta}}(M,h) &= \rho(M,h) + \gamma \intop P^{\pi_{\theta}}( (M,h) \mid (x,h-1) ) \rho(dx,h-1) + \\
	&\qquad \quad \gamma^2 \intop \intop P^{\pi_{\theta}} ( (M,h) \mid y, h-1 ) P^{\pi_{\theta}} ( (dy,h-1) \mid (x,h-2)) \rho(dx,h-2) + \ldots 
\end{align*}
where each of the integrals are differentiable in $\theta$ using the same argument as above. This implies differentiability of $\eta_{\pi_{\theta}}$.

%For any period $h \in \{0,\ldots, H-1\}$, state $s_h=(x,h)$ and a measurable set $\Mc \subset \mathcal{I}_{h+1}$, the transition kernel under $\pi_{\theta}$, $P_{\theta_h}(s_h,\Mc) = \E_{w_h} [ \mathbf{1}(x + \pi_{\theta_h}(s_h) - w_h \in \Mc) ]$ is differentiable for any $x \neq \theta_h$. Clearly, $|\partial / \partial \theta_h P_{\theta_h}(s_h, \Mc)|$ is also bounded as $|\partial / \partial \theta_h \pi_{\theta_h}(s_h)| \leq 1 \,\, \forall s_h \neq \theta$. 
%$|\partial / \partial \theta_h \pi_{\theta_h}(s)| \leq 1 \,\, \forall \, s \neq \theta_h$.
%$P_{\theta_h}(s,A) = \int_{\Sc_{h+1}} \mathbbm{1}(x \in A) \Prob_{\theta_h}(s,x)dx$ where $\Prob_{\theta_h}(s,x) = \E_{w_h} [ \mathbbm{1}(s + \pi_{\theta_h}(s) - w_h = x) ]$ \jb{check again}. Clearly, $\Prob_{\theta_h}(s,x)$ and hence $P_{\theta_h}(s,A)$ is differentiable for any $s \neq \theta_h$. 
%Therefore, when $\rho$ is supported over $\Sc_h$, the one step transition kernel
%\begin{align}
%	\label{eq:transition kernel inventory}
%\Prob^{\pi_{\theta}}_\rho(\Mc) = \int_{S_h} P_{\theta_h}(s_h,\Mc) \, d\rho(s_h)
%\end{align}
%is differentiable for any $\theta_h \in \Theta_h$. A similar argument holds for the t-step counterpart of \eqref{eq:transition kernel inventory}, which is a product of the one step transition kernels. Therefore, $\eta_{\theta}$ is differentiable in $\theta$.
%For instance, consider any $A \in \Sc_{h+2}$
%\[
%\lambda P^2_{\theta}(A) = \int_{\Sc_h} P_{\theta_h}(s,dy) P_{\theta_{h+1}}(y,A) \lambda(s) ds
%\]
%which is clearly differentiable in $\theta$. 
%Hence, for any $A \in \Sc_h$ and $h \in \{1,\ldots,H+1\}$, the state-occupancy measure $\eta_{\theta}(A) = \sum_{i=1}^h \rho P^{i}_{\theta}(A)$ is differentiable in $\theta$. It is noteworthy to see that $\eta_{\theta}$ is supported over all $\Sc$ as the start distribution $\rho$ is supported over each $\Sc_h$ for $h \leq H$.

To show differentiability of $\Bc(\thetabar|\eta_{\theta}, J_{\pi_{\theta}})$, consider the Bellman update $T_{\thetabar} J_{\theta}$ for any $\theta, \thetabar \in \Theta$. For any starting state $s_0=(x_0,h_0)$ and $h_0 < H$, we can write
\begin{align}
	\label{eq:Bellman update differentiability inventory}
	T_{\thetabar} J_{\theta}(s_0) = \left[ g(x_0, \pi_{\thetabar}(s_0)) + \sum_{t=1}^{H-h_0} g(x_t,a_t) \right]
\end{align}
where $\pi_{\thetabar}(s_0) = \max\{0, \thetabar_{h_0}-x_0\}$, $a_t = \pi_{\theta}(s_t) = \max\{0, \theta_{h_t} - x_t\}$ and the expected per-step cost function is given by $g(x_t,a_t) = c a_t + \E_{w_t}[r(x_t + a_t - w_t)]$. Here, $r: \mathbb{R} \to \mathbb{R}$ is defined as $r(z) = b\max(0,z) + p\max(0,-z)$ and denotes the holding/backlogging costs. Consider derivatives of the first term, 
\[
\frac{\partial}{\partial \thetabar_{h_0}} g(x_0,\pi_{\thetabar}(s_0)) = c  \cdot \underbrace{\frac{\partial \pi_{\thetabar}(s_0)}{\partial \thetabar_{h_0}}}_{(a)} + \underbrace {\frac{\partial}{\partial \thetabar_{h_0}} \E_{w_0}[r(x_0 + \pi_{\thetabar}(s_0) - w_0)]}_{(b)}
\]
Here, (a) exists everywhere except at $x_0=\thetabar_{h_0}$. For (b), we use that $r(x_0 + \pi_{\thetabar}(s_0) - w_0)$ is differentiable everywhere except at $x_0=\thetabar_{h_0}$ and $x_0 + \pi_{\thetabar}(s_0) = w_0$ as well as the fact that $|\frac{\partial}{\partial \thetabar_{h_0}} r(x_0 + \pi_{\thetabar}(s_0) - w_0)| \leq \max\{b,p\}$. Therefore, using Leibniz rule, the expectation in (b) is differentiable and hence $g(x_0,\pi_{\thetabar}(s_0))$ is differentiable everywhere except $x_0=\thetabar_{h_0}$. Also note that as $|\frac{\partial \pi_{\thetabar}(s_0)}{\partial \thetabar_{h_0}}| \leq 1$, this implies $|\frac{\partial}{\partial \thetabar_{h_0}} g(x_0,\pi_{\thetabar}(s_0))|$ is bounded.

%For the second term, we used that $r(x_0 + \pi_{\thetabar}(s_0) - w_0)$ is differentiable everywhere except at $x_0=\thetabar_{h_0}$ as well as at $x_0 + \pi_{\thetabar}(s_0) = w_0$ and $|\frac{\partial}{\partial \thetabar_{h_0}} r(x_0 + \pi_{\thetabar}(s_0) - w_0)| \leq \max\{b,p\}$. Therefore, using Leibniz rule, the expectation in (b) is differentiable in $\thetabar_{h_0}$. 
Let's now consider the remaining terms,
\[
\frac{\partial}{\partial \thetabar_{h_0}} g(x_t,a_t) = c \cdot \frac{\partial a_t}{\partial \thetabar_{h_0}} + \frac{\partial}{\partial y_t} \E_{w_t} [r(y_t - w_t)] \bigg \vert_{y_t = x_t + a_t} \left(\frac{\partial x_t}{\partial \thetabar_{h_0}} + \frac{\partial a_t}{\partial \thetabar_{h_0}}\right) 
\]
%\begin{align*}
%\frac{\partial}{\partial \thetabar_{h_0}} g(x_t,a_t) &= c \cdot \frac{\partial a_t}{\partial \thetabar_{h_0}} + \frac{\partial}{\partial y_t} \E_{w_t} [r(y_t - w_t)] \bigg \vert_{y_t = x_t + a_t} \frac{\partial y_t}{\partial \thetabar_{h_0}} \\
%&= c \cdot \frac{\partial a_t}{\partial \thetabar_{h_0}} + \frac{\partial}{\partial y_t} \E_{w_t} [r(y_t - w_t)] \bigg \vert_{y_t = x_t + a_t} \left(\frac{\partial x_t}{\partial \thetabar_{h_0}} + \frac{\partial a_t}{\partial \thetabar_{h_0}}\right) 
%\end{align*}
Again, the function $r(y-w_t)$ is differentiable in $y$ except at $y=w_t$ and $|\frac{\partial}{\partial y} r(y - w_t)| \leq \max\{b,p\}$. As the demand distribution is assumed to have a density over $[0, w_{\max}]$, the expectation term is differentiable using Leibniz rule. We can also write
\[
\frac{\partial a_t}{\partial \thetabar_{h_0}} = \frac{\partial \pi_{\theta}(s_t)}{\partial \thetabar_{h_0}} = \frac{\partial \pi_{\theta}(s_t)}{\partial x_t} \cdot \frac{\partial x_t}{\partial \thetabar_{h_0}}
\]
Repeatedly using the fact that threshold policies are differentiable everywhere except at one point, a little bit of algebra shows that $x_t$, $a_t$ and hence $g(x_t,a_t)$ is differentiable in $\thetabar_{h_0}$ except only at a finite number of points and $|\frac{\partial}{\partial \thetabar_{h_0}} g(x_t,a_t)|$ is bounded. Equation \eqref{eq:Bellman update differentiability inventory} shows that the same holds for $T_{\thetabar} J_{\theta}$, implying differentiability of $\Bc(\thetabar|\eta_{\pi_{\theta}},J_{\pi_{\theta}})$. Our arguments can be similarly extended to argue differentiability of $J_{\theta}$ and $\ell(\theta)$. We omit them for brevity.















==> formulation.tex <==
%!TEX root = policy_grad_optimality.tex

\section{Problem formulation}
\label{section:problem_formulation}

Consider a Markov decision process (MDP), which is a six-tuple $\left(\Sc, \Ac, g, P, \gamma, \rho \right)$, consisting of a state space $\Sc$, action space $\Ac$, cost function $g$, transition kernel $P$, discount factor $\gamma \in (0,1)$ and initial distribution $\rho$. In our general problem formulation we avoid measure theoretic subtleties by assuming the state space is either finite or countably infinite. See Remark \ref{rem: countable state} for a discussion. For each state $s\in \Sc$,  $\Ac_s\subset \mathbb{R}^k$ is the set of feasible actions. We take $\Ac=\cup_{s} \Ac_s$. The transition kernel $P$ specifies the probability $P(s'|s,a)$ of transitioning to a state $s'$ upon choosing action $a$ in state $s$. The cost function  $g(s,a)$ denotes the instantaneous expected cost incurred when selecting action $a$ in state $s$. We assume that per-period costs are uniformly bounded, meaning $\sup_{s\in \Sc, a\in \Ac_s} |g(s,a)|<\infty$.

A stationary policy is a function $\pi: \Sc \to \Ac$ is a function that prescribes a feasible action $\pi(s)\in \Ac_s$ for each state $s\in \Sc$. Let $\Pi$ denote the set of all stationary policies. Rather than develop separate notation for randomized and deterministic policies, in specific settings like Example \ref{ex:tabularMDPs}, we accommodate randomized policies by letting $a\in \Ac_s$ denote a choice of probability vector.  We write $\E_{\nu}^{\pi}[\cdot]$ to indicate an expectation is taken over the Markov chain $(s_0, s_1, \cdot)$ induced by policy $\pi$ when the initial state $s_0$ is drawn from $\nu$. With this notation, $\E_{\nu}[f(s_0)]$ is the expectation over a random state drawn from $\nu$. 


\paragraph{Cost-to-go-functions and Bellman operators.}
Let $\Jc = \{J : \Sc \to \mathbb{R} :  \|  J\|_\infty <\infty \}$ denote the set of bounded functions on the state space. For each stationary policy $\pi \in \Pi$, we use the compact notation $g_{\pi} \in \Jc$ for the function $g_{\pi}(s)=g(s, \pi(s))$ for all $s\in \Sc$. The cost-to go function $J_{\pi} \in \Jc$ associated with policy $\pi$ is defined by $J_{\pi}(s) = \E^{\pi}_{s}\left[ \sum_{t=0}^{\infty} \gamma^t g_{\pi}(s) \right]$. Define the Bellman operator $T_{\pi}: \Jc \to \Jc$ under the policy $\pi$ as 
\[
\left(T_{\pi} J\right)(s) := g_{\pi}(s) + \gamma \E^{\pi}_{s}[J(s_1)]  =g(s, \pi(s)) +  \sum_{s' \in \Sc} P(s' | s, \pi(s)) J(s'). 
\] 
The cost-to-go function under policy $\pi$ is the unique solution to the Bellman equation $J_\pi = T_{\pi} J_\pi$. The Bellman optimality operator is denoted by $T: \Jc \to \Jc$ and defined by $(TJ)(s) = \min_{\pi \in \Pi} (T_{\pi} J)(s)$. For simplicity of exposition, we assume throughout that this minimum is exists. The unique fixed point of $T$, denoted by $J^*$, is called the optimal cost-to-go function and satisfies $J^*(s) = \min_{\pi} J_{\pi}(s)$ for all $s\in \Sc$. There is at least one optimal policy, $\pi^*$, that attains this minimum for every $s\in \Sc$. It is well known that $T$ and $T_{\pi}$ are monotone and are contraction operators with respect to the maximum norm $\| \cdot \|_{\infty}$. %Additional background is given in Appendix \ref{sec: app_bellman_background}. 

The state-action cost-to-go function corresponding to a policy $\pi\in \Pi$,
\begin{equation}\label{eq: def q function}
Q_{\pi}(s,a)= g(s,a)+ \gamma \sum_{s' \in \Sc} P(s'\mid s,a) J_{\pi}(s'),
\end{equation}
measures the cumulative expected cost of taking action $a$ in state $s$ and applying $\pi$ thereafter. The state-action value function provides an alternative notation for Bellman operators. Define $Q^*(\cdot, \cdot) = Q_{\pi^*}(\cdot, \cdot)$ for some optimal policy $\pi^*$. This is the same as \eqref{eq: def q function} except the optimal cost-to-go function $J^*$ appears on the right hand side. Notice that for any polices $\pi,\pi'\in \Pi$, we have the relations 
\begin{align}\label{eq: q to bellman}
Q_{\pi}(s,\pi(s)) =  J_{\pi}(s),  \qquad    Q_{\pi}(s,\pi'(s)) =  (T_{\pi'} J_{\pi})(s),  \qquad  \min_{a\in \Ac_s} Q_{\pi}(s,a) = (TJ_{\pi})(s).
\end{align}


%\paragraph{Vector notation.}
%We use vector and matrix notation that is standard in the study of Markov decision processes, including for problems with infinite state spaces. The readers can refer to \cite[Sections 5.5, 6.1-6.2, Appendix C]{puterman2014markov} for background. 
%For each stationary policy $\pi \in \Pi$, we use the compact notation $g_{\pi} \in \Jc$ for the function $g_{\pi}(s)=g(s, \pi(s))$ for all $s\in \Sc$. As in \cite{puterman2014markov}, we call $P_{\pi} = (P(s'| s, \pi(s)))_{s,s'\in \Sc}$ the transition matrix and let $P_{\pi}^t$ denote the $t$-step transition matrix. Readers unfamiliar with infinite state space Markov chains should note that all expressions are  generalizations of those for finite Markov chains\footnote{The Chapman Kolmogorov equation states that $P_{\pi}^t = P_{\pi}^{t-1} P_{\pi}$ can be written in terms of operator composition, as when raising a square matrix to the $t$--th power. The left and right linear operators correspond to left or right matrix multiplication. They can be expressed as summations, $(P_{\pi}J)(s) = \sum_{s' \in \Sc} P(s'| s, \pi(s) ) J(s')$ and $(\nu P_{\pi})(s) = \sum_{s' \in \Sc} \nu(s')P(s| s', \pi(s'))$.   For a finite Markov chain, the Neumann series  $\sum_{t=0}^{\infty} \gamma^t P_{\pi}^t =$ converges and is equal to  $(1-\gamma P_{\pi})^{-1}$ because the spectral radius of $\gamma P_{\pi}$ is bounded by $\gamma <1$. Similarly, convergence holds here because $\gamma P_{\pi}$ is contractive when viewed either as left or right operator:  $\| \gamma P_{\pi} J\|_{\infty} \leq \gamma <1$ for each $J$ with $\|J\|_{\infty} = 1$ and   $\| \gamma \nu P_{\pi}\|_{1} \leq \gamma$ when $\| \nu\|_1 =1$.}. Transition matrices operate on elements $J\in \Jc$ on the right as $(P^t_{\pi}J)(s) = \E_s^{\pi}[J(s_t) ]$ and probability distributions $\nu$ (viewed as row vectors) on the left  as $(\nu P^t_{\pi})(s)= \Prob_{\nu}^{\pi}(s_t=s)$.  In this notation, one can write the Bellman operator concisely as $T_{\pi }J = g_{\pi} + \gamma P_{\pi}J$ and the cost to-go function as 
%\[ 
%J_\pi = g_\pi + \gamma P_\pi  J_\pi = \cdots = \sum_{t=0}^\infty \gamma^t P_{\pi}^t  g_\pi = (I-\gamma P_\pi)^{-1}  g_\pi. 
%\]

\paragraph{Scalar loss function and initial distributions.} Although classical dynamic programming methods seek a policy $\pi^* \in \argmin_{\bar{\pi} } J_{\bar{\pi}}(s)$ that simultaneously minimizes the expected cost incurred \emph{from every} state, for policy gradient methods it is more natural to study a scalar loss function  
\[
\ell(\pi)=  (1-\gamma) \E_{\rho}^{\pi}\left[\sum_{t=0}^{\infty} \gamma^t g_{\pi}(s_t) \right] =  (1-\gamma) \E_{\rho}[J_{\pi}(s_0)].  
\]
in which the states are weighted by their initial probabilities under $\rho$ and we have normalized costs by $(1-\gamma)$ for convenience.  We assume throughout that $\rho$ is supported on the entire state space, meaning that $\rho(s)>0$ for all $s\in \Sc$. Since $\rho$ places positive probability on each state, $\ell(\pi)> \ell(\pi^*)$ except when  $J_{\pi}(s) = J_{\pi^*}(s)$ at every state, implying optimality in the classical sense. As commented in Subsection \ref{subsec: scope}, policy gradient methods have poor convergence properties if applied without an exploratory initial distribution. See Appendix \ref{sec: app_iniital_distribution} for a full discussion


\paragraph{State distributions.}  We define the discounted state-occupancy measure under any policy $\pi$ and initial state distribution $\rho$ as, $\eta_{\pi}(s) = (1-\gamma)\sum_{t=0}^{\infty} \gamma^t \Prob_{\rho}^{\pi}[s_t = s]$. This evaluates the discounted fraction of time the system spends at state $s$ under policy $\pi$. This can be written in vector notation as: 
\begin{equation} \label{eq: discounted_state_occupancy_measure}
\eta_{\pi} =  (1-\gamma)\sum_{t=0}^{\infty} \gamma^{t} \rho P_{\pi}^t = (1-\gamma) \rho (I - \gamma P_\pi)^{-1}.
\end{equation}
When the state space is finite, $\eta_{\pi}$ and $\rho$ are both row vectors. Notice that $\ell(\pi) = \E_{\eta_{\pi}}\left[ g_{\pi}(s_0)  \right]$ is equal to the average cost for a state drawn from a $\pi$'s state occupancy measure.  %Recognize that $\rho P_{\pi}^t$ is the distribution of the state at time  $t$, and so $\eta_{\pi}(s)$

\paragraph{Parameterized policies.}
Policy gradient methods search over a parameterized class of policies, $\Pi_{\Theta} = \{ \pi_\theta(\cdot): \theta \in \Theta \} \subset \Pi$ which have corresponding cost-to-go functions $\Jc_{\Theta} = \{ J_{\pi_\theta} : \theta \in \Theta \}$. Assume $\Theta \subset \mathbb{R}^d$ is convex. To indicate that we are referring to a policy in the restricted policy class, rather than an arbitrary stationary policy $\pi \in \Pi$, we typically either write $\pi_\theta$ or specify that $\pi \in \Pi_{\Theta}$. We overload notation, writing $\ell(\theta) = \ell(\pi_{\theta})$. Policy gradient methods aim to minimize this loss function using gradient descent or a related first-order method.  We will state later results under smoothness conditions ensuring differentiability.

%We next assume appropriate smoothness conditions on the policy class and on the cost and transition functions to ensure that $g(s, \pi_{\theta}(s))$ and $P(s'| s,\pi_{\theta}(s))$ are differentiable functions of $\theta$. 

%To deal with infinite state spaces, we need also an assumption that gradient norms are uniformly bounded. The final regularity condition, involving the sum of the derivatives, comes from considering  forward expectations of the form $\sum_{s' \in \Sc} P(s' | s, \pi_\theta(s)) J(s')$. Assuming the summation and derivative can be exchanged, the partial derivative is  $\sum_{s' \in \Sc}\frac{\partial}{\partial \theta_i}  P(s' | s, \pi_\theta(s)) J(s')$. We would like this derivate be finite for each $J\in \Jc$, which requires  $\sum_{s' \in \Sc}\left|\frac{\partial}{\partial \theta_i}  P(s' | s, \pi_\theta(s)) \right| <\infty$. An alternate view is that this is precisely the condition that the partial derivative is integrable under the counting measure, which is the condition needed to apply the Leibniz rule justifying the interchange of the summation and derivative. 
% %Unfortunately, there is some added complexity to the assumption statement since differentiability is defined with respect to open sets and the sets $\Ac_s$ and $\Theta$ are naturally closed in some examples. As is common in optimization, we assume functions are differentiable on open sets that contain the closed set of feasible actions. As a simple case, we sometimes have $g(s, a) = \sum_{i=1}^{k} c^{s}_i a_i$ where $a$ is constrained to be a probability vector. While the set of probability vectors is closed, $g(s, \cdot)$ has a natural extension to a linear (hence differentiable) function over all of $\mathbb{R}^k$. 
%\begin{assumption}\label{ass: regularity}	For all $s, s'\in \Sc$, $a\mapsto g(s,a)$ and $a\mapsto P(s'|s,a)$ are continuously differentiable functions on an open set containing $\Ac_s$ and $\theta \mapsto \pi_{\theta}(s)$ is continuously differentiable on an open set containing $\Theta$. In addition, $\sup_{s\in \Sc, a\in \Ac_s} \| \nabla_a g(s,a) \|< \infty$, $\sup_{s\in \Sc, \theta \in \Theta} \|  \nabla_\theta \pi_{\theta}(s) \|< \infty$, and for any $i\in \{1,\cdots, d\}$, $\sup_{s\in \Sc, \theta \in \Theta} \sum_{s' \in \Sc} \left| \frac{\partial}{\partial \theta_i} P(s' | s, \pi_{\theta}(s)) \right|  < \infty$.   
%\end{assumption}




\paragraph{Norms.} Define the weighted $p$-norm, $\| J\|_{p,w} = \left(\sum_{s} |J(s)|^p \, w(s)\right)^{1/p}$.  When $w(s)=1$ for all $s\in \Sc$, we simplify notation and write $\| J \|_{p}$. The maximum norm is $\| J\|_{\infty} =  \sup_{s \in \Sc} |J(s)|$. For a matrix $A \in \mathbb{R}^{n\times m}$, we write $\| A \| = \max_{x: \| x\|_2 = 1 }  \| Ax\|_2$ for the operator norm. 


\begin{rem}[Interpretation as an average cost problem with random restarts.] 
	Discounted problems are known to be equivalent to a modified un-discounted problem, where, in every period, there is a constant probability $1-\gamma$ that the problem ``restarts'' in a random state drawn from the initial distribution $\rho$. In this modified problem, $\eta_{\pi}(s)$ denotes the long run fraction of time spent in state $s$ and so $\ell(\pi)$ denotes the long run average cost. This interpretation allows one to easily adapt results or algorithms derived for average cost, episodic, problems to our setting. 
\end{rem}

\begin{rem}[On the restriction to countable state spaces.]\label{rem: countable state}
	The assumptions that state spaces are at most countably infinite and per-period costs are bounded are standard \citep{puterman2014markov, bertsekas1995dynamic} in textbook treatments of dynamic programming.  A rigorous study of dynamic programming with uncountable state spaces and infinite actions spaces is possible, but it requires restrictions that ensure various functions are measurable \citep{hernandez2012discrete} or the theory of universally measurable policies \citep{shreve1979universally}. To avoid excessive technicality while being fully rigorous, our general results are stated in for countably infinite state spaces. In specific problems like inventory control, there are no measurability issues and so we safety substitute infinite summations for integrals. 
\end{rem} 

%The $t$-step counterparts to left and right linear operators can be naturally written as a composition. 
%For example, $P_{\pi}^2 J= P_{\pi}  (P_{\pi} J)$ satisfies $(P_{\pi}^2 J)(s)  = \E_{\pi}[J(s_2) | s_0=s]$. 
%When the state space is finite,  $P_{\pi} \in \mathbb{R}^{n\times n}$ denotes the Markov transition matrix  under $\pi$ whose $(i,j)$'th entry is equal to $P(j|i, \pi(i))$. The left operator is left-multiplication by a row vector, the right operator is right-multiplication by a column vector, and operator composition is matrix multiplcation. 

% which is interpreted as an expectation with respect to two-step transition $P_{\pi}^2 \cdot J(s) = \sum_{s'' \in \Sc} \sum_{s' \in \Sc} P(s''|s', \pi(s')) P(s'|s, \pi(s)) J(s'')$.
%Similarly, let $P_{\pi}: \Jc \to \Jc$ be the transition operator defined by $(P_{\pi}J)(s) =\sum_{s' \in \Sc} P(s'|s, \pi(s)) J(s')$. 

%Define the Bellman operator $T_{\pi}: \Jc \to \Jc$ under the policy $\pi$ as $T_{\pi} J := g_{\pi} + \gamma P_{\pi} J$. The cost-to-go function $J_{\pi}\in \Jc$ under policy $\pi$ is the unique solution to the Bellman equation $J_\pi = T_{\pi} J_\pi$ and can be written out as 
%Invertability the Neuman series formula $(I - \gamma P_{\pi})^{-1} = \sum_{t=0}^\infty \gamma^t P_{\pi}^t$ are justified since $\gamma P_{\pi}$ has operator norm less than one, meaning $ \| \gamma P_{\pi} J\|_{\infty} \leq \gamma \|J\|_{\infty}$ and $\gamma <1$. 









 %We formalize the claim in the following remark, but this construction is standard in dynamic programming. 
%\begin{rem}
%	Suppose $\Sc$ is a finite and fix $\pi \in \Pi$. Consider a Markov chain $(s_{0}, s_{1}, \cdots)$ 
%	with transition probabilities 
%	\[ 
%	\Prob\left(s_t = s| s_{t-1}, \cdots, s_{0} \right) = (1-\gamma) \rho(s) + \gamma P(s | s_{t-1}, \pi(s_{t-1})) \qquad s \in \Sc.
%	\] 
%	Then, as $T\to \infty$,
%	\begin{align*}
%  \frac{1}{T} \sum_{t=0}^{T-1} g_{\pi}(s_t)  \overset{a.s.}{\longrightarrow} \ell(\pi) \qquad \text{and} \qquad 	\frac{1}{T} \sum_{t=0}^{T-1} \mathbf{1}(s_t=s)  \overset{a.s.}{\longrightarrow}
%  \eta_{\pi}(s)	  \,\, \forall s\in \Sc. 
% \end{align*} 
%\end{rem}





==> geometric_rates.tex <==
%!TEX root = policy_grad_optimality.tex

\section{Geometric convergence in finite action problems}
\label{section:tabularMDPS}
While most of this paper was completed simultaneously with \cite{agarwal2019optimality}, this section is inspired directly by their work. In particular, one contribution of that work is to provide rates of convergence for policy gradient methods -- and in particular, natural policy gradient methods -- with exact gradient evaluations in finite state and action problems with a policy class consisting of all stochastic policies. Depending on the precise algorithm, their proofs show policy gradient methods find an $\epsilon$--optimal policy within either $O\left(\frac{1}{\epsilon}\right)$ or $O\left(\frac{1}{\epsilon^2}\right)$ iterations by posing these as smooth nonlinear optimization problems and suggesting small stepsizes to control for the error due to local linearization. In this work, we highlight that many first order methods applied to $\ell(\cdot)$, including natural policy gradient methods, can work with extremely large stepsizes and attain a \emph{linear} rate of convergence, or equivalently, they require only $O(\log(1/\epsilon))$ iterations to reach an $\epsilon$--optimal policy. Figure \ref{fig:tabular convergence} illustrates this convergence behavior for projected and natural policy gradient methods for a relatively small example with exact gradient computations. See \jb{either appendix or github link} for more details.

\begin{figure}
	\centering
	\begin{subfigure}{.5\textwidth}
		\centering
		\includegraphics[width=0.86\linewidth]{Figures/Fig_Tabular_PGD_NPG.pdf}
	\end{subfigure}%
	\begin{subfigure}{.5\textwidth}
		\centering
		\includegraphics[width=0.86\textwidth]{Figures/Fig_Tabular_PGD_NPG_log.pdf}
	\end{subfigure}
	\caption{Geometric convergence of projected and natural policy gradient methods for a 50 state, 10 action MDP with randomly generated rewards and transition probabilities, $\gamma=0.9$ and a uniform start state distribution. We use backtracking line search to set stepsizes for projected gradient descent and a small constant stepsize for natural gradient updates.}
	\label{fig:tabular convergence}
\end{figure}

Throughout this paper, we have reduced the analysis of policy gradient methods to that of first order methods on the weighted policy iteration cost function, $\Bc(\bar{\pi} | \eta, J_{\pi} )$. The special feature of the finite action case is that the policy iteration step reduces to a linear optimization problem over the probability simplex, a trivial problem which simply selects the best element among a finite set. First order methods can potentially solve such problems in just a single iteration using a large stepsize. From this, we are able to deduce a geometric rate of convergence for policy gradient methods, akin to making exact policy iteration updates. 

\subsection{Setup}
Recall the problem setup for finite state action MDPs as shown in Example \ref{ex:tabularMDPs}. There are $n$ state and $k$ deterministic actions to choose from. We take the set of feasible actions, $\Ac=\Delta^{k-1}$, to be the set of all probability distributions over these  $k$ actions. We consider the following two commonly used policy parameterizations:
\begin{description}
	\item[Natural parameterization.]  Here, $\pi\in \mathbb{R}^{n \times k}$ denotes a stochastic policy, viewed as a matrix where each row is a probability distribution over actions for a given state. The set $\Pi  = \{ \pi \in \mathbb{R}^{n\times k}_{+}  :  \sum_{i=1}^{k} \pi_{s,i}  =1  \,\, \forall s\in \{1,\cdots, n\}  \}$ deontes the set of all stationary randomized policies. 
	\item[Softmax parameterization.] For unconstrained $\theta \in \mathbb{R}^{n \times k}$, the softmax policy specifies an action-distribution  $\pi_{\theta}(s) \in \Delta^{k-1}$ for each $s\in \{1,\cdots,n\}$. The vector $\pi_{\theta}(s)\equiv(\pi_{\theta}(1|s),\cdots, \pi_{\theta}(k|s))$ has components
	\[
	\pi_{\theta}(i|s) = \frac{e^{\theta_{s,i}}}{\sum_{j =1}^{k} e^{\theta_{s,j}}}  \qquad i=1,\cdots,k.
	\]
\end{description}


%Consider a problem where $\Sc=\{1,\cdots, n\}$ is a finite set. For notational simplicity, assume the set of feasible actions $\Ac_s$ is the same for every state $s$ and denote this by $\Ac$. We assume there is a finite set of $k$ deterministic actions to choose from and take $\Ac=\Delta^{k-1}$ to be the set of all probability distributions over these actions. That is, any action $a \in \Ac$ is a vector of probabilities where each component $a_i$ denotes the probability of taking the $i\text{th}$ action. Cost and transition functions can be naturally extended to functions on the probability simplex by defining:
%\begin{align}\label{eq: tabular costs and transitions}
%g(s,a) = \sum_{i=1}^{k} g(s,e_i) \, a_i && P(s'| s,a)=\sum_{i=1}^{k} P(s'| s, e_i) \, a_i.
%\end{align}
%where $e_i$ is the $i$-th standard basis vector, representing one of the $k$ possible deterministic actions. We consider two commonly used policy parameterizations:
%\begin{description}
%	\item[Natural parameterization.]  Here $\pi_{\theta}(s) = \theta_s \in \Delta^{k-1}$ associates each state with a probability distribution over actions. Rather than track the policy parameter $\theta=(\theta_s : s=1,\cdots n)\in \mathbb{R}^{n\times k}$ we work directly with a stochastic policy $\pi\in \mathbb{R}^{n \times k}$, viewed as a matrix whose rows are probability vectors. In this case, the set of all stationary randomized policies can be written as $\Pi  = \{ \pi \in \mathbb{R}^{n\times k}_{+}  :  \sum_{i=1}^{k} \pi_{s,i}  =1  \,\, \forall s\in \{1,\cdots, n\}  \}$. 
%	\item[Softmax parameterization.] For unconstrained $\theta \in \mathbb{R}^{n \times k}$, the softmax policy specifies an action-distribution  $\pi_{\theta}(s) \in \Delta^{k-1}$ for each $s\in \{1,\cdots,n\}$. The vector $\pi_{\theta}(s)\equiv(\pi_{\theta}(1|s),\cdots, \pi_{\theta}(k|s))$ has components
%	\[
%	\pi_{\theta}(i|s) = \frac{e^{\theta_{s,i}}}{\sum_{j =1}^{k} e^{\theta_{s,j}}}  \qquad i=1,\cdots,k.
%	\]
%\end{description}
 % Since the policy parameters are constrained to the simplex, optimizing over this policy class requires using a first order algorithms that maintain feasibility like projected gradient descent, exponentiaed gradient descent, or conditional gradient descent. See section \ref{subsec: optimization background}.  We will discus challenges with direct gradient descent over the unconstrained class of softmax policies in Section \ref{}. 
\paragraph{Policy gradients.} Gradient calculations take on a particular transparent form in tabular problems. Let $e_i$ be the $i$-th standard basis vector, representing one of the $k$ possible deterministic actions. We can rewrite the policy iteration cost function as 
\begin{align}
\label{eq:WPIobjective_tabular}
\Bc(\pibar | \eta_{\pi}, J_{\pi} ) = \sum_{s=1}^{n} \eta_{\pi}(s)\left( \sum_{i=1}^{k} \pibar_{s,i} \cdot Q_{\pi}(s,e_i)  \right)= \langle \pibar\, , \, Q_{\pi} \rangle_{\eta_\pi \times 1 }
\end{align}
where $\langle v,u\rangle_{W} = \sum_{s=1}^{n}\sum_{i=1}^{k} v(s,i) u(s,i) W(s,i)$ denotes the $W$-weighted inner product and $\eta_\pi \times 1$ denotes a weighting that places weight $\eta_{\pi}(s) \cdot 1$ on any state-action pair $(s,i)$. The policy gradient theorem (Lemma \ref{lem: PG theorem}) shows $\nabla \ell(\pi)  =  \nabla \Bc(\pibar | \eta_{\pi}, J_{\pi}) \big\vert_{\pibar=\pi}$. Expressed in terms of partial derivatives, this gives $\frac{\partial}{\partial \pi_{s,i}} \ell(\pi) = \frac{1}{1-\gamma}\eta_{\pi}(s) Q_\pi(s, e_i)$. First order methods use the local linear approximation to $\ell$,
\begin{align*}
\ell(\pibar) &= \ell(\pi) +  \langle \nabla \ell(\pi)\, ,\,  \pibar -\pi \rangle + O(\| \pibar - \pi \|^2 )\\
&= \ell(\pi) + \langle Q_{\pi} \, , \, \pibar-\pi  \rangle_{\eta_\pi \times 1 } + O(\| \pibar - \pi \|^2 ).
\end{align*}
It is important that $\eta_{\pi}(s)>0$ for all $s$, since $\rho(s)>0$. %The view of $\nabla \ell(\pi)$ as an inner product is was developed by \cite{konda2003onactor}.  
\subsection{Algorithms}\label{subsec: algo tabular}
We now specialize several first-order algorithms to this setting.  Recall the set of stochastic policies $\Pi  = \{ \pi \in \mathbb{R}^{n\times k}_{+}  :  \sum_{i=1}^{k} \pi_{s,i}  =1  \,\, \forall s\in \{1,\cdots, n\}  \}$, and note that $\Pi = \Delta^{k-1}(1) \times \cdots \times \Delta^{k-1}(n)$ is the $n$-fold product of the probability simplex. This form of the policy class will cause certain policy gradient updates to decouple across states. 

\begin{description}
	\item[Frank-Wolfe.] Starting with some policy $\pi\in \Pi$, an iteration of the Frank-Wolfe algorithm computes
	\begin{equation}\label{eq: tabular-franke-wolfe-optimization}
	\pi' = \argmin_{\pibar \in \Pi}  \, \langle \nabla\ell(\pi), \pibar \rangle =  \argmin_{\pibar \in \Pi} \, \langle Q_{\pi}, \pibar \rangle_{\eta_{\pi} \times 1} 
	\end{equation}
	and then updates the policy to $\pi^+ =(1-\alpha) \pi + \alpha \pi'$. In this case, $\pi'$ is exactly a policy iteration update to $\pi$ so \emph{Frank-Wolfe mimics a soft-policy iteration step}, akin to the update in \cite{kakade2002approximately}. Note, the minimization problem in \eqref{eq: tabular-franke-wolfe-optimization} decouples across states to optimize a linear objective over the probability simplex, so $\pi^{+}(s) \in \argmin_{d \in \Delta^{k-1}} \eta_{\pi}(s) d^{\top} Q_{\pi}(s, \cdot)$ is a point-mass that places all weight on $\argmin_{i} Q_{\pi}(s, e_i)$. 
	\item[Projected Gradient Descent.] Starting with some policy $\pi\in \Pi$, an iteration of the projected gradient descent algorithm with constant stepsize $\alpha$ updates to the solution of a quadratically regularized problem
	\[ 
	\pi^{+} = \argmin_{\pibar \in \Pi}  \langle \nabla\ell(\pi), \pibar \rangle + \frac{1}{2\alpha} \|  \pibar-\pi \|_2^2 =  \argmin_{\pibar \in \Pi} \langle Q_{\pi}, \pibar \rangle_{\eta_{\pi} \times 1}  + \frac{1}{2\alpha} \|  \pibar-\pi \|_2^2.
	\] 
	As $\alpha \to \infty$ (the regularization term tends to zero), $\pi^+$ converges to the solution of \eqref{eq: tabular-franke-wolfe-optimization}, which is exactly the policy iteration update as noted above. For intermediate values of $\alpha$, the projected gradient update decouples across states and takes the form: $\pi^{+}_{s}  = {\rm Proj}_{2, \Delta^{k-1}}(\pi_s - \alpha Q_{\pi}(s, \cdot))$, a gradient step followed by a projection onto the probability simplex. Note that from an implementation perspective, projections onto the probability simplex involves a computationally efficient ($\mathcal{O}(k \log k)$) soft-thresholding operation \citep{duchi2008efficient}. 
	\item[Mirror-descent.] The mirror descent method adapts to the geometry of the probability simplex by using a non-euclidean regularizer. We focus on using the Kullback Leibler (KL) divergence, a natural choice for the regularizer, under which an iteration of mirror descent updates policy $\pi$ to $\pi^+$: 
	\begin{align*}
	\pi^{+} = \argmin_{\pibar \in \Pi}  \langle \nabla\ell(\pi), \pibar \rangle + \frac{1}{\alpha} \sum_{s=1}^{n} D_{\rm KL}( \pibar_s \, || \, \pi_s  )&= \argmin_{\pibar \in \Pi} \langle Q_{\pi}, \pibar \rangle_{\eta_{\pi} \times 1}  + \frac{1}{\alpha}\sum_{s=1}^{n} D_{\rm KL}( \pibar_s \, || \, \pi_s  ),
	\end{align*}
	where KL divergence is defined as $D_{\rm KL}(p||q)=\sum_{i=1}^{k} p_i\log(p_i /q_i)$. Equivalently, $\pi^+$ can be written as the exponentiated gradient update,
	\[
	\pi^{+}_{s,i} = \frac{\pi_{s,i} \cdot \exp\{ -\alpha \eta_{\pi}(s) Q_{\pi}(s,e_i) \} }{ \sum_{j=1}^{k} \pi_{s,j} \cdot \exp\{ -\alpha \eta_{\pi}(s) Q_{\pi}(s,e_j) \}}. 
	\]
	Again, we can see that $\pi^+$ converges to a policy iteration update as $\alpha \to \infty$. 
	\item[Natural policy gradient and TRPO.] We consider the natural policy gradient (NPG) algorithm of \cite{kakade2002natural} applied to the softmax parameterization described above. This is closely related to the widely used TRPO algorithm of \cite{schulman2015trust}. NPG with softmax policies is actually an instance of mirror descent with a specific regualrizer. In particular, beginning with some policy $\pi \in \Pi$, an iteration of NPG updates to $\pi^+$:
	\begin{align*}
	\pi^{+} &= \argmin_{\pibar \in \Pi}  \langle \nabla\ell(\pi), \pibar \rangle + \frac{1}{\alpha} \sum_{s=1}^{n} \eta_{\pi}(s) D_{\rm KL}( \pibar_s \, || \, \pi_s  )\\
	&= \argmin_{\pibar \in \Pi} \langle Q_{\pi}, \pibar \rangle_{\eta_{\pi} \times 1}  + \frac{1}{\alpha}\sum_{s=1}^{n} \eta_{\pi}(s) D_{\rm KL}( \pibar_s \, || \, \pi_s  ), \\
	& = \left(\frac{\pi_{s,i} \cdot \exp\{ -\alpha  Q_{\pi}(s,e_i) \} }{ \sum_{j=1}^{k} \pi_{s,j} \cdot \exp\{ -\alpha Q_{\pi}(s,e_j)  \} }\right)_{ s\in \{1,\cdots, n \},  i\in\{1,\cdots, k\}  } 
	\end{align*}
	Here, we have used a natural regularizer that penalizes changes to the the action distribution at states in proportion to their occupancy measure $\eta_{\pi}$. This yields a type of soft policy iteration update at each state. 
	
	A potential source of confusion is that natural policy gradient is usually described as steepest descent in a variable metric defined by a certain fisher information matrix. But it is known to be equivalent to 
	mirror descent under some conditions \citep{raskutti2015information}. In this case, readers can check that the exponentiated update above matches the explicit formula for the NPG update given in \cite{kakade2002natural} and \cite{agarwal2019optimality}. 
	
	 %The method depends on a choice Bregman divergence $D_h(\pibar, \pi)= h(\pibar)-h(\pi) - \langle \nabla h(\pi)\, ,\, h(\pibar) - h(\pi) \rangle$ defined by a choice of strongly convex $h(\cdot)$. The natural choice in our case is the sum of negative entropy functions $h(\pi) = \sum_{s} \sum_{i=1}^{k} \pi_{s,i} \log \pi_{s,i}$ in which case $D_{h}(\pibar, \pi) = \sum_{j=1}^{n} $	 
\end{description}
The choice of stepsizes is an important issue for most first order methods. Each a of the algorithms above can be applied with a sequence of stepsizes $\{\alpha_{t}\}$ to produce a sequence of policies $\{\pi_t \}$.  At iteration $t$, the rules above actually specify a one dimensional family of updated policies $\pi^{\alpha}_{t+1}$ that depends on the choice of stepsize $\alpha$. An idealized stepsize rule is \emph{exact line search}, which directly optimizes over this choice of stepize at each iteration: 
\begin{equation}\label{eq: exact linesearch}
\alpha_{t} = \argmin_{\alpha \geq 0}  \ell(\pi_{t}^{\alpha})
\end{equation}
If this minimum is not attained, then all results apply by choosing an $\epsilon$--optimal solution in \eqref{eq: exact linesearch}, for some arbitrarily small $\epsilon$. 

\subsection{Geometric convergence}
So far, we have described different vaariants of implementing policy gradients for tabular settings. Essentially, all of these algorithms make policy iteration updates for sufficiently large stepsizes. Intuitively, it makes sense to expect that their convergence behavior closely resemble results for policy iteration rather than the analysis of gradient descent. We quantify this precisely in Theorem \ref{thm: tabular rates} below.


%While we have described many variants of policy gradient that correspond to different first-order methods applied to $\ell(\cdot)$, they all essentially make policy iteration updates to the policy when step-sizes are taken to be sufficiently large. From this, it is clear their convergence behavior should reflect that policy iteration rather than the usual analyses of gradient descent. It remains to quantify this precisely. 

Our first result confirms that all of the algorithms we presented in the previous section will converge geometrically if stepsizes are set by exact line search on $\ell(\cdot)$. Again, the idea is that a policy gradient \emph{is} a policy iteration update for an appropriate choice of stepsize. 
Our proof effectively shows that exact line search updates make atleast as much progress in reducing $\ell(\cdot)$ as a policy iteration update.
%Our proof effectively shows that exact line search cannot choose a step-size much worse than a policy iteration update.
The mismatch between the policy gradient loss $\ell(\cdot)$, which governs the stepsize choice, and the maximum norm, which governs policy iteration convergence, is the source of the $\min_{s\in \Sc} \rho(s)$ term in the bound. 

Our second and third results show that dependence on the initial distribution can be avoided by forcing the algorithm to use appropriately large constant stepsizes. The simplest result applies to the Frank-Wolfe algorithm, which we already showed to be exactly equivalent to a soft policy iteration update. However, the NPG result is likely more important since variants of this algorithm are widely used in practice. We show NPG with exact gradient updates will reach an $\epsilon$ optimal policy in $O(\log(1/\epsilon))$ iterations with sufficiently large stepsizes. 
%\jb{A remark in case we choose to present it in form (c) which I prefer.} 
The constant error term is inversely related to the stepsize $\alpha_t$ and reflects the fact that NPG updates with finite stepsizes only approximately resemble the policy iteration updates. As $\alpha_t \to \infty$, we recover the exact result as one would expect for policy iteration.

%Our second and third results show that dependence on the initial distribution can be avoided by forcing the algorithm to use  appropriately large constant stepsizes. This is no coincidence, as these algorithms coincide with policy iteration if stepsizes are sufficiently large. 
%
%The simplest results apply to the Frank-Wolfe algorithm, since we have observed the algorithm is nearly equivalent to policy iteration. However, the NPG result is likely more important since variants of this algorithm are widely used in practice. We show NPG with exact gradient updates will reach an $\epsilon$ optimal policy in $O(\log(1/\epsilon))$ iterations with sufficiently large stepsizes.. 

Many caveats apply to these results. The literature claims to effectively approximate natural policy gradient updates with complex deep neural networks \citep{schulman2015trust}, but it is unclear whether understanding of other first order algorithms contributes to developing practical algorithms. Small stepsizes may be critical in practice for controlling certain approximation errors and for stabilizing algorithms. None of these issues are present in simple tabular RL problems, however, and we believe it is valuable for researchers to have a clear understanding of rates of convergence in this idealized case. 

\begin{restatable}[Geometric convergence]{thm}{geometricthm}
	\label{thm: tabular rates}
	Suppose one of the first-order algorithms in subsection \ref{subsec: algo tabular} is applied to minimize $\ell(\pi)$ over $\pi \in \Pi$ with stepsize sequence $(\alpha_t: t \in \{0,1,2, \cdots \})$. Let $\pi^0$ denote the initial policy and $(\pi^{t} : t \in \{0,1,2, \cdots)$ denote the sequence of iterates. The following bounds apply:
	\begin{enumerate}[label=(\alph*)]
		\item  \textbf{Exact line search.} If either Frank-Wolfe, projected gradient descent, mirror descent, or NPG is applied with step-sizes chosen by exact line search as in \eqref{eq: exact linesearch}, then
		% $\alpha_{t} = \argmin_{\alpha\geq 0 }\ell(\pi_{t} - \alpha \nabla \ell(\pi_t) )$, 
		\[ 
		\|  J_{\pi^t} - J^* \|_{\infty}  \leq (1-\min_{s\in \Sc} \rho(s)\left( 1-\gamma \right)^t \|  J_{\pi^0} - J^* \|_{\infty}. 
		\] 
		\item \textbf{Constant stepsize Frank-wolfe.} Under Frank Wolfe with constant stepsize $\alpha\in (0,1]$, 	\[ 
		  \|  J_{\pi^t} - J^* \|_{\infty}  \leq (1-\alpha(1-\gamma))^t \|  J_{\pi^0} - J^* \|_{\infty}. 
		\]
		\item \textbf{Constant stepsize natural policy gradient.} Fix any $\epsilon>0$. Under NPG with stepsize sequence $\alpha_t \geq  \frac{2\log(2)}{(1-\gamma) \epsilon}$, 
		\[
		\norm{J_{\pi^t}-J^*}_{\infty} \leq \left(\frac{1+\gamma}{2} \right)^t \norm{J_{\pi^0}-J^*}_{\infty} + \epsilon.
		\]
		% Alternate version
%		\item \textbf{Constant stepsize natural policy gradient.} Fix any $\epsilon>0$. Under NPG with  stepsize sequence $\alpha_t \geq  \frac{4\log(2)}{(1-\gamma) \epsilon}$, 
%		\[
%		\norm{J_{\pi^t}-J^*}_{\infty} \leq \epsilon \quad \text{if} \quad t \geq \log \left( \frac{4 \|J_{\pi^0}-J^*\|_\infty}{(1+\gamma) \epsilon} \right).
%		\] 
%		\item[Constant stepsize natural policy gradient.] Fix any $\epsilon>0$. Under NPG with  stepsize sequence $\alpha_t \geq  4\log(2)/\epsilon$, 
%		\[
%		\norm{J_{\pi^{t+1}}-J^*}_{\infty} \leq \epsilon \quad \text{if} \quad t \geq \frac{\log(1/\epsilon)}{1-\gamma/2}.
%		\] 
	\end{enumerate}
\end{restatable} 




==> non_stationary_policies.tex <==
%!TEX root = policy_grad_optimality.tex
\section{Beyond closed policy classes: the case of nonstationary policy classes}\label{sec: nonstationary}
For finite horizon problems with non-stationary policy classes, we can guarantee that there are no spurious local minima for policy gradient under a much weaker condition. Rather than require the policy class is closed under improvement, it is sufficient that the policy class contains the optimal policy\footnote{Closure of the policy class implies that it contains the optimal policy.}. For this reason, our theory will cover as special cases a broad variety of finite horizon dynamic programming problems for which structured policy classes are known to be optimal.  Interestingly, this result relies critically on the use of a non-stationary policy class. In particular, Example \ref{ex: counterexample} shows that policy gradient performed with respect to stationary policy classes can get stuck in bad local minima even if the policy class contains an optimal policy. 

As motivation, consider the finite-horizon inventory control in Example \ref{ex:inventorycontrol}. \cite{kunnumkal2008using} have previously showed through a somewhat intricate analysis that a stochastic approximation algorithm converges to the optimal policy, despite non-convexity of the objective.  
\begin{example}[Finite horizon inventory control]
	\label{ex:inventorycontrol}
	Consider a multi-period inventory control problem (also popularly known as the multi-period newsvendor problem) with backlogged demands. A seller operates over $H$ periods. At time $t\in \{0, \cdots, H-1\}$, they select a non-negative quantity $a_t\geq 0$ of inventory to order on the basis of the current inventory level $x_t \in \R$. After ordering inventory, a random i.i.d demand $w_t$ is realized and the inventory level evolves according to  $x_{t+1} = x_t + a_t - w_t$. Negative inventory levels correspond to backlogged demand that is filled when additional inventory becomes available. The seller's objective is to minimize total expected cost
	\begin{align}
	\label{eq:inventory_cost_to_go}
	\E \left[ \sum_{t=0}^{H-1} (ca_t + b\max\{s_t+a_t-w_t, 0\} + p\max\{-s_t+a_t-w_t, 0\} ) \right]
	\end{align}
	where $c,b,p > 0$ denote the per unit costs of ordering, holding and backlogging items, respectively. We assume that $p > c$. Otherwise, the optimal policy never orders inventory.  
	It is well known that a (multi-period) base-stock policy is optimal for this setting \citep{bertsekas1995dynamic}. Let $s_t= (x_t, t)$ denote the state at time $t$, encoding all information needed to make an optimal ordering decision. A base stock policy depends on a vector of target inventory levels $(\theta_0, \cdots, \theta_{H-1}) \in \mathbb{R}^H_+$ \  At state $(x,t)$, the policy orders inventory $\pi_{\theta}((x, t)) =  \max\{0, \theta_t - x\}$. That is, it orders enough inventory to reach a target level $\theta_t$, whenever feasible.  We restrict to the policy class $\Pi_{\Theta}=\{ \pi_{\theta} : \theta \in \Theta \}$ with bounded parameter space $\Theta=  [0, M]^{H}$ for $M\geq 2w_{\max}$. With a selection of $\theta_t = M$, the seller can ensure $x_{t+1} \geq w_{\max}$ is large enough to meet all demand with probability one. Inventory levels above this are clearly suboptimal, due to their excessive holding costs.  
	 % We also assume the initial distribution, $\rho$, supported on $\{1,\ldots, H\} \times \mathbb{R}$ to have a positive density on $\mathbb{R}$ for each $h$. 
\end{example}

We can state our formal result without introducing new notation for the finite horizon setting, by a well known trick that treats finite-horizon time-inhomogeneous MDPs as a special case of infinite horizon MDPs (see e.g. \cite{osband2017deep}). Essentially, one can imagine that the state space factorizes into $H+1$ components, thought of as stages or time periods of the decision problem. For any policy, a state $s \in \Sc_i$ transitions to a state in $\Sc_{i+1}$ until stage $H+1$ is reached and the interaction effectively ends. We also assume the policy class factors into separate components. This structure allows us to change the policy in stage $h$ without influencing the policy at other stages and essentially encoding time-inhomogeneous policies.  
\begin{restatable}[]{cond}{condFiniteHorizon}
	\label{cond: finite_horizon}
	Suppose the state space factors as $\Sc=\Sc_1 \cup \cdots \cup \Sc_{H} \cup \Sc_{H+1}$, where for a state $s\in \Sc_h$ with $h\leq H$, $\sum_{s'\in \Sc_{h+1}} P(s'| s, a)=1$ for all $a\in \Ac_s$. The final subset $\Sc_{H+1}=\{\tau\}$ contains a single costless absorbing state, with $P(\tau| \tau,a)=1$ and $g(\tau,a)=0$ for any action $a$. The parameter space is the product set $\Theta=\Theta_{1} \times \cdots \times \Theta_H$, where  a policy parameter $\theta=(\theta_{1}, \ldots, \theta_{H})\in \Theta$ is the concatenation of $H$ sub-vectors. For any fixed $s\in \Sc_h$, $\pi_{\theta}(s)$ depends only on $\theta_{h}$. We assume $\rho$ to be supported over the entire state space $\Sc$. 
\end{restatable}
Let us emphasize that, in this setting, the assumption that $\rho$ is supported over $\Sc$ means that the agent may begin in a subproblem with fewer than $H$ periods remaining. This would typically be possible in simulation based optimization and it is necessary for the results we derive. 

%For the finite horizon inverntory problem, we assume the demand distribution to be bounded. Therefore, $\Sc_h, \Theta_h = \Mc = [-M,M]$ for some finite $M$\footnote{We only need to search over the set of possible states to find the optimal threshold.}. 
Condition \ref{cond: finite_horizon} can be seen as an alternative to the closure property imposed in Condition \ref{cond: closure}. We also relax Condition \ref{cond: stationary}, which considered stationary points of single-period problems, $\theta \mapsto \Bc(\theta|\eta,J_\pi)$, induced by any policy $\pi \in \Pi_{\Theta}$. The weaker condition below only imposes a regularity condition on the weighted policy iteration objectives corresponding to the optimal cost-to-go function, $J^*$.  
\begin{cond}
	\label{cond:finite_horizon_stationarity}
	For any distribution $\eta$ with full support on $\Sc=\cup_{h=1}^{H+1}$, the problem $\min_{\theta \in \Theta} \Bc(\theta|\eta,J^*)$ has no suboptimal stationary points.
\end{cond}
For the inventory control problem in Example \ref{ex:inventorycontrol}, a simple argument shows that $\theta \mapsto \Bc(\theta | \eta, J^*)$ has no suboptimal stationary points for state-distributions $\eta$ obeying appropriate regularity conditions. The result, shown in Appendix \ref{subsec: finite horizon proof}, essentially follows by using that the optimal Q-function, $Q^*(s,a)$ is convex in $a$ (see Chapter 3 in \cite{bertsekas1995dynamic} for details).


We now state the main result of this subsection, which applies under conditions much weaker than those for Theorem \ref{thm: no bad stationary points general}. The full proof is given in Appendix \ref{subsec: finite horizon proof} and proceeds by backward induction. We first show how all stationary points must play according to an optimal policy at the final-period states $s\in \Sc_H$. From this, we argue that at any stationary point the policy must act optimally from any state in $\Sc_{h}$ for $h < H$. 

%We now state the main result of this subsection, which relaxes some conditions in Theorem \ref{thm: no bad stationary points general} for problems satisfying Condition \ref{cond: finite_horizon}. Note that assuming $\Pi_{\Theta}$ contains an optimal policy is weaker than Condition \ref{cond: closure}. Also, the requirement that the single-period cost function $\theta \mapsto \Bc(\theta \mid \eta, J^*)= \E_{s\sim \eta}\left[ Q^*(s, \pi_{\theta}(s))\right]$ has no suboptimal stationary points is weaker that Condition \ref{cond: stationary}, which also considers stationary points of single-period problems $\theta \mapsto \Bc(\theta | \eta, J_{\pi})$ induced by suboptimal policies.    

%\begin{restatable}[]{thm}{finiteHorizon}
%	\label{thm: finite_horizon}
%	Suppose Condition \ref{cond: finite_horizon} holds and $\theta \mapsto \Bc(\theta \mid \eta, J^*)$ has no suboptimal stationary points, for any distribution $\eta$ supported over each $\Sc_h$ for $h \leq H$. If the parameterized policy class $\Pi_\Theta$ contains an optimal policy $\pi^*$, then any stationary point $\theta$ of $\ell:\Theta \to \mathbb{R}$ satisfies $J_{\pi_\theta} = J^*$. 
%\end{restatable}

\begin{restatable}[]{thm}{finiteHorizon}
	\label{thm: finite_horizon}
	Suppose Conditions \ref{cond: finite_horizon} and \ref{cond:finite_horizon_stationarity} hold. Further assume that $\rho$ is supported over each $\Sc_h$ for $h \leq H$. If the parameterized policy class $\Pi_\Theta$ contains an optimal policy, then any stationary point $\theta$ of $\ell:\Theta \to \mathbb{R}$ satisfies $J_{\pi_\theta} = J^*$. 
\end{restatable}


==> notes_to_self.tex <==
%!TEX root = policy_grad_optimality.tex

\section{Notes to self on PG Theorem}
\paragraph{Deriving the policy gradient}
By Bellman's equation, 
\[ 
J_{\pi_{\theta'}}-J_{\pi_\theta} =  \left(T_{\pi_{\theta'}}J_{\pi_{\theta'}}-T_{\pi_{\theta'}}J_{\pi_{\theta}}\right) +\left( T_{\pi_{\theta'}}J_{\pi_{\theta}} - J_{\pi_\theta} \right) = \gamma P_{{\pi_\theta'}} \left(J_{\pi_{\theta'}}-J_{\pi_{\theta}}\right) + \left( T_{\pi_{\theta'}}J_{\pi_{\theta}} - J_{\pi_\theta} \right)
\] 
Rearranging gives, 
\begin{align*}
J_{\pi_{\theta'}} &=J_{\pi_\theta}+ \left(I-\gamma P_{\pi_{\theta'}} \right)^{-1} \left( T_{\pi_{\theta'}}J_{\pi_{\theta}} - J_{\pi_\theta} \right)\\
&=J_{\pi_\theta}+ \left(I-\gamma P_{\pi_{\theta}} \right)^{-1} \left( T_{\pi_{\theta'}}J_{\pi_{\theta}} - J_{\pi_\theta} \right) + r(\theta, \theta') 
\end{align*}
where the remainder function
\[
r(\theta, \theta')=\left[ \left(I-\gamma P_{\pi_{\theta'}} \right)^{-1}  - \left(I-\gamma P_{\pi_{\theta}} \right)^{-1}  \right] \left( T_{\pi_{\theta'}}J_{\pi_{\theta}} - J_{\pi_\theta} \right)
\] 
is $O(\| \theta'-\theta \|^2)$ as $\theta' \to \theta$ under appropriate smoothness conditions are required to ensure it is second order. 


This gives a local approximation to $J_{\pi_{\theta'}}$ around $\theta'=\theta$. We see that changes in $\theta'$ influence the cost-to-go only through the term  $\left(I-\gamma P_{\pi_\theta}\right)^{-1} T_{\pi_{\theta'}}J_{\pi_{\theta}}$. 



\paragraph{Technical conditions under which the policy gradient theorem applies.}
One way to derive the the expression \eqref{eq: PG expression 1} is to apply the policy gradient expression due to \cite{silver2014deterministic}. For problems with compact state space and satisfying sufficient smoothness conditions, they calculate the gradient as
\[ 
\grad \ell(\theta) = \E_{s\sim \eta_{\pi_\theta} }\left[ 
\left(\frac{\partial \pi_{\theta}(s)}{\partial \theta}\right) \grad_a Q_{\pi_{\theta}}\left( s, a \right)\bigg\vert_{a= \pi_{\theta}(s)} \right]
\]
where $\frac{\partial \pi_{\theta}(s)}{\partial \theta}$ is a Jacobian matrix. This is equivalent to \eqref{eq: PG expression 1} and hence \eqref{eq: policy gradient expression 2}. This result is dubbed a deterministic policy gradient theorem, since the authors focus on problems with deterministic actions. But this result also generalizes the stochastic policy gradient theorem \citep{sutton2000policy} if one interprets the action $a$ as a probability vector as we have done in section \ref{sec: tabuluar}. 

We prefer to derive the policy gradient result \eqref{eq: policy gradient expression 2} directly from the implicit function theorem, because this approach extends gracefully to problems with infinite state spaces. To sketch the idea, assume for now that the state space is finite with $\Sc=\{1,\cdots, n\}$.  Use the shorthand $J_\theta=J_{\pi_\theta}$ and $\dot{J}_\theta$ for its derivative. Note that by Bellman's equation we can view $J_{\theta}$ as the unique root of the function $f(\theta, J) = T_{\pi_\theta} J - J$. Since $T_{\pi}J= g_{\pi}+P_{\pi}J$ is an affine function of $J$, we can calculate the partial derivative $f_{2}(\theta, J) = \frac{\partial}{\partial J} f(J,\theta) = -(I-\Gamma P_{\pi_\theta})$. The implicit function theorem then states that 
\begin{equation}\label{eq: functional pg expression}
\dot{J}_\theta = (I-\gamma P_{\pi_\theta})^{-1} f_{1}(\theta, J_{\theta})
\end{equation} 
assuming the partial derivative $f_1(\cdot)$ exists and is continuous. Here $f_{1}(\theta, J_\pi)=\frac{\partial}{\partial \theta} T_{\pi_\theta} J_\pi$ evaluates changes to the Bellman update to $J_\pi$ as the policy parameter changes and is intimately related to the differentiating the policy iteration cost function. The desired formula can be reached by left multiplying both sides of \eqref{eq: functional pg expression} by the initial distribution $\rho$. This argument also applies when the state space is infinite, but because $J_\theta : S \to \mathbb{R}$ is a function one must invoke results from functional analysis.  We state here technical lemmas ensuring the policy gradient expression \eqref{eq: policy gradient expression 2} holds. Proofs follow as described above and are given in the appendix. 


\subsection{Relating policy gradients to weighed policy iteration}
Policy gradient theorems give expressions for $\nabla \ell(\theta)$. The most common expressions found in the textbook \cite{sutton2018reinforcement} hold for problems with finite action spaces and allow stochastic gradients of $\ell(\cdot)$ to be computed simply. Here, we'll review a more general policy gradient expression, due to \cite{silver2014deterministic} that also applies to problems with infinite action spaces. 



Under appropriate technical conditions, the gradients of the total cost $\ell(\theta)$ exist and satisfy the following formula: for any vector $d\theta$,  
\begin{equation}\label{eq: PG expression 1}
\ell(\theta + d\theta) = \E_{s\sim \eta_{\pi_\theta}}\left[ Q_{\pi_\theta}\left(s, \pi_{\theta + d\theta}(s) \right) \right]  + o(\| d\theta\|),
\end{equation}
where the notation $o(\| d\theta\|)$ represents an arbitrary remainder function $r(d\theta)$ satisfying $r(d\theta)/\|d\theta\| \to 0$ as $\| d\theta\| \to 0$. Later in this subsection we'll state technical regularity conditions under which this expression holds. For now, let us focus on its implications. 

Presenting the policy gradient theorem in this way emphasizes its deep connections to  the weighted policy iteration objective \eqref{eq: convexity lqr} we discussed in the previous subsection. Let us generalize \eqref{eq: convexity lqr} by introducing the weighted policy iteration objective 
\begin{equation}%\label{eq: weighted PI objective}
C(\pi' \mid \eta, \pi)  = \E_{s\sim \eta}\left[  Q_{\pi}(s, \pi'(s))  \right]  %= \E_{s\sim \eta}\left[  g(s, \pi'(s)) + \gamma\sum_{s'} P(s' \mid s, \pi'(s)) J_{\pi}(s') \right]  
\end{equation}
and overload notation to write $C(\theta \mid \eta, \pi)  = C(\pi_\theta \mid \eta, \pi)$. When $\eta$ is supported on all states, minimizing \eqref{eq: weighted PI objective} over all policies $\pi'$ is equivalent to classical policy iteration. As is common, let $C_{1}(\pi_\theta \mid \eta, \pi) = \frac{\partial}{\partial \theta} C(\theta \mid \eta, \pi)$ denote the partial derivative of $C$ with respect to its first argument. Then \eqref{eq: PG expression 1} states that 
\begin{equation}\label{eq: policy gradient expression 2} 
\nabla \ell(\theta) = C_{1}(\theta \mid \eta_{\pi_\theta}, \pi_{\theta}).
\end{equation}  
In this way, policy gradient methods are quite sharply related to the weighted policy iteration scheme
\begin{equation}\label{eq: weighted constrained PI}
\theta_{t+1} = \argmin_{\theta \in \Theta} C(\theta \mid \eta, \pi_{\theta_t}),
\end{equation}  
which preforms policy iteration style updates over the parameterized policy class. Policy gradient methods differ in two ways. First, they are incremental, making a parameter update based on a gradient of \eqref{eq: weighted PI objective} rather than solving it exactly. Second, the state-weighting $\eta$ is updated over time to reflect the states visited by the current policy. 

\paragraph{Technical conditions under which the policy gradient theorem holds.}
The policy gradient expressions \eqref{eq: PG expression 1} and \eqref{eq: PG expression 2} hold broadly, including all of the examples we consider. Unfortunately, it is subtle to give a single result that unifies problems with discrete state spaces, problems with continuous states where the state space is a bounded, and problems like linear quadratic control with the state space is unbounded and cost-to-go functions are potentially infinite. We instead provide a few separate results, which put together confirm that the policy gradient expression holds broadly. All results can be proved in the same way and standalone proofs are given the appendix. 

\begin{lem}(Policy Gradient Theorem for Finite State Spaces)
	If $\Sc = \{1,\cdots n \}$, and $\theta\mapsto \pi_{\theta}(s)$  $a\mapsto g(s, a)$ and $a\mapsto P(s' \mid s, a)$ are continuously differentiable for all $s,s'\in \Sc$ then $\ell(\theta)$ is differentiable and \eqref{eq: policy gradient expression 2}  holds. 
\end{lem}

\begin{lem}(Policy Gradient Theorem for Compact State Spaces)
	Suppose $\sup_{s,a} \| g(s,a)\|_\infty <\infty$, $\sup_{s,a} \| g(s,a)\|_\infty <\infty$,  \ldots \textbf{Fill in sufficient conditions such the $f$ is continuously Frechet differentiable}
\end{lem}
We next consider the policy gradient formula for linear quadratic control. Here, we all results need some qualification because some linear controllers are unstable and incur infinite expected cost.
\begin{lem}[Policy Gradient Theorem for LQ Control] Consider the linear quadratic control problem formulated in Example \ref{ex: lq control}. Let $\theta \in \mathbb{R}^{n\times k}$. For any $\theta$ satisfying $\| A  - B\theta\|_2 \leq 1$, $\ell(\theta)<\infty$ and equation \eqref{eq: policy gradient expression} holds. 
\end{lem}




\subsection{Relating policy gradients to weighed policy iteration}
Policy gradient theorems give expressions for $\nabla \ell(\theta)$. The most common expressions found in the textbook \cite{sutton2018reinforcement} hold for problems with finite action spaces and allow stochastic gradients of $\ell(\cdot)$ to be computed simply. Here, we'll review a more general policy gradient expression, due to \cite{silver2014deterministic} that also applies to problems with infinite action spaces. 



Under appropriate technical conditions, the gradients of the total cost $\ell(\theta)$ exist and satisfy the following formula: for any vector $d\theta$,  
\begin{equation}\label{eq: PG expression 1}
\ell(\theta + d\theta) = \E_{s\sim \eta_{\pi_\theta}}\left[ Q_{\pi_\theta}\left(s, \pi_{\theta + d\theta}(s) \right) \right]  + o(\| d\theta\|),
\end{equation}
where the notation $o(\| d\theta\|)$ represents an arbitrary remainder function $r(d\theta)$ satisfying $r(d\theta)/\|d\theta\| \to 0$ as $\| d\theta\| \to 0$. Later in this subsection we'll state technical regularity conditions under which this expression holds. For now, let us focus on its implications. 

Presenting the policy gradient theorem in this way emphasizes its deep connections to  the weighted policy iteration objective \eqref{eq: convexity lqr} we discussed in the previous subsection. Let us generalize \eqref{eq: convexity lqr} by introducing the weighted policy iteration objective 
\begin{equation}\label{eq: weighted PI objective}
C(\pi' \mid \eta, \pi)  = \E_{s\sim \eta}\left[  Q_{\pi}(s, \pi'(s))  \right]  %= \E_{s\sim \eta}\left[  g(s, \pi'(s)) + \gamma\sum_{s'} P(s' \mid s, \pi'(s)) J_{\pi}(s') \right]  
\end{equation}
and overload notation to write $C(\theta \mid \eta, \pi)  = C(\pi_\theta \mid \eta, \pi)$. When $\eta$ is supported on all states, minimizing \eqref{eq: weighted PI objective} over all policies $\pi'$ is equivalent to classical policy iteration. As is common, let $C_{1}(\pi_\theta \mid \eta, \pi) = \frac{\partial}{\partial \theta} C(\theta \mid \eta, \pi)$ denote the partial derivative of $C$ with respect to its first argument. Then \eqref{eq: PG expression 1} states that 
\begin{equation}\label{eq: policy gradient expression 2} 
\nabla \ell(\theta) = C_{1}(\theta \mid \eta_{\pi_\theta}, \pi_{\theta}).
\end{equation}  
In this way, policy gradient methods are quite sharply related to the weighted policy iteration scheme
\begin{equation}\label{eq: weighted constrained PI}
\theta_{t+1} = \argmin_{\theta \in \Theta} C(\theta \mid \eta, \pi_{\theta_t}),
\end{equation}  
which preforms policy iteration style updates over the parameterized policy class. Policy gradient methods differ in two ways. First, they are incremental, making a parameter update based on a gradient of \eqref{eq: weighted PI objective} rather than solving it exactly. Second, the state-weighting $\eta$ is updated over time to reflect the states visited by the current policy. 

\paragraph{Technical conditions under which the policy gradient theorem holds.}
The policy gradient expressions \eqref{eq: PG expression 1} and \eqref{eq: PG expression 2} hold broadly, including all of the examples we consider. Unfortunately, it is subtle to give a single result that unifies problems with discrete state spaces, problems with continuous states where the state space is a bounded, and problems like linear quadratic control with the state space is unbounded and cost-to-go functions are potentially infinite. We instead provide a few separate results, which put together confirm that the policy gradient expression holds broadly. All results can be proved in the same way and standalone proofs are given the appendix. 

\begin{lem}(Policy Gradient Theorem for Finite State Spaces)
	If $\Sc = \{1,\cdots n \}$, and $\theta\mapsto \pi_{\theta}(s)$  $a\mapsto g(s, a)$ and $a\mapsto P(s' \mid s, a)$ are continuously differentiable for all $s,s'\in \Sc$ then $\ell(\theta)$ is differentiable and \eqref{eq: policy gradient expression 2}  holds. 
\end{lem}

\begin{lem}(Policy Gradient Theorem for Compact State Spaces)
	Suppose $\sup_{s,a} \| g(s,a)\|_\infty <\infty$, $\sup_{s,a} \| g(s,a)\|_\infty <\infty$,  \ldots \textbf{Fill in sufficient conditions such the $f$ is continuously Frechet differentiable}
\end{lem}
We next consider the policy gradient formula for linear quadratic control. Here, we all results need some qualification because some linear controllers are unstable and incur infinite expected cost.
\begin{lem}[Policy Gradient Theorem for LQ Control] Consider the linear quadratic control problem formulated in Example \ref{ex: lq control}. Let $\theta \in \mathbb{R}^{n\times k}$. For any $\theta$ satisfying $\| A  - B\theta\|_2 \leq 1$, $\ell(\theta)<\infty$ and equation \eqref{eq: policy gradient expression} holds. 
\end{lem}


%we have under broad technical conditions  








%\paragraph{Review of policy gradient theorems}

%Before giving our main results, we first provide some technical background which is used throughout the paper. We begin by stating a more general policy gradient theorem and comment on some regularity conditions required for its existence. 
%\vspace{-2mm}
%The most common form of the policy gradient theorem \cite{sutton2000policy} applies to problems with finite action spaces and smoothly parameterized stochastic policies. In particular, let $\pi_\theta(a\mid s)$ denote the probability of choosing action $a\in \{1,\cdots, k\}$ in state $s$. Then, the actor-critic form of the policy gradient theorem shows that:
%\[ 
%\nabla\ell(\theta) = \E_{s\sim \eta_{\pi_\theta}, a\sim \pi_{\theta}(\cdot \mid S}) \, \left[ Q_{\pi_\theta}(s,a)  \nabla_\theta \log \pi_\theta(a|s) \right].
%\]
%It is noteworthy that this form of the policy gradient  only depends on states and actions drawn by following the current policy $\pi_\theta$ and therefore is well suited to simulation based Monte-Carlo approximation. However, a more general form of the policy gradient theorem due to \cite{silver2014deterministic} will be useful for us. Let $\frac{\partial \pi_{\theta}(s)}{\partial \theta}$ denote the Jacobian matrix of $\pi_{\theta}(s)$. 
%\begin{restatable}[Policy gradient theorem of \cite{silver2014deterministic}]{lem}{policygradstatement}\label{lem: policy gradient thm}
%	Under suitable regularity assumptions, 
%	\[ 
%	\grad_{\theta} \ell(\pi_{\theta}) = \sum_{s \in \Sc}\eta_{\pi_{\theta}}(s) 
%	\left[\frac{\partial \pi_{\theta}(s)}{\partial \theta}\right] \grad_a Q_{\pi_{\theta}}\left( s, a \right)\bigg\vert_{a= \pi_{\theta}(s)} 
%	\]
%\end{restatable}
%Though this is usually viewed as a deterministic policy gradient result, it also generalizes the policy gradient theorem by \cite{sutton2000policy} taking an action $a$ to be a probability vector.



%\paragraph{Relating policy gradients to weighed policy iteration}
%In Example \ref{ex: lq control} we highlighted the importance of a weighted policy iteration objective \eqref{eq: convexity lqr}. This section calls out precise connections between policy gradient methods and such problems. 
%\paragraph{Weighted policy iteration.}
%We generalize \eqref{eq: convexity lqr} by introducing the weighted policy iteration objective 
%\[
%C(\pi' \mid \eta, \pi)  = \E_{s\sim \eta}\left[  Q_{\pi}(s, \pi'(s))  \right]  %= \E_{s\sim \eta}\left[  g(s, \pi'(s)) + \gamma\sum_{s'} P(s' \mid s, \pi'(s)) J_{\pi}(s') \right]  
%\] 
%and overload notation to write $C(\theta \mid \eta, \pi)  = C(\pi_\theta \mid \eta, \pi)$. For distributions $\eta$ that are supported on the entire state space, policy iteration is the algorithm 
%\begin{equation}\label{eq: weighted PI}
%\pi_{t+1} = \argmin_{\pi \in \Pi} C(\pi \mid \eta, \pi_{t}).
%\end{equation}

%To see this, note that $\pi_{t+1}(s) \in \argmin_{a\in \Ac(s)} Q_{\pi_t}(s,a)$ almost surely for $s$ drawn from $\eta$. But unlike the usual formulation of policy iteration as the solution to a multi-objective minimization problem, there is a simple analogue of \eqref{eq: weighted PI} for the restricted policy class $\Pi_{\Theta}$:
%\begin{equation}\label{eq: weighted constrained PI}
%\theta_{t+1} = \argmin_{\theta \in \Theta} C(\theta \mid \eta, \pi_{\theta_t}).
%\end{equation}  
%We will study the gradients of this optimization. Define the the notation for partial gradients:
%\[ 
%g(\theta \mid \eta, \pi) = \frac{\partial }{\partial \theta} C(\theta \mid \eta, \pi) \in \mathbb{R}^d
%\]
%Here, $g$ should be understood as a function associating the tuple $(\theta, \eta, \pi)$ with an element of $\mathbb{R}^d$. 


%We give a more general expression for the policy gradient theorem which highlights its deep connections to the iteration \eqref{eq: weighted constrained PI}. The policy gradient theorem says that, under appropriate smoothness conditions,
%\begin{equation}
%\nabla \ell(\theta) = C_{1}(\theta \mid \eta_{\pi_\theta}, \pi_{\theta}).
%\end{equation}  
%This means that for a vector $d\theta$,  
%\[
%\ell(\theta + d\theta) = \E_{s\sim \eta_{\pi_\theta}}\left[ Q_{\pi_\theta}\left(s, \pi_{\theta + d\theta}(s) \right) \right]  + o(\| d\theta\|),
%\]
%where the notation $o(\| d\theta\|)$ represents an arbitrary remainder function $r(d\theta)$ satisfying $r(d\theta)/\|d\theta\| \to 0$ as $\| d\theta\| \to 0$. From this, we can see the policy gradient is closely related to the policy iteration scheme \eqref{eq: weighted constrained PI}, except that the state-weighting is adapted throughout iterations of the the algorithm and we make only a gradient update to the policy rather than solving the optimization problem to optimality. 


%\paragraph{General policy gradient theorems.}
%Below, we state formally several lemmas ensuring that \eqref{eq: policy gradient expression} holds in problems of practical interest. We include a simple proof for finite state spaces using the implicit function theorem. When the state space is infinite, the same argument can be used but appropriate smoothness conditions must be treated more carefully. We provide proofs in Appendix \ref{}. 

%To understand this, let us suppose the state space $\Sc=\{1,\cdots,n\}$ is finite. Then, $J_{\theta}\equiv J_{\pi_\theta}$ is the unique solution to $f(\theta, J_\theta)=0$ where 
%\[
%f(\theta, J)= g_{\theta} + \gamma P_{\theta} J \in \mathbb{R}^n
%\]
%and we have used the shorthand notation $g_{\theta}(s) = g(s, \pi_\theta(s))$ and $P_{\theta}(s,s')=P(s'\mid s, \pi_\theta(s))$. Assuming appropriate smoothness conditions 
%ecall that under broad conditions

%\begin{lem}
%If $\Sc = \{1,\cdots n \}$, and $\theta\mapsto \pi_{\theta}(s)$  $a\mapsto g(s, a)$ and $a\mapsto P(s' \mid s, a)$ are continuously differentiable for all $s,s'\in \Sc$ then $\ell(\theta)$ is differentiable and \eqref{eq: policy gradient expression} holds. 
%\end{lem}
%\begin{proof}
%First let us define some shorthand notation. Let $J_\theta = J_{\pi_\theta}$, set $g_{\pi_\theta} \in \mathbb{R}^n$ to be a vector with elements $g_{\pi}(s)=g(s,\pi(s))$ and $P_{\pi}\in \mathbb{R}^{n\times n}$ to be a matrix with elements $P_{\pi}(s, s')= P(s'\mid s, \pi_{\theta}(s)$. Assuming it exists, let $\dot{\theta}$ denote the derivative $J_\theta$ with respect to $\theta$. 

%The cost-to-go function $J_\theta$ is the unique solution to the Bellman equation $f(\theta, J_\theta)=0$ where %$f: \Theta \times \mathbb{R}^{n} \to \mathbb{R}^n$ is defined by 
%\[ 
%f(\theta, J) := g_{\pi_\theta} + \gamma P_{\pi_\theta} J -J.
%\] 
%This function has continuous partial derivatives we denote by $f_{1}(\theta, J) = \frac{\partial}{\partial \theta} f(\theta, J) \in \mathbb{R}^d$ and $f_{2}(\theta, J) = \frac{\partial}{\partial J} f(\theta, J) = (I-\gamma P_{\pi_\theta})$. By the implicit function theorem, $J_\theta$ is continuously differentiable with derivative 
%\[ 
%\dot{J}_\theta=  - f_{2}(\theta, J_\theta)^{-1}f_{1}(\theta, J_\theta)  = (I-\gamma P_{\pi_\theta})^{-1} f_{1}(\theta, J_\theta).
%\] 
%Recall that $(I-\gamma P_{\pi_\theta})^{-1}=\sum_{t=0}^{\infty}\alpha^t P_{\pi_\theta}^t$ and hence $\rho^\top (I-\gamma P_{\pi_\theta})^{-1}=\eta_{\pi_\theta}$ is the discounted state occupancy measure. This implies, 
%$\E_{s\sim \eta}[\dot{J}_\theta(s)]= \eta_{\pi_\theta}^\top f_{1}(\theta, J_\theta).$
%This concludes the proof since the right hand side is exactly $C_{1}(\theta \mid \eta_{\pi_\theta}, \pi_{\theta})$ in \eqref{eq: policy gradient expression}. 
%\end{proof}



\subsection{Temporary notes on an alternative proof in the tabular case}
\begin{lem}[Policy gradient expression for directional derivatives] For policies $\overline{\pi}$ and $\pi$, define $\pi^\alpha = (1-\alpha) \pi + \alpha \overline{\pi}$. Then 
	\[\frac{d}{d\alpha} J_{\pi^\alpha} \bigg\vert_{\alpha = 0} = (I-\gamma P_{\pi} )^{-1} (T_{\overline{\pi}}J_{\pi} - J_{\pi})\]
	%    and 
	%    \[
	%    \frac{d}{d\alpha} J_{\pi^\alpha} \bigg\vert_{\alpha = 0} = \frac{\eta_{\pi} (T_{\overline{\pi}}J_{\pi} - J_{\pi})}{1-\gamma}  
	%    \]
\end{lem}
\begin{proof}
	By the linearity of \eqref{eq: tabular costs} and \eqref{eq: tabular transitions}, we can see $T_{\pi^\alpha}J=(1-\alpha) T_{\pi}J+\alpha T_{\overline{\pi}}J$ for any vector $J\in \mathbb{R}^n$. Applying equation \eqref{eq: near solutions to bellmans equation}, we compute 
	\begin{align*}
	J_{\pi^\alpha} - J_{\pi} =\left( I-\gamma P_{\pi^\alpha}\right)^{-1}  (T_{\pi^\alpha} J_\pi  - J_\pi) 
	&= \left( I-\gamma P_{\pi^\alpha}\right)^{-1} ( (1-\alpha)T_{\pi}J_{\pi} +  \alpha T_{\overline{\pi}} J_\pi  - J_\pi)\\ 
	&= \alpha \left( I-\gamma P_{\pi^\alpha}\right)^{-1}  ( T J_{\pi}  - J_{\pi}) 
	\end{align*}
	Note that $P_{\pi^\alpha}=(1-\alpha)P_{\pi}+\alpha P_{\overline{\pi}} \to P_{\pi}$ as $\alpha \to 0$.  Dividing each side by $\alpha$ and taking $\alpha\to 0$ gives the directional derivative 
	\[ 
	\frac{d}{d\alpha}J_{\pi^\alpha}  \bigg\vert_{\alpha = 0} = \lim_{\alpha\to 0} \left( I-\gamma P_{\pi^\alpha}\right)^{-1}  ( T_{\overline{\pi}} J_{\pi}  - J_{\pi}) = \left( I-\gamma P_{\pi^\alpha}\right)^{-1}  ( T_{\overline{\pi}} J_{\pi}  - J_{\pi})
	\] 
	%     The establish the second claim we use the definition $\eta_{\pi}=(1-\gamma) \rho (I-P_{\pi})^{-1}$ to calculate,
	%         \begin{align*}
	%         \frac{d}{d\alpha} \ell({\pi^\alpha})  \bigg\vert_{\alpha = 0} = \rho \left(\frac{d}{d\alpha}J_{\pi^\alpha}\right) = \rho \left( I-\gamma P_{\pi}\right)^{-1}( T J_{\pi}  - J_{\pi}) =  \frac{\eta_\pi( T J_{\pi}  - J_{\pi})}{1-\gamma}.
	%     \end{align*}
\end{proof}
Now we give a trivial proof of Theorem \ref{thm: tabular stationary points}. 
\begin{proof}[Proof of Theorem \ref{thm: tabular stationary points}]
	Set $\pi^\alpha = (1-\alpha)\pi  + \alpha\pi^+$. Note that  $T_\pi^+ J_\pi= T J_\pi$ by definition of $\pi^+$ as a policy iteration update. We apply lemma together with the geoemetric series expression $(I-\gamma P_{\pi} )^{-1} = \sum_{t=0}^{\infty} \gamma^t P_{\pi}^t$ to conclude
	\begin{align*}
	\frac{d}{d\alpha} \ell({\pi^\alpha})  \bigg\vert_{\alpha = 0} = \rho \left(\frac{d}{d\alpha}J_{\pi^\alpha}\right)  = \sum_{t=0}^{\infty} \gamma^t \rho P_{\pi}^t ( T J_{\pi}  - J_{\pi})
	\leq  \rho ( T J_{\pi}  - J_{\pi}) = -\| T J_{\pi}  - J_{\pi}  \|_{1,\rho}.
	\end{align*}
	The inequality uses that $TJ_{\pi}(s) \leq J_{\pi}(s)$ for all states $s$ (see equation \eqref{eq: bellman update reduces cost}) and that $\rho P_{\pi}^t$ is non-negative. (In fact, it is the probability vector encoding the distribution of the state at time $t$).  
\end{proof}


==> numerical.tex <==
%!TEX root = policy_grad_optimality.tex

\section{Numerical Illustration}
In fact, simple numerical experiments show that gradient descent with backtracking line search performed on $\ell(\theta)$ converges rapidly to the global optimum. We show sample plots for the optimal stopping problem and the inventory control case in Figure \ref{fig:only_figure} below. For linear quadratic control we refer readers to Figure 1 in \cite{fazel2018global}. 
\begin{figure}
	\centering
	\begin{subfigure}{.5\textwidth}
		\centering
		\includegraphics[width=0.8\linewidth]{Figures/Fig_Asset_Selling.pdf}
		\caption{Contextual optimal stopping}
	\end{subfigure}%
	\begin{subfigure}{.5\textwidth}
		\centering
		\includegraphics[width=0.8\textwidth]{Figures/Fig_Inventory_Control.pdf}
		\caption{Newsvendor problem}
	\end{subfigure}
	\caption{We plot the optimality gap (difference in average cost/reward with respect to the optimal policy) as a function of gradient steps. Full experiment details are available in \cite{bhandari2019global} }
	\label{fig:only_figure}
\end{figure}

Our work aims to understand this phenomenon. Why did gradient descent on a non-convex function reach the global minimum? These examples share important structural properties. Consider a linear quadratic control problem. Starting with a linear policy and performing a policy iteration step yields another linear policy. That is, the policy class is \emph{closed} under policy improvement. In addition, although the cost-to-go function is a nasty non-convex function of the policy, the policy iteration update involves just solving a quadratic minimization problem. In fact, for each of the first three examples, the policy class is closed under policy improvement and the policy-iteration objective (i.e. the $Q$-function) is smooth and convex in the chosen action. Similar ideas, apply to the fourth example, but weaker conditions are needed to ensure convergence for some finite-horizon problems. Given this insight, strikingly simple proofs show that any stationary point of $\theta \mapsto \ell(\pi_\theta)$ is a global minimum. We also reach the stronger conclusion that $\ell$ satisfies a gradient dominance condition, a well known condition in nonlinear optimization that allows for convergence rate guarantees similar to the case of convex functions.  The major contribution here is in offering a new lens into this problem, through which some powerful conclusions can be reached \emph{without any complex calculations or analysis}. 


==> tabular.tex <==
%!TEX root = policy_grad_optimality.tex

\section{Simple results in the tabular case}\label{sec: tabuluar}
This section studies the quality of near-stationary points in finite state and action MDPs. In particular, we show that the poor optimization landscape in Example \ref{ex: counterexample} is cured by using a richer policy class consisting of all stochastic stationary policies.  While the results here are subsumed by the more the general results in the coming sections, this concrete setting provides strong intuition. In addition, the tabular setting allows us to give proofs that mirror the textbook analysis of policy iteration.   

Consider a problem where $\Sc=\{1,\cdots, n\}$ is a finite set. For notational simplicity, assume the set of feasible actions $\Ac(s)$ is the same for every state $s$ and denote this by $\Ac(s)$. We assume there is a finite set of $k$ deterministic actions that could be chosen and take $\Ac=\Delta^{k-1}$ to be the set of all probability distributions over these actions. That is, any action $a \in \Ac(s)$ is a vector of probabilities where each component $a_i$ denotes the probability of taking the $i\text{th}$ action. Cost and transition functions are naturally extended to functions on the probability simplex by defining the expected cost function to be:
\begin{equation}\label{eq: tabular costs}
g(s,a) = \sum_{i=1}^{k} g(s,i) \, a_i
\end{equation}
and transition function to be:
\begin{equation}\label{eq: tabular transitions} 
P(s'| s,a)=\sum_{i=1}^{k} P(s'| s, i) \, a_i.
\end{equation} 
We consider the natural policy parameterization where $\pi_{\theta}(s) = \theta_s \in \Delta^{k-1}$ associates each state with a probability distribution over actions. Rather than track the policy parameter $\theta=(\theta_s : s=1,\cdots n)\in \mathbb{R}^{n\times, k}$ we work directly with a stochastic policy $\pi\in \mathbb{R}^{n \times k}$, viewed as a matrix whose rows are probability vectors. In this case, the set of all stationary randomized policies can be written as $\Pi  = \{ \pi \in \mathbb{R}^{n\times k}_{+}  :  \sum_{i=1}^{k} \pi_{s,i}  =1  \,\, \forall s\in \{1,\cdots, n\}  \}$.  Since the policy parameters are constrained to the simplex, optimizing over this policy class requires using a first order algorithms that maintain feasibility like projected gradient descent, exponentiaed gradient descent, or conditional gradient descent. See section \ref{subsec: optimization background}.  We will discus challenges with direct gradient descent over the unconstrained class of softmax policies in Section \ref{}. 

\subsection{No suboptimal stationary points}
The following theorem shows that $\ell(\cdot)$ has no suboptimal stationary points by constructing a specific descent direction. The direction is chosen to point toward the policy iteration update, and we show the corresponding directional derivative scales with the average magnitude of the Bellman error $J_{\pi}-TJ_{\pi}$ weighted under the initial distribution $\rho$. Because of the assumption that $\rho(s)>0$ for all $s$, we have shown that any policy that is a stationary point of $\ell(\cdot)$ has a cost-to go function that satisfies Bellman's equation $J_{\pi}=TJ_{\pi}$ and hence is an optimal policy. 
\begin{thm}\label{thm: tabular stationary points}
	Fix any policy $\pi \in \Pi$ and choose $\pi^+\in \Pi$ to satisfy $\pi^+(s)\in \argmin_{a \in \Ac(s)} Q_{\pi}(s,a)$ for all $s\in \Sc$. Then, 
	\[ 
	\frac{d}{d\alpha}\ell(\pi^\alpha+ \alpha(\pi^+ -\pi) ) \bigg\vert_{\alpha=0}   \leq - \| TJ_\pi - J_\pi  \|_{1, \rho} 
	\] 
\end{thm} 


\begin{proof}
	We fix $\alpha>0$, but the proof follows with all inequalities reversed if $\alpha<0$. Set $\pi^\alpha = (1-\alpha)\pi  + \alpha\pi^+$. By the linearity of \eqref{eq: tabular costs} and \eqref{eq: tabular transitions}, we can see that $\pi \mapsto T_\pi J \in \mathbb{R}^{|\Sc|}$ is a linear function of $\pi$ for any $J$. Using also that $T_\pi^+ J_\pi= T J_\pi$ by definition of $\pi^+$ as a policy iteration update, we have 
	\[ 
	T_{\pi^\alpha}J_\pi  = (1-\alpha)T_\pi J_\pi + \alpha T_{\pi^+} J_\pi = (1-\alpha) J_\pi + \alpha TJ_\pi  = J_{\pi} - \alpha (J_{\pi}-TJ_{\pi}) 
	\] 
	Note that $T J_{\pi} \preceq  T_\pi J_{\pi} = J_{\pi}$ and so this shows $T_{\pi^\alpha}J_\pi \preceq J_\pi$. By the monotonicity property of Bellman operators, applying $T_{\pi^\alpha}$ repeatedly to each side of this inequality gives 
	\[
	J_{\pi} \succeq T_{\pi^\alpha}J_\pi \succeq T_{\pi^\alpha}^2 J_\pi \succeq \cdots \succeq J_{\pi^\alpha}.
	\] 
	Then, 
	\[ 
	\frac{ J_{\pi^\alpha} - J_{\pi} }{\alpha} \preceq \frac{ T_{\pi^\alpha} J_{\pi} - J_{\pi} }{\alpha} = - (J_{\pi}- T J_\pi ) 
	\] 
	This is an inequality over vectors. Taking the expectation under the initial distribution $\rho$, this becomes 
	\[ 
	\frac{\ell(\pi^\alpha) - \ell(\pi)}{\alpha} \leq -\sum_{s \in \Sc} \rho(s) \left( J_{\pi}(s) - TJ_{\pi}(s) \right) = - \| J_\pi - TJ_\pi   \|_{1, \rho}
	\] 
	where the final equality uses that $J_\pi - TJ_\pi$ has non-negative entries. The result follows by taking $\alpha$ to zero. 
\end{proof}

\subsection{Gradient dominance}
The result above constructs a descent direction with significant cost improvement whenever the gap in Bellman's equation is large. Since policies the nearly satisfy Bellman's euqation are nearly optimal, we obtain a corollary that shows policies which are nearly stationary points of $\ell(\cdot)$ must be near optimal. The result depends on a problem dependent constant $\kappa_\rho$ which roughly measures the extent to which errors in Bellman's equation can be detected by sampling from $\rho$: 
\[
\kappa_\rho  = \inf_{J\in \Jc_{\Theta}} \frac{\| TJ - J\|_{1,\rho} }{\| TJ - J\|_{\infty}} \geq \min_{s\in \Sc} \rho(s)>0.
\] 
Recall that $\Jc_{\Theta} = \{ J_{\pi} \mid \pi \in \Pi_{\Theta}\}$ is the set of cost-to-go functions corresponding to policies in the policy class. 
\begin{cor}
	\[ 
	\frac{d}{d\alpha}\ell(\pi^\alpha+ \alpha(\pi^+ -\pi) ) \bigg\vert_{\alpha=0}   \leq - \kappa_\rho (1-\gamma) \left(\ell(\pi)-\ell(\pi^*)\right)
	\] 
\end{cor}
\begin{proof}
	From the definition of $\kappa_\rho$, Theorem \ref{thm: tabular stationary points} gives
	\[
	\frac{d}{d\alpha}\ell(\pi^\alpha+ \alpha(\pi^+ -\pi) ) \bigg\vert_{\alpha=0}   \leq - \kappa_\rho \| J_{\pi} - TJ_{\pi}\|_\infty
	\]
	Using that $T$ is a contraction in the supremum norm with fixed point $J^*$, we find
	\begin{align*}
	\|  J_\pi - J^*\|_\infty &\leq \|  J_\pi - TJ_\pi\|_\infty + \| T J_\pi - J^*\|_\infty \\
	&= \|  J_\pi - TJ_\pi\|_\infty + \| T J_\pi - TJ^*\|_\infty \\
	&\leq \|  J_\pi - TJ_\pi\|_\infty + \gamma \| J_\pi - J^*\|_\infty.
	\end{align*}
	Rearranging gives a lower bound on $\|J_\pi - TJ_\pi\|_\infty$ which completes the proof. 
\end{proof}


\subsection{Necessity of an exploratory initial distribution}
The above results depend crucially on the initial distribution $\rho$ placing sufficient weight on all relevant parts of the state space. It is well known that, without such an assumption, policy gradient methods can get stuck at suboptimal policies.   


Performance difference lemma
\[
\| J^* - J_\pi \|_{1,\rho} = \|  J_\pi - T J_{\pi} \|_{1, \eta_\pi^*}.  
\] 



==> unused_proofs.tex <==
%!TEX root = policy_grad_optimality.tex

% Proof of contractivity of Bellman operators for LQ control.
\paragraph{Part (3)} Let $\| Q\|_{2} = \sup_{s\in \mathbb{R}^n} \frac{\| Qs\|_2}{\|s\|^2_2}$ denote the spectral norm for any matrix $Q \in \mathbb{R}^{n\times n}$. Then,
	\[ 
	\| J - \bar{J}\|_{\infty,w} = \sup_{s \in \mathbb{R}^n} |J(s)-\bar{J}(s)| w(s) = \sup_{s \in \mathbb{R}^n} \frac{\left| s^\top  \left( K- \bar{K} \right)s  \right|}{\| s \|_2^2}  = \left\| K-\bar{K}  \right\|_2.  
	\]   
	From definition of the Bellman operator, we have
	\begin{align*}
	\| T_{\pi_\theta} J - T_{\pi_\theta} \bar{J} \|_{\infty, w} &=  \sup_{s \in \mathbb{R}^n} \frac{1}{\| s \|_2^2} \,\cdot  \, \gamma \left[ J\left([A+B\theta] s \right) - \bar{J}\left([A+B\theta] s \right)  \right] \\
	&= \sup_{s \in \mathbb{R}^n} \frac{1}{\| s \|_2^2} \cdot \gamma s^\top  [A+B\theta]^{\top} \left( K -\bar{K}  \right) [A+B\theta] s  \\
	&= \gamma \left\|  [A+B\theta] \left( K - \bar{K}\right)[A+B\theta] \right\|_{2}\\
	&\leq \gamma \|A+B\theta\|_2^2 \left\| K - \bar{K}\right\|_2 \\
	&\leq  \gamma \left\| K - \bar{K}\right\|_2.
	\end{align*}
	which uses the fact that indcued operator norms are subultiplicative. The final inequality follows using $\|A+B\theta\|_2 \leq 1$ as we assumed $\pi_{\theta}$ to be a stable linear policy. 
	
	Given the contraction property for  $T_{\pi_{\theta}}(\cdot)$ for any stable policy, $\theta \in \Theta_\text{S}$, we show the contraction result for the Bellman optimality operator: $TJ = \min_{\theta \in \Theta_\text{S}} T_{\pi_{\theta}} J \,\,\, \forall \, J \in \Jc_{q}$. Note that it is sufficient to search over the set of stable policies as we assumed the system (A, B) to be controllable. Starting with $J \in \Jc_{q}$ such that $\|J\|_{\infty,w}$ is finite, applying the Bellman operator can only decrease costs from every state. This implies,
	\begin{align*}
		\|TJ - TJ'\|_{\infty,w} = \sup_{s \in \mathbb{R}^n} \frac{1}{\|s\|^2} \, |TJ(s)-T\bar{J}(s)|
		&=  \sup_{s \in \mathbb{R}^n} \frac{1}{\|s\|_2^2} \,|\min_{\theta \in \Theta_\text{S}} T_{\pi_{\theta}}J(s)- \min_{\theta \in \Theta_\text{S}} T_{\pi_{\theta}}\bar{J}(s)| \\
		&\overset{(a)}{\leq} \sup_{s \in \mathbb{R}^n} \frac{1}{\|s\|_2^2} \, \max_{\theta \in \Theta_\text{S}}|T_{\pi_{\theta}}J(s)-T_{\pi_{\theta}}\bar{J}(s)| \\
		& \leq \max_{\theta \in \Theta_\text{S}} \| T_{\pi_\theta} J - T_{\pi_\theta} \bar{J} \|_{\infty, w} \\
		&\overset{(b)}{\leq} \gamma \left\| K - \bar{K}\right\|_2 = \| J - \bar{J}\|_{\infty,w}.
	\end{align*}
	where (b) follows from the contraction property of $T_{\pi_{\theta}}$ for any $\theta \in \Theta_\text{S}$. Inequality (a) follows from the following short result.
	Consider any two functions $f, g$ and a set $\Z \subseteq \text{Dom}(f) \cap \text{Dom}(g)$. Then,
	\begin{align*}
		\left|\min_{z_1 \in \Z}f(z_1) - \min_{z_2 \in \Z}g(z_2)\right| \leq \max_{z \in \Z} \left|f(z) - g(z)\right|.
	\end{align*}
	To see this, note
	\begin{align*}
		\min_{z_1 \in \Z}f(z_1) - \min_{z_2 \in \Z}g(z_2) &= \min_{z_1 \in \Z} \, [f(z_1) + \max_{z_2 \in \Z} -g(z_2)] = \min_{z_1 \in \Z} \max_{z_2 \in \Z}\, [f(z_1) - g(z_2)] \leq \max_{z \in \Z}\, [f(z) - g(z)] \\
		\min_{z_2 \in \Z}g(z_2) - \min_{z_1 \in \Z}f(z_1) &= \min_{z_2 \in \Z} \, [g(z_2) + \max_{z_1 \in \Z} -f(z_1)] = \min_{z_2 \in \Z} \max_{z_1 \in \Z} \, [g(z_2) - f(z_1)] \leq \max_{z \in \Z} [g(z) - f(z)].
	\end{align*}
	

\subsection{Proof of Lemma \ref{lem: PG theorem}}\label{subsec: pg theorem proof}
For the reader's convenience, we restate the claim. 
\pgTheorem* 
\begin{proof} 
	We have already shown
	\begin{align*}
	\ell(\thetabar) &= \ell(\theta)+  \eta_{\theta} \left( T_\thetabar J_\theta - J_\theta \right) +  \left[  (\eta_\thetabar - \eta_\theta)\left( T_\thetabar J_\theta - T_{\theta} J_\theta \right)\right]\\
	&= \ell(\theta)+  \eta_{\theta}J_\theta + \underbrace{\sum_{s \in \Sc} \eta_{\theta}(s) Q_{\pi_\theta}(s, \pi_{\thetabar}(s))}_{(a)}  + \underbrace{\left[  (\eta_\thetabar - \eta_\theta)\left( T_\thetabar J_\theta - T_{\theta} J_\theta \right)\right]}_{(b)}
	\end{align*}
	where the second equality applies the basic relation between $Q$ functions and Bellman operators, $(T_{\pi'}J_{\pi})(s)=Q_{\pi}(s, \pi'(s))$. 	We show the gradient $\nabla \ell(\thetabar) |_{\thetabar=\theta}$ exists and calculate it, treating separately the terms (a) and (b).  
	
	\underline{\bf Step 1:} \emph{ Recall the Leibniz rule:}\\
	Recall the Leibniz rule states that, for any base measure $\mu$ and function $f$, 
	$\intop_{\Sc} f(\theta, s) d\mu(s)$ is continuously differentiable with respect to $\theta$, with 
	\[ 
	\frac{\partial}{\partial \theta_i} \intop_{\Sc} f(\theta, s) d\mu(s) =  \intop_{\Sc} \frac{\partial}{\partial \theta_i} f(\theta, s) d\mu(s),
	\]
	provided $\frac{\partial}{\partial \theta_i} f(\theta, s)$ is continuous and integrable, meaning $ \intop_{\Sc} \left|\frac{\partial}{\partial \theta_i} f(\theta, s)\right| d\mu(s) < \infty$. Here we make repeated use of this fact when $\mu$ is either the counting measure or $\mu(s) = \eta_{\theta}(s)$. 
	
	\underline{\bf Step 2:} \emph{ $\frac{\partial}{\partial \thetabar_i} Q_{\pi_{\theta}}(s, \pi_{\thetabar}(s))$ is continuous in $\thetabar$ and satisfies $\sup_{s \in \Sc, \thetabar \in \Theta} \left| \frac{\partial}{\partial \thetabar_i} Q_{\pi_{\theta}}(s, \pi_{\thetabar}(s)) \right| $ }\\ 
	Write,
	\[
	Q_{\pi_{\theta}}(s, \pi_{\thetabar}(s)  )  = g(s, \pi_{\thetabar}(s)) + \sum_{s' \in \Sc} P(s' | s, \pi_{\thetabar}(s) ) J_{\theta}(s').
	\]
	This first term, $g(s, \pi_{\thetabar}(s))$,  is easily seen to be continuously differentiable, since $g(s,a)$ is continuously differentiable with respect to $a$ and $\pi_{\thetabar}(s)$ is continuously differentiable with respect to $\thetabar$. In addition, 
	\[
	\left| \frac{\partial}{\partial \thetabar_i} g(s, \pi_{\thetabar}(s) ) \right|  =  \left| \big\langle \frac{\partial}{\partial \thetabar_i}\pi_{\thetabar}(s)  \, , \,   \frac{\partial}{ \partial a}  g(s, a) \bigg\vert_{a=\pi_{\thetabar}(s)} \big\rangle \right| \leq \sup_{s \in \Sc, \thetabar \in \Theta}  \left\| \frac{\partial}{\partial \thetabar_i}\pi_{\thetabar}(s)\right\|_2 \left\|  \frac{\partial}{ \partial a}  g(s, a) \bigg\vert_{a=\pi_{\thetabar}(s)}  \right\|_2 < \infty 
	\]
	is bounded uniformly by Assumption \ref{ass: regularity}. 
	
	Now consider the second term.  	Observe that $\thetabar \mapsto P(s'| a, \pi_{\thetabar}(s))$ is also continuously differentiable by the chain rule. Its partial derivatives are integrable, since 
	\[
	\sum_{s' \in \Sc}  \left| \frac{\partial}{\partial \thetabar_i} P(s' | s, \pi_{\thetabar}(s) ) J_{\theta}(s')\right| \leq \| J_{\theta}\|_{\infty}  \sum_{s' \in \Sc}\left| \frac{\partial}{\partial \thetabar_i} P(s' | s, \pi_{\thetabar}(s) ) \right| <\infty 
	\] 
	where Assumption \ref{ass: regularity} implies the infinite sum is finite. This shows $\thetabar \mapsto \sum_{s' \in \Sc} P(s' | s, \pi_{\thetabar}(s) ) J_{\theta}(s')$ is continuously differentiable with
	\[ 
	\frac{\partial}{\partial \thetabar_i} \sum_{s' \in \Sc} P(s' | s, \pi_{\thetabar}(s) ) J_{\theta}(s') = \sum_{s' \in \Sc} \frac{\partial}{\partial \thetabar_i}  P(s' | s, \pi_{\thetabar}(s) ) J_{\theta}(s')
	\]
	Assumption \ref{ass: regularity} shows these partial derivatives are uniformly bounded, with, 
	\[
	\sup_{s \in \Sc, \thetabar \in \Theta} \left|  \frac{\partial}{\partial \thetabar_i} \sum_{s' \in \Sc} P(s' | s, \pi_{\thetabar}(s) ) J_{\theta}(s')  \right| < \frac{\| g\|_{\infty} }{1-\gamma}  	\sup_{s \in \Sc, \thetabar \in \Theta} \left|  \sum_{s' \in \Sc} \frac{\partial}{\partial \thetabar_i}  P(s' | s, \pi_{\thetabar}(s) ) \right|  < \infty, 
	\]
	where we used the bound $\|J_\theta\|_{\infty} \leq \| g \|_{\infty}/(1-\gamma)$.\\
	
	{\bf Step 3} \emph{Calculating the derivative of term (a)}.\\
	The result of step (2), together with the Leibniz rule implies we can exchange the summation and derivative, to find 
	\[
	\frac{\partial}{\partial \thetabar_i} \sum_{s \in \Sc} \eta_{\theta}(s) Q_{\pi_{\theta}}(s, \pi_{\thetabar}(s) ) = \sum_{s \in \Sc} \eta_{\theta}(s)\frac{\partial}{\partial \thetabar_i}  Q_{\pi_{\theta}}(s, \pi_{\thetabar}(s) )
	\]
	and this partial derivative is continuous in $\thetabar$. 		
	
	\underline{\bf Step 4:} \emph{Show that $\lim_{\thetabar \to \theta} \left\| T_{\thetabar}J_{\theta} - T_{\theta} J_{\theta} \right\|_{\infty} =0$ }. \\
	We have,
	\begin{align*}
	\left|T_{\thetabar}J_{\theta}(s) -T_{\theta}J_{\theta}(s)\right| = \left|Q_{\pi_{\theta}}(s,\pi_{\thetabar}(s) )- Q_{\pi_{\theta}}(s,\pi_{\theta}(s) )\right| \leq \|\thetabar -\theta\| \sup_{s \in \Sc, \thetabar\in \Theta} \left| \nabla_{\thetabar} Q_{\pi_{\theta}}(s,\pi_{\thetabar}(s) ) \right|<\infty 
	\end{align*}
	where the derivative on the right hand side is bounded uniformly by Step 1. 
	
	\underline{\bf Step 4:} \emph{Show that the operator $\eta \to \eta P_{\theta}$ is Lipschitz with respect to the maximum norm, meaning that there exists $c<\infty$ such that for any distribution $\eta$ over $\Sc$ and any $\theta,\thetabar \in \Theta$
		\[ 
		\| \eta P_{\theta} - \eta P_{\thetabar} \|_{\infty} \leq c \|\thetabar - \theta\|.
		\]
	}
	We have, 
	\begin{align*}
	\| \eta P_{\theta} - \eta P_{\thetabar} \|_{\infty} &= \sup_{s' \in \Sc} \left| \sum_{s \in \Sc} \eta(s)\left( 	P(s'| s, \pi_{\thetabar}(s) - P(s'| s, \pi_{\theta}(s) \right) \right| \\
	&\leq \sup_{s, s' \in \Sc}\left| 	P(s'| s, \pi_{\thetabar}(s) - P(s'| s, \pi_{\theta}(s)) \right|\\
	&= \sup_{s, s' \in \Sc}\left| 	P(s'| s, \pi_{\thetabar}(s) - P(s'| s, \pi_{\theta}(s)) \right| \\
	&\leq  \underbrace{\left(\sup_{s, s' \in \Sc} \sup_{\tilde{\theta}\in \Theta}  \| \nabla	P(s'| s, \pi_{\tilde{\theta}}(s))\|_2 \right)}_{:=c} \|\thetabar-\theta\|_2.
	\end{align*}
	That $c<\infty$ is a direct consequence of Assumption \ref{ass: regularity}. The final equality can be derived by Taylor's theorem, which ensures that for each $s, s'\in \Sc$ there exists $\tilde{\theta} \in \{ t\theta + (1-t) \thetabar  \, : \, t \in [0,1]  \}$ on the line segment joining $\theta$ and $\thetabar$ such that 
	\[
	P(s'| s, \pi_{\thetabar}(s) - P(s'| s, \pi_{\theta}(s)) =  \langle \nabla_{\tilde{\theta}}  P(s' | s, \pi_{\tilde{\theta}}(s))\, , \, \thetabar -\theta \rangle.  
	\]
	The right hand side is then bounded by Cauchy Swartz.  
	
	
	\underline{\bf Step 5:} \emph{Treat term (b)  by showing  $\nabla_\thetabar  \left[  (\eta_\thetabar - \eta_\theta)\left( T_\thetabar J_\theta - T_{\theta} J_\theta \right)\right] \bigg\vert_{\thetabar = \theta} =0$  }.  \\
	To show this, we show $ \left\| \eta_\thetabar - \eta_\theta \|_{\infty} = O(\| \thetabar - \theta \right\|_2)$, which together with step 4 shows,  
	\[
	\lim_{\thetabar \to \theta}  \frac{\left\| (\eta_\thetabar - \eta_\theta)\left( T_\thetabar J_\theta - T_{\theta} J_\theta \right) \right\|_{\infty}}{\| \thetabar -\theta\|_2 }  =0,
	\]
	implying our claim. We have 
	\[
	\eta_{\theta} = (1-\gamma) \rho + \gamma \eta_{\theta} P_{\theta} 
	\]
	That is, $\eta_{\theta}$ is the unique solution to the fixed point equation 
	\[ 
	\eta_\theta = F_{\theta}(\eta_\theta)
	\]
	where $F_{\theta}(\eta) := (1-\gamma)\rho + \eta P_{\theta}$. 	Viewed as a left operator $\eta\mapsto \eta P_{\theta}$ is a mapping from $\ell_1$ to $\ell_1$ defined by
	\[ 
	(\eta P_{\theta}(s')) = \sum_{s \in \Sc} \eta(s) P(s'| s, \pi_{\theta}(s)). 
	\]
	This shows $\|\eta P_{\theta} \|_{\infty} \leq \|\eta\|_{\infty}$, i.e. $P_{\theta}$ is a non-expansion in the maximum norm.  From this, we have that $F_{\theta}$ is a contraction with modulus $\gamma$ with respect to the maximum norm since 
	\[ 
	\|F_{\theta}(\eta') - F_{\theta}(\eta)\|_{\infty} = \gamma \| (\eta'-\eta)  P_{\theta} \|_{\infty} \leq \gamma \| \eta'-\eta \|_{\infty }. 
	\]
	Contractivity implies,	
	\begin{align*}
	\|\eta_{\thetabar} - \eta_{\theta}\|_{\infty} &= \left\| F_{\thetabar}\left(\eta_{\thetabar} \right)  - F_{\theta}\left(\eta_{\theta} \right) \right\|_{\infty} \\ 
	&\leq \left\| F_{\thetabar}\left(\eta_{\thetabar} \right)  - F_{\thetabar}\left(\eta_{\theta} \right) \right\|_{\infty} + \left\| F_{\thetabar}\left(\eta_{\theta} \right)  - F_{\theta}\left(\eta_{\theta} \right) \right\|_{\infty}\\
	&\leq \gamma 	\|\eta_{\thetabar} - \eta_{\theta}\|_{\infty} + \left\| F_{\thetabar}\left(\eta_{\theta} \right)  - F_{\theta}\left(\eta_{\theta} \right) \right\|_{\infty},
	\end{align*}
	which can be rewritten as
	\[
	\|\eta_{\thetabar} - \eta_{\theta}\|_{\infty} \leq \frac{1}{1-\gamma} \left\| F_{\thetabar}\left(\eta_{\theta} \right)  - F_{\theta}\left(\eta_{\theta} \right) \right\|_{\infty} \leq c \|\thetabar - \theta\|
	\]
	where the inequality follows from step 4. 
\end{proof}	
	
